Accelerated Expansion of the Universe in Nonmetricity-based Modified Gravity

This thesis explores the cosmological implications of modified gravity, focusing on nonmetricity-based $f(Q)$ gravity as an alternative to the $\Lambda$CDM model in explaining cosmic acceleration. Chapter I lays the theoretical groundwork by reviewing General Relativity (GR), $\Lambda$CDM, and the limitations of the standard model, motivating $f(Q)$ gravity. Chapter II constructs cosmological reconstructions of $f(Q)$ gravity within the FLRW framework, deriving forms of $f(Q)$ that replicate the $\Lambda$CDM expansion and using the e-folding parameter to show compatibility with various cosmic histories. Chapter III addresses challenges with arbitrary $f(Q)$ forms by applying Gaussian Process (GP) reconstruction using observational Hubble data. This model-independent method reconstructs the Hubble parameter H(z), leading to a data-driven $f(Q)$ form. Motivated by this, a new parametrization $f(Q) = -2\Lambda + \epsilon Q^2$ is proposed, and power-law and exponential models are tested for consistency. Chapter IV incorporates a quintessence scalar field in power-law $f(Q)$ gravity to study inflation and late-time acceleration. Using GP, the scalar potential $V(\phi)$ is reconstructed and analyzed. Results show that early dark energy has little impact today, but reconstructed quintessence models offer insights into cosmic acceleration. Chapter V examines interacting dark energy and matter under power-law $f(Q)$ using dynamical systems. Two interaction types are studied, and fixed points linked to de Sitter and quintessence solutions are identified. Chapter VI concludes and suggests future work.

==> Heping_Tools/Biography.tex <==
\addcontentsline{toc}{chapter}{Biography}
\section*{Brief Biography of the Candidate:}
\textbf{Mr. Sankarsan Tarai} has obtained his M.Sc. degree in Mathematics from Utkal University, Odisha in 2012. He has qualified for GATE in 2013. He has worked as JRF in the SERB-DST project under the supervision of Dr. Bivudutta Mishra. He has also qualified RGNF-SC, University Grants Commission, Govt. of India in 2017-2018. He has published seven research papers in international and national SCI journals and presented research paper in national and international conferences. He was also selected for international travel grant for presenting research paper in international conference. 
\section*{Brief Biography of the Supervisor:}
\textbf{Dr. Bivudutta Mishra} is an Associate Professor in the department of Mathematics of Birla Institute of Technology and Science-Pilani, Hyderabad Campus. He has received his Ph.D. degree from Sambalpur University, Odisha, India in 2003. His main area of research is Cosmology and Relativity and currently working on the theoretical aspects  of Dark Energy and Modified Theory of Gravity. He has already published around 85 research papers in these areas of research in journals of national and international repute. He has presented several research papers and delivered invited talks in these areas in national and international conferences held in India and abroad. He has conducted several academic and scientific events in the department. He has become the member of scientific advisory committee of national and international academic events. He has successfully completed two sponsored projects: one each from University Grants Commission (UGC), New Delhi and Science and Engineering Research Board, Department of Science and Technology, (SERB-DST), New Delhi. He is also an awardee of DAAD-RISE, 2019. He has also reviewed several research papers of highly reputed journals, Ph.D. examiner and BoS member of several universities. He has also visited countries like Canada, UAE, Germany, Republic of China, Malaysia, Italy, Czech Republic, Russia, Australia, Switzerland, Japan and presented his research work in different scientific events. He is also a Visiting Associate of Inter University Centre for Astronomy and Astrophysics (IUCAA), Pune. At the same he is also active in academic administration like: Head of the Department, Mathematics from 2012-2016,  Associate Dean of International Programmes and Collaborations since July 2018. 

\section*{Brief Biography of the Co-supervisor:}
\textbf{Dr. Pradyumn Kumar Sahoo} is presently working as Associate Professor in Dept. of Mathematics, Birla Institute of Technology and Sciences, Pilani, Hyderabad Campus. He received his Ph.D. degree in Mathematics from Sambalpur University, Sambalpur, India in 2004. He has been actively involved in research, teaching, and academic administration for the past fifteen years. He has authored more than 80 research publications in various renowned national and international peer-reviewed journals. He has also presented several research works and delivered invited talks in national and international conferences held in India and aboard. He serves as an expert reviewer and editorial member for a number of reputed scientific research journals, and also Ph.D. examiner in several universities. He is also recipient of Science Academics Summer Research Fellowship, UGC Visiting fellow, Expert Reviewer, Physical Science Projects, SERB-DST, Govt. of India and lifetime membership of many scientific societies. He has successfully executed two projects from UGC, Govt. of India in 2014, and DAAD-RISE Worldwide in 2018. He has also visited counties like Canada, South Korea, Germany, Belgium, Japan, Poland, Switzerland, UK and presented his research work and delivered invited talks in different scientific events.



==> Heping_Tools/Publications.tex <==
\newpage
\addcontentsline{toc}{chapter}{List of Publications and Presentations}

\chapter*{List of Publications and Presentations}\label{Chapter:listofpub}
\vspace{-2.0cm}
\section*{Publications}
\begin{itemize}
\item
B. Mishra, S. K. Tripathy, {\bf Sankarsan Tarai}: Cosmological models with a hybrid scale factor in an extended gravity theory, \textit{Mod. Phys. Lett. A}, \textbf{33}(9), 1850052 (2018).
\item 
{\bf Sankarsan Tarai}, B. Mishra: Dynamical aspects of the magnetized anisotropic cosmological model in extended gravity, \textit{Eur. J. Phys. Plus}, \textbf{133}, 435 (2018).
\item
B. Mishra, {\bf Sankarsan Tarai}, S. K. Tripathy: Dynamical features of anisotropic cosmological model, \textit{Ind. J. Phys.}, \textbf{92}(9), 1199(2018).
\item 
B. Mishra, {\bf Sankarsan Tarai}, S. K. Tripathy: Anisotropic cosmological reconstruction in $f(R,T)$ gravity, \textit{Mod. Phys Lett. A}, \textbf{33}(29), 1850170 (2018).
\item
B. Mishra, {\bf Sankarsan Tarai}, S. K. J. Pacif: Dynamics of Bianchi $VI_{h}$ universe with bulk viscous fluid in modified gravity, \textit{Int. J. of Geom. Methods in Mod. Phys.}, \textbf{15}, 1850036 (2018).
\item
B. Mishra, {\bf Sankarsan Tarai}, S. K. Tripathy: Dynamics of an Anisotropic Universe in $f(R, T)$ gravity, \textit{Adv. High Energy Phys.}, \textbf{2016} , 8543560, (2016).
\item
B. Mishra, P. K. Sahoo, {\bf Sankarsan Tarai}: Non-static Cosmological models in $f(R,T)$ gravity, \textit{Astrophys. Space Sci.}, \textbf{359}, 15 (2015). {\bf{(Not included in the thesis)}}
\end{itemize}

\section*{Presentation in Conferences and Workshop Attended}
\begin{itemize}
\item
Non-static Cosmological model in $f(R, T)$ gravity, \textit{International Conference on General Relativity}, held at Department of Mathematics, Amravati University, Amravati during 25th-28th Nov., 2015.
\item
Attended workshop on \textit{Cosmological and theoretical applications of exact solutions of Einstein’s equations}, held at Centre for Theoretical Physics, JMI, New Delhi during 12th-23rd Feb., 2016.
\item
Attended workshop on \textit{Introductory Workshop on Astrophysics and Cosmology}, held at Aliah University, Kolkata during 27th -28th Sept., 2016.
\item
Attended workshop on \textit{Structure Formation in standard Cosmology}, held at Department of Mathematics, BITS-Pilani Hyderabad Campus during 19th -23rd Dec., 2016.
\item
Anisotropic cosmological reconstruction in $f(R, T)$ gravity,  \textit{National Workshop on Celebrating Centenary of Einstein's  General Relativity-2017 : Hundred years with $\Lambda$} ,held at Department of Mathematics, University of Burdwan, Kolkata during 26th Jul.-1st Aug., 2017.
\item
Dynamics of anisotropic universe in $f(R,T)$ gravity with hybrid scale factor, \textit{National conference on Differential Geometry and General Relativity}, held at Department of Mathematics, Sardar Patel University, Anand, Gujarat during 28th -29th Nov., 2017.
\item
Dynamical features of an anisotropic cosmological model, \textit{30th meeting of the Indian Association of General Relativity and Gravitation}, held at Department of Physics, BITS-Pilani, Hyderabad Campus during 3rd-5th Jan., 2019.
\end{itemize}
\vfill

==> Report_format_thesis/Certificate.tex <==
\pagestyle{empty} 
\begin{center} 
\vspace{0.25in} 

{\Large\bf CERTIFICATE}\\ 
\end{center} 
\vspace{0.22in} 
\normalsize{\par This is certified that, the thesis entitled
\emph{\bf  "Investigation of late time dynamics of our universe along with anisotropic dark energy models"}, which is a 
record of bonafide work carried out by
\emph{\bf Mr. Pratik Premadarshi Ray} under my supervision and guidance for the degree of \emph{\bf Doctorate of Philosophy in Mathematics} in \emph{\bf Dept. of Mathematics, Birla Institute of Technology and Science-Pilani, Hyderabad Campus}. To the best of my knowledge and belief, the thesis embodies the work of the candidate herself, has duly been completed, fulfils the requirment of the ordinance relating to the Ph.D degree of the university and is up to the standard both in respect of contents and language for being refered to the examiner. 


\vspace{1.5in} 
\vfill
                                                                                
\begin{tabular}{c}
 \noindent
\hspace*{2in} {\large \sc Dr. Bivudutta Mishra,}\\
\hspace*{2in} Supervisor\\
\hspace*{2in} Associate Professor, Department of Mathematics,\\
\hspace*{2in} BITS- Pilani University, Hyderabad Campus, Hyderabad, India\\
\hspace*{2in} \today
\end{tabular}
\vfill
\vfill
\begin{tabular}{c}
 \noindent
\hspace*{2in} {\large \sc Dr. Pradyumn Kumar Sahoo,}\\
\hspace*{2in} Co-Supervisor\\
\hspace*{2in} Associate Professor, Department of Mathematics,\\
\hspace*{2in} BITS- Pilani University, Hyderabad Campus, Hyderabad, India\\
\hspace*{2in} \today
\end{tabular}
\vfill
\vfill

\newpage


==> Report_format_thesis/Chapter1.tex <==
\chapter{Introduction}

\pagebreak



\section{ Introduction}




\section{Einstein's general theory of relativity}




\section{Dark energy}

\subsection{DE models}

\subsection{Chaplygin gas}

\subsection{Holographic DE}

\subsection{Pilgrim DE}

\subsection{Modified holographic Ricci DE}





\section{Problems investigated}



\section{Summary}



 

==> Report_format_thesis/Chapter2.tex <==

\lhead{\fancyplain{}{\nouppercase{\rightmark }}}
\chapter{Modeling the universe: Theoretical framework followed by mathematical formalism }
\vspace{5cm}

%\footnote{rwgheihgeiugheo}

\pagebreak

This chapter aims to frame a solid background on anisotropic DE universes with followed by Bianchi type space-times. The necessities of preferring Bianchi models, especially Bianchi V type, are discussed in detail. A brief literature survey, based on Bianchi models, have been carried out in this chapter. The mathematical formalism to frame the cosmological model has been presented at the back drop of GR.     

\section{Introduction}

The simplest model of the observed universe is well represented by  Friedmann – Lemaître –  Robertson – Walker (FLRW) models, which are both spatially homogeneous and isotropic. These models are good in sense of global approximation of the universe. But it is also believed that in early universe the FLRW model does not give a correct matter description. The anomalies found in the CMB and the large structure observations stimulated a growing interest in anisotropic cosmological models of universe. Observations by the Differential Microwave Radiometers on Cosmic Background Explorer (COBE) registered anisotropy in various angle scales. Ellis \cite{ellis06} pointed out that although the observed universe seems to be almost isotropic on large scales, the early and very late universe could be anisotropic. Moreover, this interest is encouraged in recent years due to the argument that going on the analysis and the interpretation of anisotropic  WMAP data. 

Hence, all these observations need a Bianchi type morphology which resolve the issue of the departure from global isotropy \cite{bianchi98}. Bianchi universes are the class of cosmological models that are homogeneous but not necessarily isotropic on spatial slices, named after Luigi Bianchi. These are generalization of open FRW universe where the spatial isotropy is relaxed. Thus, in recent years Bianchi universes have been gaining an increasing interest of observational cosmology. Besides, maximal spatial symmetry of the FRW metrics do not allow the theoretical study of cosmological models containing anisotropic fluids as long as fluids are co-moving.  Therefore, spatially anisotropic space-times are considered to study the cosmological anisotropic energy momentum sources such as bulk viscous fluid, cosmic strings, magnetic field as well as hypothetical fluids considered in the context of DE. 

\section{Anisotropic cosmology}
Experimental studies of the isotropy of the CMB radiation and reflection of the amount of helium formed in the initial stages of the evolution of the universe, stimulated theoretical study of anisotropic cosmological models. At present stage of evolution the universe is spherically symmetric and the distribution of matter in it is generally isotropic and homogeneous. But in the early stages of evolution the picture might not be as smooth as near the Big Bang singularity. The assumption of spherical symmetry and isotropy could not be strictly valid. The anisotropy of the cosmic expansion, which is supposed to disappear with time, is a very important quantity. Recent experimental data as well as theoretical arguments support the existence of anisotropic expansion phase. DE is also associated with the breakdown of global isotropy and can display small scale anisotropic features. This very facts generate interest to study evolution of the universe with the anisotropic background. 

Mostly, cosmologists use the term anisotropy to describe the uneven temperature distribution of the cosmic microwave background radiation. There are several indications of departures from statistical anisotropy across the CMB sky through some anomalous behavior. Employing the Union compilation of Type Ia Supernovae, a weak anisotropy is found in dark energy, mostly observable for higher redshift group ($z>0.56$,) towards the CMB dipole. According to WMAP data, departure from global isotropy with asymmetric expansion has been claimed. The preliminary Planck data show a slight redshit of the power spectrum from exact scale invariance. Cosmic anisotropy has also been seen in the alignment of galaxies' rotation axes and polarization angles of quasars. The first anisotropic models to study the realistic cosmological problems was used by Lemaitre \cite{lemaitre33}. The aim of his work was to investigate whether the Big Bang singularity in the FRW model is simply the consequence of the proposed symmetry. Zel’dovichv\cite{zeldovich70} and Thorne \cite{thorne66} discussed the probability of a primordial magnetic field  considering the anisotropic models. Similarly, Hawking and Tayler \cite{hawking66} studied about the factors in anisotropic models that can influence on the quantity of primordial helium in the Bing Bang cosmology. Kristian and Sachs \cite{kristian66} as well as Kantowski and Sachs \cite{kantowski66} considered the anisotropic models in order to study the degree of isotropy of our Universe.

The sources with anisotropic stresses have been rarely studied in cosmology until recent years. Barrow and Maartens \cite{barrow97,barrow99} have investigated the effects of some known anisotropic stresses according to cosmological evolution. Moreover, various discussions \cite{cruz07,hoftuft09} have promoted the general interest not only in the Bianchi type cosmological models but also in the possibility of anisotropic nature of the DE. These discussions conclude that WMAP data need a Bianchi type morphology rather than FRW type for more successful explanation of anisotropic evolution. Recently, Campanelli et al. \cite{campanelli11a,campanelli11b} investigated the possibility that a DE component with anisotropic EoS could generate an ellipsoidal Universe with the correct characteristics to explain the low quadrupole in the CMB fluctuations. They proposed that an ellipsoidal Universe allowed better matches with the large scale CMB anisotropy data. This idea is also consistent with their more recent study \cite{campanelli11b}, where they analyzed the magnitude redshift data of SNIa included in the Union catalog by considering Bianchi type I space-time in the presence of a DE fluid with anisotropic EoS. Axelsson et al. \cite{axelsson11} studied possible imperfect nature of DE and the large angle anomalous features in the CMB by considering seven years' WMAP temperature observations data. 

Based on evidences of anisotropic red-shift observations, a special kind of metric have been proposed that describes the observations best. Those are known as Bianchi type space-times, which are homogeneous as well as anisotropic in nature. These models appropriately introduce anisotropic DE candidates to break the spatial isotropy of the Universe. Moreover, yielding anisotropic pressure, the fluids considered in the context of DE, may produce results that can be produced in the presence of isotropic fluid in accordance with the $\Lambda$CDM cosmology. Also, calculations of nucleosynthesis and microwave background anisotropies in Bianchi models have been compared against data from the real Universe. 

\section{Bianchi universes}

Bianchi models provide the basis of modern cosmological models as the zeroth approximation. In quantum gravity and quantum cosmology, these models are called the minisuperspace models. In many of the investigations in these fields, topological features of models have been neglected and models with the simplest space topology have been treated. Such treatments are allowed if the interest is only in local structures and dynamics of models. However, to study global structures and dynamics of models, the effects of space topology must be taken into account. In particular, when a minisuperspace model in quantum gravity is considered, a Bianchi model with compact space used in order to make the canonical variables well defined.
When Bianchi models with non-trivial topologies are considered, various new features arise. First, space topology is strongly restricted by the Bianchi type. In particular, there exists no spatially compact model that has local symmetry of the Bianchi type IV or VIh . Second, there appear new dynamical degrees of freedom called the moduli, which describe the degrees of freedom when the global structure of space is deformed, while preserving the local structure and the topology.  This is a higher dimensional analogue of the well-known moduli freedom for the flat 2-dimensional torus. This appearance of the moduli freedom is very important in the analysis of minisuperspace models based on Bianchi models,
because it significantly alters the canonical structure and dynamics of the systems.

Moreover, in recent years Bianchi universes have been gaining an increasing interest of observational cosmology, since the WMAP data seem to require an addition to the standard cosmological model with positive cosmological constant that resembles the Bianchi morphology \cite{jaffe06,campanelli07,akarsu11}. According to this, the universe should achieved a slightly anisotropic special geometry in spite of the inflation, contrary to generic inflationary models and that might be indicating a non-trivial isotropization history of universe due to the presence of an anisotropic energy source. In principle, once the metric is generalized to Bianchi types, the EoS parameter of the fluid can also be generalized in a way conveniently to wield anisotropy with the considered metric. Goliath and Ellis \cite{goliath99} have shown that some Bianchi models isotropise due to inflation. For example flat and open FRW models are particular case of Bianchi type I, V respectively. In such models, where both the metric and EoS parameter of the fluid are allowed to exhibit an anisotropic character, the universe can exhibit non trivial isotropization histories and it can be examined whether the metric or the EoS parameter of fluid evolve toward isotropy. Thus, the Bianchi models which remains anisotropic are of rather academical interest.
Also, these models remain widely studied for their homogeneity property in space. This implies that the Einstein equations reduce from partial to ordinary differential equations in time, making them tractable exact solutions of Einstein's field equation.

\subsection{Classifications and aspects}
 
Here we give a short description about all Bianchi models as well as their importance  in observational universe based on few considerations. The metric form of all Bianchi types are given below:

Bianchi type-I metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+B^{2}dy^{2}+C^{2}dz^{2},
\end{equation}
Locally Rotationally Symmetric Bianchi type-I metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+B^{2}(dy^{2}+dz^{2}),
\end{equation}
Bianchi type-II metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}(dx-zdy)^{2}+B^{2}dy^{2}+C^{2}dz^{2},
\end{equation}
Bianchi type-III metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+B^{2}e^{-2\alpha x}dy^{2}+C^{2}dz^{2},
\end{equation}
where  $\alpha$ is a constant.\\
Bianchi type-IV metric:
\begin{equation}
ds^{2}=-dt^{2}+e^{-2z}[Adx^{2}+(Az^{2}B)dy^{2}+2Azdxdy]+C^{2}dz^{2},
\end{equation} 
Bianchi type-V metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+e^{2\alpha x}(B^{2}dy^{2}+C^{2}dz^{2}),
\end{equation}
Bianchi type-$VI_{0}$ metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+B^{2}e^{-2\alpha x}dy^{2}+C^{2}e^{2\alpha x}dz^{2},
\end{equation}

Bianchi type-$VII_{0}$ metric: 
\begin{equation}
ds^{2}=-dt^{2}+(Acos^{2}z+B sin^{2}Z)dx^{2}+(Asin^{2}z+Bcos^{2}z)dy^{2}+(A+B)sin2zdxdy+Cdz^{2},
\end{equation}
Bianchi type-VIII metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+B^{2}dy^{2}+(A^{2}sinh^{2}y+B^{2}cosh^{2}y)dz^{2}-2B^{2}coshydxdz,
\end{equation}
Bianchi type-IX metric:
\begin{equation}
ds^{2}=-dt^{2}+A^{2}dx^{2}+B^{2}dy^{2}+(B^{2}sin^{2}y+A^{2}cos^{2}y)dz^{2}-2A^{2}cosydxdz,
\end{equation}

For the homogeneous Bianchi space time in all cases above $A$, $B$, $C$ are the directional scale factors and functions of cosmic time $t$ alone. In the following research topics, these space-times are used\\
One can mention :
\begin{itemize}
\item Supernova of type Ia observations.
\item Cosmic microwave background radiation.
\item Growth of inhomogeneities and the large scale structure of the universe.
\item Statistics of gravitational lensing.
\item X-ray luminosity of galaxy clusters.
\item Age restrictions from high redshift objects.
\item New methods of diagnostics of the dark energy equation of state for future supernovae observations.
\end{itemize}

Exact general relativistic cosmological models in the presence of anisotropic fluid, in the context of DE, using kinematical ansatze have been studied in the framework of various Bianchi metrics. %Bianchi I [29, 30, 35, 36, 37, 38], Bianchi VI0 [39, 40, 41, 42, 43], Bianchi III [31, 44, 45], Bianchi V [46, 47], Bianchi VI [32] and locally rotationally symmetric (LRS) Bianchi type II [51].Such models have also been studied in f(R) theory of gravity instead of GR within the framework of Bianchi VI0 [52] and Bianchi III [53] metrics. [] Showed that the compact Bianchi models of the types V, VIIh and IX have no moduli freedom. 
As is well known, among the Bianchi models with simply connected spaces, the types VIh, VIII and IX are the most generic models, both for the vacuum and the fluid cases, in the sense that the dimension of the solution space is the largest. Further, the Bianchi type VII0 is more general than the type I in the same sense. This generality argument based on the parameter count is the starting point of the isotropization problem in spatially homogeneous cosmology and it also plays a basic role in mathematical cosmology[132]. However, the situation drastically changes when the space is compactified. 

Luigi Bianchi \cite{bianchi98} introduced the classifications of Bianchi universes as spatially homogeneous space times with three parameter isometry group acting on spatial slices. Ellis and MacCullum \cite{ellis69} and Krasinski et al.\cite{krasinski03}  have classified the Bianchi cosmologies in two classes: class A and class B and then further divided into subgroups using the eigenvalues of the matrix.  Then Taub \cite{taub51}has introduced explicitly the nine types of Bianchi models, which are necessarily spatially homogeneous. In particular, the type V becomes the most generic among all types.
 

\subsection{Significance of Bianchi V type}

Among all nine space-times of Bianchi, Bianchi V space-time is very intuitive as it has least degrees of freedom characterized by Lie groups and generates pseudo spherical space. The study of Bianchi type V cosmological models create more interest as these models contain isotropic special cases and permit arbitrary small anisotropy levels at some instant of cosmic time. This property makes them suitable as model of our universe. The general form of Bianchi V space-time is given as, 
\begin{equation}  \label{eq1}
ds^{2}= dt^{2}-\sum_{i=1}^{3}e^{2a_{i}x}b_{i}^{2} dx_{i}^{2}
\end{equation}
where, $b_{i}=b_i(t),i=1,2,3$ are the directional scale factors considered to be different along three orthogonal directions and thereby provide a source for anisotropic expansion. In our thesis, we choose $a_1=0,$ $a_{2}=a_{3}=a,$ $a$ being a non zero arbitrary constant to obtain axially symmetric and simply anisotropic Bianchi V type universe. Hence, this model has axially anitropies already contained in it. To investigate about behavior of anisotropic DE models, the job is now reduced only to constructed the field equations of the model considering DE and/or baryonic fluids along R.H.S of Einstein's equation. 
 
The Bianchi type -V locally rotationally symmetric cosmologies (LRS type V) have commanded the attention of many researchers during the past decade. The reason is that, while their dynamical behavior can be far more general than the simple FRW and Bianchi type I models, they are still less complicated than the Bianchi types V,VI and IX. These properties make the models suitable as models of our universe.

Collins and Hawking \cite{collins73} suggested that out of these nine Bianchi types, Bianchi types V can tend towards isotropy at an arbitrarily large times. Therefore, it permits the formation of galaxies. Koike et al. \cite{koike94}. Hence, it is interesting to see how the introduction of fluid alters the parameter count and to extend the analysis to the Bianchi types V universe.
 
\section{Mathematical formulation to generate a anisotropic DE universe}

To frame any cosmological model, we need three basic tools: one theory to govern the evolution equations, one space-time to analyze the geometry of universe and one or mixture of matter sources to observe its behavior through out the evolution. In order to construct an anisotropic DE cosmological model in the back drop of GR, we have considered  Bianchi type V space-time in the form, 

\begin{equation} \label{eq:2.1}
ds^{2}= dt^{2}-a_1^2 dx^2-e^{2\alpha x}\left(a_2^2 dy^2+a_3^2 dz^2\right)
\end{equation}
where, the directional scale factors $a_i (i=1,2,3)$ are functions of cosmic time only, $a_i=a_i(t)$. In general, $a_i$s are considered to be different and thereby provide a description for anisotropic expansions along the three orthogonal spatial directions. The model reduces to FRW model when the directional scale factors become equal. Here, $\alpha$ is a non zero arbitrary positive constant. We choose the unit system such that $8\pi G=c=1$, $G$ is the Newtonian gravitational constant and $c$ is the speed of light.


In contrast to the isotropic pressure of usual cosmic fluid, we wish to incorporate some degree of anisotropy in the DE pressure and consider the energy momentum tensor for DE as

\begin{eqnarray} \label{eq:2.2}
T^{DE}_{\mu\nu} & = & diag[-\rho_{DE}, p_{DE_x},p_{DE_y},p_{DE_z}] \nonumber\\ 
			  & = & diag[-1, \omega_{DE_x},\omega_{DE_y},\omega_{DE_z}]\rho_{DE}\\ \nonumber
			  & = & diag[-1, \omega_{DE}+\delta,\omega_{DE}+\gamma,\omega_{DE}+\eta]\rho_{DE} ,
\end{eqnarray}
where $\omega_{DE}$ is the DE equation of state parameter and $\rho_{DE}$ is the DE density. The skewness parameters $\delta$, $\gamma$ and $\eta$ are the deviations from $\omega_{DE}$ along $x$, $y$ and $z$ axes respectively. The DE pressure becomes isotropic when $\delta$, $\gamma$ and $\eta$ vanish identically.

In order to construct the evolution equations, we need to calculate few tensorial terms based on physical space geometry applications, which are presented below. 

\subsubsection{Christoffel symbols}

Christoffel's equation is given by,

\begin{align}
\Gamma^{l}_{jk}=g^{lm}\Gamma_{m, jk}=\frac{1}{2}g^{lm}\left(\frac{\partial g_{jm}}{\partial x^{k}}+\frac{\partial g_{km}}{\partial x^{j}}-\frac{\partial g_{jk}}{\partial x^{m}}\right)
\end{align}


Hence, the non-vanishing symmetric Christoffel symbols are:

$$\Gamma^{1}_{14}=\frac{1}{2}g^{11}\left(\frac{\partial g_{11}}{\partial x^{4}}+\frac{\partial g_{41}}{\partial x^{1}}-\frac{\partial g_{14}}{\partial x^{1}}\right)=\frac{\dot{a_{1}}}{a_{1}}= \Gamma^{1}_{41} $$

$$\Gamma^{1}_{22}=\frac{1}{2}g^{11}\left(\frac{\partial g_{21}}{\partial x^{2}}+\frac{\partial g_{21}}{\partial x^{2}}-\frac{\partial g_{22}}{\partial x^{1}}\right)= - \frac{a_{2}^{2}}{a_{1}^{2}} \alpha e^{2 \alpha x}$$

$$\Gamma^{1}_{33}=\frac{1}{2}g^{11}\left(\frac{\partial g_{31}}{\partial x^{3}}+\frac{\partial g_{31}}{\partial x^{3}}-\frac{\partial g_{33}}{\partial x^{1}}\right)=-\frac{ a_{3}^{2}}{a_{1}^{2}}\alpha e^{2 \alpha x}$$

$$\Gamma^{2}_{12}=\frac{1}{2}g^{22}\left(\frac{\partial g_{12}}{\partial x^{2}}+\frac{\partial g_{22}}{\partial x^{1}}-\frac{\partial g_{12}}{\partial x^{2}}\right)= \alpha = \Gamma^{2}_{21}$$

$$\Gamma^{2}_{24}=\frac{1}{2}g^{22}\left(\frac{\partial g_{22}}{\partial x^{4}}+\frac{\partial g_{42}}{\partial x^{2}}-\frac{\partial g_{24}}{\partial x^{2}}\right)=\frac{\dot{a_{2}}}{a_{2}}= \Gamma^{2}_{42}$$

$$\Gamma^{3}_{13}=\frac{1}{2}g^{33}\left(\frac{\partial g_{13}}{\partial x^{3}}+\frac{\partial g_{33}}{\partial x^{1}}-\frac{\partial g_{13}}{\partial x^{3}}\right)= \alpha = \Gamma^{3}_{31} $$

$$\Gamma^{3}_{34}=\frac{1}{2}g^{33}\left(\frac{\partial g_{33}}{\partial x^{4}}+\frac{\partial g_{34}}{\partial x^{3}}-\frac{\partial g_{34}}{\partial x^{3}}\right)=\frac{\dot{a_{3}}}{a_{3}}= \Gamma^{3}_{43}$$

$$\Gamma^{4}_{11}=\frac{1}{2}g^{44}\left(\frac{\partial g_{14}}{\partial x^{1}}+\frac{\partial g_{14}}{\partial x^{1}}-\frac{\partial g_{11}}{\partial x^{4}}\right)=a_{1}\dot{a_{1}}$$

$$\Gamma^{4}_{22}=\frac{1}{2}g^{44}\left(\frac{\partial g_{24}}{\partial x^{2}}+\frac{\partial g_{24}}{\partial x^{2}}-\frac{\partial g_{22}}{\partial x^{4}}\right)= a_{2} \dot{a_{2}}e^{2 \alpha x}$$

$$\Gamma^{4}_{33}=\frac{1}{2}g^{44}\left(\frac{\partial g_{34}}{\partial x^{3}}+\frac{\partial g_{34}}{\partial x^{3}}-\frac{\partial g_{33}}{\partial x^{4}}\right)=a_{3}\dot{a_{3}} e^{2 \alpha x}$$


\subsubsection{Ricci tensor and Ricci scalar}

Formula to get Ricci tensor is given as,
\begin{align}
R_{ij}=R^{a}_{ij},a=\frac{\partial}{\partial x^{j}}\Gamma^{b}_{ib}-\frac{\partial}{\partial x^{b}}\Gamma^{b}_{ij}+\Gamma^{a}_{ib}\Gamma^{b}_{ja}-\Gamma^{a}_{ij}\Gamma^{b}_{ab}
\end{align}

The non-vanishing Ricci tensors are obtained as,

$$R_{11}=\frac{\partial}{\partial x^{1}}\Gamma^{b}_{1b}-\frac{\partial}{\partial x^{b}}\Gamma^{b}_{11}+\Gamma^{a}_{1b}\Gamma^{b}_{1a}-\Gamma^{a}_{11}\Gamma^{b}_{ab}= 2 \alpha^{2} - a_{1} \ddot{a_{1}}-\frac{a_{1}\dot{a_{1}}\dot{a_{2}}}{a_{2}}-\frac{a_{1}\dot{a_{1}}\dot{a_{3}}}{a_{3}}$$

$$R_{14}=\frac{\partial}{\partial x^{4}}\Gamma^{b}_{1b}-\frac{\partial}{\partial x^{b}}\Gamma^{b}_{14}+\Gamma^{a}_{1b}\Gamma^{b}_{4a}-\Gamma^{a}_{14}\Gamma^{b}_{ab}=\frac{\alpha \dot{a_{2}}}{a_{2}}+\frac{ \alpha \dot{a_{3}}}{a_{3}} - 2 \dfrac{\alpha \dot{a_{1}}}{a_{1}}$$

$$R_{22}=\frac{\partial}{\partial x^{2}}\Gamma^{b}_{2b}-\frac{\partial}{\partial x^{b}}\Gamma^{b}_{22}+\Gamma^{a}_{2b}\Gamma^{b}_{2a}-\Gamma^{a}_{22}\Gamma^{b}_{ab}= a_{2} e^{2 \alpha x} \left( \dfrac{2 \alpha^{2} a_{2}}{a_{1}^2} - \ddot{a_{2}} - \dfrac{\dot{a_{1}} \dot{a_{2}}}{a_{1}}- \dfrac{\dot{a_{2}} \dot{a_{3}}}{a_{3}} \right)$$

$$R_{33}=\frac{\partial}{\partial x^{3}}\Gamma^{b}_{3b}-\frac{\partial}{\partial x^{b}}\Gamma^{b}_{33}+\Gamma^{a}_{3b}\Gamma^{b}_{3a}-\Gamma^{a}_{33}\Gamma^{b}_{ab}=a_{3} e^{2 \alpha x} \left( \dfrac{2 \alpha^{2} a_{3}}{a_{1}^2} - \ddot{a_{3}} - \dfrac{\dot{a_{1}} \dot{a_{3}}}{a_{1}}- \dfrac{\dot{a_{2}} \dot{a_{3}}}{a_{2}} \right)$$

$$R_{44}=\frac{\partial}{\partial x^{4}}\Gamma^{b}_{4b}-\frac{\partial}{\partial x^{b}}\Gamma^{b}_{44}+\Gamma^{a}_{4b}\Gamma^{b}_{4a}-\Gamma^{a}_{44}\Gamma^{b}_{ab}=\frac{\ddot{a_{1}}}{a_{1}}+\frac{\ddot{a_{2}}}{a_{2}}+\frac{\ddot{a_{3}}}{a_{3}}$$

Hence, the Ricci scalar can be formed as,

$$R=\sum_{i,j=1}^{4} R_{ij}g^{ij}=2\left(\frac{\ddot{a_{1}}}{a_{1}}+\frac{\ddot{a_{2}}}{a_{2}}+\frac{\ddot{a_{3}}}{a_{3}}\right)+2\left(\frac{\dot{a_{1}}\dot{a_{2}}}{a_{1} a_{2}}+\frac{\dot{a_{2}}\dot{a_{3}}}{a_{2} a_{3}}+\frac{\dot{a_{1}}\dot{a_{3}}}{a_{1} a_{3}}\right)-\frac{6 \alpha_{2} }{a_{1}^{2}}$$


\subsubsection{Einstein tensor}

The tensorial part in L.H.S of Einstein's equation of GR \eqref{EGR6} is known as Einstein tensor, given as,
$$G_{ij}=R_{ij}-\frac{1}{2}R g^{ij}$$

So, now the non-vanishing Einstein tensors are


$$G_{11}=R_{11}-\frac{1}{2}Rg_{11}=a_{1}^{2}\left(\frac{\ddot{a_{2}}}{a_{2}}+\frac{\ddot{a_{3}}}{a_{3}}+\frac{\dot{a_{2}}\dot{a_{3}}}{a_{2} a_{3}}- \alpha^{2} \right)$$

$$G_{14}=R_{14}-\frac{1}{2}Rg_{14}= \alpha \left( \frac{\dot{a_{2}}}{a_{2}}+\frac{\dot{a_{3}}}{a_{3}}-\frac{2 \dot{a_{1}}}{a_{1}} \right)$$

$$G_{22}=R_{22}-\frac{1}{2}Rg_{22}= a_{2}^{2} e^{2 \alpha x} \left(\frac{\ddot{a_{1}}}{a_{1}}+\frac{\ddot{a_{3}}}{a_{3}}+\frac{\dot{a_{1}}\dot{a_{3}}}{a_{1} a_{3}}-\frac{\alpha^{2}}{a_{1} ^{2}}\right)$$

$$G_{33}=R_{33}-\frac{1}{2}Rg_{33}=a_{3}^{2} e^{2 \alpha x} \left(\frac{\ddot{a_{1}}}{a_{1}}+\frac{\ddot{a_{2}}}{a_{2}}+\frac{\dot{a_{1}}\dot{a_{2}}}{a_{1} a_{2}}-\frac{\alpha^{2}}{a_{1}^{2}}\right)$$

$$G_{44}=R_{44}-\frac{1}{2}Rg_{44}=-\frac{\dot{a_{1}}\dot{a_{2}}}{a_{1} a_{2}}-\frac{\dot{a_{2}}\dot{a_{3}}}{a_{2}a_{3}}-\frac{\dot{a_{1}}\dot{a_{3}}}{a_{1} a_{3}}+\frac{3 \alpha^{2}}{a_{1}^{2}}$$





\subsubsection{The evolution equations}

Since all terms needed to calculate the Eintein field equations have already defined, we can express the set of evolution equations for our model, incorporating \eqref{EGR6}, as;

\begin{equation}
\frac{\ddot{a_2}}{a_2}+\frac{\ddot{a_3}}{a_3}+\frac{\dot{a_2}\dot{a_3}}{a_2a_3}-\frac{\alpha^{2}}{a_1^{2}}=T_{11}  
\end{equation} 

\begin{equation}
\frac{\ddot{a_1}}{a_1}+\frac{\ddot{a_3}}{a_3}+\frac{\dot{a_1}\dot{a_3}}{a_1a_3}-\frac{\alpha^{2}}{a_1^{2}}=T_{22}
\end{equation}

\begin{equation}
\frac{\ddot{a_1}}{a_1}+\frac{\ddot{a_2}}{a_2}+\frac{\dot{a_1}\dot{a_2}}{a_1a_2}-\frac{\alpha^{2}}{a_1^{2}}=T_{33}
\end{equation}

\begin{equation}
\frac{\dot{a_1}\dot{a_2}}{a_1a_2}+\frac{\dot{a_2}\dot{a_3}}{a_2a_3}+\frac{\dot{a_3}\dot{a_1}}{a_3a_1}-\frac{3\alpha^{2}}{a_1^{2}}=T_{44}
\end{equation}

\begin{equation} 
2\frac{\dot {a_1}}{a_1}-\frac{\dot{a_2}}{a_2}-\frac{\dot{a_3}}{a_3}=T_{14},
\end{equation}
where an over dot represents the differentiation with respect to time $t$. 
%One can note that, anisotropy is incorporated in two different manner in the field equations: one due to the inherent anisotropic DE fluid and the other through the presence of aligned cosmic strings along x-axis. These anisotropic components leads to the anisotropy in the cosmic geometry described through the BV space time. 

\section{Requirement of mix-fluid along with their energy- momentum tensors}
 
It is well known that the EMT characteristics physical property of universe and its divergence vanishes $(\bigtriangledown_{b} T^{ab}=0).$ However, some models, studied by considering EMT of perfect fluid or individual ordinary matters are failed to describe the complete evolution of accelerating universe. This gives raise to an idea that since universe is textured with various celestial matters and energy, the
mixture of fluid or matter can be considered in the R.H.S of Einstein equation. Moreover, early epoch dominated cosmic fluids (viscous fluid, cosmic string, magnetic fluid etc.) that contribute to matter of universe can be considered along with DE fluid. As investigations shows that DE is dominant towards late phase of cosmic evolution, then the combination of these fluids may give an insight to the transition from early deceleration epoch to present acceleration phase.\\

Xin \cite{xin05} studied an interacting two-fluid scenario for quintom dark energy. Xin-He et al. \cite{xin-He07} considered Friedmann cosmology with a generalized EoS and bulk viscosity to explain DE dominated universe. Recently, several authors \cite{rong09,khodam11} have examined and discussed the DE models in different context of combination of two fluids. Moreover, spatially homogeneous but totally anisotropic and non-flat Bianchi type V cosmological model has been studied in general relativity in the presence of two minimally interacting fluids; a baryonic fluid as the matter fluid and a hypothetical anisotropic fluid as the dark energy fluid. Inspired by the above discussion, in this thesis, we consider combination of two non interacting fluids that contribute to the matter in the R.H.S of Einstein's equation \eqref{EGR6}.
Thus \eqref{eq:2.2} will be reconstructed as the energy momentum tensor for an environment of two non interacting fluids, given by,
\begin{equation}\label{eq:3}
T_{\mu\nu}=T_{\mu\nu}^{MS}+T_{\mu\nu}^{DE} 
\end{equation}
where $T_{\mu\nu}^{MS}$ and $T_{\mu\nu}^{D}$ respectively denote the contribution to energy momentum tensor from matter source and DE.

%cases wrt matter fluid

\section{Conclusion}

In this chapter, we have discussed the necessity of studying anisotropic universe. We have gone though well behaving cases of few literature where the anisotropy of the expansion and the anisotropy of the fluid converge to finite values in the late Universe. We have also showed that although the metric we consider is totally anisotropic, the anisotropy of the dark energy is constrained to be axially symmetric, as long as the overall energy momentum tensor possesses zero shear stress. Then we have explained the evolution of various Bianchi type models which triggered enormous research areas recently.

Moreover, Some new exact solutions of Einstein’s field equations in a spatially homogeneous and anisotropic Bianchi type V space-time with minimally interaction of matter fluid and dark energy components have been obtained. We have developed a technique of construction of these exact solutions. Formulation of field equations followed by few important tensor tools have been calculated in detailed followed by their significance in cosmology. Applications of mix fluid character along with DE models  have been analyzed.

Using the above facts as a starting point, in the subsequent chapters, we will investigate anisotropic dark energy cosmological models based two fluid situations Physical and geometric properties of spatially homogeneous and anisotropic cosmological models are  also discussed and shown a new path to answer few unsolved problems till today.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







==> Report_format_thesis/Chapter3.tex <==
\chapter{Dynamics of anisotropic DE Universe with Bulk Viscous fluid in power law and de-Sitter cosmology}

\footnote{\bf{The contents of this chapter has been published in Advances in High Energy Physics, \textbf{2018}, 63068484 (2017)}}


\pagebreak

Following the aim of our thesis, we are interested to study the behavior of anisotropy Bianchi universe in the DE cosmological model treated with different sources of matter fluid. In the present chapter, we start considering the barotropic bulk viscous fluid to exert an anisotrpy to the model along with DE. This experiment shows very important results in terms of dynamical behavior of our universe that resembles with present day observations.

\section{Introduction} 

Many researchers extensively studied the evolution of isotropic cosmological models with perfect fluid; however it would be worthy to study cosmology with richer structure both geometrically and physically than the standard perfect fluid models. Bulk viscosity is such a dissipative phenomena that plays an important role in the study of accelerated expansion of the universe. Viscous fluid models have been used in an attempt to explain the observed highly isotropic matter distribution on the high entropy per baryon in the present state of the universe. The strong dissipation due to neutrino viscosity may considerably reduce the anisotropy of black body radiation. The viscosity mechanism in cosmology can explain the anomalously high entropy per baryon in the present universe. There have been considerable interests in cosmological models with bulk viscosity, since bulk viscosity leads to the accelerated expansion phase of the early universe, popularly known as the inflationary phase. Several cosmological models were obtained with constant deceleration parameter where the matter is in the form of perfect fluid or ordinary matter. However, many of those matters are not enough to describe the dynamics of an accelerating universe relating to anisotropy. This motivates us to consider the model of the accelerating universe filled with non-interacting fluids \cite{tripathy017}. Akarsu and Kilinc \cite{akarsu010a, akarsu010b} have assumed constant deceleration parameter to construct and investigate DE models in Bianchi I and Bianchi III space-time. Theoretical models of interacting and non-interacting DE along with viscous fluid have been discussed widely in the literature \cite{amirhashchi013, pradhan011, sheykhi011}. 
 
From an observational viewpoint, one of the most important result is the theorem of Wald \cite{wald84}, which states that universe with accelerating expansion tends towards isotropy at late phase. As a matter of fact, if the universe undergoes an early period of inflation, the present day universe will seem to be highly isotropic. Further, since the universe has now started accelerating, any kind of anisotropy will remain small in the late phase of cosmic acceleration. Bianchi universes are the class of cosmological models that are homogeneous but not necessarily isotropic on spatial slices. It contains, as a subclass, the standard isotropic model known as FRW universe. Calculations of nucleosynthesis and microwave background anisotropies in Bianchi models have been compared against data from the real Universe, typically gives null results which can be translated into upper limits on anisotropy. Tentative detections of non-zero anisotropic shear by Jaffe et al. \cite{jaffe06a} are currently believed to be in consistent with other known cosmological parameters and with polarization of the microwave background in power law cosmology as well as volumetric law cosmology . However these models remain widely-studied for their pedagogical value, mainly, making them tractable exact solutions of Einstein's field equation.

The chapter is  arranged as follows: in section 3.2, a mathematical formalism of an anisotropic DE universe is presented along with the relevant physical parameters. Two dark energy cosmological models one with power law cosmology and the other one with de Sitter universe has been constructed and analysed in section 3.3. The summary is given in section 3.4.
 
\section{Formalism}

In order to construct an anisotropic DE two fluid model in GR, we have Bianchi type V space-time defined in \eqref{eq:2.1}. The EMT of matter fluid for an environment of two non interacting fluids in \eqref{eq:2.2} can now be specified as,

\begin{align}\label{eq:3.1}
T_{\mu\nu}=T_{\mu\nu}^{vis}+T_{\mu\nu}^{DE}.
\end{align} 

Hence, EMT consists of two different components; the barotropic bulk viscous fluid $(T_{ij}^{vis})$ and DE fluid $(T_{ij}^{DE})$. 


In case of barotropic cosmic fluid, the proper pressure $p$ is given as, $p= \xi \rho,$ $(0 \leq \xi \leq 1)$. The pressure with the contribution from bulk viscosity is also directly proportional to energy density, i.e, $3 \zeta H= \epsilon_{0} \rho$, where $\epsilon_{0} \geq 0$ is the proportionality constant \cite{tripathy010, brevik015} and $\zeta u^i_{;i}=3\zeta H$. Hence, the effect of both proper pressure and barotropic bulk viscous pressure together can be expressed as,
\begin{align}\label{eq:3.2}
\bar{p} = p-3 \zeta H = (\xi - \epsilon_{0}) \rho= \epsilon \rho
\end{align}

where $\epsilon$ is the bulk viscous coefficient. One can infer that such a relation bears similarity to the pressure term with the contribution from perfect fluid ($p=\omega \rho$), where $\omega$ is the equation of state parameter for perfect fluid. However, a major part of the EoS in $\bar p$ of the present model comes from barotropic bulk viscosity. So, in no viscosity condition, the pressure term $\bar p$,  reduces to the pressure of perfect fluid. Hence, the EMT for viscous fluid is given as,

\begin{align}\label{eq:3.3}
T_{ij}^{vis}= (\rho + \bar{p}) u_{i}u_{j}- \bar{p} g_{ij}
\end{align}

where, $u^{i}$ is the four velocity vectors of the fluid. It may be noted that there is no observational reasons to conclude that pressure is isotropic in DE. However, since the fluids are co-moving, one may get this isotropic pressure in DE. Subsequently both the DE fluid and EoS parameter are direction dependent. Hence, the EMT of DE fluid is considered in the form,

\begin{align}  \label{eq:3.4}
T_{ij}^{de} &= diag[\rho^{de}, -p^{de}_{x}, -p^{de}_{y}, -p^{de}_{z}]  \notag
\\
&= diag[\rho, -\omega^{de}_{x}, -\omega^{de}_{y}, -\omega^{de}_{z}] \rho^{de}
\notag \\
&= diag[1, -(\omega^{de}+ \delta), -(\omega^{de}+ \gamma), -(\omega^{de}+
\eta)]\rho^{de}
\end{align}

where, $\omega^{de}$ is the EoS parameter of the DE fluid along the dimensional axis $x$,$y$, and $z$. $\rho^{de}$ is the dark energy density. The deviations of $\omega^{de}$ from $x$,$y$, and $z$ axes respectively denotes the skewness parameters $\delta$, $\gamma$ and $\eta$. 


Now, in the presence of EMT, Einstein's field equations \eqref{EGR6} corresponding to Bianchi type V space-time \eqref{eq:2.2} lead to the following set of evolution equations:

\begin{align}
& \frac{\ddot{b_{2}}}{b_{2}}+\frac{\ddot{b_{3}}}{b_{3}}+\frac{\dot{b_{2}}%
\dot{b_{3}}}{b_{2}b_{3}}-\frac{a^{2}}{b_{1}^{2}}=-p+3 \zeta
H-(\omega^{de}+\delta)\rho^{de}  \label{eq:3.5} \\
& \frac{\ddot{b_{1}}}{b_{1}}+\frac{\ddot{b_{3}}}{b_{3}}+\frac{\dot{b_{1}}%
\dot{b_{3}}}{b_{1}b_{3}}-\frac{a^{2}}{b_{1}^{2}}=-p+3 \zeta
H-(\omega^{de}+\gamma)\rho^{de}  \label{eq:3.6} \\
& \frac{\ddot{b_{1}}}{b_{1}}+\frac{\ddot{b_{2}}}{b_{2}}+\frac{\dot{b_{1}}%
\dot{b_{2}}}{b_{1}b_{2}}-\frac{a^{2}}{b_{1}^{2}}=-p+3 \zeta
H-(\omega^{de}+\eta)\rho^{de}  \label{eq:3.7} \\
& \frac{\dot{b_{1}}\dot{b_{2}}}{b_{1}b_{2}}+\frac{\dot{b_{2}}\dot{b_{3}}}{%
b_{2}b_{3}}+\frac{\dot{b_{3}}\dot{b_{1}}}{b_{3}b_{1}}-\frac{3a^{2}}{b_{1}^{2}%
}=\rho+\rho^{de}  \label{eq:3.8} \\
& 2\dfrac{\dot{b_{1}}}{b_{1}}-\dfrac{\dot{b_{2}}}{b_{2}}-\dfrac{\dot{b_{3}}}{%
b_{3}} =0  \label{eq:3.9}
\end{align}
where an over dot over the field variable represents the derivatives with respect to the cosmic time $t$. Moreover, the unit of cosmic time is considered as, 1 unit of cosmic time = 10 billion years. 


\section{Retrieving observational parameters from evolution equations}

In this section, instead of solving the evolution equations, we are interested to know the behavior of few important physical parameters during cosmic evolution. This will help us to analyze the dynamics of the parameters geometrically and graphically. 


The average scale factor $R$ and volumetric scale factor $V$ for the model are respectively $R=(b_1b_2b_3)^\frac{1}{3}$ and $V=R^3=b_1b_2b_3$. \\
The generalized mean Hubble parameter $H$ can be expressed as, 
\begin{align}
H=\frac{\dot{R}}{R}=\frac{1}{3}(H_x+H_y+H_z),
\end{align}
where $H_x=\frac{\dot{b_1}}{b_1}, H_y=\frac{\dot{b_2}}{b_2}$ and $H_z=\frac{\dot{b_3}}{b_3}$ are the directional Hubble parameters in the direction of $x$, $y$ and $z$ respectively. 


Now, the field equations \eqref{eq:3.5} to \eqref{eq:3.9} can be framed in Hubble terms as,

\begin{align}
& \dot{H_{y}}+ \dot{H_{z}}+ H_{y}^{2} + H_{z}^{2} + H_{y}H_{z}-\frac{%
a^{2}}{b_1^{2}} = -\bar{p} - (\omega^{de}+ \delta)\rho^{de}  \label{eq:3.10} \\
& \dot{H_{x}}+ \dot{H_{z}}+ H_{x}^{2} + H_{z}^{2} + H_{x}H_{z}-\frac{%
a^{2}}{b_1^{2}} = -\bar{p} - (\omega^{de}+ \gamma)\rho^{de}  \label{eq:3.11} \\
& \dot{H_{x}}+ \dot{H_{y}}+ H_{x}^{2} + H_{y}^{2} + H_{x}H_{y}-\frac{%
a^{2}}{b_1^{2}} = -\bar{p} - (\omega^{de}+ \eta)\rho^{de}  \label{eq:3.12} \\
& H_{x}H_{y}+ H_{y}H_{z}+ H_{z}H_{x}-\frac{3 a^{2}}{b_1^{2}} = \rho +
\rho^{de}  \label{eq:3.13} \\
& 2H_{x}-H_{y}-H_{z}=0,  \label{eq:3.14}
\end{align}

The energy conservation equation for viscous fluid, $T^{(vis)ij}_{;j}=0$ ,
yields

\begin{equation}  \label{eq:3.15}
\dot{\rho}+3(\bar{p}+\rho)H=0
\end{equation}
The energy conservation equation for dark energy fluid, $T^{ij(de)}_{;j}=0$,
yields

\begin{equation}  \label{eq:3.16}
\dot{\rho}^{de}+3 \rho^{de}(\omega^{de}+1)H+ \rho^{de}(\delta H_x+\gamma
H_y+\eta H_z)=0
\end{equation}
From \eqref{eq:3.15}, incorporating the relation between Hubble parameter and average scale factor we get,   
\begin{align}  \label{eq:3.17}
\rho=\rho_{0} R^{-3(\epsilon +1)}= \rho_{0} (b_{1} b_{2} b_{3})^{-(\epsilon
+1)},
\end{align}
where $\rho_0$ is the integration constant or rest energy density.\newline

From \eqref{eq:3.13}, we have, 
\begin{equation}  \label{eq:3.18}
\rho^{de}= H_{x}H_{y}+H_{y}H_{z}+H_{z}H_{x}-\dfrac{3 a^{2}}{b_{1}^2}- \rho
\end{equation}
In order to solve eqn. \eqref{eq:3.16}, we split the conservation equation into two parts one
corresponds to the deviation of equation of the state parameters as $\rho^{de}(\delta H_x+\gamma H_y+\eta H_z)=0$ and other one is the deviation free part as  $\dot{\rho}^{de}+3 \rho^{de}(\omega^{de}+1)H=0$ \cite{akarsu3}. It can be observed that the behaviour of energy density $\rho^{de}$ is controlled by the deviation free part of EoS parameter whereas anisotropic pressure along different directions can be obtained from second part of the above conservation equation as it corresponds to the conservation of matter field with equal pressure along all directions. Hence, we obtained the dark energy density as,
\begin{equation}  \label{eq:3.19}
\dot{\rho}^{de}+3\rho^{de}(\omega^{de}+1)H=0 \Rightarrow
\rho^{de}=\rho_{0}^{de} R^{-3(\omega^{de}+1)}
\end{equation}


Now from \eqref{eq:3.12}, incorporating the value of $\eta$, we get,

\begin{align}  \label{eq:3.20}
-\omega^{de} \rho^{de}= & \biggl(\frac{H_y+H_z}{3H}\biggr)\frac{\ddot{b_{1}}}{%
b_{1}}+\biggl(\frac{H_x+H_z}{3H}\biggr)\frac{\ddot{b_{2}}}{b_{2}}+\biggl(%
\frac{H_x+H_y}{3H}\biggr)\frac{\ddot{b_{3}}}{b_{3}}+ \\
& \frac{H_z}{3H}\frac{\dot{b_{1}}\dot{b_{2}}}{b_{1}b_{2}}+\frac{H_x}{3H}%
\frac{\dot{b_{2}}\dot{b_{3}}}{b_{2}b_{3}}+\frac{H_y}{3H}\frac{\dot{b_{1}}%
\dot{b_{3}}}{b_{1}b_{3}}-\frac{a^{2}}{b_{1}^{2}}+p-3 \zeta H  \notag
\end{align}

Again from eqn. \eqref{eq:3.9}, with the choice of integrating constant to be unity, we get, $b_{1}^2=b_{2}b_{3}$. Moreover for an anisotropic relation, we assume $b_{2}=b_{3}^m$, where $m$ is the average anisotropy parameter \cite{mishra015a}. Hence,
\begin{equation}  \label{eq:3.21}
b_{1}=b_{3}^{\frac{m+1}{2}}
\end{equation}

Now, the dark energy density and effective EoS parameter with the function $\Phi(H)= \left(\dfrac{2 \dot{H}+3H^{2}}{m+1}\right)$ can be reformulated respectively as 

\begin{align}  \label{eq:3.22}
\rho^{de}=\left[ 2 \dfrac{(m^{2}+4m+1)}{(m+1)^{2}} \right] H^{2}- \dfrac{3
a^{2}}{b_{1}^{2}}- \rho
\end{align}


\begin{align}  \label{eq:3.23}
\omega^{de} \rho^{de}= -\dfrac{2}{3} \left( \dfrac{m^{2}+4m+1}{m+1} \right)
\Phi(H) + \dfrac{a^2}{b_{1}^{2}}-\bar{p},
\end{align}

With the help of eqns. \eqref{eq:3.17}-\eqref{eq:3.20}, eqns. \eqref{eq:3.10}-\eqref{eq:3.12} can be expressed in functional form, known as skewness parameters, as: 
\begin{eqnarray} 
\gamma = \left(\frac{5+m}{6 \rho^{de}} \right) \chi(m) F(H) \label{eq:3.24}\\
\eta = - \left( \frac{5m+1}{6 \rho^{de}} \right) \chi(m) F(H)  \label{eq:3.25} \\
\delta = - \left( \frac{m-1}{3 \rho^{de}} \right) \chi(m) F(H),   \label{eq:3.26}
\end{eqnarray}

where, $\chi(m)= \dfrac{m-1}{m+1},$ $F(H)= \Phi(H)+\dfrac{3H^{2}}{m+1}$ .


From the above formalism it is quite clear that obtaining an exact solution to the field equations is a  cumbersome process. Therefore without violating any physical meaning of the expression and in order to study the cosmological model in this formalism, we have assumed two scale factors one leads to power law expansion and the other to de Sitter expansion.

 
In view of this, in the following, we discuss the dynamical features of two possible kind of  models in this frame work.



\section{Case study I: Dynamic features of Power law expansion model}


Recently many observational results as well as experiments predict a tensor-to-scalar ratio that provides a convincing results for standard inflationary scenario even though it contradicts the limits from Planck
data. During a power law expansion, the inflationary scenario predicts the generation of gravitational waves. In this model, the scale factor for power law cosmology can be represented as $R=t^k$, where $k$ is a positive constant and $k={\left(\frac{m+1}{2} \right) n}$. Also, $m$ and $n$ are positive constants. Now, the volume scale factor,$V = t^{3k}$ and Hubble parameter $H =\frac{k}{t}$. It is obvious that, for $k > 1,$ the model will be an accelerating one. Now, subsequently the directional Hubble parameters can be obtained as $H_{x} = \left(\frac{m+1}{2} \right)\frac{n}{t}$, $ H_{y} = \frac{mn}{t}$ and $ H_{z} =\frac{n}{t}$ and consequently, the mean deceleration parameter becomes $q = -1 + \frac{2}{n(m+1)}$. The deceleration parameter is a negative constant quantity for $n > \frac{2}{m+1}$, since $m$ and $n$ are positive constants and is good agreement with the present observational data that predicts an accelerating universe, therefore in order to get an accelerating model with this power law scale factor, the exponent $n>1$ if $m < 1$ otherwise it has to be decided from $n>\frac{2}{m+1}$. \\

The universe in general is isotropic, but recent observations from CMB temperature anisotropy, the anisotropic nature is favoured. However, any anisotropy in spatial expansion must be considered as a little perturbation of the isotropic behaviour which suggests that the exponent $m$ must be close to 1. In fact, according to the present result from the analysis of anisotropy as predicted from Planck data \cite{planck015} and Mishra \cite{mishra015a,mishra015b} , $m\approx 1.0001633$ . The power law model is quite successful in the sense that it neither encounter the horizon problem nor witness the flatness problem with $n \geqslant \frac{2}{m+1}$. The energy density contribution coming from the usual cosmic fluid for the power law model reduces to,

\begin{align}  \label{eq:3.27}
\rho= \frac{\rho_{0}}{t^{\frac{3}{2}(m+1)(\epsilon+1)n}}
\end{align}

Now, with the help of eqn. \eqref{eq:3.27}, the dark energy density and dark energy EoS parameter as described in \eqref{eq:3.22} and \eqref{eq:3.23} can be respectively reduced to,

\begin{align}  \label{eq:3.28}
\rho^{de}= \left[ \dfrac{(m^{2}+4m+1)n^{2}}{2} \right] \dfrac{1}{t^{2}} - 
\dfrac{3 a^{2}}{t^{n(m+1)}}-\dfrac{\rho_{0}}{t^{\frac{3}{2}%
(m+1)(\epsilon+1)n}}
\end{align}
and 
\begin{equation} \label{eq:3.29}
\omega ^{de}=\dfrac{1}{\rho ^{de}}\left[ \left\{ \dfrac{%
n(m^{2}+4m+1)(4-3n(m+1))}{6(m+1)}\right\} \dfrac{1}{t^{2}}+\dfrac{a ^{2}%
}{t^{n(m+1)}}-\bar{p}\right] ,
\end{equation}

where, $\bar{p}=\epsilon \rho _{0}^{de}$. 


The skewness parameters $\delta ,$ 
$\gamma $ and $\eta $ reduce to 
\begin{eqnarray} 
\gamma  &=&\frac{\left( 5+m\right) \left( m-1\right) }{3\left( m+1\right)
^{2}}\left( \frac{3k^{2}-k}{t^{2}}\right) \dfrac{1}{\rho ^{de}}\label{eq:3.30} \\
\eta  &=&-\frac{\left( 5m+1\right) \left( m-1\right) }{3\left( m+1\right)
^{2}}\left( \frac{3k^{2}-k}{t^{2}}\right) \dfrac{1}{\rho ^{de}} \label{eq:3.31}\\
\delta  &=&-\frac{2\left( m-1\right) ^{2}}{3\left( m+1\right) ^{2}}\left( 
\frac{3k^{2}-k}{t^{2}}\right) \dfrac{1}{\rho ^{de}}\label{eq:3.32}
\end{eqnarray}

where $k=\frac{n(m+1)}{2}$. It is seen that both $\rho$ and $\rho^{de}$ decrease with the increase in time. The decrease in $\rho^{de}$ is decided by three different factors i.e $t^{-2}$ in the first term , $t^{-n(m+1)}$ in the second term and $t^{3/2 (1+ \epsilon)(m+1)n}$ in the third term. The role of bulk viscous cosmic fluid comes through the third term. One may note that, if $\epsilon =-1$, even though the contribution coming from the usual cosmic fluid does not vanish, it does not contribute to the time variation of the dark energy density. For $\epsilon = -\frac{1}{3}$, the time variation of second and third terms can be clubbed together. Consequently, for this choice the skewness parameters becomes a constant quantity appears to be a simple time independent deviations from usual isotropic pressure.  

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{PL1rhoR2.pdf} 
\caption{ Variation of $\rho$ versus  $t$  for representative values of the parameter $m=1.0001633, n=1.7, \rho_0=0.001$ with different $\epsilon=-\frac{1}{3},-\frac{2}{3}, -1$}
\endminipage
\end{figure}

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{PL2rdeR2.pdf}
\caption{Variation of $\rho^{de}$ versus  $t$ for representative values of the parameter $m=1.0001633, n=1.7, a=0.01, \rho_0=0.001$ with different $\epsilon=-\frac{1}{3}$
}
\endminipage
\end{figure}

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{PL3wdeR2.pdf} 
\caption{Variation of $\omega^{de}$ versus  $t$ for representative values of the parameter $m=1.0001633, n=1.7, a=0.01, \rho_0=0.001$ with different $\epsilon=-\frac{1}{3},-\frac{2}{3}, -1$
}
\endminipage
\end{figure}


The figures in the manuscript have been drawn for different physical quantities which are expressed in Planckian unit system $(c=G=k_B=h=1)$. Also, 1 unit of cosmic time = 10 billion years. In figure 3.1 and figure 3.2, we have observed respectively that the matter energy density $\rho$ and the dark energy density $\rho^{de}$ remains positive during the cosmic evolution for the representative value of the constants ($m=1.0001633,n=1.7,a=0.01, \rho_0=0.001$). Hence, it indicates that both weak energy condition (WEC) and null energy condition (NEC) are satisfied in the derived model. Further, both $\rho$ and $\rho^{de}$ decreases with increase in time and slowly reaches to a small positive values in the present epoch. The value of dark energy density comes closer to zero and then smoothly approaches to small positive value which indicates the considered two fluid affects the dark energy density. It is worthy to note here that irrespective of the value of the viscous coefficient $\epsilon$, the behaviour of $\rho^{de}$ remains alike. So, in figure 3.2, we have chosen the value of the viscous coefficient to be $-\frac{1}{3}$. However, a small effect of viscous fluid in dark energy density cannot be ruled out. Figure 3.3, represents the variation of $\omega^{de}$ with cosmic time for different values of viscous coefficients $\epsilon$. The range value of EoS parameter suggested by combination of SNIa data with CMB anisotropy and galaxy clustering statistics is [-1.33,-0.79] \cite{kumar011}; whereas the range suggested by recent observations are reduced to more stringent constraints around -1  \cite{planck013a, planck013b}. However, we consider here the earlier data range since power law behaviour dominates the cosmic dynamics in early phase of cosmic evolution \cite{mishra015a}. For $\epsilon=-1/3,-2/3,-1$, FIG. 3 clearly shows that $\omega$ evolves with in a range, which is almost aligned with SN Ia and CMB observations. Moreover, it is observed that when the bulk viscous coefficients increases, the EoS parameter gradually converges to $\Lambda_{CDM}$ at late time.\\

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{PL4sk1R2.pdf}
\caption{Variation of $\delta, \gamma, \eta$ versus $t$ for representative values of the parameter $m=1.0001633, n=1.7, a=0.01, \rho_0=0.001$ for $\epsilon=-\frac{1}{3}$
}
\endminipage
\end{figure}

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{PL4sk2R2.pdf} 
\caption{Variation of $\delta, \gamma, \eta$ versus $t$ for representative values of the parameter $m=1.0001633, n=1.7, a=0.01, \rho_0=0.001$ for $\epsilon=-\frac{2}{3}$}
\endminipage
\end{figure}

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{PL4sk3R2.pdf}
\caption{Variation of $\delta, \gamma, \eta$ versus $t$ for representative values of the parameter $m=1.0001633, n=1.7, a=0.01, \rho_0=0.001$ for $\epsilon=-1$}
\endminipage
\end{figure}

The behaviour of the skewness parameters obtained in eqns. \eqref{eq:3.30}-\eqref{eq:3.32} has been graphically represented in figure 3.4, figure 3.5 and figure 3.6 respectively for $\epsilon=-1/3$, $\epsilon=-2/3$ and $\epsilon=-1$. In these figures, it can be noted that the behaviour of skewness parameter are totally controlled by the behaviour of the anisotropic parameter $m$ as shown by Mishra \cite{mishra015a}. For $m=1$, the skewness parameters vanish giving an indication that the viscous matter affects the skewness parameter. We have observed that, at an early cosmic phase, $\eta$ starts with a negative value far from zero, increases with the cosmic time to became maximum and then becomes constant with further increase in cosmic time. The skewness parameter $\delta$ also starts from a small negative value close to zero and becomes constant with respect to cosmic time. The evolutionary behavior of $\gamma$ is just the mirror image of $\eta$. It can be noted that the pressure anisotropy factors along $x$, $y$ and $z$ axis $(\eta, \delta,\gamma)$ evolves with different nature, attain their extreme values in a definite range of cosmic time $0.001<t<0.003$ and remain constant at later time.Therefore, it can be inferred that, in power law cosmology, at an early phase of cosmic evolution, the pressure was assumed to be isotropic; however in the late phase, pressure anisotropies still remain. It can also be noted that, the behavior of skewness parameters are independent of the choice of the bulk viscous coefficient.

\section{Case study II: Dynamic features of de Sitter expansion model}

In de Sitter model, the scale factor is taken as $R=e^{(\frac{m+1}{2})\xi t}$, where $\xi$ is a positive constant. In this model, the Hubble parameter is a constant quantity and remains the same through out the cosmic evolution. The directional Hubble rates along different spatial directions are also constants and can be expressed as $H_{x}=\left(\frac{m+1}{2} \right) \xi,$ $H_{y}=m \xi,$ $H_{z}= \xi$. So, $\xi$ can be expressed as $\xi= \frac{2H}{m+1}$. With this assumption of the scale factor, the energy density contribution coming from the usual cosmic bulk viscous fluid for the de Sitter model reduces to, 
\begin{equation}
\rho =\frac{\rho _{0}}{e^{\frac{3}{2}(1+\epsilon )(m+1)\xi t}}  \label{eq32}
\end{equation}%
The energy density increases with the decrease in the value of $\epsilon $ and vice-versa. For the particular choice $\epsilon =-1,$ $\rho $ becomes independent of time and assumes a constant value $\rho _{0}$ throughout the cosmic evolution (FIG.7).\\
The rest energy density $\rho^{de}$and the dark energy EoS parameter $\omega ^{de}$ for the de Sitter universe can now be obtained as,

\begin{equation}
\rho ^{de}=\xi ^{2}\left( \dfrac{m^{2}+4m+1}{2}\right) -\dfrac{3a^{2}}{%
e^{\xi (m+1)t}}-\dfrac{\rho _{0}}{e^{\frac{3}{2}(1+\epsilon )(m+1)\xi t}}
\label{eq33}
\end{equation}

\begin{equation}
\omega ^{de}=\dfrac{1}{\rho ^{de}}\left[ -\dfrac{\left( m^{2}+4m+1\right)
\xi ^{2}}{2}+\dfrac{a^{2}}{e^{\xi (m+1)t}}-\bar{p}\right]  \label{eq34}
\end{equation}

where, $\bar{p}=\epsilon \rho _{0}^{de}$. Subsequently, the skewness parameters $\delta ,$ 
$\gamma $ and $\eta $ can be expressed as 
\begin{eqnarray}
\gamma  &=&\frac{\left(5+m\right) \left( m-1\right) }{4}\left(\frac{\xi^{2}}{\rho
^{de}}\right) \label{35}\\
\eta  &=&-\frac{\left(5m+1\right) \left( m-1\right)}{4}\left(\frac{\xi^{2}}{\rho
^{de}}\right) \label{36}\\
\delta  &=&-\frac{2\left( m-1\right) ^{2}}{4}\left(\frac{\xi ^{2}}{\rho ^{de}}\right) \label{37}
\end{eqnarray}

In the de Sitter model, the dark energy density decreases with increase in time and asymptotically reduces to a positive constant. The decrement in $\rho^{de}$ is decided by four different  factors in the second and third term viz., $m, \xi, a, \rho_0$. The role of bulk viscous cosmic fluid comes through the third term. The contribution from the bulk viscous cosmic fluid becomes time independent for $\epsilon=-1$. The pressure anisotropies defined earlier in  different axis depend on the behavior of skewness parameters whereas the dark energy density $\rho_{de}$ depends on the barotropic equation of state $\epsilon$ (FIG. 8).\\

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{DS1rhoR2.pdf} 
\caption{Variation of $\rho$ versus $t$ for representative values of the parameter $m=1.0001633, \rho_0=0.001, \xi=0.08$ with different $\epsilon=-\frac{1}{3},-\frac{2}{3}, -1$}
\endminipage
\end{figure}
\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{DS2rdeR2.pdf}
\caption{Variation of $\rho^{de}$ versus $t$ for representative values of the parameter $m=1.0001633, \rho_0=0.001,a=0.01, \xi=0.08$ with different $\epsilon=-\frac{1}{3},-\frac{2}{3}, -1$}
\endminipage
\end{figure}
\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{DS3wdeR2.pdf} 
\caption{Variation of $\omega^{de}$ versus $t$ for representative values of the parameter $m=1.0001633, \rho_0=0.001,a=0.01, \xi=0.08$ with different $\epsilon=-\frac{1}{3},-\frac{2}{3}, -1$}
\endminipage
\end{figure}
The EoS parameter in FIG. 9 is very much sensitive to the choice of $\epsilon$. For different choices, they starts from different values at the early phase and maintain the same evolutionary state at late phase falling in the observed range as obtained in 2015 Planck data $\omega=-1.019^{+0.075}_{-0.080}$ \cite{planck015}.   The behaviour of EoS parameters are directly proportional to the increasing values of viscous coefficient $\epsilon$ at early phase but behave differently at late phase, gathered some amount of energy at early phase. The reason being the dynamics of EoS is greatly affected at early phases is that the bulk viscous has a substantial contribution to the density parameter at that corresponding phase. But at late phase, the dark energy dominates in spite of the presence of bulk viscous fluid. Hence, cosmic bulk viscous fluid has a very little impact on the dynamics of EoS parameter.\\

\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{DS4sk1R2.pdf}
\caption{Variation of $\delta, \gamma, \eta$ versus $t$ for representative values of the parameter $m=1.0001633,  \rho_0=0.001,\alpha=0.01, \xi=0.08$ for $\epsilon=-\frac{1}{3}$
}
\endminipage
\end{figure}
\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{DS4sk2R2.pdf} 
\caption{$\delta, \gamma, \eta$ versus $t$ for representative values of the parameter $m=1.0001633, \rho_0=0.001,a=0.01,   \xi=0.08$ for $\epsilon=-\frac{2}{3}$}
\endminipage
\end{figure}
\begin{figure}[tbph]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=\textwidth]{DS4sk3R2.pdf}
\caption{$\delta, \gamma, \eta$ versus $t$ for representative values of the parameter $m=1.0001633, \rho_0=0.001,a=0.01, \xi=0.08$ for $\epsilon=-1$}
\endminipage
\end{figure}

The DE skewness parameters are plotted as a function of cosmic time for three representative values of bulk viscous coefficient, $\epsilon= -1, - \frac{2}{3}, -\frac{1}{3}$. The corresponding skewness parameters are shown for these three viscous coefficients respectively in FIG. 10, FIG.11 and FIG. 12. With increase of viscous coefficient of matter, skewness parameters show non evolving behaviour in past epoch and rapidly evolve at late phase. The anisotropy in the DE pressure along $x$-direction is almost unaffected by cosmic expansion for all three considered viscous coefficient
values. So, the pressure anisotropy vanishes along $x$- axis. $\delta$'s are less affected by the presence of cosmic fluid compared to $\gamma$'s and $\eta$'s. The DE pressure along $y$ and $z$-directions are mostly affected. The reason behind the sensitivity may be due to the consideration of assuming mean Hubble parameter same as directional Hubble parameter along $x$-axis. At early times, the universe is predicted to have almost isotropic fluid which became anisotropic with the growth of cosmic time. Due to presence of bulk viscous fluid, the anisotropy in DE pressure continues along with the cosmic expansion and decreases slowly at the later period as shown in FIG. 10, FIG.11 and FIG 12. 

\section{Conclusion}

In the present work, we have investigated the role of anisotropic components on the dynamical aspects of DE model in Bianchi V space-time in a two fluid situations. Two cosmological  models have been constructed one pertaining to power law cosmology and the other one to de Sitter universe. The present model favours a quintessence energy dominated universe in the later universe as $-1<\omega^{de}<0$; however in early universe it favours phantom region. In power law model, EoS parameter lies within the predicted range by observational data. In the de Sitter model, DE dominates at late phase of EoS parameter and bulk viscous fluid plays an important role at early universe. The skewness parameters are dynamically evolving with respect to cosmic expansion. In power law, skewness parameter evolves with different values at early phase, where as, it remains constant at late phase, indicating constant anisotropy rate. However, in de Sitter model, the skewness parameters decreases at the later cosmic period and shows a small amount of anisotropy in future cosmic time. The behaviour of skewness parameters are independent of the choice of the bulk viscous coefficient. There is a lot of observational evidences to support the $\Lambda_{CDM}$, such as CMB and redshift-distance relation. However, our considered model is a generalization of FRW model or $\Lambda_{CDM}$ model as discussed in section II. Also, our model is scale factor dependent and may change its behaviour in different scale factors; however the formalism developed here clearly indicates the accelerating behaviour of the expanding universe. Moreover, the resemblance of data of considered model with standard $\Lambda_{CDM}$ model, our model found here also aligned with the present day observational outcomes. \\
  
There are ways to know whether the model approaching to  $\Lambda_{CDM}$ model is accurate or not. One way is $\Lambda_{CDM}$ universes may converge to de Sitter universe under special conditions as de Sitter model has the exponential growth. In our investigation also, the EoS parameter in de Sitter universe is similar to EoS parameter of $\Lambda_{CDM}$ model at late cosmic time of evolution. Another way is the state finder diagnostics, which checks the validity of the model. $\Lambda_{CDM}$ model has state finder pair ${(r,s)}={(1,0)}$. The model discussed here also confirms the acceptability by state finder analysis with the pair ${(1,0)}$ for both the de Sitter universe and for power law for large value of the exponent $m$. 

==> Report_format_thesis/Chapter4.tex <==
\chapter{Significance of hybrid expanded models in order to characterize dynamics of anisotropic DE Universe embedded with Bulk Viscous fluid }


\footnote{\bf{The contents of this chapter has been published in Eur. Phys. J. C, \textbf{79}, 34 (2019)}}


\pagebreak



\section{Introduction}
Cosmologists have given a lot of importance to viscous fluid matter which is in contrasts with the traditional approach. In this approach, usually the cosmic fluid remains ideal (non-viscous). Hydrodynamicists suggest that because of the turbulence phenomena, inclusion of viscosity becomes mandatory even in homogeneous space without any limits. There are two viscous coefficients discussed in literature such as the the shear viscosity and bulk viscosity. Shear viscosity is the  dominating one as compared to bulk viscosity \cite{land}. Since a lot of interesting results are available on viscous cosmology on the past universe, the methods from particle physics can also be applied to understand the influence of viscosity on the evolution of universe in homogeneous DE models. Also referring the present observational results for the Hubble parameter and standard Friedman formalism, we may explain the description of the universe back up to the inflationary era, or else we may go to the opposite extreme and analyse the probable ultimate fate of the universe. In early universe, the results of both shear and bulk viscosity were explained by Hogeveen et al. \cite{hoge} using kinetic theory. Also, it is indicated that in early universe the impact of viscosity is very small whereas in future universe the impact is significant. Brevik et al.\cite{brev1, brev2} have investigated viscous cosmology in the early universe for both homogeneous and inhomogeneous EoS and examined the viscosity effects on the various inflationary observables. They have also analysed the viscosity-induced crossing through the quintessence-phantom divide and examined the viscosity-driven cosmological bounces .Since viscosity appears to be an important dissipative phenomena in FRW cosmology, therefore it is  expected that cosmological models embedded with bulk viscosity fluid would produce some remarkable  results in the two fluid situations. Moreover, viscosity embedded cosmological models indicates a substantial contribution of bulk viscosity at the inflationary phase \cite{barr, zimda, pavon}. The bulk viscous driven inflation leads to a negative pressure term, which in process results in repulsive gravity and ultimately became a cause for the rapid expansion of the universe \cite{tripa1,maar,Mak02,Zeya14, Brevik15}. \\

In mixed fluids environment such as dark fluid matter along with usual ordinary matter (Baryonic matter), a number of literature has motivated the researchers to investigate different models in the back drop of General Relativity with different Bianchi forms. DE models with constant deceleration parameter have been constructed and investigated by Akarsu and Kilinc \cite{akarsu1, akarsu2} for  Bianchi type I and III space time. With a variable Equation of State (EoS) parameter, Yadav et al. \cite{yadav1} constructed BV DE cosmological models where the deceleration parameter was assumed to be constant. Several theoretical two fluids DE models either interacting or non-interacting have been discussed widely in the literature \cite{shey, amir1, amir2, tripa3, suresh}. Few have constructed DE cosmological models with two non interacting fluid situations such as DE fluid with cosmic string and nambu string. In both the models, they have shown that the models are mostly dominated by Phantom behaviour. In a similar approach of two fluid, DE cosmological models were constructed in different general scale factors . 



\section{Mathematical Formalism of the model}

The total energy momentum tensor (EMT) in presence of both the viscous and DE fluids can be expressed as,
\begin{equation} \label{eq4.2}
T_{ij}= T_{ij}^{vis} + T_{ij}^{de},
\end{equation}
where, EMT of barotropic bulk viscous fluid is 
\begin{align} \label{eq4.3}
 T_{ij}^{vis}=  (\rho + \bar{p}) u_{i}u_{j}- \bar{p} g_{ij},
\end{align}
and EMT of DE fluid is
\begin{align} \label{eq4.4}
 T_{ij}^{de} \nonumber &= diag[\rho^{de}, -p^{de}_{x}, -p^{de}_{y}, -p^{de}_{z}]\\ \nonumber &= diag[1, -\omega^{de}_{x}, -\omega^{de}_{y}, -\omega^{de}_{z}] \rho^{de}\\  &= diag[1, -(\omega^{de}+ \delta), -(\omega^{de}+ \gamma), -(\omega^{de}+ \eta)]\rho^{de},
\end{align}

Here, $u^{i}$ is the four velocity vector of the fluid in a co-moving coordinate system. $\omega^{de}$ and $\rho^{de}$ are respectively the EoS parameter of the DE fluid and DE density parameter. The skewness  parameters $\delta$ on $x$-axis, $\gamma$ from $y$-axis and $\eta$ on $z$-axis are deviations from the EoS parameter $\omega^{de}$ on these three directions. With these consideration on the parameters, in the subsequent section, we have developed the mathematical formalism of the problem.\\





\begin{align}
& \frac{\ddot{B}}{B}+\frac{\ddot{C}}{C}+\frac{\dot{B}\dot{C}}{BC}-\frac{\alpha^{2}}{A^{2}}=-p+3 \zeta H-(\omega_{DE}+\delta)\rho_{DE} \label{eq4.5} \\ 
& \frac{\ddot{A}}{A}+\frac{\ddot{C}}{C}+\frac{\dot{A}\dot{C}}{AC}-\frac{\alpha^{2}}{A^{2}}=-p+3 \zeta H-(\omega^{de}+\gamma)\rho_{DE} \label{eq4.6} \\ 
& \frac{\ddot{A}}{A}+\frac{\ddot{B}}{B}+\frac{\dot{A}\dot{B}}{AB}-\frac{\alpha^{2}}{A^{2}}=-p+3 \zeta H-(\omega^{de}+\eta)\rho_{DE} \label{eq4.7} \\ 
& \frac{\dot{A}\dot{B}}{AB}+\frac{\dot{B}\dot{C}}{BC}+\frac{\dot{C}\dot{A}}{CA}-\frac{3\alpha^{2}}{A^{2}}=\rho+\rho_{DE} \label{eq4.8}\\
& 2\dfrac{\dot{A}}{A}-\dfrac{\dot{B}}{B}-\dfrac{\dot{C}}{C} =0 \Rightarrow A^2=k_1BC \label{eq4.9}
\end{align}
where an over dot represents the derivatives of corresponding field variable with respect to $t$ and in Eqn. \eqref{eq4.9} $k_1=1$. It can be noted that the product of the field variables $A$, $B$ and $C$ gives the volume scale factor from where the average scale factor can be deduced as $R = V^{\frac{1}{3}}$. If $H_x$, $H_y$ and $H_z$ respectively denotes the Hubble parameter's in the direction of $x$,$y$ and $z$ respectively, then the mean Hubble's parameter $H =\frac{1}{3}\Sigma {H_i}=\frac{\dot{R}}{R}$, where $i=x,y,z$. \\

The proper pressure $p$, in case of barotropic cosmic fluid,  is given as, $p= \xi \rho,$ $(0 \leq \xi \leq 1)$. Moreover, the bulk viscosity related to energy density with the help of Hubble's parameter as $3 \zeta H= \epsilon_{0} \rho$. So, the effective pressure which is the mixture of proper pressure and barotropic bulk viscous pressure can be written as,  $\bar{p} = p-3 \zeta H = (\xi - \epsilon_{0}) \rho= \epsilon \rho$, where, $\epsilon$ can be considered as effective viscous coefficient. It can be noted that, $3\zeta H$ is the bulk viscous pressure which is considered in the present work to be a barotropic one. Tripathy et al.\cite{tripa1, tripa2}, have suggested this form of barotropic bulk viscous pressure from a dimensional analysis. Moreover, as claimed by Tripathy et al.\cite{tripa1, tripa2} and others \cite{Singh08,Li09}, such a bulk viscous pressure may provide a negative pressure which may be helpful for the understanding of the late time cosmic speed up. Now, replacing pressure terms $(p-3 \zeta H)$ in field equations as $\bar{p}$ and framing field variables in terms of Hubble parameter, we obtain

\begin{align}
& 2 \dot{H}+ 4  \dfrac{(m^{2}+m+1)}{(m+1)^{2}} H^{2}-\frac{\alpha^{2}}{A^{2}} = -\bar{p} - (\omega_{DE}+ \delta)\rho_{DE} \label{eq4.10} \\
& \left(\dfrac{m+3}{m+1}\right)\dot{H}+ \dfrac{(m^{2}+4m+7)}{(m+1)^{2}} H^{2}-\frac{\alpha^{2}}{A^{2}} = -\bar{p}  - (\omega_{DE}+ \gamma)\rho_{DE} \label{eq4.11}\\
& \left(\dfrac{3m+1}{m+1}\right)\dot{H}+\dfrac{(8m^{2}+4m+1)}{(m+1)^{2}} H^{2}-\frac{\alpha^{2}}{A^{2}} = -\bar{p} - (\omega_{DE}+ \eta)\rho_{DE} \label{eq4.12}\\
& \dfrac{(2m^{2}+6m+4)}{(m+1)^{2}} H^{2}-\frac{3 \alpha^{2}}{A^{2}} = \rho + \rho_{DE} \label{eq4.13}
\end{align}

The energy conservation equation for viscous fluid, $T^{ij(vis)}_{;j}=0$ and DE fluid, $T^{ij(de)}_{;j}=0$ can be obtained respectively as 

\begin{equation} \label{eq4.14}
\dot{\rho}+3(\bar{p}+\rho)\frac{\dot{R}}{R}=0
\end{equation}

and

\begin{equation} \label{eq4.15}
\dot{\rho}_{DE}+3 \rho_{DE}(\omega_{DE}+1)\frac{\dot{R}}{R}+ \rho_{DE}(\delta H_x+\gamma H_y+\eta H_z)=0
\end{equation}

From \eqref{eq4.14}, incorporating the relation between Hubble parameter and scale factor,  we get the energy density for the matter field as,
\begin{align} \label{eq4.16}
\rho=\frac{\rho_{0}}{\left[ e^{\int{H}.dt}\right]^{3(\epsilon +1)}}
\end{align}
where $\rho_0$ is the integration constant or rest energy density of present time.\\

From the literature, it is evident that bulk viscous fluid has an important role in the study of the recent claim of accelerated expansion of the universe. It is already mentioned that the barotropic bulk viscous pressure includes the contributions both from the usual cosmic fluid and from the coefficient of bulk viscosity $\epsilon$. The contribution from bulk viscosity to cosmic pressure is assumed to be proportional to the rest energy density of universe \cite{tripa1}. From the analysis of $p=\epsilon \rho$, we can note that, in case contribution from bulk viscosity becomes more than the usual perfect fluid pressure then the total effective pressure becomes negative with a negative $\epsilon$. The accelerated expansion in the present epoch is usually attributed to a fluid with negative pressure and hence, it can be thought that the contribution coming from the bulk viscosity is greater than the usual pressure. If the usual pressure from perfect fluid equals to the contribution from cosmic bulk viscosity, then the cosmic fluid in the model behaves like a pressure less dusty universe.  However, the presence of an exotic DE form leads to a negative pressure of the universe which simulates an anti-gravity effect that drives the acceleration. If the time variation of the mean Hubble rate is known, then the rest energy density of the universe can be calculated from \eqref{eq4.16} for a given value of $\epsilon$. \\

From \eqref{eq4.13} and \eqref{eq4.16}, we can retrieve, the DE density as,

\begin{equation} \label{eq4.17}
\rho_{DE}=\dfrac{2(m^2 +4m +1)}{(m+1)^2} \left( \dfrac{\dot{R}^2}{R}\right)-\dfrac{3 \alpha^{2}}{R^2}- \rho_{0} R^{-3(\epsilon + 1)}
\end{equation}


With the help of the second part of  the conservation equation \eqref{eq4.15},which corresponds to the deviation of equation of the state parameters and other is deviation free part and incorporated value of $\eta$ from \eqref{eq4.12}, we  formalize the EoS parameter of DE as,

\begin{align}\label{eq4.18}
\omega_{DE}= -\dfrac{1}{\rho_{DE}} \left[ \dfrac{2(m^{2}+4m+1)}{3(m+1)^{2}} \left( F(R)- 3 \dfrac{\dot{R}^{2}}{R^{2}} \right) - \dfrac{\alpha ^{2}}{R^{2}} + \epsilon \rho_{0} R^{-3(\epsilon +1)} \right]
\end{align}

where, $F(R)= \frac{\ddot{R}}{R}+ 4 \frac{\dot{R}^{2}}{R^{2}}$. With the help of eqns. \eqref{eq4.17}-\eqref{eq4.18}, eqns.  \eqref{eq4.10}-\eqref{eq4.12} can be formulated as:

\begin{align}
\delta = & - \left( \frac{m-1}{3 \rho^{de}} \right) \chi(m)  F(R) \label{eq4.19}\\
\gamma = & \left(\frac{5+m}{6 \rho^{de}} \right) \chi(m) F(R) \label{eq4.20}\\
\eta =& - \left( \frac{5m+1}{6 \rho^{de}} \right) \chi(m) F(R) \label{eq4.21}
\end{align}

Where, $\chi(m)= \dfrac{m-1}{(m+1)^2}$.

\section{Solution of the model using Hybrid scale factor}
Based on the recent outcomes on the present universe, mostly the scale factors are chosen to be either the exponential law expansion universe or power law expansion, whose deceleration parameter turns out to be constant. However, the time dependence of the directional scale factor would be decided by specific choices of scale factors. In the present work, we have considered the specific scale factor, the hybrid scale factor which at late time results into a constant deceleration parameter. The hybrid scale factor has two factors in the form, $R=e^{at}t^{b}$, where $a= \left( \frac{m+1}{2} \right) \xi$ and $b= \left( \frac{m+1}{2} \right)n$ are positive constants. The cosmic dynamics is dominated by the power law $(t^{b})$in the early phase, whereas it is dominated by the exponential factor $(e^{at})$ at late phase. However, eventually, the hybrid scale factor is found to be more dominant in the late phase of the evolution. It can be noted that in the hybrid scale factor, when the exponent $a=0$ and $b=0$, it recovers power law and exponential law respectively. For this model, the Hubble parameter and the directional Hubble parameter can be obtained respectively as $H = H_{x} = a +\frac{b}{t}$, $H_{y}=\frac{2m}{m+1} (a +\frac{b}{t})$ and $H_{z}=\frac{2}{m+1} (a +\frac{b}{t})$. Hence, with the hybrid scale factor the energy density of the matter from \eqref{eq4.16} would be $\rho=\frac{\rho_{0}}{\left[ e^{\int{H}.dt}\right]^{3(\epsilon +1)}}= \rho_{0} (e^{\xi t}t^{n})^{-\frac{3}{2}(m+1)(\epsilon +1)}$. Subsequently, DE density and the effective EoS parameter can be written as,

\begin{align} \label{eq4.22}
\rho_{DE}= \dfrac{(m^{2}+4m+1)(n+ \xi t)^{2}}{2t^{2}}-\dfrac{3 \alpha^{2}}{(e^{\xi t}t^{n})^{(m+1)}}-\dfrac{\rho_{0}}{(e^{\xi t}t^{n})^{\frac{3}{2}(m+1)(\epsilon+1)}}
\end{align}

and  
\begin{align} \label{eq4.23}
-\omega_{DE} \rho_{DE}= -2(m^{2}+4m+1) \Phi (t)+ \alpha^{2} (e^{\xi t}t^{n})^{-(m+1)} - \epsilon \rho.
\end{align}

where $\Phi(t)= \left[\frac{\xi^2t^2+n^2-2\xi nt}{4t^2}-\frac{n}{3(m+1)t^2}\right]$. Similarly, the skewness parameters can be expressed as,

\begin{align}
\delta = & - \left(\frac{m-1}{\rho^{de}}\right)(m-1)f(t)
 \label{eq4.24}\\ 
\gamma = & \left(\frac{5+m}{2\rho^{de}} \right)(m-1)f(t) \label{eq4.25}\\ 
\eta =& - \left( \frac{5m+1}{2 \rho^{de}} \right)(m-1)f(t) \label{eq4.26}
\end{align}
Here, $f(t)=\left[\Phi(t)+\left(\frac{\xi t+n}{2t}\right)^2\right]$.

It is observed that both $\rho$ and $\rho_{DE}$ are decreasing when time period is gradually increasing. The decrease in $\rho_{DE}$ is decided by three different factors i.e. $\frac{1}{t^{2}}$ , $\frac{1}{t^{n(m+1)}}$ and $\frac{1}{t^{\frac{3n}{2}(m+1)(\epsilon + 1)}}$. However, only the third term contains the bulk viscous coefficient for the DE density. When, $\epsilon=-1$,  the contribution from cosmic fluid for the DE density becomes time invariant. Similarly whenever  $\epsilon=-\frac{1}{3}$, the denominator of second and third term of \eqref{eq4.22} becomes same and the rest energy density along with the constant $\alpha$ decides the behaviour of DE density. Since bulk viscous coefficient $(\epsilon)$ acts as EoS parameter $(p=\epsilon \rho)$ for viscous source of matter, the above two values of $\epsilon$ reduces the model to vacuum and radiation dominated respectively in absence of DE. So, in order to understand the behaviour of the matter throughout, we have chosen a value $\epsilon=-\frac{2}{3}$, which is in the range $[-1,-\frac{1}{3}]$. Consequently, for this choice, in spite of the presence of the time factor $f(t)$,the skewness parameters become constant and independent of time, so the change in the isotropic pressure in all directions remain constant. To investigate some more details on the DE model, we have derived some physical parameters of the model. The scalar expansion and shear scalar are respectively given by,
\begin{align}
\theta=3H=3\left(a+\frac{b}{t}\right)
\end{align}
\begin{align}
\sigma^2=\frac{1}{2}(H_x^2+H_y^2+H_z^2-\frac{\theta^2}{3})=\biggl(\frac{m-1}{m+1}\biggr)^2\biggl(a+\frac{b}{t}\biggr)^2       
\end{align}
The anisotrpic parameter can be expressed as,
\begin{equation}
\mathcal{A}_m=\frac{1}{3}\sum \biggl(\frac{\vartriangle H_i}{H}\biggr)^2=\frac{2}{3}\biggl(\frac{m-1}{m+1}\biggr)^2
\end{equation}
Here, the parameter $m$ dealt with the anisotropic behaviour of the model and became isotropic for $m=1$. The parameters $H, \theta$ and $\sigma ^{2}$ start with with an extremely large values and continue to decrease with expansion of universe; whereas the spatial volume grows with cosmic time which mimic the present scenario of the universe. 

\section{Dynamical Behaviour of the model}

The deceleration parameter $q=- \frac{R \dot{R}}{\dot{R}^2}$  describes the cosmic dynamics of universe. Positive value of it indicates decelerating universe where as negative values confirms the accelerated expansion of the universe. In view of the observations of high red shift supernova, Type Ia supernova observations combined with BAO and CMB, models transiting from early decelerating universe to late time accelerating universe gained much importance in recent times. According to recent observational data at present time, the most favourable value for $q$ to be $ -0.81 \pm 0.14$. The deceleration parameter for the hybrid scale factor, turns to be $q= -1 + \dfrac{2n}{(m+1)(\xi t+ n)^{2}}=-1 + \dfrac{b}{(at+b)^{2}}$. So, at an early phase of cosmic evolution, i.e. whenever $t\rightarrow 0$, $q\rightarrow -1+\dfrac{1}{b}$ whereas  at late phase i.e. whenever $t\rightarrow \infty$, $q \simeq -1$. The parameter $b$ is constraint here to be in range $0<b<\frac{1}{3}$ to get a transient universe \cite{mishra015a}. In Fig-4.1, we have represented the deceleration parameter with cosmic time. At early phase the deceleration parameter is positive decreases rapidly and at late phase it appears to be negative. At present time, the deceleration parameter value found to be $(\simeq- 0.9)$, which is in alignment with the observational data. \\

\begin{figure}[h!]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=65mm]{dece.pdf}
\caption{DE deceleration parameters  vs. time }
\endminipage\hfill
\minipage{0.40\textwidth}
\includegraphics[width=65mm]{rho.pdf}
\caption{DE density parameter  vs. time  }
\endminipage 
\end{figure}

In Fig. 4.2, we observe, the DE density $(\rho_{DE})$ remains positive till late phase of evolution, satisfying weak energy condition (WEC) and  null energy condition (NEC) for the present model. It is worth to mention that, behaviour of DE density does not depend on change in value of viscous coefficient$(\epsilon)$ and remains alike. $\rho_{DE}$ decreases with increase in cosmic time and reaches to a positive value at present epoch instead of coming closer to zero as in case of the hybrid model embedded in string fluid. This indicates that viscous fluid has smaller effect on $\rho_{DE}$ than string fluid. However, this small effect due to mix fluid matter cannot be ruled out.\\


\begin{figure}[h!]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=65mm]{omega.pdf}
\caption{DE EoS parameter  vs. time for different viscous coefficients }
\endminipage\hfill
\minipage{0.40\textwidth}
\includegraphics[width=65mm]{omegaRho0.pdf}
\caption{DE EoS parameter  vs. time for different $\alpha$ with $\epsilon=-0.66$  }
\endminipage 
\end{figure}


\begin{figure}[h!]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=65mm]{skewness.pdf}
\caption{DE skewness parameters  vs. time }
\endminipage\hfill

\end{figure}

Fig.4.3 represents variation of EoS parameter $(\omega_{DE})$ w.r.t appropriate choices of bulk viscous coefficients $(\epsilon= 0, -\frac{1}{3}, -\frac{2}{3}, -1)$. When compared to the de Sitter model and power law model, we found nature of EoS parameters are directly proportional to the increasing value of viscous coefficients $(\epsilon)$ till late phase. But the behaviours of the parameters greatly affect the dynamics at early phase of evolution where as the late phase is smooth and mildly affected by the viscous coefficient values, falling in the preferred range, determined by observational data. The reason of this drastically affected early phase is due to the substantial contribution of bulk viscous fluid. The pink line $(\epsilon=-1)$ confirms that the less is the viscous coefficient value, lesser is the possibility of occurring $\omega_{DE}$ within the observed length (Quintessence region). However, for much lower value of $(\epsilon)$ (beyond $\epsilon=-1$), the decrement of EoS parameter is more rapid. Also, $\omega_{DE}$ decreases with increase in cosmic time in these cases. With increase in viscous coefficient value, this model gathers some energy in early phase and behave differently. The black line $(\epsilon=0)$ represents the cosmic fluid without usual matter but only of dark fluid. This line is most closer to $\Lambda$CDM line than other EoS parameter lines which are embedded with viscous fluid. It also indicates that without any viscous fluid, the model behaves like quintessence field with cosmic growth. The green line $(\epsilon=-\frac{2}{3})$ and blue line $(\epsilon=-\frac{1}{3})$ emerge at early phase, showing little deflection due to presence of viscous fluid and decrease smoothly in the quintessence region with evolution. At late phase of cosmic evolution, $\omega_{DE},$ for all the cases considered here except $(\epsilon=-1),$ decrease to achieve larger negative value. In spite of the presence of bulk viscous fluid, the DE seems to be dominant the universe. Hence, it indicates that there is a very little impact of bulk viscous on the dynamics of EoS, that too in the early phase of evolution.\\

DE EoS parameters can also be useful in testing the model w.r.t certain other parameters. In fact, one has the liberty to test the impact of EoS parameter for different choices of parameter $\alpha$, shown in Fig. 4.4. $\omega_{DE}$ remains in the quintessence region for all considered values of $\alpha$ but the behaviour changes over time and inclined towards $\Lambda$CDM line. Behaviour of $\omega_{DE}$ is same as compared to different viscous coefficient values. But when the value of $\alpha$ increases, $\omega_{DE}$ increases most rapidly. Also, the value of $\omega_{DE}$ for $\alpha=0.05$(red line) is more for higher values of $\alpha$ and lies very similar to $\omega_{DE}$ for more suitable viscous coefficient value $(\epsilon= -\frac{2}{3}).$\\

In absence of cosmic bulk viscous fluid (dotted lines), the anisotropic parameters execute almost non-evolving behaviour in most of the early phase evolve a little towards late phase. The DE pressure along x- direction,  remains unaffected mostly during evolution. But the anisotropy in DE pressure along y-direction, $\gamma$(blue dotted line) increase a little, where as, along z-direction, DE pressure $\eta$(black dotted line) decrease a little at late times. One can also conclude that, at initial phase of phase of evolution, the skewness parameter may merge into one line indicating the isotropic universe but at late phase is anisotropic w.r.t small scale contribution. In presence of cosmic bulk viscous fluid, the early phase is dominated and affected mostly by bulk viscous but remain unaltered as in case of no viscous fluid, towards$\delta$(red dotted line) late phase. $\gamma$(blue solid line) and $\eta$(black solid line) show similar increasing and decreasing behaviour, being affected by viscous fluid. In fact, they both evolve as mirror image to each other in both presence and absence of cosmic viscous fluid. However, the viscous fluid affects the skewness parameter $\delta$(red solid line) mostly as compared to the other two skewness parameters. $\delta$ increases as it moves towards late phase and changes sign at some cosmic time. This impact on $\delta$ may be due to the fact that, we have considered the mean Hubble parameter is same as directional Hubble parameter along x-axis $(H=H_{x})$. Also, the effects of anisotropic parameter ($m$), parameters $\alpha$ and $n$ are investigated w.r.t pressure anisotropy. But they do not find to have any significant impact on the overall behaviour of skewness parameters.\\



\section{Conclusion}

In this work, we have investigated the anisotropic behaviour of the cosmological model constructed in a two fluid situations: the usual bulk viscous fluid and DE fluid. The scale factor considered here is the hybrid scale factor which can be attributed to power law cosmology and de Sitter universe for appropriate value of the constant. The parameters of the scale factor has been chosen appropriately from some physical background. Along, $x$-direction, the anisotropy in DE pressure has a very little effect on the pressure anisotropy  whereas along $y$-direction, it increases and along $z$-direction decreases at late times. Presence of viscous fluid substantially affects the DE density at early phase of cosmic evolution; however at late phase late phase DE density dominates over viscous fluid. One more observation is that, the DE EoS parameter remains unaffected for different viscous coefficients however it for different value of the constant $\alpha$, it remains in the quintessence region. The anisotropic parameters remain almost non-evolving in most of the early phase in the absence of viscous fluid however in the presence of viscous fluid it has impact. In the late phase the DE fluid has the dominance over bulk viscous fluid. From the evolutionary behaviour of the state finder pairs, we can infer that the model may bear a similarity to the $\Lambda CDM$ universe at a non-perturbative level.


==> Report_format_thesis/Chapter5.tex <==
\chapter{Dynamical features of an anisotropic two fluid Bianchi V DE universe dipped in geometric string fluid and treated with hybrid scale factor }

\footnote{\bf{The contents of this chapter has been published in Int. J. Geom. Mod. Phys, \textbf{14}, 1750124 (2017)}}
\pagebreak


\section{Introduction}

 In this present chapter, we have constructed anisotropic DE model at the back ground of Bianchi V space time in GR and investigated the dynamics of the model considering two different non interacting fluids contributing to the matter field. The first one is usual cosmic string fluid and the second one is due to the DE. The outline of the chapter is as follows; In section 5.2, we have set up the mathematical formulation of the problem along with its corresponding physical parameters. In section 5.3, the significance of hybrid scale factor has been analysed which mimic a cosmic transition. The physical and kinematical properties of the model has been discussed in section 5.4. In section 5.5, the results and summaries are discussed.
 
\section{Mathematical Formalism of the model}

We know from General Relativity that all sources can be described by an observer or class of observers by the energy momentum tensor $(T_{ij})$. Therefore in any model, we are interested to find the governing equations of motion along with some source of matter of universe, we take help of Einstein's field  equation. The R.H.S of the equation contains $T_{ij}$ of the corresponding source matter along with a coupling constant, that governs the dynamics of the curved space time. The energy momentum tensor for the given environment with two non interacting fluids is,

\begin{equation}
T_{ij}=T_{ij}^{(cs)}+T_{ij}^{(de)} \label{eq:5.2}
\end{equation}
where $T_{ij}^{(cs)}$ and $T_{ij}^{(de)}$ respectively denote the contribution to energy momentum tensor from one dimensional cosmic string and DE. For cosmic string,the energy momentum tensor can be defined as 

\begin{equation}\label{eq:5.3} 
T^{(cs)}_{ij} = (\rho + p) u_{i} u_{j}- pg_{ij}+ \lambda x_{i}x_{j}
\end{equation}
where $u_{i}u_{j}=x_{i}x_{j}=1$ (along x- direction). In a co moving coordinate system $u^i$ is the four velocity vector of the fluid. The pressure $p$ for this fluid is taken to be isotropic, $\rho$ as proper energy density for a cloud of strings and $\lambda$ as string tension density. The energy momentum tensor for DE can be described as

\begin{eqnarray} \label{eq:5.4}
T^{(de)}_{ij}  = diag[-\rho_{de}, p_{de_x},p_{de_y},p_{de_z}]\\ \nonumber
			   = diag[-1, \omega_{de_x},\omega_{de_y},\omega_{de_z}]\rho_{de}\\ \nonumber
			   =diag[-1, \omega_{de}+\delta,\omega_{de}+\gamma,\omega_{de}+\eta]\rho_{de} ,
\end{eqnarray}

where $\omega_{de}$ is the equation of state parameter (EoS)for DE and $\rho_{de}$ is the DE density. The skewness parameters, the deviations
from $\omega_{de}$ on $x$, $y$ and $z$ axes are respectively represented as $\delta$, $\gamma$ and $\eta$ . Now, the field equations for a two fluid i.e the cosmic string and DE with  Bianchi type V space-time in the frame work of GR are obtained as  

\begin{equation}\label{eq:5.5}
\frac{\ddot{B}}{B}+\frac{\ddot{C}}{C}+\frac{\dot{B}\dot{C}}{BC}-\frac{\alpha^{2}}{A^{2}}=-p-\lambda-(\omega_{de}+\delta)\rho_{de}  
\end{equation} 

\begin{equation}\label{eq:5.6}
\frac{\ddot{A}}{A}+\frac{\ddot{C}}{C}+\frac{\dot{A}\dot{C}}{AC}-\frac{\alpha^{2}}{A^{2}}=-p-(\omega_{de}+\gamma)\rho_{de} 
\end{equation}

\begin{equation}\label{eq:5.7}
\frac{\ddot{A}}{A}+\frac{\ddot{B}}{B}+\frac{\dot{A}\dot{B}}{AB}-\frac{\alpha^{2}}{A^{2}}=-p-(\omega_{de}+\eta)\rho_{de}
\end{equation}

\begin{equation}\label{eq:5.8}
\frac{\dot{A}\dot{B}}{AB}+\frac{\dot{B}\dot{C}}{BC}+\frac{\dot{C}\dot{A}}{CA}-\frac{3\alpha^{2}}{A^{2}}=\rho+\rho_{de} 
\end{equation}

\begin{equation} \label{eq:5.9}
2\frac{\dot {A}}{A}-\frac{\dot{B}}{B}-\frac{\dot{C}}{C}=0
\end{equation}

where an over dot is represented as the derivatives with respect to time $t$. Eqn. \eqref{eq:5.9} yields $A^2=k BC$. Suitably the integration constant absorbed into the metric potential $B$ or $C$ to yield $A^2=BC$. In order to study the models, some physical parameters can be defined as : the cosmic spatial volume and the scalar expansion $\theta$ can be obtained respectively as $V=R^3=ABC$ and $\theta=3H$, where $H=\frac{\dot{R}}{R}=\frac{1}{3}(H_x+H_y+H_z)$.  $H_x$, $H_y$ and $H_z$ are directional Hubble parameter in the direction of $x$, $y$ and $z$ respectively. The shear scalar $\sigma^2=\frac{1}{2}(H_x^2+H_y^2+H_z^2-\frac{\theta^2}{3})$ and the deceleration parameter can be calculated from $ q=-\frac{R\ddot{R}}{\dot{R}^2} $. In order to get an anisotropic relation between the scale factors of different directions, we assume $B=C^m, m\neq1$. Accordingly the scale factors in different directions can be expressed as , $A=R, B=R^{\frac{2m}{m+1}}, C=R^{\frac{2}{m+1}}$. As the behaviour of the model would be studied through the behaviour of Hubble parameter, therefore the directional Hubble parameters can be calculated as, $H_x=H$, $H_y=\big(\frac{2m}{m+1}\big)H$ and $H_z=\big(\frac{2}{m+1}\big)H$. The anisotropic parameter $\mathcal{A}$ can be obtained as

\begin{equation} \label{eq:5.10}
{\mathcal A}=\frac{1}{3}\sum \biggl(\frac{\vartriangle H_i}{H}\biggr)^2
\end{equation}

The energy conservation equation for the anisotropic fluid, $T^{ij}_{;j}=0$ can be defined as 

\begin{equation} \label{eq:5.11}
\dot{\rho}+3(p+\rho)H+\lambda H_x+\dot{\rho_{de}}+3\rho_{de}(\omega_{de}+1)H+\rho_{de}(\delta H_x+\gamma H_y+\eta H_z)=0
\end{equation}

From eqn. \eqref{eq:5.11}, the energy conservation equation for string fluid, $T^{ij(cs)}_{;j}=0$ and DE fluid $T^{ij(de)}_{;j}=0$ respectively obtained as:

\begin{equation} \label{eq:5.12}
\dot{\rho}+3(p+\rho)H+\lambda H_x=0
\end{equation}
and
\begin{equation} \label{eq:5.13}
\dot{\rho_{de}}+3\rho_{de}(\omega_{de}+1)H+\rho_{de}(\delta H_x+\gamma H_y+\eta H_z)=0
\end{equation}

We assume $\rho=\xi \lambda$ and $p=\omega \rho $ in \eqref{eq:5.12}. The constants, $\xi$ and $\omega$ are state parameter variables which can be positive and negative and  $\omega \in[-1,1]$. A positive $\xi$ value indicates the presence of one dimensional string in cosmic fluid and a negative $\xi$ value shows the strips of the string phase of the universe. Hence, we obtain
\begin{equation} \label{eq:5.14}
\rho=(ABC)^{-(1+\omega)}A^{-\frac{1}{\xi}}\rho_0
\end{equation}
where $\rho_0$ is the integration constant or rest energy density. Subsequently, pressure and string density can be obtained as:

\begin{eqnarray} 
p=\frac{\omega \rho_0 A^{-\frac{1}{\xi}}}{(ABC)^{1+\omega}};\label{eq:5.15}\\
\lambda=\frac{\rho_0 A^{-\frac{1}{\xi}}}{\xi (ABC)^{1+\omega}} \label{eq:5.16}
\end{eqnarray}

Now, eqn. \eqref{eq:5.8} and eqn. \eqref{eq:5.14} yields,

\begin{equation}\label{eq:5.17}
\rho_{de}= \frac{\dot{A}\dot{B}}{AB}+\frac{\dot{B}\dot{C}}{BC}+\frac{\dot{C}\dot{A}}{CA}-\frac{3\alpha^{2}}{A^{2}}-\frac{\rho_0 A^{-\frac{1}{\xi}}}{(ABC)^{1+\omega}}
\end{equation}

We can split \eqref{eq:5.13} into two parts; one corresponds to the deviation of EoS parameter and other is deviation free part as:

\begin{equation} \label{eq:5.18}
\dot{\rho_{de}}+3\rho_{de}(\omega_{de}+1)H=0 
\Rightarrow \rho_{de}=\rho_{de_0} R^{-3(\omega_{de}+1)}
\end{equation}

\begin{equation} \label{eq:5.19}
\rho_{de}(\delta H_x+\gamma H_y+\eta H_z)=\rho_{de} \left(\delta +\gamma \left(\frac{2m}{m+1}\right)+\eta \left(\frac{2}{m+1}\right)\right)\frac{\dot{R}}{R}=0  
\end{equation}
According to the eqn. \eqref{eq:5.18}, the DE density behaviour $(\rho_{de})$ is diagnosed by the deviation free part of EoS parameter of DE , where $\rho_{de_0}$ indicates DE density at present epoch. The second equation deals with the anisotropic part i.e. the deviations from the total DE pressure along different spatial directions.\\

Algebraic manipulation of equations \eqref{eq:5.5} ,\eqref{eq:5.6}, \eqref{eq:5.7} and
using $\lambda$ from eqn. \eqref{eq:5.16}, the skewness parameters take the form,
\begin{eqnarray}
\gamma= \frac{1}{3\rho_{de}}\biggl[\frac{(m+5)}{(m+1)} \chi(m) F(R)+\frac{\rho_0}{\xi} G(R)\biggr] \label{eq:5.20}\\
\eta=-\frac{1}{3\rho_{de}}\biggl[\frac{(5m+1)}{(m+1)} \chi(m) F(R)-\frac{\rho_0}{\xi} G(R)\biggr] \label{eq:5.21}\\
\delta=-\frac{2}{3\rho_{de}}\biggl[\frac{(m-1)}{(m+1)} \chi(m) F(R)-\frac{\rho_0}{\xi} G(R) \biggr] , \label{eq:5.22}
\end{eqnarray}
where  $\chi (m)= \dfrac{m-1}{m+1}$, represents the amount of difference from isotropic behaviour of the model.   $F(R)=\biggl( \dfrac{\ddot{R}}{R}+ \dfrac{2 \dot{R}^{2}}{R^{2}} \biggr)$ and $G(R)=\dfrac{1}{R^{3(1+ \omega+\frac{1}{3\xi})}}.$\\
To get the model isotropic, $\chi(m)$ vanishes and consequently,
the skewness parameters will retain only the string terms, because the anisotropic part vanished. Subsequently, the DE density $\rho_{de}$ and the EoS parameter $\omega_{de}$ can be  obtained as,

\begin{align} \label{eq:5.23}
\rho_{de} =   \dfrac{\dot{R}^2}{2R^2}\left[ \phi(m) \right]- 3 \dfrac{\alpha ^2}{R^2}- \rho_{0} G(R) 
\end{align}

\begin{align} \label{eq:5.24}
- \omega_{de} \rho_{de} & = \dfrac{4\ddot{R}}{3 R} \left[ \phi(m) \right]  +  \dfrac{2\dot{R}^2}{3R^2} \left[ \phi(m) \right] + \rho_{0} G(R) \left[ \dfrac{1}{3 \xi} + \omega \right] - \dfrac{\alpha ^{2}}{R^2}, 
\end{align}

where, $\phi(m)= \dfrac{m^{2} + 4 m + 1}{(m+1)^2}$.

The functional $F(R)$ and the DE density $\rho_{de}$ completely controlled the behaviour of skewness parameters and the functional $\chi (m)$ depends upon the exponent $m$. EoS parameter for DE is decided by the anisotropic nature of the model through this
exponent $m$, the time dependence of mean Hubble parameter $H$, the hybrid scale factor $R$ and the rest energy density $\rho_{0}$. It is interesting to note that, the DE density and the DE EoS parameter depend on the usual cosmic string fluid too. 

\section{Hybrid scale factor and Cosmic transit}

Based on the recent outcomes on the present universe, the appropriate choice for the scale factor are the de Sitter solution and the power law expansion. The behaviour of both power law and exponential law of the scale factor lead to a constant deceleration parameter. However, the time dependence of the directional scale factor would be decided by specific choices of scale factors. In the present work, we have considered the specific scale factor, the hybrid scale factor which at late time results into a constant deceleration parameter. The hybrid scale factor has two factors in the form, $R=e^{at}t^{b}$, where $a$ and $b$ are positive constants. In this combined form of the scale factor one form is on exponential expansion and the other is on power law expansion. The cosmic dynamics is dominated by the power law $(t^{b})$ in the early phase, whereas it is dominated by the exponential factor $(e^{at})$ at late phase. However, eventually, the hybrid scale factor pulls itself away towards later phase of evolution in a more dominant fashion which may mimic the accelerated expansion of universe. When $a=0,$ the scale factor reduces to the power law and for $b=0,$ the exponential law recovered. So, a cosmic transition from early deceleration to late time acceleration can be obtained by a hybrid scale factor.\\

For this model, the Hubble parameter and the directional Hubble parameter can be obtained respectively as $H = a+\dfrac{b}{t}$ and $H_{x} = a+\dfrac{b}{t}, H_{y}=\dfrac{2m}{m+1}\left(a+\dfrac{b}{t}\right) $ and $Hz = \dfrac{2}{m+1}\left(a+\dfrac{b}{t}\right)$ \cite{akarsu3, kumar2, pradhan3}. Tripathy \cite{tripa2} has considered a general form of such  parameter in the form $H = a+ \dfrac{b}{t^{n}}$ , $n$ being a constant.\\

The deceleration parameter $q = - \dfrac{\ddot{R}}{R^2}$ describes cosmic dynamics concerning the late time acceleration. A positive deceleration parameter indicates a decelerating universe, negative value describes a universe with acceleration expansion and a null value predicts a universe expanding with constant rate. Since most of observational data favour an accelerating universe, models with late time cosmic dynamics have got much focus in recent times. In this present work, we are interested in the kinematics of late time accelerating
universe while the deceleration parameter is assumed to vary slowly or becoming a constant with cosmic time. According to type Ia Supernovae observations, the deceleration parameter for the accelerating universe in the present time is $q = -0.81 \pm 0.14$ \cite{rapet}. Type Ia Supernovae data in combination with BAO and CMB observations declare the deceleration parameter as $q = -0.53 ^{+0.17}_{-0.13}$ \cite{giost}. Eventually, the deceleration parameter becomes $q =   -1+ \dfrac{b}{(at+b)^{2}}$ . At an early phase of cosmic evolution when $t \longrightarrow 0,$ $ q \simeq -1 + \dfrac{1}{b}$ and at late phase of cosmic evolution with $t \longrightarrow \infty , q \simeq -1 $. To find a transient universe with early deceleration and late acceleration, we constrain the parameter $b$ to be in the range $0 < b < 1$ so that at early time $q$ can be positive whereas at late time $q$ assumes a negative value in conformity with the recent observational data.  We can infer from deceleration parameter evaluated here that, the cosmic transit occurs at a time $t = -\dfrac{b}{a}\pm \dfrac{\sqrt{b}}{a}$. The negativity of the second term leads to a concept of negative time which may be unphysical in the context of Big Bang cosmology and therefore, the cosmic transit may have occurred at time $t =\dfrac{\sqrt{b}-b}{a}$, which again restricts $b$ in the same range $0 < b < 1$. The variation of deceleration parameter vs. time for the representing value of the constant $a=0.1$ and $ b=0.3$ has been depicted in Fig. 5.1 which also shows that the transition occurs at $t=2.47$.\\

\begin{figure}[h!]

\minipage{0.56\textwidth}
\includegraphics[width=75mm]{q1stP.pdf}
\caption{Variation of deceleration parameter $q$  vs. time with a=0.1 and b=0.3}
\endminipage
\end{figure}

With this consideration of hybrid scale factor the directional scale factors can be expressed as $ A=R=e^{at}t^b; B=R^{\frac{2m}{m+1}}=(e^{at}t^b)^{\frac{2m}{m+1}};$ and $ C=R^{\frac{m}{m+1}}=(e^{at}t^b)^{\frac{2}{m+1}}$. Subsequently, eqns. \eqref{eq:5.20} - \eqref{eq:5.23} can be recasted as, 

\begin{eqnarray}
\gamma &=& \frac{1}{3\rho_{de}}\biggl[\frac{(m+5)}{(m+1)} \chi(m) F(t)+\frac{\rho_0}{\xi} \dfrac{1}{R^{3(1+ \omega-\frac{1}{3\xi})}}\biggr] \label{eq:5.25}\\
\eta &=&-\frac{1}{3\rho_{de}}\biggl[\frac{(5m+1)}{(m+1)} \chi(m) F(t)-\frac{\rho_0}{\xi} \dfrac{1}{R^{3(1+ \omega-\frac{1}{3\xi})}}\biggr] \label{eq:5.26}\\
\delta &=& -\frac{2}{3\rho_{de}}\biggl[\frac{(m-1)}{(m+1)} \chi(m) F(t)-\frac{\rho_0}{\xi} \dfrac{1}{R^{3(1+ \omega-\frac{1}{3\xi})}}\biggr] , \label{eq:5.27}
\end{eqnarray}

where $F(t)=\frac{3a^2t^2+6abt+3b^2-b}{t^2}$. The DE density and EoS parameter can be expressed as,

\begin{align} \label{eq:5.28}
\rho_{de} =  \frac{2(m^2+4m+1)(a+\frac{b}{t})^2-
 3 \alpha^2(e^{at}t^b)^{-2}(m+1)^2}{(m+1)^2} -  \rho_0(e^{at}t^b)^{\frac{1}{\xi}-3(1+\omega)}
\end{align}

\begin{align} \label{eq:5.29}
\omega_{de}& = \frac{-4(m^2+4m+1)(a^2 t^2+2abt+b(b-1))}{6(m^2+4m+1)(at+b)^2-9 \alpha^2(m+1)^2 e^{-2at-2b+2} -3 \rho_{0} (m+1)^{2} t^{2} (e^{at}t^{b})^{\frac{1}{\xi}-3(1+\omega)} } \nonumber
\\  &\nonumber -
\frac{2(m^3+5m^2+5m+1)(at+b)^2}{6(m^2+4m+1) (m+1)(at+b)^2-9 \alpha^2(m+1)^3 e^{-2at-2b+2}-3 \rho_{0} (m+1)^{3} t^{2} (e^{at}t^{b})^{\frac{1}{\xi}-3(1+\omega)} } \nonumber \\&
- \frac{[(\frac{1}{3\xi}+\omega)\rho_0(e^{at}t^b)^{-\frac{1}{\xi}-3(1+\omega)}-\alpha^2(e^{at}t^b)^{-2}](m+1)^2}{2(m^2+4m+1)(a+\dfrac{b}{t})^2 - 3 \alpha^{2} (e^{at}t^{b})^{-2} (m+1)^2 - \rho_{0} (m+1)^{2}(e^{at}t^{b})^{\frac{1}{\xi}-3(1+\omega)} }
\end{align}

The density parameter of the cosmic string fluid $\Omega_{cs}$  and the density parameter of DE fluid $\Omega_{de}$ can be derived respectively as 

\begin{align} \label{eq:5.30}
\Omega_{cs}= \dfrac{\rho_{0}}{3} \dfrac{(e^{at}t^{b})^{\frac{1}{\xi}-3}}{\left(a+\dfrac{b}{t}\right)^2}
\end{align}

\begin{align} \label{eq:5.31}
\Omega_{de}= \dfrac{2}{3} \dfrac{(m^2+4m+1)}{(m+1)^2}-\dfrac{\alpha^{2}(e^{at}t^{b})^{-2}}{\left(a+\dfrac{b}{t}\right)^2}-\dfrac{\rho_{0}(e^{at} t^{b})^{\frac{1}{\xi}-3}}{3 \left(a+\dfrac{b}{t}\right)^2}
\end{align}

and subsequently the total density parameter can be obtained as, 

\begin{align} \label{eq:5.32}
\Omega_{T} \equiv \Omega_{cs} + \Omega_{de} = \mathcal{A} +\dfrac{4m}{(m+1)^2} -\dfrac{\alpha^{2}(e^{at}t^{b})^{-2}}{\left(a+\dfrac{b}{t}\right)^2},
\end{align}

where, $\mathcal {A}$ = $\dfrac{2 \sigma^{2}}{3H^{2}}= \dfrac{2}{3} \left( \dfrac{m-1}{m+1} \right) ^{2}$ is the anisotropy parameter of expansion. Here also we can see that for $m=1$, the anisotropy parameter is zero, which further confirms the isotropic behaviour of the model. 


\section{Physical Properties of the model}

\begin{figure}[h!]

\minipage{0.56\textwidth}
\includegraphics[width=75mm]{rho1stP.pdf}
\caption{Variation of DE density $\rho_{de}$ vs cosmic time with $m=2,$ $a=0.1,$ $b=0.3,$ $\alpha = 0.05,$ $\rho_{0}=0.2$ and $\xi =1$}
\endminipage
\end{figure}


From Fig. 5.2, we observed that during cosmic evolution, the DE density $(\rho_{de})$ remains positive. Therefore, in the derived model, both weak energy condition (WEC) and null energy condition (NEC) are satisfied. Further, $\rho_{de}$ decreases with time and leads to a small positive values in present time. The value of DE density comes closer to zero at late phase $(t \in [400,500])$ and then smoothly approaches to small positive value which indicates that the considered two fluid affects the DE density.  Similarly, it can be shown the string energy density $(\rho)$ will follow the same behaviour as of $\rho_{de}$. Fig. 5.3, depicts the variation of EoS parameters $(\omega_{de})$ with cosmic time, as a representative case with appropriate choice of constants of integration and other physical parameters for accelerating phase of universe.  The SN Ia data suggests the range value of EoS parameter as $-1.67 < \omega_{de} < -0.62$ where as the limit imposed by a combination of SN Ia data with CMB anisotropy and galaxy clustering statistics is in the range $-1.33 < \omega_{de} < -0.79.$ Again Fig. 5.3 shows that $\omega_{de}$ evolves in the range, which is in agreement with SN Ia and CMB observations. Also, the value of EoS parameter increases strictly in a range $(t \in [5,10])$, then decreases smoothly and remains constant in the preferred range. The behaviour of $\omega_{de}$ is different from other discussed literature but the value lies in the same range as in the observational result. So, we can infer here that the considered two fluid matter affects the EoS parameter of the model. \\

To check whether our model is realistic or not, the energy densities of the fluid need to be worked out. For a large value of $t$, the density parameter approaches to a finite value as $\Omega_{de}=\frac{2}{3}\frac{m^2+4m+1}{(m+1)^2}$. Further, the parameter started decreasing at an initial value and subsequently increases from the representing value of the cosmic time $t=0.462$ and remain constant at large $t$. In the case of string fluid, the density parameter $\Omega_{cs}$ initially increases and started decreasing at a representing value of $t=0.478$ and subsequently vanishes at infinite time. However,  the total density parameter is found to be $\Omega_T=0.97$, which also in accordance with the present observational data.  Also, it has been observed that the string density parameter dominates for a small time period i.e. at $t=0.471$ to $t=0.473$ and beyond that the DE density parameter dominates further.  The details are depicted in Fig. 5.4. \\

Fig. 5.5 shows that the evolution of skewness parameters with cosmic dynamics. In this figure, it can be noted that the behaviour of skewness parameters are totally controlled by the  parameter $m$. For $m=1$, the skewness parameters retain only the cosmic string nature giving an indication that the cosmic string matter affects the skewness parameters. We observed, at early cosmic phase $\eta$ starts with a small positive value, decreases with the cosmic time to became minimum and then becomes constant with further increase in cosmic time. The skewness parameter $\gamma$ also starts from a small negative value, attains maximum and becomes constant with respect to cosmic time. The evolutionary behaviour of $\delta$ is just the similar image of  $\delta$ but it retains a negative constant value at late phase. It can be noted that the pressure anisotropy factors along $x$, $y$ and $z$ axis $(\eta, \delta,\gamma)$ evolves with different nature, attain their extreme in a definite range of cosmic time $1<t<2$ and remain constant at later time. Hence we can infer that, the pressure anisotropies remain even at the late phase of cosmic evolution though in the early phase pressure was assumed to be isotropic. Also, it is interesting to note that, at the switching over cosmic time $t=0.02$, all the skewness parameters vanish.  

\begin{figure}[h!]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=65mm]{omega1stP.pdf}
\caption{Dynamics of EoS parameter of DE with respect to cosmic vs time with $m=2,$ $a=0.1,$ $b=0.3,$ $\alpha = 0.05,$ $\rho_{0}=0.2$ and $\xi = 1$}
\endminipage\hfill
\end{figure}
\begin{figure}[h!]
\minipage{0.56\textwidth}
\includegraphics[width=65mm]{OMEGA1stP.png}
\caption{Density parameter of DE $\Omega_{de}$, string fluid $\Omega_{cs}$ and the total density parameter $\Omega_T$ with respect to cosmic time with $m=2,$ $a=0.1,$ $b=0.3,$ $\alpha = 0.05,$ $\rho_{0}=0.2$ and $\xi = 1$}
\endminipage
\end{figure}


\begin{figure}[h!]
\minipage{0.56\textwidth}
\includegraphics[width=65mm]{skewness1stP.pdf}
\caption{Dynamical evolution of Skewness parameters along three spatial directions with respect to cosmic time with $m=2,$ $a=0.1,$ $b=0.3,$ $\alpha = 0.05,$ $\rho_{0}=0.2$ and $\xi = 1$}
\endminipage
\end{figure}

The scalar expansion $ \theta=3H=3(a+\frac{b}{t})$ and shear scalar $\sigma^2=\frac{1}{2}(H_x^2+H_y^2+H_z^2-\frac{\theta^2}{3})=\biggl(\frac{m-1}{m+1}\biggr)^2\biggl(a+\frac{b}{t}\biggr)^2 $  start off with extremely large values and continue to decrease with expansion of universe. The anisotropic parameter $\mathcal{A}_m=\frac{1}{3}\sum \biggl(\frac{\vartriangle H_i}{H}\biggr)^2=\frac{2}{3}\biggl(\frac{m-1}{m+1}\biggr)^2$, which is a measure of deviation from the isotropic expansion. If $\mathcal{A}=0$, the model is isotropic, otherwise anisotropic. In this case for $m=1$, the model becomes isotropic. Moreover, the average anisotropic parameter of the model is time independent which gives the indication that the anisotropy in expansion rates is maintained throughout the cosmic evolution. The state finder diagnostic pair $(r,s)$ provide an idea about the geometrical nature of the model and also through this the viability of the DE model can be tested. The pair can be obtained as $r=\frac{\tau^3-3b\tau+2b}{\tau^3}$ and $s= \frac{4b-6b\tau}{6b\tau-9\tau^3}$, where $\tau=at+b$. The state finder pair values depend on the constants $a$ and $b$ of the scale factor chosen. The state finder pair for the present model at the initial time is $\left({\frac{b^2-3b+2}{b^2}}, \frac{2}{3b}\right)$ and at the late time of cosmic evolution the value of state finder pair is $(1,0)$, which confirms that the model behaves like $\Lambda$ CDM.

\section{Conclusion}

In the present work, we have constructed an anisotropic DE cosmological model in the framework of GR and Bianchi type V space time. In order to study the evolution of skewness parameters and the EoS parameters, we have developed the DE models in two fluid situations. The EoS parameter of DE evolves within the range predicted by the observations. In the present epoch, the DE dominates the universe. This may be attributed to the current accelerated expansion of the universe. The parameter $m$ is responsible for the anisotropic behaviour and the matter behaviour of the model in the sense that, if $m=1$, we get isotropic model where only string matter part exist and for $m \neq 1,$ anisotropic and two fluid nature will be retained. In the present models,as expected, the matter energy density and DE density remains positive. Therefore, the energy conditions are satisfied, which in turn imply that the derived models are physically realistic. Moreover, it is showed that, there remain pressure anisotropies even at the late phase of cosmic evolution, though in the early phase pressure was assumed to be isotropic. Further the state finder pair is varying with time and decrease with the cosmic evolution in late time. Further the EoS of parameter changed with cosmic time and which indicates that during evolution there exists a relationship between the mean pressure of the cosmic fluid and energy density. The total density parameter $\Omega_T$, which quantifies the density of matter in the universe is found to be in the observational range $-1<\Omega_T<1$. In most part of the evolution, the DE density dominates the matter density; however for a small range of the cosmic time, the matter density dominates the DE density. So, we can conclude through the behaviour of the density parameter, that our model also mimics the cosmic acceleration in the early phase and also in late phase.\\

==> Report_format_thesis/Chapter6.tex <==
\chapter{Reconstruction of accelerating Bianchi v string cosmological model with dark energy anisotropy }

\footnote{\bf{The contents of this chapter has been published in Astrophysics and Space Science, \textbf{363}, 86 (2018)}}

\pagebreak


\section{Introduction}

In the present Chapter, we consider a general form of non interacting dark energy with anisotropic pressures along  different spatial directions and have investigated the effect of anisotropic components on the dark energy density parameter and the equation of state. In addition to the anisotropic DE fluid, cosmic strings aligned along x-direction are also considered to incorporate some anisotropic effect. In some of our earlier studies, we have investigated the dynamical behavior of pressure anisotropies either in the framework of GR or alternative gravity theory \cite{mishra015a, mishra015b}. Cosmological studies involving one dimensional cosmic strings are interesting in the sense that, they may provide some explanation to the Physics of the early universe. Moreover, cosmic strings are believed to arise as topological defects during the spontaneous symmetry breaking. They may help in the formation of large structures like galaxies. There are some interesting investigations on different aspects of string cosmological models in recent times \cite{SKT08, SKT09a, SKT09b,SKT09c, Saha08}.

The chapter is organized as follows. In Sect. 6.2, we discuss the basic formalism of an anisotropic dark energy. The effect of anisotropy on dark energy and the DE equation of state (EoS) parameter is discussed in Sect. 6.3 and we summarize our results in Sect. 6.4.
 
\section{Basic Formalism}

We have considered a spatially homogeneous and anisotropic Bianchi V (BV) space time in \eqref{eq:2.1}. The energy momentum tensor for a given environment of two non interacting fluids in \eqref{eq:2.2} is  now given by,

\begin{equation}
T_{\mu\nu}=T_{\mu\nu}^{s}+T_{\mu\nu}^{D} \label{eq:6.1}
\end{equation}
where $T_{\mu\nu}^{s}$ and $T_{\mu\nu}^{D}$ respectively denote the contribution to energy momentum tensor from one dimensional cosmic strings and DE. For a cosmic fluid containing one dimensional strings \cite{letelier, stachel}, the energy momentum tensor is 

\begin{equation}\label{eq:6.2} 
T^{s}_{\mu\nu} = (\rho + p) u_{\mu} u_{\nu}- pg_{\mu\nu}+ \lambda x_{\mu}x_{\nu}
\end{equation}
where $u^{\mu}u_{\mu}=-x^{\mu}x_{\mu}=1$ and $u^{\mu}x_{\mu}=0$. In a co moving coordinate system, $u^{\mu}$ is the four velocity vector and $p$ is the isotropic pressure of the fluid. $x^{\mu}$ represents the direction of cosmic strings (here x-direction). $\rho$ is the proper energy density and is composed of energy density due to massive particles and the string tension density $\lambda$. In the absence of any string phase, the total contribution to the baryonic energy density comes from particles only. In contrast to the isotropic pressure of usual cosmic fluid, we wish to incorporate some degree of anisotropy in the DE pressure and consider the energy momentum tensor for DE as

\begin{eqnarray} \label{eq:6.3}
T^{D}_{\mu\nu} & = & diag[-\rho_{D}, p_{D_x},p_{D_y},p_{D_z}] \nonumber\\ 
			 % & = & diag[-1, \omega_{de_x},\omega_{de_y},\omega_{de_z}]\rho_{de}\\ \nonumber
			  & = & diag[-1, \omega_{D}+\delta,\omega_{D}+\gamma,\omega_{D}+\eta]\rho_{D} ,
\end{eqnarray}
where $\omega_{D}$ is the DE equation of state parameter and $\rho_{D}$ is the DE density. The skewness parameters $\delta$, $\gamma$ and $\eta$ are the deviations from $\omega_{D}$ along $x$, $y$ and $z$ axes respectively. The DE pressure becomes isotropic when $\delta$, $\gamma$ and $\eta$ vanish identically.

The field equations, $G_{\mu\nu}=T_{\mu\nu}$, for a two fluid system consisting of cosmic strings and DE in a BV metric are obtained as  

\begin{equation}\label{eq:6.4}
\frac{\ddot{a_2}}{a_2}+\frac{\ddot{a_3}}{a_3}+\frac{\dot{a_2}\dot{a_3}}{a_2a_3}-\frac{\alpha^{2}}{a_1^{2}}=-p-\lambda-(\omega_{D}+\delta)\rho_{D}  
\end{equation} 

\begin{equation}\label{eq:6.5}
\frac{\ddot{a_1}}{a_1}+\frac{\ddot{a_3}}{a_3}+\frac{\dot{a_1}\dot{a_3}}{a_1a_3}-\frac{\alpha^{2}}{a_1^{2}}=-p-(\omega_{D}+\gamma)\rho_{D} 
\end{equation}

\begin{equation}\label{eq:6.6}
\frac{\ddot{a_1}}{a_1}+\frac{\ddot{a_2}}{a_2}+\frac{\dot{a_1}\dot{a_2}}{a_1a_2}-\frac{\alpha^{2}}{a_1^{2}}=-p-(\omega_{D}+\eta)\rho_{D}
\end{equation}

\begin{equation}\label{eq:6.7}
\frac{\dot{a_1}\dot{a_2}}{a_1a_2}+\frac{\dot{a_2}\dot{a_3}}{a_2a_3}+\frac{\dot{a_3}\dot{a_1}}{a_3a_1}-\frac{3\alpha^{2}}{a_1^{2}}=\rho+\rho_{D} 
\end{equation}

\begin{equation} \label{eq:6.8}
2\frac{\dot {a_1}}{a_1}-\frac{\dot{a_2}}{a_2}-\frac{\dot{a_3}}{a_3}=0,
\end{equation}
where an over dot represents the differentiation with respect to time $t$. One can note that, anisotropy is incorporated in two different manner in the field equations: one due to the inherent anisotropic DE fluid and the other through the presence of aligned cosmic strings along x-axis. These anisotropic components leads to the anisotropy in the cosmic geometry described through the BV space time.

The cosmic spatial volume and the scalar expansion $\theta$ can be obtained respectively as $V=R^3=a_1a_2a_3$ and $\theta=3H$, where $H=\frac{\dot{R}}{R}=\frac{1}{3}\sum_{i=1}^{3} H_i$ is the mean Hubble parameter.  $H_i=\frac{\dot{a_i}}{a_i}$ are the directional Hubble parameters along different spatial directions. The shear scalar is given by $\sigma^2=\frac{1}{2}(\sum_{i=1}^{3} H_i^2-\frac{\theta^2}{3})$ and the deceleration parameter can be calculated from the relation $ q=\frac{d}{dt} \left(H^{-1}\right)-1$. 

It is straightforward to obtain $a_1^2=a_2a_3$ from \eqref{eq:6.8}. In order to get an anisotropic relation between the directional scale factors, we assume 
\begin{equation}\label{eq:6.9}
a_2=a_3^k,
\end{equation}
where $k$ is an arbitrary positive constant else than 1. Consequently, the scale factors along different directions can be $a_1=R,~ a_2=R^{\frac{2k}{k+1}}$ and $a_3=R^{\frac{2}{k+1}}$. The directional Hubble parameters can be obtained as, $H_1=H$, $H_2=\big(\frac{2k}{k+1}\big)H$ and $H_3=\big(\frac{2}{k+1}\big)H$.  The anisotropic parameter $\mathcal{A}$ can be obtained as 
\begin{equation} \label{eq:6.10}
{\mathcal A}=\frac{1}{3}\sum \left(1-\frac{H_i}{H}\right)^2=\frac{2}{3}\left(\frac{k-1}{k+1}\right)^2.
\end{equation}
The anisotropic nature of model can also be  quantified through the estimation of $\frac{\sigma}{H}$ at the present epoch. In many earlier works, there have been discussions on this quantity which may come out to be constant with time \cite{SKT10, Muh18,Saha12,Collins77, Collins80, Roy85, Roy95, Bali08, Sharif10}. For the BV model, this quantity can be obtained as 

\begin{equation} \label{eq:6.11}
\frac{\sigma}{H}= \left[\frac{5k^2+2k+5}{2(k+1)^2}-1.5\right]^{\frac{1}{2}}.
\end{equation}
Observational limits to this quantity have been obtained by many workers in recent times. From an analysis of COBE data, Bunn et al. have obtained a limit of $\left(\frac{\sigma}{H}\right)_0 < 3 \times 10^{-9}$ \cite{bunn16}. Saadeh et al. put a tighter constraint of  $\left(\frac{\sigma}{H}\right)_0 < 4.7 \times 10^{-11}$ which strongly disfavours the anisotropic expansion of the universe \cite{saadeh16}. We may constrain the parameter $k$ according to these bounds. In the present work, we have formulated a model, which can be suited better for any amount of cosmic anisotropy. However, we use the previous constraint on $k$ i.e $k=1.0001633$ so that  $\left(\frac{\sigma}{H}\right)_0$ becomes $8.164 \times 10^{-5}$ \cite{mishra015a} to obtain some considerable effects on the dynamical features of the universe.


The energy conservation equation for the anisotropic fluid, $T^{\mu\nu}_{;\nu}=0$ yields 

\begin{equation} \label{eq:6.12}
\dot{\rho}+3(p+\rho)H+\lambda H_1+\dot{\rho_{D}}+3\rho_{D}(\omega_{D}+1)H+\rho_{D}(\delta H_1+\gamma H_2+\eta H_3)=0.
\end{equation}

We consider the cosmic string and DE to be non interacting and obtain two separate equations from \eqref{eq:6.12},

\begin{equation} \label{eq:6.13}
\dot{\rho}+3H\left(\rho+p+\frac{\lambda}{3}\right)=0
\end{equation}
and
\begin{equation} \label{eq:6.14}
\dot{\rho_{D}}+3H\rho_{D}(\omega_{D}+1)+\rho_{D}(\delta H_1+\gamma H_2+\eta H_3)=0.
\end{equation}
The equations of state for strings and isotropic fluid can be considered respectively as 
\begin{eqnarray*}
\lambda &=& 3\xi \rho,\\
p &=& \omega \rho,
\end{eqnarray*}
where $\xi$ and $\omega$ are assumed to be non evolving state parameters. 

From \eqref{eq:6.13}, we get
\begin{equation} \label{eq:6.15}
\rho=\rho_0R^{-3(1+\omega+\xi)}
\end{equation}
where $\rho_0$ is rest energy density due to the matter field at the present epoch. Subsequently, pressure and string tension density can be obtained as

\begin{eqnarray} 
p &=& \omega\rho_0R^{-3(1+\omega+\xi)},\label{eq:6.16}\\
\lambda &=& 3\xi\rho_0R^{-3(1+\omega+\xi)}. \label{eq:6.17}
\end{eqnarray}

The DE density is obtained from \eqref{eq:6.7} and \eqref{eq:6.15} as

\begin{equation}\label{eq:6.18}
\rho_{D}= 3\left(\Omega_{\sigma}-\Omega_k\right)\left(\frac{\dot{R}}{R}\right)^2-\rho,
\end{equation}
where $\Omega_{\sigma}= 1-\frac{\mathcal{A}}{2}$ and $\Omega_k=\frac{\alpha^{2}}{\dot{R}^{2}}$.
The density parameters can be expressed as
\begin{eqnarray}
\Omega_{D} &=& \Omega_{\sigma}-\Omega_k-\Omega_m, \label{eq:6.19}\\
\Omega_m &=& \frac{\rho}{3H^2}.\label{eq:6.20}
\end{eqnarray}
The total density parameter becomes
\begin{equation}
\Omega=\Omega_m+\Omega_{D}= \Omega_{\sigma}-\Omega_k. \label{eq:6.21}
\end{equation}
Obviously, for a flat isotropic universe with $\alpha=0$ and $k=1$, the total density parameter reduces to be 1. However, in an anisotropic background the dynamics of dark energy density parameter is substantially affected according to the behavior of $\Omega_{\sigma}$.

Eq. \eqref{eq:6.14} can be split into two parts corresponding to the deviation free part and the one involving  the deviation from EoS parameter:

\begin{eqnarray} 
\dot{\rho_{D}}+3\rho_{D}(\omega_{D}+1)H & =& 0,\label{eq:6.22}\\
\delta H_1+\gamma H_2+\eta H_3 &=&0. \label{eq:6.23}
\end{eqnarray}

These equations can be expressed as 
\begin{eqnarray}
\dot{\rho_{D}}+3\rho_{D}(\omega_{D}+1)\frac{\dot{R}}{R} &=& 0,\label{eq:6.24}\\ 
\left[\delta +\gamma \left(\frac{2k}{k+1}\right)+\eta \left(\frac{2}{k+1}\right)\right]\rho_{D} \frac{\dot{R}}{R} &=& 0. \label{eq:6.25}
\end{eqnarray}

%Integration of \eqref{eq:20} yields the DE density as
%\begin{equation} \label{eq:22}
%\rho_{D}=\rho_{D_0} R^{-3(\omega_{D}+1)}.
%\end{equation}
%
%It is obvious that, the behavior of DE density $(\rho_{D})$ is diagnosed by the deviation free part of DE EoS. Here, $\rho_{D_0}$ is the DE density at present epoch. 

We obtain the skewness parameters from the field equations \eqref{eq:6.4},\eqref{eq:6.5}and \eqref{eq:6.6} as
\begin{eqnarray}
\delta &=& -\frac{2}{3\rho_{D}}\left[\zeta^2(k) F(R)+\lambda\right] , \label{eq:6.26}\\
\gamma &=& \frac{1}{3\rho_{D}}\biggl[\frac{(k+5)}{(k+1)} \zeta(k) F(R)+\lambda\biggr], \label{eq:6.27}\\
\eta &=& -\frac{1}{3\rho_{D}}\biggl[\frac{(5k+1)}{(k+1)} \zeta(k) F(R)-\lambda\biggr], \label{eq:6.28}
\end{eqnarray}
where  $\zeta (k)= \dfrac{k-1}{k+1}$, represents the amount of deviation from isotropic behavior of the model and $F(R)=\biggl( \dfrac{\ddot{R}}{R}+ \dfrac{2 \dot{R}^{2}}{R^{2}} \biggr)$. Besides the control of the parameter $k$, the pressure anisotropies are decided by the behavior of the functional $F(R)$ and the string tension density. In some of the models in GR, the functional $F(R)$ may vanish leading to an isotropic DE fluid in the absence of any aligned cosmic strings. For isotropic model  with $k=1$, $\zeta(k)$ vanishes and the pressure anisotropies are developed only due to the presence of one dimensional cosmic strings.

The DE EoS parameter $\omega_{D}$ is now obtained as,

\begin{align} \label{eq:6.29}
- \omega_{D} \rho_{D} & = \left[\dfrac{2\ddot{R}}{ R} +  \left(\dfrac{\dot{R}}{R}\right)^2 \right] \Omega_{\sigma}-\dfrac{\alpha ^{2}}{R^2}+ \rho \left(\omega+ \xi \right) , 
\end{align}



It is interesting to note that, in a cosmic fluid that blends DE with one dimensional cosmic strings in a non interacting manner, the dynamics of the DE EoS parameter will also be governed by the presence of the cosmic string fluid. In the absence of  any matter field, the skewness in pressure anisotropies and the DE EoS reduce to 
\begin{eqnarray} 
\delta &=& -\frac{2}{3\rho_{D}}\biggl[\zeta^2(k) F(R)\biggr] , \label{eq:6.30}\\
\gamma &=& \frac{1}{3\rho_{D}}\biggl[\frac{(k+5)}{(k+1)} \zeta(k) F(R)\biggr], \label{eq:6.31}\\
\eta &=& -\frac{1}{3\rho_{D}}\biggl[\frac{(5k+1)}{(k+1)} \zeta(k) F(R)\biggr], \label{eq:6.32}\\
- \omega_{D} \rho_{D} & =& \left[\dfrac{2\ddot{R}}{ R} +  \left(\dfrac{\dot{R}}{R}\right)^2 \right] \Omega_{\sigma}-\dfrac{\alpha ^{2}}{R^2}. \label{eq:6.33}
\end{eqnarray}
The above expressions \eqref{eq:6.30}-\eqref{eq:6.33} are the same as obtained in our earlier work \cite{mishrampla}. One should note that, the evolutionary behavior of the pressure anisotropies and the DE EoS depend on the assumed dynamics of the present day universe. In particular, if we have a presumed dynamics of the universe in the form of a scale factor pertaining to the late time cosmic speed up, the background cosmology can be well studied. Consequently, the evolutionary behavior of these properties can be well assessed. In view of this, in the present work, we consider a hybrid scale factor ( as in Refs. \cite{mishra015a, BM18}) that can simulate a transit universe from a decelerated phase to an accelerated phase.


\section{Model with a Hybrid scale factor}

It has been an usual practice to consider the scale factor to behave either as de Sitter type expansion or  as the power law expansion. Both the power law and exponential law of the scale factor lead to a constant deceleration parameter. However, the belief that the universe has undergone a transition from a decelerated phase of expansion to an accelerated one requires the deceleration parameter to evolve from some positive values at remote past to negative values at late phase of cosmic evolution. Such a behavior can be generated by a hybrid scale factor \cite{mishra015a, akarsu3, BM18}. The hybrid scale factor behaves as power law in the early cosmic phase and as de Sitter type at late phase of cosmic acceleration. It is expressed through two adjustable parameters $a$ and $b$ as $R=e^{at}t^{b}$. For this model, the Hubble parameter is expressed as $H = a+\dfrac{b}{t}$. Moreover, Tripathy \cite{tripa2} has considered a general form $H = a+ \dfrac{b}{t^{n}}$ of the Hubble parameter to address the role of skewness in anisotropic models where $n$ is a positive constant . The present case can be considered as a special case of that in Ref. \cite{tripa2}. The deceleration parameter for this model is obtained as $q =   -1+ \dfrac{b}{(at+b)^{2}}$. The parameter $b$ can be constrained in the range $0<b<1$ from simple arguments but $a$ can be constrained from a detailed analysis of $H(z)$ data \cite{mishra015a}. In the present work, we consider the same range for $b$ and leave $a$ as an open parameter.

The deceleration parameter generated by a hybrid scale factor is shown in figure 6.1. Deceleration parameter for power law cosmology and de Sitter type expansion have also been shown in the figure for comparison. The deceleration parameter for hybrid scale factor evolves from positive values at past epochs to negative values at late time. The transition from deceleration to acceleration occurs at some transition redshift $z_t$ which is decided by the parameter $a$. In the present work, we have considered two representative values of $a$ i.e. $0.1$ and $0.075$ corresponding to $z_t=0.8$ and $0.4$ respectively. It is worth to mention here that, the value of transition redshift has been constrained in a recent work as $z_t=0.806$ \cite{Jesus17}. Also, Farooq et al. obtained similar results from an analysis of Hubble parameter data \cite{Farooq17}. It is clear from the figure that at an early time, the behavior is dominated by the power law factor and the exponential factor dominates at late times . The rate of transition depends on the parameter $a$; transition is faster for higher value of $a$.

\begin{figure}[h!]
%\minipage{0.40\textwidth}
\includegraphics[scale=0.45]{fig1}
\caption{Deceleration parameter $q$  as a function of redshift.}
%\endminipage
\end{figure}

%\begin{figure}[h!]
%%\minipage{0.40\textwidth}
%\includegraphics[scale=0.5]{fig4}
%\caption{Variation of Hubble parameter $q$  as a function of redshift.}
%%\endminipage
%\end{figure}
%\begin{figure}[h!]
%%\minipage{0.40\textwidth}
%\includegraphics[scale=0.45]{fig3a}
%\caption{Evolution of skewness parameters in presence and absence of cosmic strings. $\xi$ is taken to be 1/6.}
%%\endminipage
%\end{figure}

\subsection{Dark energy density and skewness parameters}

The DE density parameter has contributions from the anisotropic aspects of the model and the matter field (including the string tension density). For an isotropic model with $k=1$, the anisotropic part $\Omega_{\sigma}$ becomes 1 (refer to eq. \eqref{eq:6.19}). It is obvious that at remote past, the matter field has a dominant contribution whereas at late phase of cosmic evolution the dark energy dominates. With an increase in the geometrical anisotropy through an increase in the parameter $k$, $\Omega_{\sigma}$ decreases from its isotopic value of 1 but the contributions from matter field and curvature part remain the same. This indicates that, with an increase in the value of $k$, there occurs a decrease in the value $\Omega_D$ at a given redshift. This feature of the DE density parameter is clearly visible in figure 6.2, where we have shown $\Omega_D$ as a function of redshift for some representative values of $k$. 

In order to investigate the effect of string phase on DE density parameter, we have considered three different values of $\xi$ namely $\xi=0, \frac{1}{6}$ and $\frac{1}{3}$ corresponding to no string phase, Nambu strings and geometric string phase respectively. Presence of string phase incorporates some kind of anisotropy. It is evident from figure 6.3 that the presence of string phase affects the DE density parameter in the early phase of cosmic evolution. With an increase in the value of $\xi$, $\Omega_D$ decreases to some lower values in the past epoch. However, at late times, aligned cosmic strings seem to have little effect on $\Omega_D$. 
%\begin{figure}[h!]
%%\minipage{0.40\textwidth}
%\includegraphics[scale=0.5]{fig3a}
%\caption{Evolution of skewness parameters in presence and absence of cosmic strings. $\xi$ is taken to be 1/6.}
%%\endminipage
%\end{figure}

\begin{figure}[t]
%\minipage{0.40\textwidth}
\includegraphics[scale=0.45]{fig2}
\caption{DE density parameter as a function of redshift for three representative values of $k$. $\xi$ is taken to be 1/6.}
%\endminipage
\end{figure}

\begin{figure}[h]
%\minipage{0.40\textwidth}
\includegraphics[scale=0.45]{fig3}
\caption{DE density parameter as a function of redshift for three representative values of $\xi$ for $k=1.0001633$.}
%\endminipage
\end{figure}

One can note from eqs. \eqref{eq:6.23}-\eqref{eq:6.31} that, the anisotropic DE pressure with the skewness parameters depend on the evolutionary behavior of the functional $\frac{F(R)}{\rho_D}$ and $\frac{\lambda}{\rho_D}$. In the absence of string phase, the pressure anisotropies depend only on the behavior of $\frac{F(R)}{\rho_D}$. In figure 6.4, the evolutionary behavior of the skewness parameters $\delta, \gamma$ and $\eta$ are shown either in presence or in absence of cosmic strings. One can note that, in absence of cosmic strings (dotted lines in the figure), the skewness parameters show almost a non evolving behavior in most of the past epochs and evolve at late phase of cosmic time.  $\delta$ and $\eta$ assume negative values whereas $\gamma$ assumes positive values during the evolutionary process. The anisotropy in the DE pressure along x-direction is almost unaffected by cosmic expansion. But the DE pressure along y-direction shows an increasing trend and the DE pressure along z-direction shows a decreasing trend at late times. In presence of cosmic strings, the behaviors of the pressure anisotropies remain almost unaltered at late phase of evolution whereas at an early epoch, the cosmic strings show their presence in a dominant manner. As a result, $\delta$ increases as we move back to past and it changes sign from negative to positive values at some redshift. $\gamma$ also show a similar increasing behavior with an increase in redshift. However, $\delta$ is more affected by the presence of cosmic strings compared to $\gamma$ and $\eta$. The DE pressure along z-direction is least affected. The reason behind the sensitivity of $\delta$ to the presence of cosmic strings may be due to the fact that, we have considered the strings to align along x-direction. We have also investigated the effect of anisotropy parameter $k$ on pressure anisotropies. It is found that, a variation of $k$, in the given range, does not have any significant effect on the overall behavior of the skewness parameters.
\begin{figure}[h]
%\minipage{0.40\textwidth}
\includegraphics[scale=0.45]{fig4}
\caption{Evolution of skewness parameters in presence of cosmic strings. The dotted lines represent the behavior of skewness parameters in the absence of cosmic strings.}
%\endminipage
\end{figure}

\begin{figure}[h!]
%\minipage{0.40\textwidth}
\includegraphics[scale=0.5]{fig5}
\caption{Evolution of DE EoS parameter for  three representative strengths of cosmic strings.}
%\endminipage
\end{figure}

\subsection{DE equation of state}
The dynamics of the universe is studied through the evolution of the DE EoS parameter $\omega_D$ in figure 6.5.  $\omega_D$ is not sensitive to the choice of the parameter $k$ at least at cosmic times spanning from some recent past to late phase. However, at early times the choice of $k$ may weakly affect the dynamics. In view of this, in the figure we have considered a representative value $k=1.6$ and examined the dynamics in presence of cosmic strings. It is obvious that, at a late phase of cosmic expansion, the dark energy strongly dominates even in the presence of cosmic strings and therefore, the DE EoS is not affected by string anisotropy. But at an early phase, the cosmic string has a substantial contribution to the density parameter and therefore, the dynamics of DE EoS is greatly affected. In the absence of any cosmic strings, the model behaves like quintessence field and the DE EoS smoothly decreases in the quintessence region. With an increase in string tension density, the model gathers some amount of energy in the early phase to behave differently. In such cases, the DE EoS first increases with cosmic time and then decreases.

\section{Conclusion}

In this chapter, we have investigated the role of anisotropic components on the dynamical aspects of dark energy. We considered the dark energy to have anisotropic pressures along different spatial directions. Some anisotropic effects have also been incorporated through the inclusion of cosmic strings aligned along x-direction. A hybrid scale factor having two adjustable parameters have been considered to mimic a cosmic transition from an early decelerating phase to a late time acceleration. The parameters of the hybrid scale factor have been fixed from some physical basis. The anisotropic parameter has been tightly bound from recent observations by different authors. In the present work, we have formulated an anisotropic model, where any amount of cosmic anisotropy can be considered and accordingly, the dynamical features of the model can be assessed. However, we have considered that $m=1.0001633$ corresponding to $\left(\frac{\sigma}{H}\right)_0 = 8.164 \times 10^{-5}$ to get some appreciable effects on the dynamical features of the universe. An increase in the anisotropic parameter decreases the DE density parameter and therefore shares some of the burden to provide an acceleration. Presence of string phase substantially modifies the DE density at early epoch. The anisotropy in DE pressure continues along with the cosmic expansion and grows a bit rapidly at a later period. In general,  the pressure anisotropies along different directions increase in the early phase dominated by cosmic strings. Along the x-direction, the anisotropic effect in DE pressure is more due to the string contribution. Along the z-direction, the presence of string phase has little affect on the pressure anisotropy. The DE EoS is also affected due to the anisotropic affect of cosmic strings at early phase. However, the dominance of DE at late times prevents the DE EoS to be affected substantially by cosmic strings.

==> Report_format_thesis/Chapter7.tex <==
\chapter{Dynamics of anisotropic dark energy universe embedded in radially directed magnetized fluid}

\footnote{\bf{The contents of this chapter has been published in Int. J. Mod. Phys D,To appear (2019)}}
\pagebreak

\section{Introduction}

Cosmological models, having the matter field as magnetic field had significant impact on the dynamics of the Universe depending on the direction of the field lines \cite{maden, king}. It has been revealed that during early time cosmic evolution of universe, magnetic field had a maximum effect in radiation dominated phase, producing large expansion anisotropies \cite{jacob}. Many investigations have considered Bianchi models to analyze the effect of magnetic field on the evolution of the Universe \cite{lebla, tsaq}. Under the above circumstances, Jacobs \cite{jacob} revealed the impact of uniform primordial magnetic field whereas the polarization and anisotropy of CMB radiation was investigated by  Milaneschi and Fabbri \cite{milan}. Also, King and Coles \cite{king} have introduced magnetized perfect fluid energy-momentum tensor in order to observe the role of magnetic field during cosmic evolution.


Several models have been investigated with perfect fluid and baryonic matter i.e. the ordinary matter. But most of them lack of describing exact dynamics of anisotropy of an accelerated universe. This motivates us to fill the  model universe with mixed fluids. One would be the exotic matter source such as the DE fluid and other can be taken as usual ordinary matter source.  Keeping this set up in background, significant works have carried out with various Bianchi forms in the back drop of general relativity \cite{akarsu010a, akarsu010a}. Yadav et al. \cite{yadav1} has worked in a DE model characterized by variable equation of state (EoS), obtained from constant deceleration parameter with  locally rotationally symmetric Bianchi V universe.  Mishra et al. \cite{mishra3} have studied the anisotropic dark energy fluid with different pressures along different spatial directions with one dimensional cosmic strings aligned
along x-direction to supplement some kind of anisotropy.Several interacting and non interacting two fluid situation DE models have been discussed widely in the literature \cite{mishra4, mishra5}.


This chapter is organized as follows: in section 7.2, we have developed the mathematical formalism for Bianchi type V space-time in a two-fluid situations and derived the physical parameters. In 7.3, the solution of the model is obtained with a hybrid scale factor to obtain a viable solution. The physical importance of the scale factor also discussed. In section 7.4, a comparison is made for EoS and skewness parameters with respect to the evolutionary behavior of the model followed by significant role of different parameters. Also comparisons made in the absence and presence of magnetic matter fluid. Moreover, state finder diagnosis has been done and discussed to show the model as physically realistic. Concluding remarks are given in section 7.5. 


\section{Mathematical set up and field equations of model}

In this work, we have investigated Bianchi type-V massive magnetized dark energy fluid cosmological model in general relativity. The magnetic field is due to an electric current produced along $z$-direction after quantizing the axis of magnetic field in the same direction. In continuation to other chapters, we have considered a spatially homogeneous and anisotropic Bianchi V space time in the form \eqref{eq:2.1}.\\
Moreover, the geometry of the considered space-time is represented by two equivalent transverse directions $y$ and $z$ and one different longitudinal direction $z$, along which the magnetic field is oriented. 


We, here, assume the energy momentum tensor $T_{ij}$ (EMT) consists of two different components; the electromagnetic fluid $(T_{ij}^{emf})$ and the hypothetical fluid in the context of DE $(T_{ij}^{de})$. So, the energy momentum tensor for the given environment with two non interacting fluids in \eqref{eq:2.2} reduced to, 

\begin{equation}
T_{\mu \nu}=E_{\mu \nu}^{(z)}+T_{\mu \nu}^{(de)}, \label{eq:7.1}
\end{equation}

where $E_{\mu \nu}^{(z)}$ and $T_{\mu \nu}^{de}$ respectively denote the contribution to energy momentum tensor from electromagnetic fluid and dark energy fluid. Here, the space-time coordinates are denoted as $\mu \nu,$ where, $\mu , \nu =1,2,3,4$ in the respective spatial and time directions. The energy momentum tensor for dark energy can be considered as

\begin{align} \label{eq:7.2}
T^{(de)}_{\mu \nu}  &= diag[\rho_d, -p_{xd},-p_{yd},-p_{zd}]\\ \nonumber
			        &= diag[1, -\omega_{xd},-\omega_{yd},-\omega_{zd}]\rho_d\\ \nonumber
			        &=diag[1, -(\omega_{d}+\delta), -(\omega_{d}+\gamma),-(\omega_{d}+\eta]\rho_d,
\end{align}

where $\omega_d$ is the dark energy equation of state parameter (EoS) and $\rho_d$ is the dark energy density. The skewness parameters $\delta$, $\gamma$ and $\eta$ are the deviations from $\omega_d$ on $x$, $y$ and $z$ axes respectively. The dark energy pressure becomes isotropic if $\delta$, $\gamma$ and $\eta$ vanish identically. Adding to this, if the electromagnetic part is set to zero, then the usual dark energy evolution is obtained \cite{chand,amirhashchi013a,saha}.\\

The energy momentum tensor corresponding to the electromagnetic field can be descried  as

\begin{equation}\label{eq:7.3} 
E_{\mu \nu}^{(z)} = \frac{1}{4 \pi} \left[ g^{sp}F_{\mu s}F_{\nu p}-\frac{1}{4} g_{\mu \nu}F_{sp}F^{sp}   \right],
\end{equation}
where $g_{\mu \nu}$ is the gravitational metric potential and $F_{sp}$ is the electromagnetic field tensor. Here, $F_{14}=F_{24}=F_{34}=0,$ assuming an infinite electrical conductivity to neglect the effect of electric field on the model. Again, the incidental magnetic fluid is quantized  the axis of the magnetic field along the axis of symmetry of latitudinal direction (along the $z$-direction). Hence, we obtained $F_{13}=F_{23}=0$. Thus, the only non-vanishing component of electromagnetic field tensor is $F_{12}$.\\

The Maxwell's equation, $F_{\mu \nu ; \gamma} + F_{ \nu \mu ; \gamma}+ F_{\gamma \mu  ;\nu }=0$ and $F^{\mu \nu}_{; \gamma}=0$ are satisfied only when the non-vanishing components can be represented as, $F_{12}=-F_{21}= M,$ where  $M$ is constant comes from the distribution of magnetic permeability along $z$-direction. Now, the components of EMT for electromagnetic fluid in the considered universe, thus, can be expressed as,
$E_{11}=-\frac{\mathcal{M}}{A_{1}^{2}} ,$ $E_{22}= -\frac{\mathcal{M}}{A_{2}^{2}e^{2 \alpha x}},$ $E_{33}=\frac{\mathcal{M}}{A_{3}^{2} e^{2 \alpha x}}  $ and $E_{44}=- \mathcal{M},$  where, $\mathcal{M}=\frac{M^{2}}{8 \pi A_{1}^{2}A_{2}^{2}e^{2 \alpha x}}$. Now assuming General Relativity (GR) is well defined at cosmic scales, we incorporate Einstein's field equations as in \eqref{EGR6},the field equations for a two fluid dark energy model in the frame work of GR can be obtained as: 

\begin{align}
& \frac{\ddot{A_{2}}}{A_{2}}+\frac{\ddot{A_{3}}}{A_{3}}+\frac{\dot{A_{2}}%
\dot{A_{3}}}{A_{2}A_{3}}-\frac{\alpha^{2}}{A_{1}^{2}}=-(\omega_{d}+\delta)\rho_{d}- \mathcal{M}  \label{eq:7.4} \\
& \frac{\ddot{A_{1}}}{A_{1}}+\frac{\ddot{A_{3}}}{A_{3}}+\frac{\dot{A_{1}}%
\dot{A_{3}}}{A_{1}A_{3}}-\frac{\alpha^{2}}{A_{1}^{2}}=-(\omega_{d}+\gamma)\rho_{d}+\mathcal{M}  \label{eq:7.5} \\
& \frac{\ddot{A_{1}}}{A_{1}}+\frac{\ddot{A_{2}}}{A_{2}}+\frac{\dot{A_{1}}%
\dot{A_{2}}}{A_{1}A_{2}}-\frac{\alpha^{2}}{A_{1}^{2}}=-(\omega_{d}+\eta)\rho_{d}+ \mathcal{M}  \label{eq:7.6} \\
& \frac{\dot{A_{1}}\dot{A_{2}}}{A_{1}A_{2}}+\frac{\dot{A_{2}}\dot{A_{3}}}{%
A_{2}A_{3}}+\frac{\dot{A_{3}}\dot{A_{1}}}{A_{3}A_{1}}-\frac{3\alpha^{2}}{A_{2}^{2}%
}= \rho_{d}- \mathcal{M}  \label{eq:7.7} \\
& 2\dfrac{\dot{A_{1}}}{A_{1}}-\dfrac{\dot{A_{2}}}{A_{2}}-\dfrac{\dot{A_{3}}}{%
A_{3}} =0  \label{eq:7.8}
\end{align}

The over dot over the field variables denote the derivatives with respect to the cosmic time $t$. Eqn. \eqref{eq:7.8} yields $A_{1}^2=A_{2}A_{3}$ after absorbing the integrating constant into the metric potential $A_{2}$ or $A_{3}$. In order to study the models, the physical parameters, such as; The cosmic spatial volume $V$ and the scalar expansion $\theta$ can be defined respectively as $V=R^3=A_{1}A_{2}A_{3}$ and $\theta=3H$. Here, the scale factor for the model universe is considered to be $R(t)$. The mean Hubble expansion parameter can be expressed in terms of directional Hubble parameters $(H_{1},H_{2},H{3})$ along spatial orthogonal directions as, $H= \frac{\dot{R}}{R}= \frac{1}{3}(H_{1}+H_{2}+H_{3})$. The shear scalar and deceleration parameter can be respectively calculated as $\sigma^2=\frac{1}{2 }(H_1^2+H_2^2+H_3^2-\frac{\theta^2}{3})$ and $ q=-\frac{R\ddot{R}}{\dot{R}^2} $. Now, the energy conservation equation, $T^{\mu \nu}_{; \nu}=0$, for the considered mixture of anisotropic fluid can be obtained as,

\begin{equation} \label{eq:7.9}
\dot{\mathcal{M}}+2 \mathcal{M} (H_{2}+H_{3})+\dot{\rho_d}+3\rho_d(\omega_d+1)H+\rho_d(\delta H_1+\gamma H_2+\eta H_3)=0,
\end{equation}

\noindent from which the the energy conservation equation for electromagnetic fluid, $E^{ij}_{;j}=0$ and dark energy fluid $T^{ij(DE)}_{;j}=0$, respectively, expressed as:

\begin{equation} \label{eq:7.10}
\dot{\mathcal{M}}+2 \mathcal{M} (H_{2}+H_{3})=0
\end{equation}
and
\begin{equation} \label{eq:7.11}
\dot{\rho_d}+3\rho_d(\omega_d+1)H+\rho_d(\delta H_1+\gamma H_2+\eta H_3)=0
\end{equation}

Now, eqn. \eqref{eq:7.7} and eqn. \eqref{eq:7.11} yields,

\begin{equation}\label{eq:7.12}
\rho_d= \frac{\dot{A_{1}}\dot{A_{2}}}{A_{1}A_{2}}+\frac{\dot{A_{2}}\dot{A_{3}}}{A_{2}A_{3}}+\frac{\dot{A_{3}}\dot{A_{1}}}{A_{3}A_{1}}-\frac{3\alpha^{2}}{A_{1}^{2}}+ \frac{k^{2}}{8 \pi A_{2}^{2} A_{3}^{2} e^{4 \alpha x}}
\end{equation}

We can split \eqref{eq:7.11} into two parts one corresponds to the deviation of equation of the state parameters and other is deviation free part as:

\begin{equation} \label{eq:7.13}
\dot{\rho_d}+3\rho_d(\omega_d+1)H=0 
\Rightarrow \rho_d=\rho_{d0} R^{-3(\omega_d+1)}
\end{equation}

\begin{equation} \label{eq:7.14}
\rho_d(\delta H_1+\gamma H_2+\eta H_3)=0  
\Rightarrow \delta \rho_d=-\frac{(\gamma H_x+\eta H_y)\rho_d}{H_z}
\end{equation}

According to \eqref{eq:7.13}, the behaviour of dark energy density $(\rho_{d})$ is controlled by deviation free part of EoS parameter of dark energy, where $\rho_{d0}$ indicates dark energy density at present epoch.  However, in equation \eqref{eq:7.13}, the corresponding EoS of DE $(\omega_{d})$ has to be assumed non-evolving in order to get the value of DE density. But then the evolutionary behavior of EoS parameters cannot be analyzed further to support the dynamics of our universe. Also, the DE density obtained in equation \eqref{eq:7.13} doesn’t have any contribution from electromagnetic fluid source. Hence, we dropped the idea of determining values $\rho_{d}$ and $\omega_{d}$ from \eqref{eq:7.13} and consider \eqref{eq:7.14} for the purpose followed by a basic mathematical formalism. Eqn.\eqref{eq:7.14} deals with the anisotropic part i.e the deviations from the total dark energy pressure along different spatial directions. In order to obtain an anisotropic relationship between the directional scale factors, we assume $A_{2}=A_{3}^m, m\neq1$ is the anisotropic factor. The anisotropic parameter $\cal(A),$ thus, can be obtained as,${\cal A}=\frac{1}{3}\sum \biggl(\frac{\vartriangle H_i}{H}\biggr)^2= \frac{2}{3} \left(\frac{(m-1)}{m+1} \right)^{2}$. Subsequently, the directional scale factors can be expressed as , $A_{1}=R, A_{2}=R^{\frac{2m}{m+1}}, A_{3}=R^{\frac{2}{m+1}}$. Now, with algebraic manipulations of eqns. \eqref{eq:7.4}-\eqref{eq:7.6} and \eqref{eq:7.12} the skewness parameters take the form,

\begin{align}
\delta=\frac{1}{\rho_d}\biggl[ H(2,3)\epsilon(m) F(R)+ H(3) 2 \mathcal{M}(R,x;z) \biggr] , \label{eq:7.15}\\
\gamma= -\frac{1}{\rho_d}\biggl[H(1,3) \epsilon(m) F(R)- H(3) 2 \mathcal{M}(R,x;z)\biggr] \label{eq:7.16}\\
\eta=\frac{1}{\rho_d}\biggl[H(1,2) \epsilon(m) F(R)-H(2,1) 2 \mathcal{M}(R,x;z)\biggr], \label{eq:7.17}
\end{align}

\noindent where  $F(R)=\biggl( \dfrac{\ddot{R}}{R}+ \dfrac{2 \dot{R}^{2}}{R^{2}} \biggr),$ $\mathcal{M}(R,x;z)=\dfrac{k^{2}R^{-2 \left( \frac{3m+1}{m+1} \right)}}{8 \pi e^{2 \alpha x}}=\mathcal{M},$ $H(2,3)=\frac{H_{2}-H_{3}}{3H},$ $H(1,3)=\frac{H_{1}+2 H_{3}}{3H},$ $H(1,2)=\frac{H_{1}+2H_{2}}{3H},$ $H(2,1)=\frac{H_{2}-H_{1}}{3H}$ and $H(3)=\frac{H_{3}}{3H}$. The functional $\epsilon (m)= \frac{1-m}{1+m},$ here, is a measure of deviation from isotropic behaviour. For an isotropic model, $\epsilon (m)$ vanishes and consequently,the skewness parameters will retain only the magnetized terms after vanishing the anisotropic part. Thus, to analyse the qualitative behaviour of these anisotropic parameters, it is convenient to normalize $\epsilon (m)$ to unity. The magnetic part,$\mathcal{M}(R,x;z)$,eventually obtained from the factor $R$ indicates the involvement of the $z$-direction magnetic field influence and the average scale factor in it. The anisotropy parameters depends on the functional F(R) in the absence of magnetic fluid. But in presence of the matter fluid, the dynamical behaviour of F(R) and $\mathcal{M}$ control the DE anisotropic pressure with skewness parameters.  Hence, choosing the average scale factor suitably plays a vital role in dynamical behaviour of the model as magnetic part directly depends on it. Subsequently, from the developed formalism, the total effective dark energy density $\rho_{eff}$ and the EoS parameter $\omega_{eff}$ are obtained as,

\begin{align} \label{eq:7.18}
\rho_{eff} = 2 \phi_{1} (m) \dfrac{\dot{R}^2}{R^2}- 3 \dfrac{\alpha ^2}{R^2}+ \mathcal{M}(R,x;z) 
\end{align}

\begin{align} \label{eq:7.19}
\omega_{eff} \rho_{eff} & = -\dfrac{4 \ddot{R}}{3 R} \left[ \phi_{1} (m) \right]  - \dfrac{2}{3} \left[ \dfrac{\dot{R}^2}{R^2}  \phi_{2} (m)  +  \mathcal{M}(R,x;z) \left( \frac{1-3m}{3(m+1)}\right) \right] + \dfrac{\alpha ^{2}}{R^2}, 
\end{align}

where, $\phi_{1} (m)= \dfrac{ (m^{2} + 4 m + 1)}{(m+1)^2}$ and $\phi_{2} (m)= \dfrac{(m^{3}+5m^{2}+5m +1)}{(m+1)^{3}}.$

The behaviour of the skewness parameters are totally controlled by the behaviour of the functional $F(R).$   The functional $\xi (m)$ depends upon the exponent $m$. EoS parameter are decided by the anisotropic nature of the model through this exponent $m$, the time dependence of mean Hubble parameter $H$, the the average scale factor $R$ and the rest energy density $\rho_{d}$. It is interesting to notice that, the effective dark energy density and the dark energy EoS parameter depend on the usual cosmic magnetic fluid too. 

\section{ Dynamical Solutions to the field equations}

It has been a usual practice to consider the scale factor to behave either as de Sitter type expansion or as the power law expansion. Both the power law and exponential law of the scale factor lead to a constant deceleration parameter. However, the belief that the universe has undergone a transition from a decelerated phase of expansion to an accelerated one requires the deceleration parameter to evolve from some positive values at remote past to negative values at late phase of cosmic evolution. Such a behavior can be generated by a hybrid scale factor \cite{mishra015a}. The hybrid scale factor behaves as power law in the early cosmic phase and as de Sitter type at late phase of cosmic acceleration. It is expressed through two adjustable parameters $h_{1}$ and $h_{2}$ as $R = e^{h_{1}t}t^{h_{2}}$. For this model, the Hubble
parameter is expressed as $H = \left( h_{1}+\frac{h_{2}}{t}\right)$. The deceleration parameter for this model is obtained as $ q = - 1 + \frac{h_{2}}{(h_{1}t+h_{2})^{2}}.$ The parameter $h_2$ can be constrained in the range $0 < h_{2} < 1$ from simple arguments but $h_1$ can be constrained from a detailed analysis of $H(z)$ data. In the present work, we consider the same range for $h_{2}$ and leave $h_{1}$ as an open parameter.

Since we considered the average scale factor as hybrid scale factor, therefore, the directional scale factors or metric potential can be expressed with hybrid scale factor as,

\begin{align*}
A_{1}=R=e^{h_{1}t}t^{h_{2}}; A_{2}=R^{\frac{2m}{m+1}}=(e^{h_{1}t}t^{h_{2}})^{\frac{2m}{m+1}};\,\,\,\, and \,\,\,\, 
A_{3}=R^{\frac{m}{m+1}}=(e^{h_{1}t}t^{h_{2}})^{\frac{2}{m+1}}
\end{align*}
Also, as the behaviour of the model would be studied through the behaviour of Hubble parameter, therefore the directional Hubble parameters can be calculated as, $H_x=H$, $H_y=\big(\frac{2m}{m+1}\big)H$ and $H_z=\big(\frac{2}{m+1}\big)H$.\\

Using the above relations, the dark energy density and the EoS parameter can be expressed as, 
\begin{align} \label{eq:7.20}
\rho_{eff} = 2  (h_1t+h_2)^{2}t^{-2}\phi_{1} (m)- 3 \alpha ^{2}e^{-2at}t^{-2b} + \mathcal{M} 
\end{align}

\begin{align} \label{eq:7.21}
\omega_{eff} \rho_{eff} & = -\dfrac{4 }{3} G(t) \phi_{1} (m)  - \dfrac{2}{3}  (h_1t+h_2)^{2}t^{-2} \phi_{2} (m)  +  \mathcal{M}(t,x;z) \left( \frac{1-3m}{m+1}\right) + \alpha ^{2} e^{-2h_1t}t^{-2h_2}, 
\end{align}

where, $G(t)=\frac{h_1^{2}t^{2}+2h_1h_2t+h_2(h_2-1)}{t^{2}}$ and $\mathcal{M}(t,x;z)=\dfrac{k^{2}(e^{h_1t}t^{h_2})^{-2 \left( \frac{3m+1}{m+1} \right)}}{24 \pi e^{2 \alpha x}}=\frac{\mathcal{M}}{3}$. Subsequently, equations \eqref{eq:7.15} - \eqref{eq:7.17} can be recasted as,
\begin{align}
&\delta=-\frac{2}{3\rho_d}\biggl[\left(\frac{m-1}{m+1}\right) \epsilon(m) F(t)- \mathcal{M}(t,x;z) \biggr] \label{eq:7.22}\\
&\gamma= \frac{1}{3\rho_d}\biggl[\left(\frac{m+5}{m+1} \right) \epsilon(m) F(t)+ 2 \mathcal{M}(t,x;z)\biggr] \label{eq:7.23}\\
&\eta=-\frac{1}{3\rho_d}\biggl[\left(\frac{5m+1}{m+1}\right) \epsilon(m) F(t)+ (3m+1) \mathcal{M}(t,x;z)\biggr] \label{eq:7.24}
\end{align}
Where $F(t)=\frac{3h_1^2t^2+6h_1h_2t+3h_2^2-h_2}{t^2}$. It is to be noted that all the equations above indicate  the explicit dependence of $\mathcal{M}$ on the physical parameters. This allows us to investigate the dynamical behavior of the model choosing the range of magnetic influence comfortably. Moreover, in the absence of the usual cosmic magnetic fluid, i.e, $\mathcal{M} \rightarrow 0,$ the values of Hubble parameter $H$, the scalar expansion $\theta,$ shear scalar $\sigma,$ volume scale factor $V$ remains as it is and the above equations reduce to the expressions obtained earlier \cite{mishra015a}. 

\section{Dynamical Behavior of the model relating to observational constraints} 

The deceleration parameter $q=- \dfrac{R \ddot{R}}{(\dot{R})^2}$  is an vital quantity describing cosmic dynamics of universe. Positive value of it indicates decelerating universe where as negative values confirms the accelerated expansion. With the advent of a lot of observations of high redshift supernova, Type Ia supernova observations combined with BAO and CMB, models transiting from early decelerating universe to late time accelerating universe gained much importance in recent times. At present time, the negative value of $q$ such as $q = -0.81 \pm 0.14$ is more favourable according to recent observational data. Supporting to this fact, the deceleration parameter for the present model, incorporating hybrid scale factor, turns to be $q= -1 + \dfrac{2n}{(m+1)(\xi t+ n)^{2}}=-1 + \dfrac{h_2}{(h_1t+h_2)^{2}}$. At an early phase of evolution $(t\longrightarrow 0)$, $q$ tends to be $-1+\dfrac{1}{h_2}$ where as $q \simeq -1 $ at late phase $(t \longrightarrow \infty )$. The parameter $h_2$ is constraint here to be in range $0<h_2<\dfrac{1}{3}$ \cite{mishra2} to get a transient universe.\\


\begin{figure}[h!]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=65mm]{rhonwfnl.pdf}
\caption{Evolution of $\rho_{eff}$ w.r.t. $z$ } 
\endminipage
\end{figure}

\begin{figure}[h!]
\minipage{0.56\textwidth}
\includegraphics[width=65mm]{omegamag.pdf}
\caption{Effective EoS paramter versus $z$ for representative values of the parameter M with $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$  $\alpha=0.35$ }
\endminipage \hfill
\end{figure}
\begin{figure}[h!]
\minipage{0.56\textwidth}
\centering
\includegraphics[width=65mm]{omegaalpha.pdf}
\caption{Variation of effective EoS paramter versus $z$ for representative values of the parameter $\alpha$ with $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$  $ M=0,05$} 
\endminipage
\end{figure}

\begin{figure}[h!]
\minipage{0.56\textwidth}
\includegraphics[width=65mm]{skewparacomp.pdf}
\caption{ Glance of Skewness parameter versus $t$ for the suitable discussed value of the parameter $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$  $\alpha=0.35, M=0,05.$ Dotted lines indicate the situation in the absence of magnetic fluid.}
\endminipage
\end{figure}

In figure 7.1, we observe, the dark energy density $(\rho_{DE})$ remains positive till late phase of evolution, satisfying weak energy condition (WEC) and  null energy condition (NEC) for the present model. It is worth to mention that, behaviour of dark energy density does not depend on change in value of magnetic coefficient but the presence of two fluid matter has notable effect w.r.t red-shift change. $\rho_{eff}$ decreases, initially, with increase in cosmic time (decrease in redshift) and reaches to a low  positive value till the inflation phase occurs. Then after the density value rises suddenly near upto present time red-shift data $(z \approx -1).$ The reason behind this phantom behaviour is may be due to the accelerated expansion of universe by the dark components \cite{noza}. How ever, the density seems to be retained a constant positive value towards late cosmic time which resembles with present observational information. This indicates that magnetic fluid has significant effect on $\rho_{eff}$ due to mix fluid matter.\\

Figure 7.2 shows variation of EoS parameter $(\omega_{eff})$ w.r.t significant choices of magnetic constant coefficients $\mathcal{M}$. One can note that nature of EoS parameters are inversely proportional to the increasing value of magnetic coefficients at past epochs.\\ 

But the behavior changes completely opposite towards late phase of evolution. The transit point or shifting point can be marked during the inflation epoch, which may be responsible for the change in behavior w.r.t. different M values. At this point, the model gathers some amount of energy and behaves differently. EoS parameters decreases more rapidly for lower values of M after the transit point. So it is very much clear that the dynamics is greatly affected by the behavior of different EoS parameters at early phase of evolution. Reason behind the mostly affected early phase is due to the substantial involvement of one directional magnetic fluid. It can be noted that, the states of matter for this model changes in late cosmic epoch in comparison to early epoch w.r.t different magnetic coefficient values. At early phase of evolution, the red line (m=0.05) confirms that less is the magnetic coefficient values, more is the possibility of accruing stiff dominated model. But at late cosmic epoch, lesser values of M indicates of achieving quintessence region by EoS parameter of the model. As a result, the red line lies most closer to $\Lambda$CDM line than other EoS parameter lines which are embedded with magnetic fluid. It also indicates that in the absence of any magnetic fluid, the model behaves like quintessence field with cosmic growth. So, we can also conclude here that the present model behaves like quintessence model in the absence of magnetic field. Hence, magnetic cosmic fluid has most impact on the dynamics of EoS that other tested cosmic fluids (in our earlier works), such as geometric string fluid, nambu string fluid, bulk viscous fluid; that too in the early phase of evolution. However, all these works, including the proposed model, shows that at late cosmic time, dark energy is dominated anyhow.\\ Hence, in the late time universe the effect of magnetic fields could be very small though in the early/inflationary universe these are observed to play a significant role.\\ 

DE EoS parameters can also be useful in testing the model w.r.t certain other parameters. In fact, one has the liberty to test the impact of EoS parameter for different choices of parameter $\alpha$, shown in Fig. 3. $\omega_{DE}$ remains in the quintessence region for all considered values of $\alpha$ but the behavioral switching over  red-shift of the universe shifts towards $\Lambda$CDM line. Behaviour of $\omega_{DE}$ is same as compared to different magnetic coefficient values, where as, with the increase in the value of $\alpha$, the increment in $\omega_{DE}$ is more rapid. Also, the value of $\omega_{DE}$ for $\alpha=0.35$(red line) is more for higher values of $\alpha$ and lies very similar to $\omega_{DE}$ for for a suitable magnetic coefficient value.\\

Figure 7.4 depicts the evolutional behaviours of anisotropic parameters in both absence and presence of matter fluid. The dotted lines of skewness parameters, indicating the absence of magnetic fluid, seem to be non evolving in the the early phase of cosmic time but evolves uniformly towards late cosmic time of evolution. The anisotropic parameter $\gamma$  assumes a positive value and shows increasing trend towards present epoch. But $\eta$ takes a negative value through out the evolution, having a decreasing trend towards present time. But both parameters retain their non-evolving behaviour towards late phase. Whereas, the parameter $\delta,$ indicates that the effective anisotropic pressure along x-direction of the universe, is independent of the cosmic expansion. Hence, the dotted lines express the anisotropic situation of the universe where only DE matter is involved. However, the presence of magnetic fluid drives a drastic change, particularly, in the early epoch. The solid lines clearly indicate the dominance of magnetic fluid during early time of evolution. Due to this effect, $\delta$ (blue solid line) starts evolving, assuming positive value and changes sign at a red shift value as we move forward to late epoch. The reason behind this sensitivity of $\delta$ to presence of magnetic fluid may be due to the consideration of normalising the average scale factor along $x$-direction $(H=H_{1}).$ Similarly, $\gamma$ and $\eta$ also show irregular evolutionary behaviour due the presence of matter. Whereas, one can clearly notice that $\eta$(red solid line) is most affected in comparison to the rest two anisotropic pressure parameters. This situation occurs due to the fact that we have designed the magnetic fluid to align along $z$-direction. \\

So, we observed that at past evolutionary epoch, just after big bang phenomnon, the evolution of anisotropy in our model (solid lines) is much different and dominant than evolution of standard anisotropic dark energy model (dotted lines). It revealed the impact of uniform primordial magnetic field. But, ultimately the merging of solid lines with the respective dotted ones clearly indicates that, at late cosmic epoch, DE is mostly dominant that drives the cosmic acceleration.


Although in the early/inflationary universe the magnetic fields are expected to play a role, in the late-time universe their effect could be small 
 
 




\section{Conclusion}
In the present work, we have constructed an anisotropic DE cosmological model in the framework of GR and Bianchi type V space time. In order to study the evolution of skewness parameters and the EoS parameters, we have developed the DE models in two fluid situations. The EoS parameter of DE evolves within the range predicted by the observations. Study on skewness parameters shows that, the universe is mostly dominant by magnetic fluid than any other source of matter. But in the present epoch, the DE dominates the universe.  This may be attributed to the current accelerated expansion of the universe. The parameter $m$ is responsible for the anisotropic behaviour and the matter behaviour of the model in the sense that, if $m=1$, we get isotropic model where only string matter part exist and for $m \neq 1,$ anisotropic and two fluid nature will be retained. In the present models,as expected, the matter energy density and DE density remains positive. Therefore, the energy conditions are satisfied, which in turn imply that the derived models are physically realistic. Moreover, it is showed that, there remain pressure anisotropies even at the late phase of cosmic evolution, though in the early phase pressure was assumed to be isotropic.

==> Report_format_thesis/Chapter8.tex <==
\chapter{Axially magnetized dark energy cosmological model}

\footnote{\bf{The contents of this chapter has been in arXiv:1811.09626v2}}

\pagebreak
\section{Introduction}
Contrary to Newtonian gravity, the recent development of expanding universe is an interesting phenomena in modern cosmology \cite{Hawley98}. Possibly this expansion is due to the Dark Energy(DE),which is instrumental in driving the galaxies apart \cite{Ryden03}. In order to explain acceleration, cosmologists have developed the idea of DE, which can be conceived as a hypothetical fluid with negative pressure and positive energy density \cite{Knop03}. Observational evidences \cite{Perlm98,Riess98,Riess04, Ade14, Ade16, Aghanim18} indicate that DE has two-third contribution to the mass energy budget of the universe and has spread across the space homogeneously. The noting part of this discovery is that DE does not interact with light and remain ineffective on the objects of small scales. Since the DE has a negative pressure, strong energy condition is not satisfied. For this reason, the evolution of the universe gets a sudden boost and there occurs a cosmic transition from early deceleration to late acceleration. It can also be noted that cosmologists have made several attempts to measure the deceleration of the expansion with a strong belief that the expansion of the universe due to gravity may slow down. However, the observational results from High-z supernovae search team totally rejected this idea and almost proved that the expansion of the universe is accelerating \cite{Riess98, Perlm99}. Subsequently strong evidences were gathered in support of the  accelerating expansion with greater accuracy \cite{Riess00, Astier06, Amanullah10, Weinberg13}. Later, the fact is supported by other observations from BAO \cite{Bond97, Wang06}, SDSS \cite{Seljak05, Adelman06}, CMB \cite{Jaffe06, Spergel07}. However, definitive observations of dark energy is far from elusive.\\

Post supernovae observations, plethora of cosmological models based on accelerating expansion of the universe have been proposed either by modifying the matter part of Einstein's Field Equations or by modifying the gravity theory. Bamba et al. \cite{Bamba12} have explained the dark energy and dark matter by a two periodic generalizations of the Chaplygin gas type models. Brevik et al. \cite{Brevik15a} constructed cosmological models by establishing an interaction between the DE and dark matter with a homogeneous equation of state parameter. In contrast to constant deceleration parameter, Mishra and Tripathy \cite{Mishra15b} considered time varying deceleration parameter to construct DE cosmological model in an anisotropic metric. Saadeh et al. \cite{Saadeh16} have presented a new framework to depart from isotropic background in Bianchi type $VII_h$ cosmologies. Fayaz and Hossienkhani \cite{Fayaz17} have considered Bianchi I space time and made a comparison between generalized Chaplygin gas model, interacting holographic and new agegraphic dark energy. Mamon et al. \cite{Mamon17} have considered dimensionless dark energy function to reconstruct the DE cosmological model. Ebrahimi et al. \cite{Ebrahimi17} have established a non-linear interaction of dark energy and dark matter to construct ghost DE cosmological model. Several cosmological models have been constructed in order to address the cosmic acceleration problem using different space time and different matter field\cite{Bamba11, Bamba12a, Mishra17, Mishra18}. Recent works on dark energy and the extended gravity can  be found in \cite{Capozziello:2010zz,Nojiri:2010wj,Bamba:2012cp,Bamba:2015uma, Cai:2015emx,Nojiri:2017ncd}.

The universe is observed to be isotropic. But there continues a debate on whether Bianchi type models are favoured at some cosmic phases or not? On the theoretical front, spatially homogeneous and isotropic FRW are usually considered for modelling the present universe. However, Bianchi type models with flat spatial sections and anisotropic directional expansion rates are considered more general compared to FRW models. In the present work, we have employed Bianchi-V space time to construct the model. The motivation is to develop a more general model which can allow us to consider anisotropy of any range (comparable to the range predicted in observations). In most of the cosmological models, we have observed that the deceleration parameter assumed to be constant and the matter field has been taken either as a perfect fluid or ordinary matter. However with this background, it is not sufficient to observe the dynamical behaviour with anisotropy for an accelerating universe. In this context, to get into the deeper inside of the problem, we consider the combination of two fluids such as the DE fluid and fluid of usual matter. Akarsu and Kilinc \cite{Akarsu10, Akarsu11}, assumed constant deceleration parameter to investigate the DE problem with the anisotropic metric Bianchi I and Bianchi III. Yadav et al. \cite{Yadav11} have supported their DE cosmological model with variable deceleration parameter and anisotropic Bianchi V space time. Theoretical models of interacting and non interacting DE have been discussed widely in the literature \cite{Mishra17, Mishra18, Mishra18a}. Several cosmological models have been constructed on cosmic magnetic field as the matter field. The role of cosmic magnetic fields has been reviewed in Refs. \cite{Kronberg:1993vk,Grasso:2000wj,Carilli:2001hj,Widrow:2002ud,Giovannini:2003yn,Giovannini:2004rj,Giovannini:2006kg,Kandus:2010nw,Yamazaki:2012pg,Durrer:2013pga,Maleknejad:2012fw,Bamba:2003av,Bamba:2004cu,Bamba:2006ga,Bamba:2008ja,Bamba:2008xa,Bamba:2018cup}.

The chapter has been arranged as follows: in section 8.2, we have developed the mathematical formalism for Bianchi type V space-time in a two-fluid situations and derived its physical parameters. In section 8.3, the solution of the model is obtained with a hybrid scale factor. In section 8.4, a comparison is made for EoS and skewness parameters with respect to different representative values and the evolutionary aspects of the skewness parameters has been discussed. The existence of big bang and big rip singularity has also been analysed in this section. Concluding remarks have been presented in section 8.5. 

\section{Mathematical Formalism with Physical Parameters}

In the context of the recent observational results made us to believe that, the universe at least at the late phase of cosmic evolution undergoes accelerating expansion. Further,it is mentioned that this result is due to the presence of an exotic DE energy form. Hence, in order to study the accelerating expansion further, we have considered here the cosmic fluid composed of DE and electromagnetic field. The motivation behind such an assumption stems from the fact that, DE has a lion share of $68.3\%$ in the mass-energy budget compared to a negligible share of around $4.9\%$ for the baryonic matter. The presence of electromagnetic field may also contribute to some extent to the cosmic speed up phenomena. Also, presence of magnetic field leads to an asymmetric cosmic expansion.  Now, the energy momentum tensor(EMT)for the cosmic fluid can be expressed as 

\begin{equation}
T_{\mu \nu}=E_{\mu \nu}+T_{\mu \nu}^{D}, \label{eq:8.1}
\end{equation}
where $E_{\mu \nu}$ is the energy momentum tensor for electromagnetic field and $T_{\mu \nu}^{D}$ is for the DE. For this investigation, we have considered an anisotropic space time in the form of Bianchi type V (BV) metric as 
  \begin{equation} \label{eq:8.2}
 ds^{2}= dt^{2}-a(t)^{2} dx^{2}-e^{2\alpha x}[b(t)^{2} dy^{2}+c(t)^{2} dz^{2}]
\end{equation}
In BV space time \eqref{eq:8.2}, it is seen that the expansion along different directions are different. The time dependent functions $a(t), b(t)$ and $ c(t)$ changes differently in the cosmic time and known here as the directional scale factor respectively for $x$, $y$ and $z$ direction.
$\alpha$ is non-zero positive constant. It is obvious that, when the three time dependent functions are equal and $\alpha=0,$ the line element \eqref{eq:8.2} reduces to flat FRW metric. In this sense, the BV metric is a general model than FRW model where some scope for anisotropic expansion can be assumed. Another geometrical significance of \eqref{eq:8.2} is that  the expansion along the longitudinal direction $x$ is different than that of the two equivalent traverse directions. In order to study an anisotropic cosmological model, we should have an anisotropic distribution of the DE fluid. So, the energy momentum tensor for DE can be defined as

\begin{align} \label{eq:8.3}
T^{D}_{\mu \nu}  &=  diag[\rho, -p_{x},-p_{y},-p_{z}]\\ \nonumber
			        &= diag[\rho, -\rho\omega_{x},-\rho\omega_{y},-\rho\omega_{z}]\\ \nonumber
			        &= diag[\rho, -\rho(\omega+\delta), -\rho(\omega+\gamma),-\rho(\omega+\eta)]
\end{align}
where $p$ is the pressure, $\rho$ is the density of DE and the DE equation of state parameter (EoS), $\omega=\frac{p}{\rho}$. Since the pressure anisotropy is one of the source of anisotropy, we have expressed that in \eqref{eq:8.3} through the skewness parameters $\delta$, $\gamma$ and $\eta$. These parameters are the deviations from EoS parameter along the respective coordinate axis. As we have added the electromagnetic field with DE, we can define its energy momentum tensor in the form 

\begin{equation}\label{eq:8.4} 
E_{\mu \nu} = \frac{1}{4 \pi} \left[ g^{sp}f_{\mu s}f_{\nu p}-\frac{1}{4} g_{\mu \nu}f_{sp}f^{sp}   \right],
\end{equation}
where $g_{\mu \nu}$ is the gravitational metric potential and $f_{\mu \nu}$ is the electromagnetic field tensor. In order to avoid the interference of electric field, we have considered an infinite electrical conductivity to construct the cosmological model. This results in the expression $f_{14}=f_{24}=f_{34}=0$. Again, quantizing the axis of the magnetic field along $x$-direction as the axis of symmetry, we obtain the expression $f_{12}=f_{13}=0,$ $f_{23}\neq 0$. Thus, the only non-vanishing component of electromagnetic field tensor is $f_{23}$.\\

With the help of Maxwell's equation, the non-vanishing component can be represented as, $f_{23}=-f_{32}= k $, where  $k$ is assumed to be a constant and it comes from the axial magnetic field distribution. For the anisotropic BV model, the components of EMT for electromagnetic field can be obtained as

\begin{align}\label{eq:8.5}
E_{11} &= \mathcal{M} a^{2},\nonumber\\
E_{22} &=- \mathcal{M} b^{2} e^{2 \alpha x},\nonumber\\
E_{33} &=- \mathcal{M} c^{2} e^{2 \alpha x},\nonumber\\
E_{44} &=- \mathcal{M},
\end{align}
where, $\mathcal{M}=\frac{k^{2}}{8 \pi b^{2}c^{2}e^{4 \alpha x}}$. When $k$ is non-zero, the presence of magnetic field has been established along the $x$-direction. If $k$ vanishes, the model will reduce to the one with DE components only. 


Assuming GR is well defined at cosmic scales, we wish to investigate the axially magnetised universe in the framework of Einstein's field equations (EFE),

\begin{equation} \label{eq:8.6}
R_{ij}-\frac{1}{2}Rg_{ij}=\kappa T_{ij},
\end{equation}
In \eqref{eq:8.6}, $R_{ij}$ is Ricci tensor and the Ricci scalar, $R=g_{ij}R^{ij}$, $\kappa = - \frac{8 \pi G}{c^{4}}$ . For physical convenience, we adopt  natural units where, $G =\frac{1}{8\pi}$ and $c=1.$ For the assumed cosmological model, the Einstein field equations become

\begin{align}
& \frac{\ddot{b}}{b}+\frac{\ddot{c}}{c}+\frac{\dot{b}%
\dot{c}}{bc}-\frac{\alpha^{2}}{b^{2}}=-(\omega+\delta)\rho- \mathcal{M}  \label{eq:8.7} \\
& \frac{\ddot{a}}{a}+\frac{\ddot{c}}{c}+\frac{\dot{a}%
\dot{c}}{ac}-\frac{\alpha^{2}}{a^{2}}=-(\omega+\gamma)\rho+\mathcal{M}  \label{eq:8.8} \\
& \frac{\ddot{a}}{a}+\frac{\ddot{b}}{b}+\frac{\dot{a}%
\dot{b}}{ab}-\frac{\alpha^{2}}{a^{2}}=-(\omega+\eta)\rho+ \mathcal{M}  \label{eq:8.9} \\
& \frac{\dot{a}\dot{b}}{ab}+\frac{\dot{b}\dot{c}}{%
bc}+\frac{\dot{c}\dot{a}}{ca}-\frac{3\alpha^{2}}{a^{2}%
}= \rho- \mathcal{M}  \label{eq:8.10} \\
& 2\dfrac{\dot{a}}{a}-\dfrac{\dot{b}}{b}-\dfrac{\dot{c}}{%
c} =0  \label{eq:8.11}
\end{align}

The single and double over dots on the metric potentials respectively denote first and second derivative with respect to the cosmic time. Field equation \eqref{eq:8.11} yields $a^2=bc$ after absorbing the integration constant into the metric potential $b$ or $c$.

In order to analyse the model, we define the spatial volume with respect to the metric potentials as $V=R^3=abc$ whereas the scalar expansion can be expressed as $\theta=3H$. Moreover, the scale factor can be denoted as $R(t)$. Now, we can also establish relationship between the directional Hubble rates ($H_{x},H_{y},H_{z}$), mean Hubble rate ($H$) and the scale factor ($R$)as $H= \frac{\dot{R}}{R}= \frac{1}{3}(H_{x}+H_{y}+H_{z})$.
The shear scalar is given by,
$\sigma^2=\frac{1}{2}(H_x^2+H_y^2+H_z^2-\frac{\theta^2}{3})$; $ q=-\frac{R\ddot{R}}{\dot{R}^2} $ is the deceleration parameter. \\

Incorporating the energy conservation, $T^{\mu \nu}_{; \nu}=0,$ for the magnetized DE fluid, we obtain

\begin{equation} \label{eq:8.12}
\dot{\mathcal{M}}+2 \mathcal{M} (H_{y}+H_{z})+\dot{\rho}+3\rho[(\omega+1)H+(\delta H_x+\gamma H_y+\eta H_z)/3]=0.
\end{equation}

\noindent For a mixture of non interacting DE fluid and electromagnetic fluid, separate energy conservation equations can be obtained from \eqref{eq:8.12} as

\begin{equation} \label{eq:8.13}
\dot{\mathcal{M}}+2 \mathcal{M} (H_{y}+H_{z})=0
\end{equation}
and
\begin{equation} \label{eq:8.14}
\dot{\rho}+3\rho[(\omega+1)H+(\delta H_x+\gamma H_y+\eta H_z)/3]=0
\end{equation}

Integrating eq. \eqref{eq:8.13}, we obtain
\begin{equation} \label{eq:8.15}
\mathcal{M}= \frac{k_{1}}{b^{2}c^{2}},
\end{equation}
where $k_{1}$ is an integration constant and we can assign $k_{1}=\frac{k^{2}}{8 \pi e^{4 \alpha x}}$ to retain the value of $\mathcal{M}$ as obtained in eq.\eqref{eq:8.15} without affecting its generality. 

The first two terms of eq.\eqref{eq:8.14} is the deviation free part of the EoS parameter wheresas the third term is the respective deviations of the EoS parameter. Now, we can obtain

\begin{equation} \label{eq:8.16}
\frac{\dot{\rho}}{\rho}= -3(\omega+1)\frac{\dot{R}}{R},
\end{equation}
and
\begin{equation} \label{eq:8.17}
\delta=-\frac{\gamma H_y+\eta H_z}{H_x}.
\end{equation}
It can be inferred from eq. \eqref{eq:8.16} that the behaviour of DE density $(\rho)$ is decided by the time evolution of the deviation free DE EoS parameter. Eq. \eqref{eq:8.17} deals with the deviation of DE pressure along different coordinate axes.\\

To investigate the dynamical and anisotropic behaviour along different directions, we adopt here the mathematical formalism developed in \cite{Mishra15b}. Now, with an axially placed magnetic field and DE, we  reveal the dynamical properties of the cosmological model. To do that we have taken an anisotropic relationship between the metric potentials as $b=c^m$ \cite{Mishra15b,Mishra17a}. Here $m$ should not be unity to avoid the isoptropic behaviour of the model. The anisotrpic parameter $\cal(A)$ can be obtained as, ${\cal A}=\frac{1}{3}\sum \left(\frac{\vartriangle H_i}{H}\right)^2= \frac{2}{3} \left(\frac{m-1}{m+1} \right)^{2}$. With this, the metric potentials with respect to scale factors are, $a=R, b=R^{\frac{2m}{m+1}}, c=R^{\frac{2}{m+1}}$ respectively. The directional Hubble parameters changed its expressions as, $H_x=H$, $H_y=\left(\frac{2m}{m+1}\right)H$ and $H_z=\left(\frac{2}{m+1}\right)H$. 

Now, with algebraic manipulation of equations \eqref{eq:8.7} ,\eqref{eq:8.8}, \eqref{eq:8.9} and \eqref{eq:8.17}, the skewness parameters take the form,

\begin{eqnarray}
\delta &=& -\frac{2}{3\rho}\left[\epsilon_1(m)F(R)+\mathcal{M}\right],\label{eq:8.18}\\
\gamma &=&  \frac{1}{3\rho}\left[\epsilon_2(m)F(R)+\mathcal{M}\right],\label{eq:8.19}\\
\eta   &=& -\frac{1}{3\rho}\left[\epsilon_3(m)F(R)-\mathcal{M}\right]\label{eq:8.20}.
\end{eqnarray}
Here $F(R)=\biggl( \dfrac{\ddot{R}}{R}+ \dfrac{2 \dot{R}^{2}}{R^{2}} \biggr)$ and the $m$ dependent functionals are $\epsilon_1(m)=\left(\frac{m-1}{m+1}\right)^2$, 
$\epsilon_2(m)=\left(\frac{m+5}{m+1}\right)\left(\frac{m-1}{1+m}\right)$ and 
$\epsilon_3(m)=\left(\frac{5m+1}{m+1}\right)\left(\frac{m-1}{1+m}\right)$.  Further, the skewness parameters are scale factor dependent; specifically on the functional $F(R)$, the magnetic contribution $\mathcal{M}$  and the DE energy density $\rho.$ For an isotropic model, $\epsilon_1(m),\epsilon_2(m), \epsilon_3(m) $ vanish and consequently the skewness parameters become proportional to the ratio $\frac{\mathcal{M}}{\rho}$ i.e $\delta=-\frac{2}{3}\frac{\mathcal{M}}{\rho}$, $\gamma=\frac{1}{3}\frac{\mathcal{M}}{\rho}$ and $\eta=\frac{1}{3}\frac{\mathcal{M}}{\rho}$. It is observed that, the presence of axial magnetic field contributes to DE pressure anisotropy along different coordinates. The above relations reduce to \cite{Mishra15b} in the absence of any magnetic field.

The dark energy density $\rho$ and the EoS parameter $\omega$ are obtained as,

\begin{eqnarray} 
\rho &=& 2 \phi_{1} (m) \dfrac{\dot{R}^2}{R^2}- 3 \dfrac{\alpha ^2}{R^2}+ 2\mathcal{M},\label{eq:8.21}\\
%\omega  & =& -\frac{1}{\rho}\left[\dfrac{4 \ddot{R}}{3 R} \phi_{1} (m)   + \dfrac{2}{3} \left( \dfrac{\dot{R}^2}{R^2}  \phi_{2} (m)  -  \mathcal{M} \right) - \dfrac{\alpha ^{2}}{R^2}\right]\label{eq:22},\\
%\omega\rho &=& -\frac{2}{3}\phi_{1} (m)\left[\dfrac{2\ddot{R}}{ R}+ \dfrac{\dot{R}^2}{R^2}  \phi_{2} (m) \right] + \frac{2}{3}\mathcal{M}+ \dfrac{\alpha ^{2}}{R^2}\\
\omega\rho &=& \left(\frac{\mathcal{A}}{2}-1\right)\left[\dfrac{2\ddot{R}}{ R}+ \dfrac{\dot{R}^2}{R^2} \right] + \frac{2}{3}\mathcal{M}+ \dfrac{\alpha ^{2}}{R^2}, \label{eq:8.22}
\end{eqnarray}

where, $\phi_{1} (m)= \dfrac{ (m^{2} + 4 m + 1)}{(m+1)^2}$. % and $\phi_{2} (m)= \frac{1}{\phi_1}\dfrac{(m^{3}+5m^{2}+5m +1)}{(m+1)^{3}}$.

From eq. \eqref{eq:8.21}-\eqref{eq:8.22}, the importance of the exponent $m$ is clearly visible in the sense that evolutionary behaviour of the EoS parameter can be assessed through this exponent $m$, the average scale factor $R$, the magnetic contribution $\mathcal{M}$ and the rest energy density $\rho$. Magnetic field certainly affects the evolutionary behaviour of the DE EoS parameter. In the absence of the axial magnetic field, the above equations reduces to the respective expressions of \cite{Mishra15b}.

\section{Hybrid scale factor and Dynamical aspects of the model}
We are indeed focussing on the variable deceleration parameter to understand the dynamical behaviour of the cosmological models. This is because there is a strong believe that universe evolved from a decelerated phase of expansion to an accelerated phase. This can be better studied if the deceleration parameter is time dependent. Keeping this in mind, we have chosen a hybrid scale factor in the form (HSF) \cite{Mishra15b,Mishra17a,Mishra18d} 
\begin{equation}
R = e^{h_{1}t}t^{h_{2}}\label{eq:8.23}
\end{equation}
where $h_{1}$ and $h_{2}$ are two adjustable parameters. With this new type of scale factor,  we can define the corresponding Hubble parameter as  $H = \left( h_{1}+\frac{h_{2}}{t}\right)$.  One should note that the deceleration parameter $q=- \dfrac{R \ddot{R}}{\dot{R}^2}$  is an important quantity in describing cosmic dynamics of universe. Positive value of it indicates decelerating universe where as negative values favour a universe with accelerated expansion. With the advent of a lot of observations from high redshift type Ia supernova combined with BAO and CMB, models  predicting a transition from early decelerating universe to late time accelerating universe gained much importance in recent times. At the present epoch, the negative value of $q$ such as $q = -0.81 \pm 0.14$ is more favourable according to recent observational data \cite{Ade14, Ade16}. Supporting to this fact, the deceleration parameter for the present model, incorporating hybrid scale factor, turns out to be $ q = - 1 + \frac{h_{2}}{(h_{1}t+h_{2})^{2}}$. At early phase of evolution $(t\rightarrow 0)$ and $q$ tends to be $-1+\dfrac{1}{h_2}$ where as $q \simeq -1 $ at late phase $(t \rightarrow \infty).$ The parameter $h_2$ can be constrained in the range $0 < h_{2} < 1$ from simple arguments; however with a detail analysis of the Hubble parameter with respect to redshift data, the range for $h_1$ can be constrained \cite{Mishra15b}. Hence, here we have considered the range for $h_{2}$ as in  \cite{Mishra15b} and $h_{1}$ as an open parameter. The directional scale factors or metric potential for an HSF can be expressed as  $a=R=e^{h_{1}t}t^{h_{2}}, b=(e^{h_{1}t}t^{h_{2}})^{\frac{2m}{m+1}} $ and $c=R^{\frac{2}{m+1}}=(e^{h_{1}t}t^{h_{2}})^{\frac{2}{m+1}}$.

For the present model with an HSF, the pressure anisotropies along different spatial directions are obtained as
\begin{eqnarray}
\delta &=& -\frac{2}{3\rho}\left[\epsilon_1(m)F(t)+\mathcal{M}\right],\label{eq:8.24}\\
\gamma &=&  \frac{1}{3\rho}\left[\epsilon_2(m)F(t)+\mathcal{M}\right],\label{eq:8.25}\\
\eta   &=& -\frac{1}{3\rho}\left[\epsilon_3(m)F(t)-\mathcal{M}\right]\label{eq:8.26}.
\end{eqnarray}
where
\begin{equation}
F(t)= \frac{3h_1^2t^2+6h_1h_2t+3h_2^2-h_2}{t^2}.\label{eq:8.27}
\end{equation}


The DE density and EoS parameter for the present model with an HSF can also be obtained in a straightforward manner using eqs. \eqref{eq:8.21}-\eqref{eq:8.23}. In the present model, we wish to put a positive constraint on the dark energy density which forces us to chose low values of the parameter $\alpha$ so that the dark energy density $\rho$ remains positive through out the cosmic evolution. This constraints enable the model to satisfy weak energy condition (WEC) and  null energy condition (NEC) for the present model. $\rho$ decreases with an increase in cosmic time and reaches to a constant positive value at late epoch. 

\section{Results and Physical Behaviours of the Model}
The model as developed in this work depends on the model parameters. Primarily five parameters  are responsible in deciding the dynamical behaviour of the model. Two parameters $h_1, h_2$ from the hybrid scale factor, $\alpha$ from the anisotropic BV metric, anisotropic parameter $m$ and $k$ from the strength of the axial magnetic field. As we have mentioned earlier, the parameter $h_1$ is considered to be within the range $0<h_1<1$ and $h_2$ is taken as a free parameter. In order to investigate various dynamical aspects of the model particularly the evolution of the EoS parameter and the directional pressure anisotropies, we have considered $h_1=0.1$ and $h_2=0.4$. These choices are motivated from the cosmic transit phenomena where we expect that the deceleration parameter smoothly decreases from a positive value at an early epoch to negative values at late times can predict a transit redshift of the order of unity ($z_t \simeq 1$). We have considered low values of $\alpha$ in the range $0<\alpha<0.5$ so that the DE density remains in the positive domain. The anisotropic parameter $m$ has been constrained in an earlier work to be $m=1.0001633$ which corresponds to an acceptable range of anisotropy \cite{Mishra15b}. The magnetic field contribution is suitably handled in the work to assess the effects of magnetic field on the EoS parameter and the skewness parameters. The values of these parameters are mentioned (wherever necessary) in the figures.

\subsection{EoS Parameter}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{fig81.pdf}
\caption{EoS parameter for different representative values of the parameter $k$ for $\alpha=0.35$.}
\end{center}
\end{figure}

\begin{figure}
\minipage{0.40\textwidth}
\centering
\includegraphics[width=65mm]{fig82.pdf}
\caption{EoS parameter for four representative values of the parameter $\alpha$ for $k=0.5$. } 
\endminipage\hfill
\minipage{0.40\textwidth}
\includegraphics[width=65mm]{fig83.pdf}
\caption{EoS parameter for four representative values of the parameter $\alpha$ for $k=1$. }
\endminipage\\
\minipage{0.40\textwidth}
\centering
\includegraphics[width=65mm]{fig84.pdf}
\caption{EoS parameter for four representative values of the parameter $\alpha$ for $k=5$. } 
\endminipage\hfill
\minipage{0.40\textwidth}
\includegraphics[width=65mm]{fig85.pdf}
\caption{EoS parameter for four representative values of the parameter $\alpha$ for $k=9$. }
\endminipage
\end{figure}
%\begin{figure}
%\minipage{0.40\textwidth}
%\centering
%\includegraphics[width=65mm]{EOSk5.pdf}
%\caption{EoS parameter for four representative values of the parameter $\alpha$ for $k=5$. } 
%\endminipage\hfill
%\minipage{0.40\textwidth}
%\includegraphics[width=65mm]{EOSk9.pdf}
%\caption{EoS parameter for four representative values of the parameter $\alpha$ for $k=9$. }
%\endminipage
%\end{figure}



%\begin{figure}[h!]
%\minipage{0.40\textwidth}
%\centering
%\includegraphics[width=65mm]{skew.pdf}
%\caption{Glance of Skewness parameter versus $t$ for the suitable discussed value of the parameter $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$  $\alpha=0.35, k=0,05$} 
%\endminipage\hfill
%\end{figure}



In Fig. 8.1,  the EoS parameter is plotted as a function of cosmic time for different strengths of the magnetic field for a constant value of $\alpha$. It has already been mentioned in the text that, the magnetic field strength is controlled by the parameter $k$. We have considered four different value of $k$ namely $0,2, 5, 9$ to assess its effect on the dynamical evolution of the EoS parameter. In general $\omega$ evolves from a positive domain to a negative domain. At late phase it saturates at around $-1$ to overlap with $\Lambda$CDM model. The EoS parameter displays peculiar behaviour with the increase in the strength of the axial magnetic field.
At an early epoch, the effect of magnetic field is substantial compared to that at late phase of cosmic evolution. At very late phase, the magnetic field has minimal effect on $\omega$ so that the curves of $\omega$ coincide and saturates at around $\omega=-1$. At an early epoch, the EoS parameter decreases with the increase in the magnetic field strength. But this behaviour is reversed in due course of cosmic evolution and $\omega$ increases with increase in magnetic field.

In order to assess the effect of the parameter $\alpha$ on the dynamical evolution of the EoS parameter, we have plotted $\omega$ for four representative values of $\alpha$ for a given axial magnetic field strength in Fig. 8.2. The red curve in the plot corresponds to $\alpha=0.35$, the green curve is for $\alpha=0.25$, pink curve for $\alpha=0.15$ and the blue curve represents for $\alpha=0.05$. It is obvious from the plot that, $\omega$ increases with the increase in $\alpha$ in very early epoch and after some cosmic phase of evolution it changes the behaviour. At some cosmic time, $\omega$ reverses the trend and decreases with the increase in $\alpha$. Just like the effect of magnetic field, $\alpha$ affects the dynamics in the early phase of evolution. However $\omega$ becomes less sensitive to $\alpha$ values at late phase. The Figures 3-5 are a repetition of Fig.8.2 with different $k$ values. From the Figs. 8.2-8.5, the effect of the magnetic field on the EoS parameter can be clearly assessed. It is certain from the analysis that, magnetic field has a substantial affect in the early phase of cosmic evolution.

\subsection{Skewness parameters}
The dynamical evolution of pressure anisotropies along different orthogonal spatial directions are investigated in terms of the skewness parameters $\delta, \gamma$ and $\eta$ in Figs. 8.6-8.11. In Fig.8.6, the skewness parameters in the absence of magnetic field are shown. In the absence of magnetic field, the The skewness parameters depend on the parameter $m$ and the parameters $h_1, h_2$ of HSF. In the present work, we have considered $m=0.0001633$, $h_1=0.1$ and $h_2=0.4$. The parameters are chosen in such a manner that, we obtain no substantial evolution of the skewness parameter along the x-direction. However, the skewness parameters along the y-direction and z-direction evolve with cosmic evolution. In the absence of magnetic field, $\gamma$ remains to be positive where as $\eta$ becomes negative.  With the cosmic evolution, the magnitude of $\gamma$ and $\eta$ increase for some period of time and then decrease after attaining a maximum. In general,the evolutionary behaviour of $\gamma$ seems to be opposite to that of $\eta$.

\begin{figure}[tbph]
%\hspace{-1cm}
\begin{center}
\minipage{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{fig86.pdf}
\caption{Skewness parameters in the absence of magnetic field ($k=0$) with $\alpha=0.35$.}
\endminipage
\minipage{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{fig87.pdf} 
\caption{Skewness parameters for $k=0.1$ with $\alpha=0.35$. }
\endminipage
\minipage{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{fig88.pdf}
\caption{Skewness parameters for $k=0.2$ with $\alpha=0.35$.}
\endminipage\\
%\hspace{-1cm}
\minipage{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{fig89.pdf}
\caption{Skewness parameters for $k=0.1$ with $\alpha=0.35$.Variation of Skewness parameters versus $t$ for $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$ $k=0.05$ and  $\alpha=0.2$ 
}
\endminipage
\minipage{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{fig810.pdf} 
\caption{Variation of Skewness parameters versus $t$ for $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$ $k=0.05$ and  $\alpha=0.4$}
\endminipage
\minipage{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{fig811.pdf}
\caption{Variation of Skewness parameters versus $t$ for $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$ $k=0.05$ and  $\alpha=0.46$}
\endminipage
\end{center}
\end{figure}

%\begin{figure}[tbph]
%\hspace{-1cm}
%\minipage{0.35\textwidth}
%\centering
%\includegraphics[width=\textwidth]{skew4a02.pdf}
%\caption{Variation of Skewness parameters versus $t$ for $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$ $k=0.05$ and  $\alpha=0.2$ 
%}
%\endminipage
%\minipage{0.35\textwidth}
%\centering
%\includegraphics[width=\textwidth]{skew4a04.pdf} 
%\caption{Variation of Skewness parameters versus $t$ for $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$ $k=0.05$ and  $\alpha=0.4$}
%\endminipage
%\minipage{0.35\textwidth}
%\centering
%\includegraphics[width=\textwidth]{skew4a046.pdf}
%\caption{Variation of Skewness parameters versus $t$ for $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.4,$ $k=0.05$ and  $\alpha=0.46$}
%\endminipage
%\end{figure}

The evolutionary behaviour of the skewness parameters in presence of magnetic field for a constant $\alpha$ are shown in Figs.8.7-8.8.  In Figs. 8.9-8.11, the time variation of skewness parameters are shown in presence of magnetic field for different representative values of $\alpha$. When the magnetic field is switched on, the skewness parameters display interesting behaviour. The skewness parameter along the x-direction, $\delta$ which was almost non evolving in the absence of magnetic field, starts to evolve with time. It becomes negative initially and evolves to become positive at late phase. $\delta$ initially decreases steadily with time and after attaining a minimum again increases. The magnitude of $\delta$ increases with the increase in the strength of magnetic field. The skewness parameter along the z-direction, $\eta$ becomes positive in an early epoch steadily increasing initially and then decreases to become negative at late times. With an increase in the strength of magnetic field, the magnitude of $\eta$ increases. Also, the time frame (within which it vanishes) increases with an increase in magnetic field. It is interesting to note that, for a given value of $\alpha$, the $\gamma$ and $\eta$ behave alike in the presence of magnetic field. However, as is evident from Figs.8.9-8.11, $\eta$ is more sensitive to the variation of the parameter $\alpha$. 

\subsection{Existence of Big-bang and Big-rip singularity}
It can be observed that, with the representative values of the parameters, the model approaches singularity at $t = 0$. Initially, the model begins with a big bang at initial epoch and and  shows a big rip behaviour with an ending at $t = \frac{t_{0} \alpha}{h_{2}} = 31.8$.  $t_{0}$ is the present time, which is 13.82 billion years from big bang. Energy density, EoS parameter, skewness parameters diverge at $t = 0$ and $t = 31.8$. We can summarise that the model starts with a big bang at $t = 0$ with decelerating expansion, and at the late phase of expansion enters into the accelerating phase. The model isotropic at $t = \frac{t_{0} \alpha}{h_{2}}$ and indicates big rip singularity. It has finite life time. At the late phase of cosmic evolution, the universe on its expansion is in agreement with the supernovae observation and in the deceleration phase, it allows the formation of large scale structure of the universe.

\begin{figure}[h!]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=65mm]{fig812.pdf}
\caption{Evolution of EoS parameter versus $t$ showing two singularities for representative values of the parameter $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.01,$ $\alpha=2.4,$ $ k=0.05$ and $x=0.2$} 
\endminipage\hfill
\minipage{0.40\textwidth}
\includegraphics[width=65mm]{fig813.pdf}
\caption{Evolution of Skewness parameters versus $t$ showing two singularities for representative values of the parameter $m=1.0001633,$ $ h_{1}=0.1,$ $h_{2}=0.01,$ $\alpha=2.4,$ $ k=0.05$ and $x=0.2$}
\endminipage
\end{figure}

\section{Conclusion}

In this chapter, in the frame work of GR, we have constructed an anisotropic DE cosmological model, with Bianchi V space time. In order to study the evolution of skewness parameters and the EoS parameters, we have developed the DE models in two fluid situations. The EoS parameter of DE evolves within the range predicted by the observations. In the present epoch, the DE dominates the universe. This may be attributed to the current accelerated expansion of the universe. The parameter $m$ is responsible for the anisotropic behaviour and the matter behaviour of the model in the sense that, if $m=1$, we get isotropic model where only string matter part exist and for $m \neq 1,$ anisotropic and two fluid nature will be retained. In the present models, as expected, the matter energy density and DE density remains positive. Therefore, some energy conditions are satisfied, which in turn imply that the derived models are physically realistic. Moreover, it is shown that, there remains pressure anisotropies even at the late phase of cosmic evolution, though in the early phase pressure was assumed to be isotropic. The EoS parameter changed with cosmic time and which indicates that during evolution there exists a relationship between the mean pressure of the cosmic fluid and energy density. The presence of magnetic field changes the dynamics substantially at least at the initial phase of cosmic evolution. The skewness parameters are found to be more sensitive to the magnetic field strength and the choice of model parameters.

==> Report_format_thesis/Chapter9.tex <==
\chapter{Role of various forms of Hubble scale factor during late time cosmic evolution in the back drop of DE anisotropy}

\footnote{\bf{The contents of this chapter has been published in Eur. Phys. J. Plus, \textbf{132}, 429 (2017)}}
\pagebreak

In this chapter, we have constructed dark energy models in an anisotropic Bianchi-V space-time and studied the role of anisotropy in the evolution of dark energy. We have considered anisotropic dark energy fluid with different pressure gradients along different spatial directions. In order to obtain a deterministic solution, we have considered three general forms of scale factor. The different forms of scale factors considered here produce time
varying deceleration parameters in all the cases that simulates the cosmic transition. The variable equation of state (EoS) parameter, skewness parameters for all the models are obtained and analyzed. The physical properties of the models are also discussed.

\section{Introduction} 
The standard cosmological model is based upon the assumption of large scale isotropy and homogeneity of space. However, a small scale anisotropies can be expected in the Universe in view of the observations of temperature anisotropy in the CMB radiation data from
WMAP and Planck. These data show some non trivial topology of the large scale cosmic geometry with asymmetric expansion \cite{ Watan09, Buiny06}. Planck data also show a slight
redshit of the power spectrum from exact scale invariance. Though the standard $\Lambda $CDM model is well supported by different measurements, at least at low multipoles, it does not fit to the temperature power spectrum data \cite{Ade14}. Dark energy is also believed to be associated with the breakdown of global isotropy and can display anisotropic features %\cite {Picon04, Jaffe05, Koivisto08a, Cooray10}. Employing the Union compilation
of Type Ia Supernovae, Cook and Lynden-Bell \cite{Cook10} found that a weak anisotropy in
dark energy, mostly observable for higher redshift group with $z>0.56$, directed roughly towards the cosmic microwave background dipole. While Friedmann Robertson Walker models (FRW) in the framework of General Relativity (GR) provide satisfactory explanations to various issues in cosmology, Bianchi type models have been constructed in recent times to
handle the smallness in the angular power spectrum of temperature anisotropy  \cite{campa1, campa3, gruppo, Koivisto06, Koivisto08, Bat09, akarsu1, akarsu2}. Moreover, Bianchi type models are the generalisation of the FRW models, where the spatial isotropy is relaxed.\\

As a sequel to our previous studies on the dynamical behaviour of pressure anisotropies \cite{Mishra15, mishrampla, skt15}, in the present work, we have considered different general form of non interacting dark energy with anisotropic pressures along different spatial directions and have investigated the effect of anisotropic components on the dynamics of dark energy. 

The present chapter is organized as follows. In section 9.2, we discuss the basic formalism of an anisotropic dark energy in a Bianchi type V space time. The effect of anisotropy on dark energy and the DE equation of state (EoS) parameter along with the behaviour of other physical parameters are discussed in section 9.3 and we summarize our results and its discussions in section 9.4.

\section{Basic Formalism of the Model and Anisotropy}

We consider the line element as Bianchi V space- time in the form \eqref{eq:2.2}. We have defined the energy momentum tensor for Dark Energy (DE) as

\begin{equation}
T_{\mu \nu }=(\rho +p)u_{\mu }u_{\nu }+pg_{\mu \nu }  \label{eq:9.1}
\end{equation}%
where $u^{\mu }u_{\mu }=1$ and in a co-moving coordinate system, $u^{\mu }$
is the four velocity vector of the fluid. $p$ and $\rho $ are respectively the isotropic
pressure of the fluid and the proper energy density. We are interested to incorporate some amount of anisotropy in the DE pressure, therefore the energy momentum tensor can be rewritten as:

\begin{eqnarray}  \label{eq:9.2}
T_{\mu\nu} & = & diag[\rho, -p_x,-p_y,-p_z]  \nonumber \\
& = & diag[1, -\omega_x,-\omega_y,-\omega_z]\rho \\
& = & diag[1, -(\omega+\delta),-(\omega+\gamma),-(\omega+\eta)]\rho, 
\nonumber
\end{eqnarray}
where $\rho$ and $\omega$ respectively denote the density and equation of state (EoS) parameter of DE. $\delta$, $\gamma$ and $\eta$ are the skewness parameters which deviates from the EoS parameter along $x$, $y$ and $z$ axes respectively. When the skewness parameters vanish identically the pressure of DE becomes isotropic. Now, the field equations \eqref{EGR6},  for this model in the frame work of GR when the matter field is in the form of DE can be obtained as,

\begin{equation}  \label{eq:9.3}
\frac{\ddot{a_2}}{a_2}+\frac{\ddot{a_3}}{a_3}+\frac{\dot{a_2}\dot{a_3}}{%
a_2a_3}-\frac{k^{2}}{a_1^{2}}=-(\omega+\delta)\rho
\end{equation}

\begin{equation}  \label{eq:9.4}
\frac{\ddot{a_1}}{a_1}+\frac{\ddot{a_3}}{a_3}+\frac{\dot{a_1}\dot{a_3}}{%
a_1a_3}-\frac{k^{2}}{a_1^{2}}=-(\omega+\gamma)\rho
\end{equation}

\begin{equation}  \label{eq:9.5}
\frac{\ddot{a_1}}{a_1}+\frac{\ddot{a_2}}{a_2}+\frac{\dot{a_1}\dot{a_2}}{%
a_1a_2}-\frac{k^{2}}{a_1^{2}}=-(\omega+\eta)\rho
\end{equation}

\begin{equation}  \label{eq:9.6}
\frac{\dot{a_1}\dot{a_2}}{a_1a_2}+\frac{\dot{a_2}\dot{a_3}}{a_2a_3}+\frac{%
\dot{a_3}\dot{a_1}}{a_3a_1}-\frac{3k^{2}}{a_1^{2}}=\rho
\end{equation}

\begin{equation}  \label{eq:9.7}
2\frac{\dot{a_{1}}}{a_{1}}-\frac{\dot{a_{2}}}{a_{2}}-\frac{\dot{a_{3}}}{a_{3}%
}=0,
\end{equation}
where an over dot represents the differentiation with respect to the cosmic time $t$. By suitably absorbing the integrating constants in the metric potentials, from eqn. \eqref{eq:9.7}, we obtain $a_{1}^{2}=a_{2}a_{3}$. To
obtain an anistropic relation among the directional scale factors, here we
have assumed $a_{2}=a_{3}^{l}$ where $l$ is an arbitrary positive constant $%
\neq 1$.\newline

We have assumed the rate of expansion in $x$-direction and the average
expansion are same. The mean Hubble parameter $H$ and directional Hubble
parameters $H_{i},i=1,2,3$ along different spatial directions can be
expressed respectively as $H=\frac{\dot{R}}{R}=\frac{1}{3}%
\sum_{i=1}^{3}H_{i} $ and $H_{i}=\frac{\dot{a_{i}}}{a_{i}}$. Also the cosmic
spatial volume $V$, scalar expansion $\theta $ and shear scalar $\sigma ^{2}$
can be defined respectively as $V=R^{3}=a_{1}a_{2}a_{3}$, $\theta =3H$, and $%
\sigma ^{2}=\frac{1}{2}(\sum_{i=1}^{3}H_{i}^{2}-\frac{\theta ^{2}}{3})$.
Moreover, the deceleration parameter can be obtained from the relation $q=%
\frac{d}{dt}\left( \frac{1}{H}\right) -1$. With the anisotropy assumptions $%
a_{2}=a_{3}^{l}$, the scale factors along different directions can be $%
a_{1}=R,a_{2}=R^{\frac{2l}{l+1}}$ and $a_{3}=R^{\frac{2}{l+1}}$.
Subsequently, the directional Hubble parameters can be obtained as, $H_{1}=H$%
, $H_{2}=\big(\frac{2l}{l+1}\big)H$ and $H_{3}=\big(\frac{2}{l+1}\big)H$. We
can also obtain the anisotropic parameter $\mathcal{A}$ as ${\mathcal{A}}=%
\frac{1}{3}\sum \left( 1-\frac{H_{i}}{H}\right) ^{2}=\frac{2}{3}\left( \frac{%
l-1}{l+1}\right) ^{2}$. For $l=1$, the anisotropy parameter $\mathcal{A}$
vanishes implying the model becomes isotropic with the rate of expansion is
equal in all spatial directions. The energy conservation equation for the
anisotropic fluid, $T_{;\nu }^{\mu \nu }=0$, which will subsequently split
into two parts, can be defined as

\begin{equation}  \label{eq:9.8}
\dot{\rho}+3\rho(\omega+1)H+\rho(\delta H_1+\gamma H_2+\eta H_3)=0.
\end{equation}
In the above equation, when the third term is zero, it reduces to eqn.%
\eqref{eq:9.9}, which defines the conservation of matter field with equal
pressure in all directions whereas when the first two terms are zero, eqn. %
\eqref{eq:9.8} reduces to eqn.\eqref{eq:9.10}, which is the deviations of
skewness parameters only.

\begin{equation}  \label{eq:9.9}
\dot{\rho}+3H(\omega +1)\rho=0
\end{equation}
and 
\begin{equation}  \label{eq:9.10}
\dot{\rho}+ \rho(\delta H_1+\gamma H_2+\eta H_3)=0.
\end{equation}

Using the mathematical scheme developed in our earlier work, \cite%
{mishrampla}, the skewness parameters can be obtained as

\begin{eqnarray}
\delta &=&-\chi (l)\left( \frac{l-1}{\rho }\right) f(H)  \label{eq:9.11} \\
\gamma &=&\chi (l)\left( \frac{l+5}{2\rho }\right) f(H)  \label{eq:9.12} \\
\eta &=&-\chi (l)\left( \frac{5l+1}{2\rho }\right) f(H)  \label{eq:9.13}
\end{eqnarray}

where $\chi (l)= \dfrac{l-1}{(l+1)^2}$, represents the amount of deviation
from isotropic behaviour of the model and from the parameter $l$. The
pressure anisotropies are also decided from the behaviour of the function $%
f(H)=\frac{2}{3}(\dot{H}+ 3H^2)$. The energy density and EoS parameter can be respectively obtained as

\begin{equation}  \label{eq:9.14}
\rho =2\left[ \frac{l^{2}+4l+1}{(l+1)^{2}}\right] H^{2}-3\frac{k^{2}}{R^{2}}
\end{equation}

\begin{equation}  \label{eq:9.15}
\omega =-\frac{2}{\rho }\left[ \frac{l^{2}+4l+1}{(l+1)^{2}}\right] \left[
f(H)-H^{2}\right] +\frac{k^{2}}{\rho R^{2}}
\end{equation}

We can observe from \eqref{eq:9.14}, the positivity condition of energy
density $\rho $ requires $2\left[ \frac{l^{2}+4l+1}{(l+1)^{2}}\right] H^{2}-3%
\frac{k^{2}}{R^{2}}>0$ implying that at any time interval we should have 
\begin{equation} \label{eq:9.16}
H^{2}>1.5k^{2}\frac{(l+1)^{2}}{l^{2}+4l+1}\frac{1}{R^{2}}\text{.}  
\end{equation}

This general condition i.e. $H^{2}>\frac{constant}{R^{2}}$ should be
satisfied while studying any models of Bianchi-V space-time. The most
general functional form of the scale factor $R$ satisfying this condition is
an exponent function. In this chapter in order to study the background
cosmology, we will consider three functional forms of scale factor
containing an exponent term.

\section{Scale Factors and Anisotropy Effect}

The variation of Hubble law may not be consistent with observations.
However, it has the advantage of providing simple functional form of the
time evolution of the scale factor. Also in order to explain the late time cosmic acceleration a simple parametrization of Hubble parameter is needed \cite{akarsu3,Pacif16}.  Hence, in order to construct the
cosmological models of the universe, in this section, we have adopted three
general forms of the scale factor $R$.

\subsection{Case I}

In this case, we have considered the scale factor which is a combination of two factors:
the one is the usual power law expansion and the second one is the
generalized form of an exponential function. Another reason to consider this
scale factor is that a cosmic transit from early deceleration to late time
acceleration can be obtained in this form of scale factor. So, the scale factor can be defined as 
\begin{equation} \label{eq:9.17}
R(t)=t^m\xi ^{n t}  
\end{equation}

where $m$, $n$, $\xi $ are positive constants and $2\leq \xi \leq 3$. For $%
\xi =2.718$ (Exponential), it reduces to hybrid scale factor cosmology \cite%
{mishrampla}. So, the Hubble parameter becomes $nln\xi +\frac{m}{t}$.
Subsequently the directional Hubble parameters can be obtained as: $%
H_{1}=H=nln\xi +\frac{m}{t}$, $H_{2}=\left( \frac{2l}{l+1}\right) \left(
nln\xi +\frac{m}{t}\right) $ and $H_{3}=\left( \frac{2}{l+1}\right) \left(
nln\xi +\frac{m}{t}\right) $. Now, we can obtain the functional $f(H)$, for
the considered Hubble parameter as 
\begin{equation} \label{eq:9.18}
f(t)=\frac{2}{3}\left[ 3\left( nln\xi +\frac{m}{t}\right) ^{2}-\frac{m}{t^{2}%
}\right]  
\end{equation}

So, the energy density \eqref{eq:9.14} and the EoS parameter \eqref{eq:9.15} can
be further simplified as:

\begin{equation}  \label{eq:9.19}
\rho=2 \left(\frac{l^2+4l+1}{l^2+2l+1}\right) \left(n ln\xi +\frac{m}{t}%
\right)^2 -3\left(\frac{k}{t^{m}\xi ^{nt}}\right)^2
\end{equation}

\begin{equation} \label{eq:9.20}
\omega =-\frac{2}{\rho }\left( \frac{l^{2}+4l+1}{l^{2}+2l+1}\right) \left[
\left( nln\xi +\frac{m}{t}\right) ^{2}-\frac{2m}{3t^{2}}\right] +\frac{1}{\rho}\left( 
\frac{k}{t^{m}\xi ^{nt}}\right) ^{2} 
\end{equation}

\begin{figure}[tbph]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-1-RHO}
\caption{ Energy density $\protect\rho$ versus time $t$ \\ 
($m=1.1,$ $n=0.05,$ $k=0.1,$ $l=0.9$)}
\endminipage
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-1-w}
\caption{ EoS parameter $\protect\omega$ versus time $t$\\
($m=1.1,$ $n=0.05,$ $k=0.1,$ $l=0.9$)}
\endminipage
\end{figure}

where $\chi(l)=\frac{l-1}{(l+1)^2}$.The plots for the energy density and EoS parameter has been shown in figure 9.1
and figure 9.2 respectively by choosing appropriate adjustable constants to see
the time evolution of these parameters. The behaviour of the energy density
would be decided by the power of the cosmic time in the expression %
\eqref{eq:9.19}. At the late cosmic
phase the energy density $\rho \simeq 2\left( \frac{l^{2}+4l+1}{l^{2}+2l+1}%
\right) \left( nln\xi \right) ^{2}$. It has been observed that both in early
time and late time the energy density remain positive. It might be negative
if the second term in eqn. \eqref{eq:9.19} dominates the first term. However,
we have already adjusted the functions in such a way that the energy density
remains positive throughout the cosmic evolution. The EoS parameter starts in the negative region and stays in the acceptable range \cite{Mathew15}. Hence, it can be infer that the matter evolves in the quintessence region at early time and remains in the same domain till late phase of cosmic time and approaching towards phantom barrier. The parameter evolves
dynamically with the expansion of the universe. This is basically governed
by the rest energy density that appears in the denominator of eqn. \eqref{eq:9.20}.
Moreover, it is worthy to mention here that since the exponent $n$ and the
value of $\xi $ are positive, at late phase $\omega \sim -1$. Subsequently,
we obtained the skewness parameters as:

\begin{equation}  \label{eq:9.21}
\delta = -\left(\frac{l-1}{\rho}\right)\left(\frac{2}{3}\chi(l)\right)\left[%
3\left(n ln\xi +\frac{m}{t}\right)^2-\frac{m}{t^2}\right]
\end{equation}

\begin{equation}  \label{eq:9.22}
\gamma = \left(\frac{l+5}{2\rho}\right)\left(\frac{2}{3}\chi(l)\right)\left[%
3\left(n ln\xi +\frac{m}{t}\right)^2-\frac{m}{t^2}\right]
\end{equation}

\begin{equation}  \label{eq:9.23}
\eta = -\left(\frac{5l+1}{2\rho}\right)\left(\frac{2}{3}\chi(l)\right)\left[%
3\left(n ln\xi +\frac{m}{t}\right)^2-\frac{m}{t^2}\right]
\end{equation}

\begin{figure}[tbph]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-1-DGE} 
\caption{Skewness parameters versus time $t$\\
($m=1.1,$ $n=0.05,$ $k=0.1,$ $l=0.9)$}
\endminipage
\label{fig:case-1-DGE}
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-1-q}
\caption{Deceleration parameter $q$ versus time $t$\\
($m=1.1,$ $n=0.05,$ $k=0.1,$ $l=0.9$)}
\endminipage
\end{figure}

The plot for the anisotropic parameters and cosmic time has been represented
in figure 9.3. The functional $\frac {f(t)}{\rho}$ is also time varying, as the
energy density $\rho$ has been changing with the time. So, the evolutionary
behaviour of the skewness parameters $\delta$, $\eta$ and $\gamma$ which are
negative at early cosmic time and positive in the late phase have been
decided by the factor $\frac {f(t)}{\rho}$. As expected, the skewness
parameter along $x-$axis does not evolve with time and mostly remains close
to zero. This expectation is because in our initial assumption along $x-$%
axis, the expansion rate is assumed to be the same as the mean Hubble rate.
It also indicates that the the pressure of the anisotropic fluid also same
with the mean pressure. It is also very much notable that the other skewness
parameters $\gamma$ and $\eta$ are found to be the mirror image of each
other. This may be due to the fact that the anisotropic parameter $l$ is
close to 1, which will describe the small anisotropic nature of the universe (figure 9.4). The constants (model parameters) are adjusted in such a way that the present numerical values of the cosmological parameters lie in the neighbourhood of predicted values by the observational data. In figure 9.4, $q(t_0)\sim-0.8$ where $t_0=13.7$ billion years. Here, 2 units of cosmic time $t$ measured as 1 billion year. So, the current assigned value for cosmic time $t_0$ = 28 units, gives $t_0\sim13.7$ billion years.\\

The scalar expansion and shear scalar of the model can be obtained
respectively as $\theta=3n ln\xi+\frac{3m}{t}$ and $\sigma^2=\left(\frac{l-1%
}{l+1}\right)^2\left(nln\xi+\frac{m}{t}\right)^2$. These parameters confirm the rate of change of local volume of the corresponding model in an increasing way since all $m$,$n$ and $\xi$ are positive. Also, the deceleration parameter can be obtained as $q=-\frac{1}{H^2}\left((nln\xi)^2+\frac{m(m-1)}{%
t^2}+\frac{m}{t}\right)$. The deceleration parameter remains negative and time dependent for $m>1$ and $n>0$ with a negative value at early phase and $q\sim -1$ at late times of acceleration agreeing with the present observational result.

\subsection{Case II}

In this case, we have considered the scale factor as a hyperbolic function
in the form 
\begin{equation}  \label{eq:9.24}
R(t)=\alpha cosh \beta t
\end{equation}
where $\alpha $, $\beta $ are positive constants and the Hubble parameter
obtained as $H=\beta tanh\beta t$. Subsequently the directional Hubble
parameters can be obtained as: $H_{1}=H=\left( \beta tanh\beta t\right) $, $
H_{2}=\left( \frac{2l}{l+1}\right) \left( \beta tanh\beta t\right) $ and $
H_{3}=\left( \frac{2}{l+1}\right) \left( \beta tanh\beta t\right) $. Now, we
can obtain the functional $f(H)$, for the considered Hubble parameter as 

\begin{equation} \label{eq:9.25}
f(t)=\frac{2}{3}\left[ \beta ^{2}\left( 1+2tanh^{2}\beta t\right) \right]
\end{equation}

The energy density and the EoS parameter can be expressed as:

\begin{equation}  \label{eq:9.26}
\rho=2 \left(\frac{l^2+4l+1}{l^2+2l+1}\right) \left(\beta tanh \beta
t\right)^2 -3\left(\frac{k}{\alpha cosh \beta t}\right)^2
\end{equation}

\begin{equation}  \label{eq:9.27}
\omega=-\frac{2}{\rho}\left(\frac{l^2+4l+1}{l^2+2l+1}\right) \left[\frac{2}{3%
}\beta^2\left(1+\frac{1}{3} tanh^2\beta t\right)\right]+\frac{1}{\rho}\left(\frac{k}{%
\alpha cosh \beta t}\right)^2
\end{equation}

\begin{figure}[tbph]
\minipage{0.40\textwidth} 
\centering
\includegraphics[width=\textwidth]{./case-2-RHO}
\caption{ Energy density $\protect\rho$ versus cosmic time $t$ \newline
($\protect\alpha =1,$ $\protect\beta =0.30,$ $k=0.1,$ $l=0.9)$}
\endminipage
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-2-w} 
\caption{ EoS parameter $\protect\omega$ versus cosmic time $t$ \newline
($\protect\alpha =1,$ $\protect\beta =0.30,$ $k=0.1,$ $l=0.9)$}
\endminipage

%\minipage{0.40\textwidth}
%\centering
%\includegraphics[width=\textwidth]{./case-2-w(z)} 
%\caption{ EoS parameter $\protect\omega$ versus redshift $z$ \newline
%($\protect\alpha =1,$ $\protect\beta =0.30,$ $k=0.1,$ $l=0.9)$}
%\endminipage

\end{figure}


It has been observed that the energy density increases with increase in time and remain flat after a
particular time period. Initially there is a sharp increase and subsequently
the increment becomes constant at late time. The details has been shown in
figure 9.5. It may be noted here that since $\rho$ needs to be positive, the
first term of \eqref{eq:9.26}, should dominates the second. Therefore the
behaviours of the parameters are constrained accordingly within the
admissible limit. The EoS parameter in figure 9.6 shows phantom behaviour in early phase of cosmic time ($t\sim 1.7 $ billion years) and evolves dynamically. However, it crosses the phantom barrier at $t=5.8$ before stabilising in the quintessence region as referred by current Planck satellite data ( $\omega=-1.49_{-0.57} ^{+0.05}$ )\cite{Mathew15, Brevik15}. The skewness parameters of the model with
this scale factor can be obtained as:

\begin{equation}  \label{eq:9.28}
\delta = -\left(\frac{l-1}{\rho}\right) \left(\frac{2}{3}\chi(l) \right)%
\left[\beta^2\left(1+2tanh^2\beta t\right)\right]
\end{equation}

\begin{equation}  \label{eq:9.29}
\gamma = \left(\frac{l+5}{2\rho}\right)\left(\frac{2}{3}\chi(l)\right)\left[%
\beta^2\left(1+2 tanh^2\beta t\right)\right]
\end{equation}

\begin{equation}  \label{eq:9.30}
\eta = -\left(\frac{5l+1}{2\rho}\right)\left(\frac{2}{3}\chi(l)\right)\left[%
\beta^2\left(1+2 tanh^2\beta t\right)\right]
\end{equation}

\begin{figure}[tbph]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-2-DGE}
\caption{Skewness parameters versus time $t$\\
($\protect\alpha =1,$ $\protect\beta =0.30,$ $k=0.1,$ $l=0.9)$}
\endminipage
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-2-q}
\caption{Deceleration parameter $q$ versus time $t$
($\protect\alpha =1,$ $\protect\beta =0.30,$ $k=0.1,$ $l=0.9)$}
\endminipage
\end{figure}


In figure 9.7, we have represented the behaviour of skewness parameters with respect
to the cosmic time. As in the previous case, in this case also the skewness
parameter $\delta$ does not evolve with time and move all along the x-axis
with increase in $t$. In fact it lies entirely on the $x-$axis at late
times. At the same time the other two skewness parameters $\gamma$ and $\eta$
remain constant at late times respectively in the positive and negative side
of $x-$axis. Both these parameters maintain a uniform distance from the
parameter $\delta$. The scalar expansion of the model can be calculated as $%
\theta=3\beta tanh\beta t$, which indicates that the expansion increases
with increase in time. The shear scalar found to be  $\sigma^2=\left(\frac{l-1}{l+1}%
\right)^2 \beta^2 tanh^2 \beta t$. Irrespective of the value of the
aniostropic value $l$, the shear scalar is positive through out the
evolution. Both the shear scalar and scalar expansion indicate that the rate of deformation is positive with respect to the cosmic evolution through the transition. Scalar expansion remains positive for positive value of $\beta$ whereas in shear scalar $l$ need to constraint as $l>1$ in order to get a positive cosmic behaviour. The deceleration parameter is found to be $q=-tanh^2\beta t$, it
indicates that the parameter always remain negative and close to $-1$ for $\beta=0.30$, adhere to a good match with the observational data. It is also observed from figure 9.8 that the accelerated expansion occur in a reasonable time period, which can be termed as the transition period.

\subsection{Case III}

In the previous two cases, we have constructed the dark energy models by
considering the scale factor as a hybrid and hyperbolic functions. In order
to have a better understanding on the anisotropic universe, in this case, we
have considered the scale factor as a fraction of exponential function in
the form:

\begin{equation}  \label{eq:9.31}
H(R)=a(R^{-n}+1)=\frac{ae^{nat}}{e^{nat}-1}
\end{equation}

where $a$, $b$ are positive constants. The scale factor $R$ can be expressed
as $R=(e^{nat}-1)^{\frac{1}{n}}$. Now, we can obtain the functional $f(H)$
as 
\begin{equation}
f(t)=\frac{2}{3}\left[ -na^{2}e^{nat}+\frac{3a^2e^{2nat}}{(e^{nat}-1)^{2}}%
\right]  \label{eq:9.32}
\end{equation}

The energy density and EoS parameter can be obtained as,

\begin{equation}  \label{eq:9.33}
\rho=2 \left(\frac{l^2+4l+1}{l^2+2l+1}\right) \left(\frac{ae^{nat}}{e^{nat}-1%
}\right)^2 -3\left(\frac{k}{(e^{nat}-1)^\frac{1}{n}}\right)^2
\end{equation}

\begin{equation}  \label{eq:9.34}
\omega =-\frac{2}{\rho }\left( \frac{l^{2}+4l+1}{l^{2}+2l+1}\right) \left[ -%
\frac{2na^{2}e^{nat}}{3}+\left( \frac{ae^{nat}}{e^{nat}-1}\right) ^{2}\right]
+\frac{1}{\rho}\left( \frac{k}{\left( e^{nat}-1\right) ^{\frac{1}{n}}}\right) ^{2}
\end{equation}

\begin{figure}[tbph]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-3-RHO} 
\caption{ Energy density $\protect\rho$ versus time $t$ \newline
($n=0.99,$ $a=0.1,$ $k=0.1,$ $l=0.9)$}
\endminipage
\minipage{0.40\textwidth} 
\centering
\includegraphics[width=\textwidth]{./case-3-w} 
\caption{ EoS parameter $\protect\omega$ versus time $t$ \newline
($n=0.99,$ $a=0.1,$ $k=0.1,$ $l=0.9)$}
\endminipage

%\minipage{0.40\textwidth} 
%\centering
%\includegraphics[width=\textwidth]{./case-3-w(z)} 
%\caption{ EoS parameter $\protect\omega$ versus redshift $z$ \newline
%($n=0.99,$ $a=0.1,$ $k=0.1,$ $l=0.9)$}
%\endminipage
\end{figure}

The energy density in figure 9.9 lies in the positive domain. Though initially, it
rises sharply but at late times it decreases rapidly. The most common type
of dark energy is the EoS parameter with the ratio of pressure and dark
energy density is a constant. Such an EoS is well known if $\omega \in[0,1]$%
, which describes a perfect fluid; however with $\omega=-1$, it defines a
cosmological constant. When $\omega <-\frac{1}{3}$, the universe is filled
with some similar substance which leads to the expansion with acceleration.
However, in most of the cases it remains in the range $({-\frac{1}{3},-1})$. From figure 9.10, it
is observed that, $\omega$ evolves in the phantom era at early cosmic time and slides through the quintessence region at late time, crossing the phantom barrier at $t=5.75$ billion years. The parameter proceeds towards still higher values in later evolution and remains in the preferred observed range. The skewness
parameters for the model can be obtained as:

\begin{equation}  \label{eq:9.35}
\delta = -\left(\frac{l-1}{\rho}\right)\left(\frac{2}{3}\chi(l) \right) %
\left[-na^2e^{nat}+\frac{3a^2e^{2nat}}{(e^{nat}-1)^2}\right]
\end{equation}

\begin{equation}  \label{eq:9.36}
\gamma = \left(\frac{l+5}{2\rho}\right)\left(\frac{2}{3}\chi(l) \right) %
\left[-na^2e^{nat}+\frac{3a^2e^{2nat}}{(e^{nat}-1)^2}\right]
\end{equation}

\begin{equation}  \label{eq:9.37}
\eta = -\left(\frac{5l+1}{2\rho}\right)\left(\frac{2}{3}\chi(l) \right)\left[%
-na^2e^{nat}+\frac{3a^2e^{2nat}}{(e^{nat}-1)^2}\right]
\end{equation}

\begin{figure}[tbph]
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-3-DGE}
\caption{Skewness parameters versus time $t$ \\
( $n=0.99,$ $a=0.1,$ $k=0.1,$ $l=0.9)$}
\endminipage
\minipage{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{./case-3-q}
\caption{Deceleration parameter $q$ versus time $t$\\
( $n=0.99,$ $a=0.1,$ $k=0.1,$ $l=0.9)$}
\endminipage
\end{figure}
figure 9.11 describes the behaviour of the skewness parameters of the model. Here also the parameter $\delta$ aligned with the $x-$axis and  $\gamma$, $\eta$ remain as the mirror image of each other. In this case, the scalar expansion and shear scalar can be obtained
respectively as $\theta=\frac{3ae^{nat}}{e^{nat}-1}$ and $\sigma^2=\left(%
\frac{l-1}{l+1}\right)^2 \left(\frac{ae^{nat}}{e^{nat}-1}\right)^2$. Scalar expansion shows the change of volume of the corresponding universe in an accelerated way as it includes exponential terms. Similarly shear scalar indicated the deformation rate of the universe is positive always for $l>1$ and $a>0$.  The
deceleration parameter $q=-\frac{n}{e^{nat}(e^{nat}-1)}-(1-n)$.  The behaviour of deceleration parameter in figure 9.12 indicates the acceleration expansion at late time; however at early time it might have decelerated. In order to get an accelerated expansion of the universe $n<1$. It can be noted that $q(t_0)\sim-0.7$ when $t_0=13.7$ billion years. 

\section{Conclusion}

We have considered three different functional forms of scale factor to
construct some DE cosmological models of the Universe in the
framework of GR in this chapter. The space time at the backdrop considered
is the spatially homogeneous anisotropic Bianchi V metric. With the help of
the forms of scale factor and Hubble expansion rates along different
directions, the anisotropic behaviour of the dark energy driven cosmological
model has been simulated. In the first and third case, we have observed that at late
phase of cosmic dynamics, the accelerated expansion of the universe has
occurred; however before this the universe might have decelerating at early
time whereas in the second case it reveals the time period of cosmic transition from early deceleration phase to late time acceleration phase. The EoS parameters in case I and III become time varying. In case I, where the scale factor is in the form of general hybrid factor, the EoS parameters entirely remain in the quintessence region. However in case II, it starts evolving from phantom phase and in case III it evolves from phantom dominated era but approaches towards false vacuum model, lying primarily in the quintessence region. \\

The skewness parameters in case I and II indicates pressure anisotropy of late phase evolving dynamically with cosmic expansion. In all the cases skewness parameters evolve fluctuating from different ranges showing greater anisotropy. In case III, the parameters continue their behaviour towards an isotropic universe but in the other two cases pressure anirotropy remains constant. In the present work, we observed that, the constant in the functional form of the scale factors are used to reconstruct different DE anisotropic models, depending on Hubble parameter, we revealed more interesting results favouring phantom kind of behaviour and quintessence dominated era. It is concluded that pressure anisotropic in DE fluid play very important and interesting role of pressure anisotropic need to be carried out for further better understanding of the accelerated expansion of the universe. 



==> Report_format_thesis/Conclusion.tex <==
\chapter{Concluding remarks and future scope of research}
\pagebreak
This chapter summarizes the elegant results presented so far in the thesis followed by wide scope of research.


The present thesis contains the investigations on the nature of conservation of anisotrpic DE  two-fluid cosmological models. The indispensable part of investigation is the reconstruction of the models with specific theoretical framework, which have been discussed in the chapters of the thesis. The reconstructions are mainly based on a newly assumed hybrid scale factor approach where the prime endeavor is to estimate, appropriately, the values of the model parameters and then to figure out the evolution of different cosmological quantities like the Hubble parameter, deceleration parameter, DE density, DE EoS parameter, skewness parameters etc.

Precisely, The motivation to GR and DE, as a source of current expanding universe, with diff DE candidates have been thoroughly discussed in chapter 1 followed by a through literature survey. An overview of cosmology is also presented where only elementary knowledge on general relativity is required. This is mainly intended for the reader who is not familiar with the subject, but particular DE cosmological model applications and recent DE experiments, which can interest the expert reader, will also appear for standard cosmological issues. Chapter 2 of the thesis frames a solid background on the concept of anisotropy in our universe followed by Bianchi space-times. The necessities of preferring Bianchi models, especially Bianchi V type, are discussed in detail. A brief literature survey, based on Bianchi models, is carried out which is more than a simple review. The mathematical framework to construct our model theory is introduced in a rather pedagogical manner, so that almost no prerequisites are needed to understand the treated arguments in next chapters.\\

In chapter 3 to 8, a number of specific anisotropic DE models using different matter fluid are introduced. The dynamical behaviors are focused on the cosmological and astrophysical aspects of the models and on their viability. Meanwhile in chapter 9, we also introduced the vital role and application of different forms of hybrid scale factor in form of a transition key during the inflation epoch which, when treated with DE components, can induce a viable scheme for the whole evolutionary history. We have studied the dynamical behavior of the model using the scale factor as HEL along with different matter fluid and analyzed their effect and nature along with DE taking in various observational red-dhift distances. \\

Another important aspect, which has been emphasized in the present work, is that we proved the physical acceptability of our proposed model comparing with $\Lambda$CDM model through two different kinds of diagnosis. Correspond results obtained for most of the models show that the models are in close proximity of $\Lambda$CDM model. In most of the cases the $\Lambda$CDM remains within 1s confidence region. Some of the models have inclination towards the phantom nature of dark energy $(\omega_{DE} > −1)$ and in some cases, quintessence nature $(\omega_{DE} < −1)$ is preferred. Though the results are model dependent, it can be concluded that the DE EoS parameter hovers around the limit $\omega_{DE}=-1.$ At this point, it is important to mention that though the $\Lambda$CDM cosmology is well consistent with most of the observational data, mainly with the observation at very low red-shift, but it might not be true for the observations at slightly higher red-shift.\\  

Our intention was to construct the model, mathematically, with in the frame work of discussed theory that would fit the data adequately with the help of our proposed formalism and confront it with recent observations. In this light, it is probably preferable to share that this theory, followed by the mathematical frame work, is best to investigate the characteristics of anisotropic DE. Moreover, the DE anisotropy in the models gradually reduces to isotropy at late time epoch along with the evolution process which is in agreement of recent DE projects as well as experiments.  

This thesis is conceived as a bridge between the mathematicians and the physicists. In fact the first one can have a look at formalism of well known mathematical techniques in the subject of cosmology and make himself an idea of some of the problems afflicting the modern interpretation of the universe. The second one instead can learn useful mathematical tools, helped by the numerous examples appearing in the physical field of cosmology, which can eventually be applied to many other physical frameworks. It is the hope of the author that both the physicist and the mathematicians will find this thesis useful to broaden their general scientific knowledge.\\

This work has a wide scope for the comparative study of anisotropic DE cosmological models in cosmology. In future, the problem can be extended to study the dynamical behavior of the cosmological model using any form of the hybrid scale factors proposed in our thesis. The anisotropic behavior can be further studied to check the possibility of getting a better range and can match its accuracy with current satellite observations. For the purpose of through comparison, in this thesis, we considered only a diagonal Bianchi type V space-time leading to anisotropic expansion. Hence, other non-diagonal Bianchi type space-times can be examined. The proposed formalism can be used to test the anisotropic behavior of DE with the isotropic FRW space-time to check anisotropy arises from isotropic background or not.

==> Report_format_thesis/Introduction.tex <==
\chapter{Introduction}


\pagebreak


In this thesis titled "Investigation of late time dynamics of the universe along with anisotropic dark energy models" based on the investigation of nature of dark energy (DE), and its contribution to
the dynamics of the universe. The comparison between the theoretical outcomes to the latest observational and calculation of exact solutions and special parameters that lead to understanding the reason behind the late time acceleration of universe has been investigated.

\section{Introduction}
In the beginning there was nothing. Not even void. Then, suddenly, the Big Bang, space and time were born. In its earliest times the Universe was filled with matter at enormous densities in exotic forms, far from the everyday experience of terrestrial matter. As the Universe expanded and cooled, matter started to congest into lumps of increasing magnitude. First quarks combined to form neutrons and protons. Then these so-called nucleons captured electrons and became atoms. Some atoms combined to form molecules and the molecules and atoms started to be pulled together by gravity to form clouds. Small inhomogeneities in the distribution of matter within the clouds were enhanced by gravitational forces and eventually the first stars and galaxies were born.

\subsection{An insight into brief evolutionary history}
On a philosophical level, cosmology is a field in which researchers' ultimate aims are to answer the fundamental questions: Where do we come from? How did it all begin? How will it all end? In ancient times, people looked to philosophers, historians and story-tellers when they wanted to know the workings of the world. Throughout the Middle Ages, the appeal to the authority of Aristotle was the answer to questions of why natural phenomena occurred. Aristotelian views, such as the final cause, telos, of things, lasted long into the Renaissance.

Towards the end of the Renaissance there was a period of great activity and  change in the natural sciences; Copernicus, Kepler, Newton and Galileo all lived and worked in this time period, which came to be known as the scientific revolution (16th–17th centuries). It was a time which dramatically changed the way to look at problem-solving. One of the main outcomes of the Scientific Revolution was to supplant Aristotle's final cause with a mechanical philosophy; that all natural phenomena can be explained by physical causes. Gradually, the Sun replaced the Earth as the center of the Universe. The idea that heavy bodies by their nature move down while lighter bodies naturally move up, was replaced by the idea that all bodies; both on Earth and in the heavens – move according to the same physical laws. The concept that a continued force is necessary to keep a body on motion, was abandoned by the inertial concept that motion, once started, continues indefinitely unless acted on by another force. Yet the most remarkable development of this time was not a specific discovery but a revolutionary new method of investigation. The new scientific method focused on mathematics as a language in which to formulate the laws of physics, and empirical research as a reference frame from which to make hypotheses and conduct experiments. Experimental outcomes replaced Aristotle's teachings as the new authority for truth.

Cosmology is the astrophysical study of the history, structure, and dynamics of the Universe. Hence it was, for much longer than other branches of physics and astronomy, a field more dominated by speculation and conjecture than by observations and experiments. There were few possibilities for the accuracy of tests and predictions starting to emerge in other disciplines in science laboratories around the world. In very recent years, however, cosmology too has entered the world of precision sciences. In November 1989, NASA launched the satellite COBE (Cosmic Background Explorer) to investigate the already detected \cite{penzias65} cosmic microwave radiation (CMB)predicted by the hot Big Bang theory. COBE confirmed that the CMB spectrum is that of a nearly perfect blackbody with a temperature of $2.725 \pm 0.002K.$ Subsequently, COBE data revealed tiny variations of temperature in different directions on the sky, at a level of one part in 100 000. These variations offer important clues to early structure formation in the Universe. For these discoveries, John C. Mather and George F. Smoot were awarded the Nobel Prize in Physics in 2006.
In the 20 years that have passed since the launch of COBE, cosmology has indeed grown to a true precision science that now places strong boundary conditions on cosmological models.

\section{General Relativity: \textit{Strongest theory to analyse late time cosmic dynamics}}

Einstein's general theory of relativity is the most promising theory in modern physics. It has major importance in its application to cosmology specifically with the evolutionary dynamics of the universe on a large scale. It is the most successful theory that describes gravity in curved space-time. Special theory of relativity formulated by Einstein in 1905 takes care of the relativity of uniform translatory motion in a region of free space where the effect of gravity is neglected. 
However, there was a serious conflict with Newton's law of gravitation $ F= - \dfrac{G M m_{G}}{r^{2}}$, where $F$ is the force exerted by a sphere of mass $M$ on a galaxy of gravitating mass $m_{G}$ located at a radius $r$ in three different ways:

First, since the expression contains only scalars, there is no obvious way to rewrite in terms of invariant. Second, it has no explicit time dependence, so gravitational effects propagate instantaneously to every location in the universe. Third, the gravitating mass $m_{G}$ appearing in Newton's law of gravitation is totally independent of the inert mass $m$ in Newton's second law and masses appear to be equal to a precision of $10^{-13}$. Hence, a theory was needed to establish link between Einstein's Special theory of relativity and Newton's law of gravitation. Mach {} postulated the idea that determines inertial properties of matter known as Mach's principle. Einstein considered it to be one of the basic underlying principles in his early work of general relativity. But subsequently, in his later publications, he has not refereed it. However, it is worthy to mention that, Mach's principle is a consequence of cosmology with Einstein's gravity. 

In view of the shortcomings of Newtonian mechanics and the limitations of special relativity, Einstein \cite{einstein15, einstein16} presented the general theory of relativity, which describes all kinds of motion and generalizes special theory of gravitation. He has combined the principle of equivalence, which incorporates gravitational effects in GR and the principle of general covariance, which helps to write the physical laws in covariant form. Einstein's theory is a geometric theory of gravitation which gives a unified description of gravity as a geometric property of space-time. In particular, the curvature of space-time is directly related to the four momenta of matter and radiation. In Einstein's theory of gravitation, the space time is described by the pseudo Riemannian metric,
\begin{align}
ds^{2}= g_{ij}dx^{i}dy^{j};\,\,\,\,\,\,\, i,j=1,2,3,4
\end{align}
and the components of the symmetric tensor $g_{ij}$ act as gravitational potentials.The gravitational field manifests through the curvature of space time and the general field equations which govern the gravitational field.

So, in the following section, we explain the mathematical framework provided by Einstein to formulate the field equations from the laws of gravitation.

\subsection{Einstein's formulation of field equation}

Einstein did not derive the field equation, but formulated it from a number of consideration (i) in the first place, according to the principle of covariance, the field equation must be a tensor equation; (ii) In the second place, there is the well known Poisson law in gravitation:

\begin{align}\label{EGR1}
\dfrac{\partial^{2} \psi}{\partial x^{2}} +  \dfrac{\partial^{2} \psi}{\partial y^{2}} + \dfrac{\partial^{2} \psi}{\partial z^{2}} = 4 \pi G \rho,
\end{align}
where $\psi$ is the gravitational potential, $\rho$ is the density of matter distribution and $G$ is Newton's gravitation constant. Under appropriate conditions, the new law of gravitation must yield an equation of the form \eqref{EGR1}. If the ten metric functions $g_{\mu \nu}$ ($g_{\mu \nu}$ being symmetric) of Einstein's theory are to correspond to a single function $\psi$ of Newton's theory, then, according to \eqref{EGR1}, the new law of gravitation must not contain higher derivatives of $g_{\mu \nu}$ than the second. The Ricci tensor $R_{\mu \nu}$ indeed does not contain higher derivatives of $g_{\mu \nu}$ than the second. The left side of \eqref{EGR1} should therefore be related to $R_{\mu \nu}$ in an appropriate form.

(iii) In the third place, the right hand side of \eqref{EGR1} containing the density of matter distribution should be related to $T_{\mu \nu},$ the energy momentum tensor, of Einstein's theory. Also, it is known known that, according to special theory of relativity, the conservation law in a  flat space-time is, 

\begin{align}\label{EGR2}
\dfrac{\partial T^{\mu \nu}}{\partial x^{\nu}}=0.
\end{align}
Obviously, \eqref{EGR2} would be valid in a geodesic co-ordinate system. In this system, the Christoffel symbol vanishes, i.e,

\begin{align}\label{EGR3}
\Gamma^{\mu}_{\alpha \beta}=0.
\end{align}

Hence, using \eqref{EGR2} and \eqref{EGR3}, 

\begin{align}\label{EGR4}
T^{\mu \nu}_{; \nu} \equiv \dfrac{\partial T^{\mu \nu}}{\partial x^{\nu}}+ \Gamma^{\mu}_{\alpha \nu} T^{\alpha \nu} + \Gamma^{\nu}_{\alpha \nu} T^{\mu \alpha} = 0
\end{align}
Equation \eqref{EGR4} is a tensor equation holding in the geodesic co-ordinate system. So \eqref{EGR4} holds in curved space-time.

[(iv)] Finally, in the fourth place, $R_{\mu \nu}$ occurs in an expression, $R_{\mu \nu}- \dfrac{1}{2} g_{\mu \nu} R,$ such that,

\begin{align}\label{EGR5}
\left( R^{\mu \nu} - \dfrac{1}{2} g^{\mu \nu} R \right)_{; \nu} = 0,
\end{align}
also known as Bianchi identity which will be introduced in next chapter.

The above four considerations (i-iv) inspired Einstein to introduce the law of gravitation as the general relativistic analogue of the Poisson equation in the following form,

\begin{align}\label{EGR6}
R_{\mu \nu} - \dfrac{1}{2} g_{\mu \nu} R = - k T_{\mu \nu},
\end{align}
where $k= \dfrac{8 \pi G}{c^{4}},$ is constant as the velocity of light $c$ in vacuum and the Newtonian gravitational constant $G$ are taken to be unity. The left hand side of \eqref{EGR6} is an Einstein tensor, $R_{ij}$ is the Ricci tensor, $R$ is the Ricci scalar curvature, $T_{ij}$ is the energy momentum tensor due to matter.

Since $(g^{\mu \nu})_{; \nu}=0,$ we can write \eqref{EGR5} in the following enlarged form with a constant $\Lambda,$

\begin{align}\label{EGR7}
\left( R^{\mu \nu} - \dfrac{1}{2} g^{\mu \nu} R + \Lambda g^{\mu \nu} \right)_{; \nu} = 0
\end{align}  
on cosmological ground.\\
Then law of gravitation can be expressed in the following form also:
\begin{align}\label{EGR8}
R_{\mu \nu} - \dfrac{1}{2} g_{\mu \nu} R + \Lambda g_{\mu \nu} = - k T_{\mu \nu}.
\end{align}
The cosmological constant $\Lambda$ was introduced by Einstein, while studying static cosmological model and was later discarded by him. Since Einstein's tensor is divergence free, the field equations \eqref{EGR8} yield,
\begin{align}
T^{ij}_{;j}=0,
\end{align}
which can be considered as the energy momentum conservation equation ans which also gives us the equations of motion of matter.

Einstein's theory of GR yields good results which are in good agreement with experimental tests of relativity, mainly the gravitational deflection  of light rays and the gravitational redshift of spectral lines. This theory serves as an effective tool for the study of cosmology and cosmological models of the universe because the basic force governing the dynamics of universe is gravity. Also, Einstein's general theory of relativity represents a grand tool of gravitation to understand uniquely the fabric of the space-time and the behavioural pattern of the cosmic bodies.

\section{Expanding universe: \textit{A revolutionary discovery in cosmology}}

The observations suggest that the Universe is expanding with an accelerating rate at present.
The accelerated expansion of the Universe is very strange because gravity is known to be
attractive. From the Friedmann equations, $\frac{\ddot{a}}{a}$ can be derived as,

\begin{align}
\dfrac{\ddot{a}}{a}= - \dfrac{4 \pi G}{3} (\rho + 3 p)
\end{align}

where, $a(t)$ is the scaling of distance between two object in the Universe at
cosmological scale, the second order time derivative of $a(t)$ is actually the acceleration. The
knowledge of standard cosmology suggests that the normal components of the energy budget
of the Universe satisfies the strong energy condition $\rho + 3 p > 0$. It indicates that the rate of expansion should decrease (decelerated expansion) which is not consistent with the present observations. The cosmic acceleration is represented in a dimensionless way using the deceleration parameter $q(t)$, defined as,
\begin{align}
q(t)= -\dfrac{1}{H^{2}(t)} \dfrac{\ddot{a}}{a}
\end{align}
If the value of $q(t)$ is negative, then the Universe is accelerating and if $q(t)$ is positive, the expansion is decelerating. The Universe has two phases of accelerated expansion. One is the early inflation which is required to explain certain observational phenomena. The second one is the late
time acceleration which is the present state of evolution of the Universe. In between this two
phases of accelerated expansion, there prevailed a phase of decelerated expansion.

The cosmological inflation is the very rapid expansion of the Universe just after the Big
Bang. It started after $10^{36}$ sec. of the Big Bang and ended around $10^{33}$ sec. to $10^{32}$ sec. Inflationary models have been introduced by Alan Guth \cite{guth81} for theoretical requirement to explain the flatness problem and the horizon problem. The flatness problem is related to the
reason of observed flatness of the spatial geometry of the Universe and the horizon problem is
related to the isotropy of the cosmic microwave background (CMB) radiation.

Late time acceleration is an observed phenomenon. It was first discovered in late nineties
by two supernova observing groups independently (Supernova Search Team led by Riess \cite{riess98, riess99} and Supernova Cosmology Project headed by Permutter \cite{perlmutter99}). The prime observation was of the magnitude red-shift curve of type Ia supernovae and it was highly consistent with the present accelerated expansion of the Universe. Later on, many other observations have confirmed the late time cosmic acceleration \cite{suzuki012, betoule014}. Analysis of observational data also suggest that the acceleration has started very recently, at around redshif $z\approx 0.5$ \cite{riess004}. It has emerged as the most puzzling phenomenon of modern cosmology.

As already mentioned, the accelerated expansion of the Universe is surprising because for
all the well known components of the Universe, even for the dark matter, gravity is attractive.
But the accelerated expansion invokes the possibility of repulsive gravity at cosmological scale.
There are different theoretical prescriptions in literature attempting to answer this puzzle. The following section is devoted to the discussions about those theoretical attempts to explain the
phenomenon of cosmic acceleration.


\section{Dark Energy: \textit{Source of accelerated expanding universe}}

Current estimates from NASA's Wilkinson Microwave Anisotropy Probe (WMAP) %\cite{Komatsu09}
show that the Universe consists of  $4\%$ baryons, $21 \%$ cold dark matter and $75 \%$ dark energy. WMAP measures the amplitude of temperature fluctuations in the cosmic microwave background radiation as a function of angular size on the sky, and from this information cosmological parameters can be inferred.

Early indications of the acceleration of the Universe actually dates back to a result from measuring the red-shifts and magnitudes of galaxies by J.-E. Solheim as far back as 1966 %\cite{Smoot92}.
The cluster galaxies were used to measure the magnitude-red-shift relation and found that the best-fit model describing the data included a non-zero cosmological constant and a negative deceleration parameter. During the 1980's, more hints were reported, but the evidence was highly uncertain. 

Supernovae of type Ia (SNIa) are the explosive deaths of white dwarf stars. These explosions are relatively uniform in their luminosities, making them ideal standard candles for measuring luminosity distances. To date, supernovae remain the most direct and well established method for constraint dark energy %\cite{Solheim66}$
. Current surveys include the SuperNova Legacy Survey (SNLS) %\cite{Richstone92}
, which expects to discover $\sim$ 700 high-red-shift supernovae, and ESSENCE Supernova Survey %\cite{Marian08}
, which aims to measure the dark energy equation of state parameter to $\pm 0.1$ by
following $\sim$  200 type Ia supernovae. Future surveys
such as The SuperNova Acceleration Probe (SNAP) will study more supernovae
at higher red-shifts as well as bringing more precise information on red-shift-dependent luminosity evolution of the supernovae. SNAP %\cite{Albrecht06}
is now being proposed as part of the Joint Dark
Energy Mission (JDEM).
Galaxy cluster and weak lensing surveys are also sensitive to dark energy. Since
the number density of clusters as a function of mass and red-shift is sensitive to the
underlying cosmological model, cluster counts can be used to constrain cosmological parameters. For example, the formation epoch of galaxy clusters depends
on the matter density parameter $\Omega_{m}$ of the Universe %\cite{Eisenstein05}
. One way of detecting
clusters is to measure peaks in the shear fields caused by weak lensing. Although
the shear peaks-method is subjected to projection effects because lensing measures mass along the line of sight, new studies show that the projected peak and
the 3-dimensional mass function scale with cosmology in an astonishingly close
way %\cite{Rassat08a}
.

In order to obtain precise weak lensing results for cosmological purposes, it will be necessary to measure the distortion of the shapes of galaxies to extremely high accuracy for millions of galaxies %\cite{Rassat07b}
. Future surveys will be bringing in the potential for a substantial increase in the accuracy of dark energy measurements if the distortion can be measured better than an accuracy of 0.0003. The launching of the Gravitational lensing Accuracy Testing 2008 (GREAT08) challenge, aimed at solving this practical problem.


Baryon Acoustic Oscillations (BAO) is a series of peaks and troughs predicted in the matter power spectrum, or equivalently a characteristic scale in the galaxy distribution. In the very early Universe the environment was so hot and dense that baryons and photons were coupled in a plasma. Fluctuations in this plasma were due to the competing forces of gravity and radiation pressure. In early 2005 a peak in the galaxy correlation function at 100$h^{-1}$Mpc was reported by
the SDSS team %\cite{Goldsmith97}
, which was an excellent match to the predicted imprint of acoustic oscillations on low-red-shift clustering of matter. The scale of the acoustic oscillations provide a standard ruler with great potential to be used for constrained dark energy from future galaxy surveys through its effect on the angular distance versus red-shift-relation.

The integrated Sachs-Wolfe (ISW) effect is caused by gravitational red- or blueshifts affecting CMB photons propagating from the last scattering surface and encountering gravitational potentials (i.e. large matter concentrations). With dark energy dominating the Universe today, the gravitational potential will be time dependent. In other words, the energy gained by photons falling into a potential well does not cancel out the energy loss as the photons climb out of the well. This large-scale effect can be measured by cross-correlating large-scale structure observations with CMB anisotropies caused by the ISW-effect %\cite{Marian08}
.
\subsection{Observational evidences on dark energy}

The basic endeavour of present cosmology is to model different observational phenomena. The observations are mainly of the electromagnetic wave of different wavelength. Earlier, the observations were limited within the optical wavelength. But at present, the astronomical observations are going in the wavelength regime starting from microwave to gamma ray.  Dark energy may have been detected by recent advances in the cosmological tests. The tests establish a good scientific case for the context, in the relativistic FRW model, including the gravitational inverse square law applied to the scales of cosmology. The mean mass density is not more than one quarter of the critical Einstein de Sitter value. The case for detection of dark energy is serious but not yet as convincing. Planned observations might be capable of detecting evolution of the dark energy density; a positive result would be a considerable stimulus to attempts to understand the micro physics of dark energy. In the following subsections, we have discussed some of the independent observations which are important in the context of late time cosmic acceleration.

\subsubsection{Type Ia supernova (SN Ia)}

In the context of late time cosmic acceleration, the pioneering observation is the type Ia supernova. The acceleration of the expansion of the universe was first discovered by Riess et al. \cite{riess98} by measuring luminosity distances of SNe Ia, used as standard candles. Perlmutter et al. \cite{perlmutter99} later confirmed the discovery with analysis of nearby and high-red-shift supernovae. The type Ia supernova is a standard candle for astronomical observation. A standard candle is defined as a class of distinguishable objects of known intrinsic brightness and it can be distinguished in a wide range of distance. As the Universe expands, the distance between the object and the observer increases and the wavelength of the radiated photons also increases. Thus the radiated photon get red-shifted. The observed brightness of the objects and the red-shift of the observed photons provide a measurement of the expansion of the Universe.

White dwarf stars that accrue mass from a companion star can eventually reach the Chandrasekhar limit, in which their masses become so big that the electron degeneracy pressure cannot continue counterbalancing the gravitational collapse \cite{hillebrandt00}. The variable star which results from the thermonuclear explosion of a white dwarf is also known as a supernova. The classification of the supernovae is based  on their spectral properties. In contrast to those of the Type II, Type I supernovae do not show any Balmer lines of hydrogen in their spectrum. The type Ia differs from
its siblings Ib and Ic by the presence of a strong ionized silicon absorption line at a high wavelength \cite{schneider006}. When a white dwarf reaches $1.4 M_{\bigodot},$ gravity becomes bigger than the Fermi degeneracy pressure and drives the star into explosion. Since SN Ia is made in the same process, it is assumed that SN Ia always have the same luminosity and it can be used as a standard candle. Measuring the apparent magnitude, the luminosity distance can be estimated. Once the absolute magnitude of the SNe Ia is determined, one can obtain the observational distance modulus as,
\begin{align}
\mu_{obs}= m-M,
\end{align}
where $m$ and $M$ are the apparent and absolute magnitudes, respectively. \\
The theoretical distance modulus of a supernova $(i)$, can be
calculated as,

\begin{align}
\mu_{th}(z_{i}) \equiv 5 \log_{10} d_{L}(z_{i})+25,
\end{align}
where $d_{L}$ is the luminosity distance.\\
Models can then be constrained through the dependence of the luminosity distance on the cosmological parameters by comparing $\mu_{obs}$ and $ \mu_{th}.$ The observed luminosity distance for nearby supernova is higher than the expected value, it can be concluded that the value of $q_{0}$ is negative. That means the present Universe is going through a phase of accelerated expansion.

\subsubsection{Cosmic Microwave Background (CMB)}

The CMB observations strongly indicate the presence of dark energy. The CMB is a snap shot of the Universe before the cosmic structure developed and has temperature anisotropies which are influenced by dark energy. This snap shot tells us the cosmic history from the photon decoupling epoch to the present. The high degree of uniformity of the CMB is the most compelling evidence of the
universe starting with a Big Bang. At the epoch when the universe was hot enough for electrons to be bounded into atoms, the collisions of photons with free electrons had maintained a thermal equilibrium between radiation and matter. The distribution of the number density of photons follow a black-body spectrum. At some time later, as the universe was expanding, the matter cooled down and became less dense. The radiation then decoupled from the matter to start a free
expansion, but the form of its spectrum was kept unchanged. \\

Anisotropies in the CMB in form of small temperature fluctuations were discovered by the COBE satellite in 1989. The WMAP measured precisely the temperature power spectrum and probed several cosmological parameters with high accuracy. A best-fitting value of $\Omega_{\Lambda}$ for the DE density parameter corresponding to a cosmological constant was found with the 9-year data.
The angular power spectrum of CMB temperature anisotropies measured by Wilkinson Microwave Anisotropy Probe (WMAP) \cite{spergel003, komatsu011} implies that it is dominated by acoustic peaks arising from gravity-driven sound waves in the photon-baryon fluid. Then the positions of these acoustic peaks are shifted by cosmic expansion. Thus the positions and amplitudes of acoustic peaks contain important cosmic information.

The combination of CMB and SN Ia observations indicates that our Universe is spatially flat and the matter component is about one quarter of the critical density,$\Omega_{m}=0.3$. This implies the need for dark energy as a missing component $\Omega_{\Lambda}= 1- \Omega_{m} \simeq 0.7, $ which
is indeed consistent with the value of $\Omega_{\Lambda} \simeq 0.7,$ suggested by SN Ia surveys.

\subsubsection{Baryon Acoustic Oscillations (BAO)}

BAO is the oscillation of the tightly coupled photon-baryon plasma before the recombination. The idea of statistical standard ruler with baryon acoustic oscillation is based on the fact that the clustering of galaxies may have a preferred scale. This preferred scale of galaxy clustering can be used to constrain the angular diameter distance. The phenomenon behind this distance correlation of galaxy clustering is actually the baryon acoustic oscillation. Before recombination, the formation of neutral hydrogen atom and the decoupling of photon from baryon matter, the mixture of baryons and photons was in the form of a hot plasma due to tight coupling between photons and baryons via Thomson scattering. The radiation pressure and the gravitational attraction acted as two competing forces and set up oscillations in the plasma. A single spherical over-density in the tightly coupled photon-baryon plasma would propagate with a speed $c_{s}=\dfrac{c}{\sqrt{3(1+ (\frac{3 \rho_{b}}{4 \rho_{\gamma}}))}},$ where $\rho_{b}$ is the baryon density and $\rho_{\gamma}$ is the photon density \cite{eisenstein007}.\\
At recombination, the photon decoupled from the baryon and propagated freely, forming
the cosmic microwave background (CMB). The size of the BAO measured from astronomical
observations indicates about the expansion history of the universe through measurements
of the Hubble rate $H(z)$. It yields measurements of the angular diameter distance,
$ d_{A},$ which is given for flat universe as \begin{align}
d_{A} \equiv \dfrac{l}{\theta} = \dfrac{1}{1+z} \int_{0}^{z} \dfrac{d \bar{z}}{H(\bar{Z}).}
\end{align}

Here, $l$ is the BAO characteristic length, $\theta$ is the angle and $d_{A} $ is related to the luminosity distance by $d_{A} = a^{2} d_{L}. $

\subsubsection{Weak gravitational lensing}

The gravitational bending of light by structure distorts the images of galaxies. Studying this gravitational lensing effect, the dark matter and its clustering can be mapped which shows us the influence of dark energy in the growth of large-scale structure. strong lensing is the deflection of light by massive structures like clusters and causes multiple images of the same background galaxy. Weak lensing distorts the shapes, sizes and brightness of galaxies. Since the shape is better than the original size and brightness of galaxy, the focus is on the change on shapes, called cosmic shear. Weak lensing normally reads only $1 \%$ change of galaxy shape. Therefore, a large number of galaxies are required to detect cosmic shear signal. The shear correlation function can be directly compared with the measurements \cite{crittenden002}.

\subsubsection{Planck collaboration}
 
Planck Collaboration provides a major source of information relevant to several cosmological and astrophysical issues, such as testing theories of the early Universe and the origin of cosmic structure. Planck has also defined the most precise measurements of several key cosmological parameters, like the average density of ordinary matter and dark matter in the Universe and the age of the universe. The main findings of Planck collaboration are:  

\begin{itemize}
\item High resolution detections of both the total intensity and polarization of primordial CMB anisotropies.
\item Creation of a catalogue of galaxy clusters.
\item observations of the gravitational lensing of the CMB.
\item Observations of bright extra-galactic radio (active galactic nuclei) and infrared (dusty galaxy) sources.
\item Observations of the Milky Way, including the interstellar medium, distributed synchrotron emission and measurements of the Galactic magnetic field.
\item Studies of the Solar System, including planets, asteroids, comets and the zodiacal light.
\end{itemize}

Planck had a higher resolution and sensitivity than WMAP, allowing it to probe the power spectrum of the CMB to much smaller scales. There are several others dark energy probes available in the literature such as the cosmic age tests from globular cluster and the white dwarfs \cite{feng005}, galaxy clusters \cite{allen011, haiman000}, observational Hubble parameter measurements \cite{yu011, freedman010} and gamma ray bursts \cite{tsutsui009, basilakos008}.

\subsection{Dark energy experiments}

There are many observational projects to detect dark energy using the four dark energy probes: SN Ia, CMB, BAO and Weak Lensing (WL). Among them the Dark Energy Task Force (DETF) report \cite{friedmann22} classifies the dark energy projects into four stages:\\
Stage I–completed projects that already released data, Stage II–on-going projects, Stage
III–intermediate-scale, near-future projects, and Stage IV–large-scale, longer-term future
projects. \\
Following table shows us the dark energy projects classified by probes and stages.


\begin{table}
  \centering
  \caption{Different stages of probes}
  
\begin{tabular}{ |p{3cm}| p{3cm}| p{3cm}| p{3cm}| p{3cm}|} 
\hline
Probes  &SN Ia & CMB & BAO & WL\\
\hline

 stage-I & Higher-Z Team, SNLS, ESSENCE, NSF, LOSS, SDSS, SCP, CfA, Palmar QUEST Survey & COBE, TOCO, BOOMERang, Maxima, WMAP &  2d FGRS, SDSS, 6dFGRS, WiggleZ& CFHTLS \\ 
 \hline
 stage-II &Pan-STARRS1, HST, KAIT& Planck, SPT, ACT& SDSS II, SDSS III, BOSS, LAMOST, WEAVE& Pan-STARRS1, DLS, KIDS\\
  \hline 
 stage-III & DES,Pan-STARRS4, ALPACA, ODI& ALPACA, CCAT & DES, HET-DEX, BigBOSS, ALPACA, SuMIRe& DES,Pan-STARRS4, ALPACA, ODI\\
  \hline
 stage-IV & LSST, WFIRST& EPIC, Lite BIRD, B-Pol & LSST, SKA, WFIRST, Euclid& LSST, SKA, WFIRST, Euclid\\
  \hline
\end{tabular}
\end{table}

Most observational applications of these methods now take place in the context of large cosmological surveys, for which constrained dark energy and modified gravity theories is a central objective. Following table lists a selection of current and planned dark energy experiments, taken from the Snowmass 2013 Dark Energy Facilities review \cite{wang98}, which focused on projects in which the U.S. has either a leading role or significant participation.

\begin{table}
  \centering
  \caption{Project Data Set}
  
\begin{tabular}{ p{2cm} p{2cm} p{2cm} p{1.5cm} p{2.3cm} p{2cm}}
 \hline\hline
 Project & Dates  &Area/deg$^2$ & Data & Spec-z Range & Methods\\
 \hline
 BOSS   & 2008-2014    & 10,000 & Opt-S & $0.3 - 0.7$ (gals) $2- 3.5$ (Ly$\alpha$F) &   BAO/RSD\\
 DES&  2013-2018  & 5000 & Opt-I & -  & WL/CL SN/BAO \\
 eBOSS &2014-2020 &7500& Opt-S& $0.6-2.0$ (gal/QSO) $2-3.5$ (LY$\alpha$F) & BAO/RSD\\
 SuMIRE   &2014-2024 & 1500& Opt-I Opt/NIR-S& $0.8 - 2.4$ (gals) &   WL/CL BAO/RSD\\
 HETTDEX& 2014-2019 & 300 & Opt-S & $1.9<z<3.5$ (gals) & BAO/RSD\\
 DESI& 2019-2024 & 14,000   & Opt-S & $0 - 1.7$ (gals) $2 - 3.5$ (Ly$\alpha$F)& BAO/RSD\\
 LSST& 2020-2030  & 20,000& Opt-I &   -& WL/CL BAO/RSD\\
 Euclid & 2020-2026 & 15,000 & Opt-I NIR-S & $0.7 - 2.2$ (gals) &  WL/CL BAO/RSD \\
 WFIRST& 2024-2030 & 2200 & NIR-I  NIR-S & $1.3 - 3.0$ (gals) & WL/CL/SN BAO/RSD \\
 \hline \hline
\end{tabular}

\end{table}

\section{Dark Energy Models: \textit{Theoretical attempts to reveal the darker side of universe}}

It has been a natural choice to try to understand the present acceleration of the universe by also using scalar fields. In this section, we will present some alternative candidates of DE based on various cosmic fluids.

\subsection{Cosmological Constant models}

One of the simplest ways to incorporate the acceleration of the Universe into theoretical models, is to revive the cosmological constant $\Lambda$ term. Ironically, $\Lambda$ was originally introduced by Einstein as a way of preventing his dynamic model of the Universe from evolving in 1917. In its simplest form, general relativity predicted that the Universe must either expand or contract. But Einstein believed the Universe is static, so he added the  $\Lambda$ term to his equations to stop the expansion. In 1917 he introduced the cosmological constant, the antigravity vacuum energy. He had adjusted the scale of $\Lambda$ to gravity so that the Universe stays static.  In the same year 1917 Willem de Sitter has calculated Einstein's equation for a vacuum Universe without matter. This solution drives inflation of the Universe. Also, in Einstein's Universe $\Lambda$ was used for a stationary Universe, but in de Sitter's Universe $\Lambda$ is the reason for inflation. Alexander Friedmann (1888-1925) realized that this was an unstable fix and proposed an expanding universe model. When in 1929 Hubble's study of nearby galaxies showed evidence that the universe was indeed expanding, Einstein saw no further use of the cosmological constant and rejected it. He famously commented to George Gamow that he viewed the introduction of the cosmological constant term as ''the greatest blunder of my life''.


However, Einstein did not drop the interest around the cosmological constant  as well. In fact, later, modern field theory reintroduced the cosmological constant with the energy density of the vacuum, and on these grounds it has been revived as a driving force for the acceleration of the Universe. Also, this approach represents the simplest model of dark energy where the introduction of a single parameter is enough to fit all the astronomical data \cite{peebles003}. From then, the cosmological constant has been revived as a model of dark energy.

Einstein was seeking statistic solutions $(\dot{a}=0)$, so he proposed a modification of his
equation.\\
Einstein’s equation with the constant $\Lambda$ is given by
\begin{align}
R_{\mu \nu}-\dfrac{1}{2}g_{\mu \nu}R- \Lambda g_{\mu \nu}= 8 \pi G T_{\mu \nu}
\end{align}

In FRW background these equations become,
\begin{align}
H^{2}= \dfrac{{\dot{a}}^{2}}{a^{2}} = \dfrac{8 \pi G}{3} \rho - \dfrac{k}{a^{2}} + \dfrac{\Lambda}{3}
\end{align}
and
\begin{align}
\dfrac{\ddot{a}}{a} = -\dfrac{4 \pi G}{3}(\rho + 3p)+\dfrac{\Lambda}{3}
\end{align}

It can be clearly seen from the above equations that sufficiently large positive value of cosmological constant $(\Lambda > 4 \pi G (\rho + 3 p))$ can drive the accelerated expansion of the universe.

The corresponding action is,
\begin{align}
S= -\dfrac{1}{16 \pi G} \int d^{4}x \sqrt{-g} (R+ 2\Lambda) + S_{M}
\end{align}
where $g$ is the determinant of the metric tensor $g_{\mu \nu}$, $R$ is the Ricci scalar, $S_{M}$ denotes the matter action. The cosmological constant here is a constant term in the Lagrange density. For the cosmological constant, $p_{\Lambda}=-\rho_{\Lambda}=-\dfrac{\Lambda}{8 \pi G}=$ constant.


The small positive cosmological constant has been supported by a number of observations. Indeed the cosmological constant is a perfect fit to the dark energy data. There are two cosmological constant problems \cite{weinberg89, weinberg000}: The first one is the smallness of vacuum energy or does not gravitate at all, and the second one is the comparison to the present mass density.

\subsubsection{Fine-tuning Problem}

If the origin of $\Lambda$ is a vacuum energy, there is a serious problem of its energy scale. The vacuum means a state of minimum energy. For a harmonic oscillating particle the potential is of the form, $V(x)=\dfrac{1}{2} \omega^{2} x^{2}$ . The vacuum state is given by the particle sitting motionless in the minimum of the potential, i.e., $x = 0$. But mechanically the position and momentum of the particle cannot be obtained at the same time because of the uncertainty principle. So, the lowest energy state has an energy, $E_{0}=\dfrac{1}{2} h \omega$. The quantum field can be considered as an infinite set of harmonic oscillators, where the minimum energy of such a field should be also infinite. However, from dimensional consideration if the theory is considered up the Planck scale then,

\begin{align}
\rho_{\Lambda} \sim (10^{18}Gev)^{4} \sim 2 \times 10^{110} \,\,\,\, \frac{era}{cm^{3}}
\end{align}
However, cosmological observations indicate,

\begin{align}
\rho_{\Lambda}^{obs} \leq (10^{-12}Gev)^{4} \sim 2 \times 10^{-10} \,\,\,\, \frac{era}{cm^{3}}
\end{align}

There is 120 orders of magnitude difference between the theoretical expectation and the observational value. This discrepancy is the worst theoretical prediction.\\

\subsubsection{Coincidence Problem}

The second cosmological constant problem is on the smallness of $\rho_{\Lambda}$ and the on the starting of cosmic acceleration. If the vacuum energy were big and dominant from the earlier epoch, there would be no chance to form structures in the Universe. The observers will only observe the states which are allowed for observers. This consideration is the  known as anthropic principle. According to this principle, universe may not be determined directly by one specific process, but there are different expanding regions at different times and space of the Universe. Therefore, the measured value of $\rho_{\Lambda}$ should be just suitable for the evolution of intelligent lives.

This anthropic consideration seems to give us the explanation for both the cosmological constant problems i.e. on the smallness and starting of acceleration. However, its verification is still remains as a challenge. The anthropic explanation of the value $\rho_{\Lambda}$ makes sense only if there is a multiverse with a lot of big bangs and different values of $\rho_{\Lambda}$. 

Mathematical physics invites the idea that space contains energy whose gravitational effect approximates Einstein's cosmological constant, $\Lambda$. This concept termed as dark energy or quintessence. Physics also suggests the dark energy could be dynamical, its density is evolving to its natural value, zero. This is small now because the expanding universe is old. Also, after the discovery of the expansion of the universe, the cosmological constant has been almost forgotten due to the fact that its contribution is not necessary to achieve a dynamical expansion in FRW cosmology.

\subsubsection{$\Lambda$ CDM model}

Present studies have shown that around 68$\%$ of the mass–energy density of the universe can be attributed to  dark energy. The canonical concordance cosmology, known as cosmological constant $\Lambda$ is the simplest possible explanation for dark energy, and is used in the current standard model of cosmology known as the $\Lambda$CDM model. It describes a flat universe composed of baryonic and dark matter, radiation and a cosmological constant. Nowadays the $\Lambda$CDM model is in astonishing agreement with observational constraints \cite{tegmark006, jones009}.

The evolution of the $i^{th}$ component is often described by the density
parameter $\Omega_{i} \equiv \dfrac{\rho_{i}}{\rho_{crit}},$ where $\rho_{crit} \equiv \dfrac{3 H^{2}}{(8 \pi G)} $ is the critical density and
$H \equiv \frac{\dot{a}}{a}$ is the Hubble function. Now, as a consequence of Friedmann's set of equations %\eqref{•},

\begin{align}
H(a)_{2}= H_{0}^{2}[\Omega_{b}(a)+ \Omega_{DM}(a)+ \Omega_{rad}(a) + \Omega_{\Lambda} (a)],
\end{align}
where the various $\Omega's$ stand for baryons, dark matter, radiation and cosmological constant contributions and a flat universe \cite{coles002}.\\
With present time scale factor $a_{0}=1,$ then above equation can be renewed as,

\begin{align}
H(a)_{2}= H_{0}^{2}[\Omega_{b} a^{-3}+ \Omega_{DM} a^{-3}+ \Omega_{rad} a^{-4} + \Omega_{\Lambda}.
\end{align}

So, it is clear that the expansion rate of the universe is determined by the energy density and the equation of state of its constituents. In order to determine the expansion history, the recent values of the cosmological parameters and the Hubble constant must be measured. %The most recent values for these quantities are from Planck Collaborations are respectively.....

\subsection{Quintessence models}

Quintessence scalar field model is the most popular among the different models of time evolving dark energy. The idea is to introduce a homogeneous time dependent scalar field $\phi(t),$ minimally coupled to the matter field. The nature of the field is characterized by a potential $V(\phi)$ associated to the scalar field. The action of a scalar field is written as,

\begin{align}
S= \int d^{4}x \sqrt{-g} (- \dfrac{1}{2} g^{\mu \nu} \partial_{\mu} \phi \partial_{nu} \phi - V(\phi)).
\end{align}


The expression of the dark energy equation of state parameter $\omega$ for a quintessence
scalar field is give by,
\begin{align}
\omega= \dfrac{\dot{\phi}^{2}- 2 V(\phi)}{\dot{\phi}^{2}+ 2 V(\phi)}.
\end{align}
It is also straightforward from the expressions of $\rho_{\phi}$ and $p_{\phi},$ as,

\begin{align}
\rho_{\phi}+ p_{\phi}= \dot{\phi}^{2} \geq 0.
\end{align}
This indicates that, for $\rho_{\phi} \geq 0,$ $\omega \geq -1.$ 

Now the quintessence potential can be expressed as,

\begin{align}
V(\phi)= \left(\dfrac{1- \omega}{1+ \omega}\right) \dfrac{\dot{\phi}^{2}}{2}.
\end{align}
This equation reveals that dark energy equation of state parameter $\omega$ for a quintessence
model is time evolving. Depending upon the nature of quintessence potential, quintessence models are classified in three different classes.

\begin{itemize}
\item If $ V(\phi) \ll \dot{\phi}^{2},$
, then $ \omega \simeq 1$ and the energy density varies as $\rho_{\phi} \propto a^{-6},$ which is equivalent to the stiff matter. This does not contribute like dark energy.

\item If $V(\phi) \gg \dot{\phi}^{2},$ then $\omega \simeq -1$ and the energy density $\rho_{\phi}=$ constant, which is equivalent to the cosmological constant.

\item For the intermediate scenario $-1 < \omega < 1,$ the energy density $\rho_{\phi} \propto a^{-n},.$ The quintessence field generates cosmic acceleration for $ 0 \leq n \leq 2.$ \cite{copeland006}.
\end{itemize}

The idea of quintessence scalar field was first introduced in the context of inflation by Ratra and Peeble \cite{ratra88} and Wetterich \cite{wetterich88}. There are ample amount of work in the literature in the context of late time cosmic acceleration with different type of quintessence potential. $V(\phi) \propto \dfrac{1}{\phi^{\alpha}},$ ($\alpha$ is a constant) type of potential was first introduced in the context of dark energy. An exponential potential can generate a power law expansion that is $a(t) \propto t^{b},$ where $b$ is a positive constant. But the exponential potential can not explain the transition from decelerated to accelerated phase of expansion. A double exponential potential can successfully generate the present acceleration and the decelerated expansion phase that prevailed in the recent past \cite{sen02a}.

The quintessence scalar models with some fine-tuning can address the problem of cosmic coincidence. Observations suggested that at present the energy density of the scalar field $(\rho_{\phi})$
and matter energy density $\rho_{\phi}$ are comparable in order of magnitude. As these two energy
densities decay at different rates, it requires a fine tuning the initial conditions to make them
comparable at present time. The idea is to introduce the quintessence potential in such a way
that the energy density $(\rho_{\phi})$ behaves in a very similar way as the dark matter density for a wide range of initial conditions. Actually the idea is that the dark energy density will follow
the evolution which is similar to the evolution of the matter density. This is known as the tracking behaviour of the quintessence dark energy. The idea of tracking quintessence was first introduced by Zlatev, Wang and Steinhardt \cite{zatev99a}. Sahlen, Liddle and Parkinson have reconstructed quintessence potential and checked the viability of tracking behavior \cite{sahlen007}. On the other hand, the thawing scalar field models behave in the opposite way. The dark energy equation of state parameter $(\omega_{DE})$ for a thawing model is close to $-1$ at earlier epoch and it increases with time. This is opposite to the scenario of the tracking quintessence where $w_{DE}$ decreases with time. The behaviour of the dark energy equation of state depends upon the relative shape of the quintessence potential. A comprehensive discussion of thawing models of dark energy can be found in \cite{scherrer008, chiba009}. Observational constraints on tracking and thawing models are
discussed by Chiba, Felice and Tsujikawa \cite{chiba013}. Comperative study of thawing and freezing
models of dark energy has been presented by Pantazis, Nesseris and Perivolaropoulos \cite{pantazis016}. Stability analysis of tracking quintessence has been discussed by Roy and Banerjee \cite{roy014}. Carvalho et al.\cite{carvalho006} showed that in a scalar field dominated cosmology, it is possible to have a transient accelerating expansion .

\subsection{k-essence}

In quintessence scalar field models of dark energy, potential energy gives rise to the accelerated
expansion of the universe. But it is also possible to have models of dark energy where the kinetic energy drives the acceleration. Originally kinetic energy driven acceleration was introduced to describe inflation of the early universe and this model was named as $k$-inflation \cite{armendariz99}. Chiba et al. \cite{chiba000} first introduced this idea to describe late time acceleration, it was generalized by Armendariz-Picon et al. \cite{armendariz000, armendariz001} and called it as $k$-essence models of dark energy. The action for the $k$-essence models is,
\begin{align}
S= \int d^{4}x \sqrt{-g} P(\phi, X),
\end{align}
where $X= -\frac{1}{2} (\triangledown \phi)^{2}$ is the kinetic energy and $P(\phi, X)$ is the Lagrangian pressure density. The idea of $k$-essence indicates kinetic energy dominated Lagrangian, i.e, when $X \rightarrow 0,$ the Lagrangian should also vanish
$(P(\phi, X) \rightarrow 0).$ Hence, the Lagrangian density around $X = 0$ can be expanded as,

\begin{align}
P(\phi , X)= k(\phi)X + L{\phi} X^{2}+ \cdots
\end{align}
Here, the higher order terms of $X$ can be neglected for $X \rightarrow 0$. Now, one can redesign the potential and Lagrangian density as,
$\phi^{new}= \int_{\phi} \sqrt{\dfrac{L}{\mid K \mid}} d\phi$ and $P(\phi^{new}, X^{new})= f(\phi^{new})(-X^{new}+ {X^{new}}^{2})$, where, $X^{new}= (\frac{L}{\mid k\mid})X$ and $f(\phi^{new})= \dfrac{k^{2} \phi}{L \phi}$. 
In a flat FRW background, the field equations of this model can be reconstructed as, 
$$ H^{2}= \dfrac{8 \pi G}{3} f(\phi)[-X + 3 X^{2}] $$
$$ \dfrac{\ddot{a}}{a}= \dfrac{8 \pi G}{3} f(\phi)[- 2X + 3 X^{2}]. $$

Observing the continuity equation, $\dot{\rho}+3H(\rho +p)=0,$ it can be stated that in a strongly radiation or matter dominated era $(\rho_{m}\gg \rho_{\phi}),$ the Hubble parameter evolves as $H=
\dfrac{2}{3 (1+ \omega_{m}) (t-t_{0})}$. The pressure and energy density of scalar field for this model in FRW background can be given as,

$$ p_{\phi}= P(\phi, X)= P(\phi, X)= f(\phi)(-X + X^{2} $$

$$\rho_{\phi}= f(\phi)(-X + 3 X^{2} $$

The equation of state can be obtained as, $\omega_{\phi}= \dfrac{p_{\phi}}{\rho_{\phi}}= \dfrac{1-X}{1-3X}.$ The accelerated expansion occurs for $\omega_{\phi} \leq \dfrac{-1}{3} \Rightarrow X < \dfrac{2}{3}.$ Eventually, the EoS of cosmological constant can be retrieved for $X=\dfrac{1}{2}$. For a constant equation of state of the scalar field (X = constant),$ f(\phi) \propto (\phi - \phi_{0})^{- \alpha}, $  where $\alpha= \dfrac{2 (1+ \omega_{\phi})}{1+ \omega_{m }}.$
For $\alpha = 2,$ the solution is a boarder between decelerating and accelerating phase. At dark energy dominated epoch $(\omega_{\phi}=-1),$ $f(\phi)$ is constant, i.e, $X = \dfrac{1}{2}.$ This corresponds to ghost condensate scenario \cite{arkani004}. In order to build a viable model of dark energy $f_{\phi}$ has to be fine-tuned to be of order the present energy density of the universe.

\subsection{Phantom models}

Phantom field was first introduced by Hoyle \cite{hoyle49, hoyle72} in his steady state theory of the universe.
Later it was used by Caldwell \cite{caldwell002} as a dark energy candidate to drive the accelerated expansion
of the universe. Phantom field has negative kinetic energy. Motivation of phantom field comes from s-brane construction. and the action is given as
\begin{align}
S= \int d^{4}x L(\phi, X)
\end{align}
$L(\phi, X)=-X-v(\phi).$
The kinetic energy of phantom field is negative. This is the difference of the phantom field models with the quintessence models of dark energy. The energy density and pressure of the phantom field are $\rho = - \dfrac{\phi^{2}}{2}+ v(\phi)$ and $p=- \dfrac{\phi^{2}}{2}- v(\phi $
respectively. Now, the EoS parameter $\omega_{\phi}= \dfrac{\dot{\phi}+2V(\phi)}{\phi^{2}-2V(\phi)}.$ So, $\omega_{\phi} < -1$ when $2 V \phi \gg \dot{\phi^{2}}$.  Phantom field models of dark energy predict different type of ultimate fate of the universe. The phantom field can roll up the potential due to its negative kinetic energy. This scalar field obey an EoS with negative kinetic energy violating the weak energy condition, $\rho + p \geq 0$. This is a serious problem for quantum instabilities. But if the potential do not have any maxima, then the universe will expand to infinity very rapidly in finite time. So every thing will rip apart as the curvature grows towards infinity and this scenario is known as Big Rip singularity.

With  potential, having a maximum, the singularity can be avoided. Suppose, $V(\phi)= \dfrac{V_{0}}{\cosh (\frac{\alpha \phi}{\phi_{0}})},$ where $\alpha$ is a constant has been suggested to avoid Big Rip. In contrast to ordinary kinematics, the phantom field evolves toward the top of the potential and crosses over on the other side. If then turns around and again returns to the top, executing damped oscillations across the top until it finally settles at $\omega_{\phi}=-1.$ In other words, the field reaches maxima of the potential at $\phi =0$ and rests after a damped oscillation. When it rests, $\dot{\phi}=0$ and $\omega_{\phi}=-1$. 
 
\subsection{Chaplygin Gas models}

An comfortable way to unify the dark sector of the universe is to consider it as a single component that acts as both DE and dark matter. In the simplest way this unification can be achieved by a universe filled with the Chaplygin gas. Chaplygin \cite{chaplygin04} introduced this as a suitable mathematical approximation for calculating the lifting force on a wing of an airplane in aerodynamics. He also observed that pure Chaplygin gas is a perfect fluid which behaves like a presuureless fluid at an early stage and a cosmological constant at a later stage. Kamenshchik \cite{kamenshchik001} rediscovered the same model in the same context with a special type of equation of state,
\begin{align} \label{chapEoS1}
p=-\dfrac{\beta}{\rho},
\end{align}
where $\beta$ is a positive constant.


The convenience of the Chaplygin gas is connected with the fact that the corresponding Euler equations have a very large group of symmetry, which implies their integrability. The relevant symmetry group has been described in modern terms \cite{bazeia98}. The negative pressure following from the Chaplygin equation of state could also be used for the description of certain effects in deformable solids\cite{stanyukovich60}, of stripe states in the context of the quantum Hall effect and of other phenomena. The Chaplygin gas has positive and bounded squared sound velocity, 
\begin{align}
v_{x}^{2}=\dfrac{\partial p}{\partial \rho}= \dfrac{A\beta}{\rho^{2}},
\end{align}
which is a non-trivial fact for fluids with negative pressure.

The Chaplygin gas equation of state has recently raised a growing attention \cite{jackiw000a} because it displays some interesting and intriguingly unique features. The Chaplygin gas is the only fluid that admits a super symmetric generalization \cite{jackiw000b}. Inspired by the fact that the Chaplygin gas possesses a negative pressure, Kamenshchik et al. \cite{kamenshchik001} have undertaken the simple task of studying a FRW cosmology illed with this type of fluid .  Further theoretical developments of the model were given in \cite{bilic002, gorini003}. One of its most remarkable properties is that it describes a transition from a decelerated cosmological expansion to a stage of cosmic acceleration. The inhomogeneous Chaplygin gas able to combine the roles of dark energy and dark matter \cite{bilic002}. Bennet \cite{bennet003}, has extended the pure Chaplygin gas to generalized Chaplygin gas. The corresponding EoS parameter contains two free parameters and can be defined as ,

\begin{align}
p=-\dfrac{\beta}{\rho^{\alpha}},\,\,\, 0<\beta<1.
\end{align}
The EoS parameter for modified Chaplygin gas \cite{benaoum012, debnath004} can be defined as 
\begin{align} \label{chapEoS2}
p= \mu \rho -\dfrac{\beta}{\rho^{\alpha}},\,\,\, 0<\beta<1,
\end{align}
where $\mu$ and $\rho$ are positive constants the EoS parameter shows radiation era $(\mu = \dfrac{1}{3})$ at one extreme $(a(t)\approx 0)$ whereas a $\Lambda$CDM model at other extreme $(a(t)\approx \infty)$. Guo and Zhang \cite{guo005} prposed Variable Chaplygin gas model with the EoS parameter \eqref{chapEoS1}, where $\beta$ is a positive function of cosmic scale factor $a$. Debnath \cite{debnath007} proposed variable modified Chaplygin gas  that satisfies \eqref{chapEoS2} with $\mu$ as a positive constant and  $\beta = \beta (a)$. Gorini et al. \cite{gorini003} and Sahni et al. \cite{sahni003} studied the two-fluid cosmological model  including both the Chaplygin gas and the usual dust like matter. The two-fluid model can suggest a solution of the cosmic coincidence conundrum \cite{gorini003}.\\

The cosmological models of the Chaplygin class have at least three significant features: (i) it  describes a smooth transition from a decelerated expansion of the universe to the present epoch of cosmic acceleration; (ii) it attempts to give a unified macroscopic phenomenological description of dark energy and dark matter; and (iii) finally, it represents the simplest deformation of traditional $\Lambda$CDM models. Another interesting feature of the Chaplygin gas is that it can be considered as the simplest model within the family of tachyon cosmological models. Frolov \cite{frolov002} showed that the Chaplygin gas cosmological model can be identified with a tachyon field theoretical model with a constant value of the field potential.

\subsection{Tachyon models}

A tachyon has negative squared mass and speed greater than light $(c)$. The EoS parameter of Tachyon model varies between -1 to 0, therefore tachyon has been chosen as a candidate of dark energy \cite{gibbons002}. Different models shows tachyon with suitable potential and can drive the acceleration \cite{padmanabhan002, copeland005}. As a consequence of negative squared mass of tachyon, it rests on the maxima of the potential and subjected to a very small perturbation. The action of tachyon model is,
\begin{align}
S=- \int d^{4}x V(\phi) \sqrt{- det (g_{ab}+ \partial_{\alpha} \phi \partial_{\beta} \phi)},
\end{align}
where $V(\phi)$ is tachyonic potential. In a flat FRW background, the energy density and pressure of the tachyon as,

$$\rho_{\phi} = \dfrac{V(\phi)}{\sqrt{1-(\dot{\phi}^{2})}}$$  and $$ p_{\phi}= - \dfrac{V(\phi)^{2}}{\rho_{\phi}}. $$

Incorporating these in Einstein's field equations, for tachyon, it can be obtained 

\begin{align}
&H^{2}= \dfrac{8 \pi G V(\phi)}{3 \sqrt{1-(\dot{\phi})^{2}}}\\
&\dfrac{\ddot{a}}{a}= \dfrac{8 \pi G}{3}
\dfrac{ V(\phi)}{\sqrt{1-(\dot{\phi})^{2}}} (1-2  \dot{\phi}^{2})
\end{align}

Now the combining equation takes the form,

\begin{align}
\dfrac{\ddot{\phi}}{1- \phi^{2}} + 3H \dot{\phi} + \dfrac{1}{V} \dfrac{dV}{d \phi} =0
\end{align}

Hence, the accelerated expansion of the universe occurs for $\dot{\phi}^{2} < \dfrac{2}{3}$. The EoS parameter, $\omega_{\phi}= \dfrac{p_{\phi}}{\rho_{\phi}}= \dot{\phi}^{2}-1$ is in the range $-1 < \omega_{\phi} < 0$. The scalar field density can be observed from the continuity equation as, $\rho \varpropto a^{-m}$, where $0< m < 3$.

\subsection{Holographic dark energy}

Theorists have been believed that understanding entirely the nature of DE is very tough till a complete theory of quantum gravity was established \cite{witten00}. Though there is a lack of quantum gravity, still some attempts can be made to probe the nature of DE according to some principles of quantum gravity. As an example, the holographic DE model, which can be constructed with the help of principle of quantum gravity theory.  The distinctive feature of the cosmological constant or vacuum energy is that its EoS is always exactly equal to -1. However, when considering the requirement of holographic principle originating from quantum gravity speculation, the vacuum energy will acquire dynamical property. In the classical gravity theory, cosmological constant is always considered to  provide an arbitrary value to the dark energy density. However, a complete theory of quantum gravity should be capable of making the properties of DE, such as the energy density and the EoS, be determined definitely and uniquely. Currently, an interesting attempt \cite{cohen99, horava00} for probing the nature of DE within the framework of quantum gravity is considered, known as the holographic dark energy. It is well known that the holographic principle is an important result of the recent researchers \cite{susskind95,hooft09} for exploring the quantum gravity as well as string theory. This principle is enlightened by investigations of quantum property of the black holes.  Nojiri and Odintsov \cite{nojiri06} proposed a generalized holographic DE model, identifying the IR cut-off with combination of FRW parameters. Granda and Oliveros \cite{granda08} took the holographic DE density to depend on the usual quadratic term in the $H$ as well as on the time derivative of $H$. 

\subsection{Pilgrim dark energy}

Wei \cite{wei12} proposed a new DE model called as Piligrim DE. It belongs to family of holographic DE. One of its key points is the formation of the black hole. This has been introduced on the basis that black hole formation can be avoided through the strong repulsive force of the type of DE. It is well known that everything will be completely torn up before universe ends in big rip caused by the phantom-like DE. Even the black hole will also be completely torn up. So the repulsive force contributed by phantom-like DE is strong enough to destroy the black hole. Babichev et al. \cite{babichev04}, also argued that black hole mass reduces due to phantom acceleration phenomenon. Wei \cite{wei12} developed cosmological parameters for pilgrim DE model with Hubble horizon and provided different possibilities for avoiding the black hole formation through pilgrim DE parameters. He adopted different possible theoretical and observational ways to make the black hole free phantom universe.\\ The first property is,

\begin{align}
\rho_{\Lambda} \geq M_{P}^{2} L^{-2}.
\end{align}
To implement the above property, Wei \cite{wei12} set piligrim DE model in the simplest way as,

\begin{align}
\rho_{\Lambda}= 3 n^{2}M_{P}^{4-s} L^{-s},
\end{align}
where $n$ and $s$ are dimensionless  constants.
\\
From both these equations, $L^{2-s} \geq M_{P}^{s-2}= l_{P}^{2-s},$ where $l_{P}$ is the reduced Planck length. Since $L \geq l_{P},$ one requires $s \leq 2$. Another requirement for pilgrim DE is that it is to be phantom-like, i.e, $\omega_{\Lambda} < -1.$ Wei \cite{wei12} obtained the EoS parameter of piligrim DE with Hubble horizon as a simplest choice of cut-off $L,$ i.e, $L=H^{-1}$ and obtained the energy density of piligrim DE as $\rho_{\Lambda} \varpropto H^{s}$. Sharif and Jawad \cite{sharif13a, sharif13b} studied the interacting piligrim DE in flat as well as non-flat universe models with different IR cut-offs. Chattopadhyay et al. \cite{chattopadhyay14}, Sharif and Rani \cite{sharif14} have also investigated the piligrim DE cosmological models in various modified theories of gravitation. Jawad and Majeed \cite{jawad15a} have discussed correspondence of pilgrim DE with scalar field models.

\subsection{Modified holographic Ricci dark energy}
The holographic DE models with Hubble or particle horizons can not explain the current accelerated expansion as the effective EoS for such vacuum energy is zero \cite{hsu04}. Also, the model suffers from some disadvantage while the event horizon is taken as the length scale. Future event horizon is a global concept of space-time whereas density of DE is a local quantity. So the relation between them will enact challenges to the causality concept. These lead to the introduction of a new holographic DE, where the length scale is given by average radius of the Ricci scalar curvature, $R^{\frac{-1}{2}}.$ Recently, Li \cite{li04} proposed that the future event horizon of the universe to be used as the characteristic length $L$. This holographic DE model not only represents a reasonable for DE density, but also leads to a solution for the cosmic accelerated expansion. In fact, the choice of the characteristic length $L$ is not unique for the holographic DE model. Gao et al. \cite{gao09} assumed that the length can be given by the inverse of Ricci scalar curvature, i.e, $L = \mid R \mid ^{\dfrac{-1}{2}}, $ which is called holographic Ricci DE model. It is argued that the model can solve the coincidence problem entirely. Thus, the properties of such holographic Ricci DE have been investigated widely soon aft\cite{huang04,zhang05}.

The modified holographic Ricci DE model introduced by Granda and Oliveros \cite{granda09}, based on space-time scalar curvatures, is fairly good in fitting with the observational data. In this model, the fine tuning and causality problems can be avoided. The coincidence problems also can be solved effectively. Chen and Jing \cite{chen09} studied a modified form of Ricci DE energy by assuming the density of DE contains $H, \dot{H}$ and $\ddot{H}.$ The expression of the DE density of this modified holographic Ricci DE is given by,

\begin{align}
\rho_{\Lambda}= 3 M_{P}^{2}(\beta_{1} H^{2} + \beta_{2} \dot{H} + \beta_{3} \ddot{H} H^{-1}),
\end{align}
where, $\beta_{1}, \beta_{2}$ and $\beta_{3}$ are constants.

Saadat \cite{saadat12} discussed FRW modified holographic Ricci DE model. Jawad \cite{jawad15b} investigated modified holographic Ricci DE in Chameleon Brans-Dicke cosmology and its thermodynamic consequences.
\section{Problems investigated}
This section is devoted to the presentation of problems investigated and results obtained in the thesis. The main objective of the present work is to study the dynamical behavior of anisotropic DE cosmological models using various cosmic matter fluids those play a vital role in composing our universe. The matter fluids of specific interest are Bulk viscous fluid, Cosmic string fluid, Directional electromagnetic fluids etc.. The noble cause behind this objective is due to the interesting fact that; the evolutionary history of our universe show the dominance of the matter fluids in the early phase of evolution {just after big bang neucleo-synthesis} but, surprisingly, the late epoch of evolution (present accelerated expansion phase) is filled and driven due to DE only. As a result of interest, many problems have been framed to understand the nature of DE along with the matter fluids during the phenomenal evolution. Many researchers have considered some dynamic form of scale factors and space-times in the frame work of GR to crack through the problems. Keeping these problems in mind, we compared among evolutionary nature of the matter fluids along with DE in respective two-fluid situations and the acceptability of the our model is proved via few popular diagnosis. Moreover, some new ideas on how to improve this situation are subsequently offered in few chapters through an enrich reconstruction of scale factors. We looked into the problems focusing the above said aspects and presented into ten chapters including the Introduction as chapter 1 and summary of results as chapter 10. All our results are in nice agreement with current cosmic observational data.


In chapter 2, anisotropic dark energy cosmological models have been investigated in a Bianchi V space-time, with the energy momentum tensor consisting of two non-interacting fluids, namely, bulk viscous fluid and dark energy fluid. Two different models are constructed based on the power law cosmology and de Sitter universe. The constructed model was also embedded with different pressure gradients along different spatial directions. The variable EoS parameter and skewness parameters for both models are obtained and analysed. The physical properties of the models obtained with the use of scale factors of power law and de Sitter law are also presented.

In chapter 3, we have constructed the cosmological model of the universe in a two-fluid environment
with a newly developed mathematical formalism. In order to construct the model, we have considered with a time varying deceleration parameter in frame work of Binachi type V space time. Both the fluids, the viscous fluid and the dark energy DE fluid have shown their dominance respectively in early time and late time of the cosmic evolution. The scale factor that simulates
the cosmic transition based on the value of the bulk viscous coefficient. Within the developed formalism, a general form of the skewness parameters is also obtained as a functional form of the scale factor. The physical parameter of the model such as EoS parameter is also derived and analyzed. The state finder diagnostic pair is also obtained to understand the geometrical nature of the model.



The next part of thesis is divided into two chapters depending on two characteristics of a single matter fluid. We have investigated the anisotropic behavior of the accelerating universe when the matter field is considered to be of two fluids: (a) the usual geometric string with DE and (b) the Nambu string with DE fluid.


In chapter 4, The matter field we have considered is of the usual geometric string fluid and dark DE fluid. In order to represent the pressure anisotropy, the skewness parameters are introduced along three different spatial directions. Also here, to achieve a physically realistic solutions to the field equations, we have considered hybrid scale factor, which simulates a cosmic transition from early deceleration to late time acceleration. It is observed that the string fluid dominates the universe at early deceleration phase but does not affect nature of cosmic dynamics substantially at late phase, whereas the DE fluid dominates the universe in present time, which is in accordance with the observations results. Hence, we analyzed here the role of two fluids in the transitional phases of universe with respect to time which depicts the reason behind the cosmic expansion and DE. The role of DE with variable EoS and skewness parameters, is also discussed along with physical and geometrical properties.\\
In a sequel to this, chapter 5 explores the role of anisotropic components on the dark
energy and the dynamics of the universe in a nambo string embedded. An anisotropic dark energy fluid with different pressures along different spatial directions is assumed to incorporate the effect
of anisotropy. One dimensional cosmic strings aligned along x-direction supplement some kind of anisotropy. Anisotropy in the dark energy pressure is found to evolve with cosmic expansion at least at late times. At an early phase, the anisotropic effect due to the cosmic strings substantially
affect the dynamics of the accelerating universe.


Similarly, in chapter 6 and 7, we have investigated an anisotropic dark energy cosmological model in
a two  fluid situations such as the usual dark energy and the magnetized  fluid along radial and horizontal direction respectively.We have assumed
the dark energy pressure to be anisotropic in different spatial directions. In order to develop the
mathematical formalism of the model we have considered the scale factor as hybrid scale factor
which is a combination of both power law and volumetric expansion law. The physical parameters
are derived and analyzed and found to be in agreement with the observational limits.


In chapter 8, In order to obtain various deterministic solutions, we have considered three general forms of scale factor. The different forms of scale factors considered here produce time-varying deceleration parameters in all the cases that simulates the cosmic transition. The variable EoS parameter, skewness parameters for all the models are obtained and analyzed. The physical properties and viabilities of the models are also discussed matching with current observational data.

\section{Conclusion}

The aim of this chapter is to provide a review on origin and evolution of dark energy, as a source of recent accelerated expansion of our universe. In the beginning, an overview of cosmology is also presented where only elementary knowledge on general relativity is required. A basic introduction to Einstein's theory of GR and field equations for a spatially flat FRW metric are presented followed by an insight to DE cosmology. Following the aim, we then, carried out a brief study on various demanding DE candidates. The models constructed with the help of these candidates triggers many research interests at present.    Hence, the aim for this approach is quite ambitious. Therefore, an effort has been made in order to include as much literature as possible in order to refer to all the works employing various DE models. The simplest and most promising models, then, will be analyzed in detail in the subsequent chapters. Models presented in the chapter and its analysis definitely put some light in the context of the uncertainty prevailing in the studies of the late time cosmic acceleration, opening a wide scope of further research. 





 

==> Report_format_thesis/References.tex <==


\begin{thebibliography}{9999}


%Chapter 1
%---------------------------------------------------
\bibitem{penzias65} A. A. Penzias and R. W. Wilson, ApJ, 142, 419–421 (1965).

\bibitem{einstein15} A. Einstein, Sitzungsber.Preuss.Akad.Wiss.Berlin (Math.Phys.), 1915, 844-847 (1915).

\bibitem{einstein16} A. Einstein, Ann. Soc. Sci. Brux., vol. 49, 769-822 (1916). 

\bibitem{guth81} A. H. Guth, Phys. Rev. D 23, 2 (1981).

\bibitem{riess98} A. G. Riess et al., Astron. J. 116, 1009 (1998).

\bibitem{riess99} A. G. Riess et al., Astron. J. 117, 707 (1999).

\bibitem{perlmutter99} S. Perlmutter et al., Astrophys. J. 517, 565 (1999).

\bibitem{suzuki012} N. Suzuki et al., Astrophys. J. 746, 85 (2012).

\bibitem{betoule014} M. Betoule et al., Astron. Astrophys. 568, A22 (2014).

\bibitem{riess004} A. G. Riess, Astrophys. J. 607, 665 (2004).


\bibitem{hillebrandt000} W. Hillebrandt and J. C. Niemeyer. , Annual Review of Astronomy and Astrophysics, 38.1, 191–230 (2000).

\bibitem{schneider006}  P. Schneider. , Springer (2006).

\bibitem{knop003} Supernova Cosmology Project Collaboration, R. A. Knop et. al., Astrophys.J., 598, 102 (2003).

\bibitem{dicke65}  R. H. Dicke, P. J. E. Peebles, P. G. Roll and D. T. Wilkinson., The Astrophysical Journal, 142 (1965).

\bibitem{weinberg008} S. Weinberg. Cosmology. Oxford University Press (2008).

\bibitem{mather94} J. C. Mather et al., The Astrophysical Journal, 420 (1994).

\bibitem{fixsen009} D. J. Fixsen., The Astrophysical Journal, 707.2 (2009).

\bibitem{spergel007} WMAP Collaboration Collaboration, D. Spergel et. al., Astrophys.J.Suppl., 170, 377 (2007).

\bibitem{komatsu011} WMAP Collaboration Collaboration, E. Komatsu et. al., Astrophys.J.Suppl. 192, 18 (2011).

\bibitem{eisenstein007} D. J. Eisenstein, H. J. Seo and M. White, Astrphys. J. 633, 560 (2007).

\bibitem{eisenstein005} SDSS Collaboration Collaboration, D. J. Eisenstein et. al., Astrophys.J., 633, 560-574 (2005).  

\bibitem{miao011} L. Miao, L. Xiao-Dong, W. Shuang and W. Yi., 56.3, 525 (2011).

\bibitem{giostri012} R. Giostri et al., JCAP, 03, 027 (2012).

\bibitem{crittenden002} R. G. Crittenden, P. Natarajan, U. L. Pen, and T. Theuns, Astrophys.J. 568, 20-27 (2002).


\bibitem{planck011}	Planck Collaboration, Astronomy and Astrophysics, 536, A1 (2011).

\bibitem{planck013a} Planck 2013 results. I, Astronomy and Astrophysics, 571, A1 (2013).
 
\bibitem{planck013b} Planck 2013 results. XVI, Astronomy and Astrophysics, 571, A16 (2013).
  
\bibitem{planck015} Planck 2015 results. XIII, Astronomy and Astrophysics, 594, A13 (2015).
 
\bibitem{feng005} B. Feng, X. L. Wang, and X. M. Zhang, Phys. Lett., B607, 35-41 (2005).

\bibitem{allen011} S. W. Allen, A. E. Evrard, and A. B. Mantz,  Ann. Rev. Astron. Astrophys., 49, 409-470 (2011).

\bibitem{haiman000} Z. Haiman, J. J. Mohr, and G. P. Holder, Astrophys. J., 553, 545 (2000).

\bibitem{yu011} H. R. Yu, T. Lan, H. Y. Wan, T. J. Zhang, and B.Q. Wang, Res. Astron. Astrophys., 11, 125-136 (2011).

\bibitem{freedman010} W. L. Freedman and B. F. Madore, Ann. Rev. Astron. Astrophys., 48, 673-710 (2010).

\bibitem{tsutsui009} R. Tsutsui et. al., Mon. Not. Roy. Astron. Soc., 394, L31-L35 (2009).

\bibitem{basilakos008} S. Basilakos and L. Perivolaropoulos, Mon. Not. Roy. Astron. Soc., 391, 411-419 (2008).

\bibitem{friedmann22} A. Friedmann, On the curvature of space. Z. Phys. 10, 377 (1922).

\bibitem{wang98} L. M. Wang and P. J. Steinhardt, Astrophys.J., 508, 483-490 (1998).


\bibitem{peebles003} P. Peebles and B. Ratra,
Rev. Mod. Phys., 75, 559-606 (2003).

\bibitem{weinberg89} S. Weinberg, Rev.Mod.Phys., 61, 1-23 (1989).


\bibitem{weinberg000} S. Weinberg, arXiv:astro-ph/0005265v1, (2000).

\bibitem{tegmark006} M. Tegmark, Phys. Rev. D, 74, 12, 123507 (2006).

\bibitem{jones009} D. H. Jones, MNRAS, 399, 683–698 (2009).

\bibitem{coles002} P. Coles and F. Lucchin, Wiley, Second edition, (2002).


\bibitem{copeland006} E. J. Copeland, M. Sami, and S. Tsujikawa, Int. J. Mod. Phys. D 15, 1753 (2006).


\bibitem{ratra88} B. Ratra and P. J. E. Peeble, Phys. Rev. D 37, 3406 (1988).


\bibitem{wetterich88} C. Wetterich, Nucl. Phys. B 302, 668 (1988).


\bibitem{sen002} A. A. Sen, S. Sethi, Phys. Lett. B 532, 159 (2002).


\bibitem{zatev99a} I. Zatev, L. Wang and P. J. Steinhardt, Phys. Rev. Lett. 82, 896 (1999).


\bibitem{sahlen007} M. Sahlen, A. R. Liddle and D. Parkinson, Phys. Rev. D 75, 023502 (2007).


\bibitem{scherrer008} R. J. Scherrer and A. A. Sen, Phys. Rev. D 77, 083515 (2008).



\bibitem{chiba009} T. Chiba, Phys. Rev. D 79, 083517 (2009); 80, 109902(E) (2009);



\bibitem{chiba013} T. Chiba, A. D. Felice and S. Tsujikawa, Phys. Rev. D 87, 083505 (2013).


\bibitem{pantazis016} G. Pantazis, S. Nesseris and L. Perivolaropoulos, Phys. Rev. D 93, 103503 (2016).


\bibitem{roy014} N. Roy and N. Banerjee, Gen. Relativity Gravity. 46, 1651 (2014).



\bibitem{carvalho006} F. C. Carvalho, J. S. Alcaniz, J. A. S. Lima and R. Silva, Phys. Rev. Lett. 97, 081301
(2006).


\bibitem{armendariz99} C. Armendariz-Picon, T. Damour, and V. Mukhanov, Phys. Lett. B, 458, 209 (1999).

\bibitem{chiba000} T. Chiba, T. Okabe and M. Yamaguchi, Phys. Rev. D 62, 023511 (2000).

\bibitem{armendariz000} C. Armendariz-Picon, V. Mukhanov, and P. J. Steinhardt, Phys. Rev. Lett. 85, 4438 (2000).

\bibitem{armendariz001} C. Armendariz-Picon, V. Mukhanov, and P. J. Steinhardt, Phys. Rev. D 63, 103510 (2001).

\bibitem{arkani004} N. Arkani-Hamed, P. Creminelli, S. Mukohyama and M.Zaldarriaga, JCAP 0404, 001 (2004)


\bibitem{hoyle49} F. Hoyle, Mon. Not. R. Astr. Soc., 109, 365 (1949).

\bibitem{hoyle72} F. Hoyle and J. V. Narlikar, Proc. Roy. Soc. A282, 305 (1972).

\bibitem{caldwell002} R.R. Caldwell, Phys.Lett. B, 54523, 29(2002).


\bibitem{chaplygin04} S. Chaplygin, Sci. Mem. Moscow Univ. (Math. Phys.), 21, 1 (1904).
 
\bibitem{kamenshchik001} A. Kamenshchik, U. Moschella and V. Pasquier,Phys.  Lett.B, 511, 265 (2001). 

\bibitem{bazeia98} D. Bazeia and R. Jackiw,Ann. Phys. (N Y)270, 246 (1998).

\bibitem{stanyukovich60} K. Stanyukovich, Unsteady Motion of Continuos Media (1960).

\bibitem{jackiw000a} R. Jackiw, A Particle Field Theorist’s Lectures on Supersymmetric,Non-Abelian Fluid Mechanics and d-Branes, physics/0010042.

\bibitem{bordemann93} M. Bordemann, J. Hoppe,Phys. Lett.B317, 315 (1993).

\bibitem{jackiw000b} R. Jackiw and A. P. Polychronakos,Phys. Rev.D62, 085019 (2000). 


\bibitem{bilic002} N. Bilic, G.B. Tupper and R. Violler,Phys. Lett.B535 (2002).


\bibitem{gorini003} V. Gorini, A.Yu. Kamenshchik and U. Moschella,Phys. Rev.D67,063509 (2003).


\bibitem{bennet003} C. L. Bennet et al., Astrophys. J. Suppl.,148,1 (2003).

\bibitem{benaoum012} H. B. Bennaoum, Advances in High Energy Phys., 357802 (2012).

\bibitem{debnath004} U. Debnath et al., Class. Quantum Gravity, 21, 5609 (2004).

\bibitem{guo005} Z. K. Guo et al., Phys. Lett. B, 608, 177 (2003).

\bibitem{debnath007} U. Debnath, Astrophys. Space Sci., 312, 295 (2004).


\bibitem{sahni003} V. Sahni, T.D. Saini, A.A. Starobinsky and U. Alam,JETP Lett.77,201 (2003).


\bibitem{frolov002} A. Frolov, L. Kofman and A. Starobinsky,Phys. Lett.B545, 8 (2002).


%tachyon

\bibitem{sen002} A. Sen, JHEP 0204, 048 (2002); JHEP 0207, 065 (2002).

\bibitem{kluson000} J. Kluson, Phys. Rev. D 62, 126003 (2000).

\bibitem{gibbons002} G. W. Gibbons, Phys. Lett. B 537, 1 (2002).

\bibitem{padmanabhan002} T. Padmanabhan, Phys. Rev. D 66, 021301 (2002).

\bibitem{copeland005} E. J. Copeland, M. R. Garousi, M. Sami and S. Tsujikawa, Phys. Rev. D 71, 043003 (2005).


%Holographic DE

\bibitem{witten000}

\bibitem{cohen99}

\bibitem{horava000}

\bibitem{susskind95}

\bibitem{hooft0009}

\bibitem{brkrnstein}

\bibitem{li004}

\bibitem{gao009}

\bibitem{nojiri006}

\bibitem{granda008}



%Piligrim DE

\bibitem{wei012}

\bibitem{babichev004}

\bibitem{sharif013a}

\bibitem{sharif013b}

\bibitem{chattopadhyay014}

\bibitem{chattopadhyay015}

\bibitem{sharif014}

\bibitem{jawad015b}


%Modified HDE

\bibitem{hsu004}

\bibitem{huang004}

\bibitem{zhang005}

\bibitem{granda009}

\bibitem{chen009}

\bibitem{chattopadhyay011}

\bibitem{saadat012}

\bibitem{jawad015a}


%Chapter2
%---------------------------------------------------
\bibitem{ellis006} G.F.R. Ellis, Gen. Relativ. Gravit., 38, 1003 (2006).

\bibitem{bianchi898} L. Bianchi, Memone di matematica edi Fisica della societa Italiana delle Scienze, serie Terza, 11, 267-352 (1898).

\bibitem{schwarz004} D. J. Schwarz et al.: Phys. Rev. Lett., 93, 221301 (2004).

\bibitem{land007} K. Land and J. Magueijo, Mon. Not. R. astr. Soc., 378, 153 (2007).

\bibitem{lemaitre33} G. H. Lemaitre, Ann. Soc. Sci. Brux., A 53, 51–85 (1933).

\bibitem{zeldovich70} Y. B. Zeldovich, J. Exper. Theor. Phys., 48, 986–988 (1970).

\bibitem{thorne66} K. S. Thorne, Bull. American Phys. Soc., 11, 340 (1966).

\bibitem{hawking66} S. W. Hawking and R. J. Taylor, Nature, 299, 1278 (1966).

\bibitem{kristian66} J. Kristian and R. K. Sachs, Astrophys. J., 143, 379–399 (1966).

\bibitem{kantowski66} R. Kantowski and R. K. Sachs, J. Math. Phys. 7, 443–446 (1966).

\bibitem{barrow97} J. D. Barrow, Phys. Rev. D, 55, 7451-7460 (1997).

\bibitem{barrow99} J. D. Barrow and R. Maartens, Phys. Rev. D 59, 043502 (1999).

\bibitem{cruz007} M. Cruz et al.: Astrophys. J. 655, 11-20 (2007).

\bibitem{hoftuft009} J. Hoftuft et al.: Astrophys. J. 699, 985-989 (2009).

\bibitem{campanelli011a} L. Campanelli et al.: Int. J. Mod. Phys. D 20, 1153-1166 (2011).

\bibitem{campanelli011b} L. Campanelli et al.: Phys. Rev. D 83, 103503 (2011).

\bibitem{axelsson011} M. Axelsson et al.: arXiv:1109.2778 [astro-ph.CO] (2011).

\bibitem{akarsu011} O. Akarsu and C. B. Kilinc, Int. J. Theor. Phys. 50, 1962-1977 (2011).

\bibitem {wald84} R. M. Wald, "General Relativity", The University of Chicago Press, Chicago, 1984.

\bibitem{jaffe006}] J. Jaffe et al., Astron. Astrophys., 460, 393 (2006).

\bibitem{campanelli007} L. Campanelli, P. Cea and L. Tedesco, Phys. Rev. D, 76, 063007 (2007).

\bibitem{goliath99} M. Goliath, G. F. R, Ellis, Phys. Rev D, 60, 023502 (1999).

\bibitem{ellis69} G. F. R. Ellis and M. A. H. MacCallum, Commun. Math. Phys., 12, 108 (1969).

\bibitem{taub51} A. Taub, Ann. Math., 53, 472 (1951).

\bibitem{siklos78} S. T. C. Siklos, Commun. Math. Phys., 58, 255 (1978).

\bibitem{akarsu010a} O. Akarsu, C. B. Kilinc, Gen. Rel. Grav., 42, 119, (2010).

\bibitem{akarsu010b} O. Akarsu, C. B. Kilinc, Gen. Rel. Grav., 42, 763, (2010).

\bibitem{wainwright97}  J. Wainwright and G. F. R. Ellis, Dynamical Systems in Cosmology, Cambridge Univ. Press (1997).

\bibitem{collins73} C. B. Collins, S. W. Hawking, Astrophys. J., 180, 317-334, (1973).

\bibitem{koike94} T. Koike, M. Tanimoto and A. Hosoya, J. Math. Phys., 35, 4855 (1994).

\bibitem{yadav011} A. K. Yadav, Astrophys. Space Sci, 335, 2, 565–575 (2011).

\bibitem{kumar011} S. Kumar and A. K. Yadav, Mod. Phys. Lett. A, 26, 647 (2011).

\bibitem{tripathy017} S.K. Tripathy, B.Mishra, P.K. Sahoo, Euro. J Phus Plus, 132, 388 (2017).

\bibitem{xin005} Z. Xin, Commun. Theor. Phys., 44, 762 (2005).

\bibitem{xin-He007} M. Xin-He et al., Commun. Theor. Phys., 47, 379 (2007).

\bibitem{rong009} C. Rong-Gen et al.: Commun. Theor. Phys., 52, 954 (2009).

\bibitem{khodam011} A. Khodam-Mohammadi and M. Malekjani, Commun. Theor. Phys., 55, 942 (2011).

\bibitem{Xiao011} Z. Xiao-Fei, Commun. Theor. Phys., 56, 1167 (2011).

\bibitem{setare009} M.R. Setare, J. Sadeghi and A. R. Amani, Phys. Lett. B, 673, 241 (2009).


\bibitem{sheykhi011} A. Sheykhi and M. R. Setare, Mod. Phys. Lett. A, 26, 1897 (2011).

\bibitem{amirhashchi013a} H. Amirhashchi, Astrophys. Space Sci., 345, 439 (2013).

\bibitem{amirhashchi013b} H. Amirhashchi, A. Pradahan, H. Zainuddin, Res in Astro Astrophys., 13, 119 (2013).

\bibitem{kumar013} S. Kumar, \emph{Grav. and Cosmology}, \textbf{19},284 ,(2013).






%Chapter 3
%----------------------------------------------------



%chapter-7

\end{thebibliography}







==> Report_format_thesis/ack.tex <==
\addcontentsline{toc}{chapter}{Acknowledgement}
\vspace*{0.5cm}
\begin{center}
%{\large \bf Birla Institute of Technology and Science- Pilani University, Hyderabad Campus, Hyderabad} \\
%\vskip 0.5pc
%{\large \bf Department of Mathematics} \\
%\vskip 5.0pc
\Large\sl {\sc Acknowledgement}
\end{center}
Being involved in the process of pursuing a scientific research programme brings the zest of finding new things, satisfies the quest for gaining knowledge and gives the unalloyed joy of contributing something to the society. Despite a wonderful journey, many times it smells of failure, struggle, uncertainty etc. However, there are many people whose motivational influences helped me throughout this journey and encouraged me to accomplish my goal. It has been great pleasure to thank all of them.\\
First and foremost, I would like to express my sincere and deepest gratitude to my research supervisor, \textbf{Dr. Bivudutta Mishra}, for his constant supports during the course of this work. It is difficult for me to imagine having better supervisor than Prof. Bivudutta Mishra, to whom I am truly grateful, not only for his guidance but also for standing by me in all my choices and for the impressive amount of patience has exhibited during my Ph.D work. It has been a great honour and privilege for me to have worked under his guidance. I also express my deepest gratitude to my Co-advisor, \textbf{Dr. Pradyumn Kumar Sahoo} for his constant supports during the course of my Ph.D years.\\
I would like to thank my DAC members, \textbf{Dr. K. Venkata Ratnam} and \textbf{Prof. Kannan Ramaswamy}  for their valuable suggestions for the improvement of my research work.\\ 
 My sincere thanks to HoD and DRC convener, Department of Mathematics, BITS-Pilani, Hyderabad Campus for their help and support.\\
 I am grateful to all the faculty members of the department of Mathematics for supported me and encourage me to give my best effort in my thesis.\\
 My greatest gratitude to our co-authors \textbf{Dr. Sunil Kumar Tripathy}, Assistant Professor,Department of Physics, IGIT Saranga, Dhenkanal, Odisha and \textbf{Dr. S. K. J. Pacif}, Assistant Professor, Department of Mathematics,VIT University, Vellore, Tamilnadu for their guidance, discussion and support.\\  
 I gratefully acknowledge to BITS-Pilani, Hyderabad Campus for providing me the necessary facilities to carry out my research work.\\


\newpage

==> Report_format_thesis/cover.tex <==
\pagestyle{empty} 
	\begin{center} 
	\Large{\textbf{\textsf{{Investigation on late time dynamics of the universe along with anisotropic dark energy models}}}} \\ 
        \vspace{1.0cm} 
        \large{\textbf{Pratik Premadarshi Ray}}\\ 
        %\textbf{}\\                              
	\vspace{1.0cm}
        \small{\em{A thesis submitted to the Birla Institute of Technology and Science-Pilani for the award of the Degree of}}\\ 
	\vspace{0.16in} 
        \small{\textbf{Doctor of Philosophy}}\\ 
       % \small{{in }}\\ 
       % \small{\textbf{ Applied Physics}}\\ 
        \vspace{0.55in} 
        \begin{center}
        \includegraphics[scale=0.1]{logo}
        \end{center}
	\vspace{1.00cm} 
	\large{\em{Under the supervision of}}\\ 
	\vspace{0.10cm} 
%	\large{\textbf{Dr. Zashmir Naik}}\\ 
%	\small{Lecturer}\\
%	\small{School of Physics}\\
%	{Sambalpur University, Jyotivihar}\\
%	\vspace{0.03cm}
%	\small{and} \\
%	\vspace{0.03cm}
	\large{\textbf{Dr. Bivudutta Mishra}}\\
	\vspace{1.00cm} 
	%\large{\em{Co-Supervisor}}\\ 
	\vspace{0.05cm} 
	\large{\textbf{Dr. Pradyumn Kumar Sahoo}}\\
%	\small{Assistant Professor}\\
%	\small{Deaprtment of Physics}\\  
%	{Indira Gandhi Institute of Technology, Sarang}\\ 
%\[
%\begin{array}{cc}
%\centering
%\large{\textbf{Dr. Sukanta Das}} & \large{\textbf{Dr. Pradipta Maji}} \\
%\small{Asst. Professor} &  \small{Asst. Professor}\\
%\small{\textbf{Dept. of Information Technology}} & \small{\textbf{Machine Intelligence unit}}\\
%\small{\textbf{Indian Institute of Engineering Science And Technology,}} & \small{\textbf{Indian Statistical institute, Kolkata}}\\
%\small{\textbf{Shivpur}} & \small{\textbf{ }}\\\\\\\\\\
%\end{array}
%\]
       \vspace{0.4in} 
	\small{\textbf{Department of Mathematics}}\\ 
	\small{\textbf{Birla Institute of Technology and Science-Pilani, Hyderabad Campus}}\\
	\small{\textbf{(Hyderabad, Telangana-500078)}}\\
	%\small{\textbf{West Bengal, India -- 711103}}\\ 
        \vspace{0.12in} 
	%\small{\textbf{\thedate}}\\ 
	\end{center} 
\newpage 



==> Report_format_thesis/notation.tex <==
\textbf{Notation}
\\
$g^{ij}:$ \,\,\,\,\,\,\, Lorentzian Metric\\
$g:$ \,\,\,\,\,\,\, Determinant of $g^{ij}$\\
$\Gamma^{\lambda}_{ij}:$ \,\,\,\,\, General Affine Connection (Christoffel Symbols)\\
$\{\begin{array}{cl}
\lambda\\
ij \end{array}\}: $\,\,\,\, Levi-Civita connection\\
$\nabla_{i}$: \,\,\,\,\, Co-variant derivative w.r.t. Levi- Civita connection\\
$(ij):$ \,\,\,\, Symmetrization over the indices $i$ and $j$\\
$[ij]:$ \,\,\,\, Anti-symmetrization over the indices $i$ and $j$\\
$R^{\lambda}_{\sigma ij}:$ \,\,\,\, Riemann tensor of $g_{ij}$\\
$R_{ij}:$\,\,\,\,\, Ricci tensor of $g_{ij}$\\
$R:$ \,\,\,\,\,   Ricci scalar of $g_{ij}$\\
$S_{M}:$ \,\,\,\,\, Matter action\\
$T_{ij}:$ \,\,\,\, Stress-energy tensor\\
$ \Delta^{\lambda}_{ij}: $ \,\,\,\, Hypermomentum

==> Report_format_thesis/title.tex <==
\pagestyle{empty} 
	\begin{center} 
	\Large{\textbf{\textsf{{Investigation on late time dynamics of the universe along with anisotropic dark energy models }}}} \\
        \vspace{1.0cm} 
        \large{\textbf{Pratik Premdarshi Ray}}\\ 
        %\textbf{}\\                              
	\vspace{1.0cm}
        \small{\em{A thesis submitted to the Birla Institute of Technology and Science-Pilani for the award of the Degree of}}\\ 
	\vspace{0.16in} 
        \small{\textbf{Doctor of Philosophy}}\\ 
       % \small{{in }}\\ 
       % \small{\textbf{ Applied Physics}}\\ 
        \vspace{0.55in} 
        \begin{center}
        \includegraphics[scale=0.1]{logo}
        \end{center}
	\vspace{1.00cm} 
	\large{\em{Under the supervision of}}\\ 
	\vspace{0.10cm} 
%	\large{\textbf{Dr. Zashmir Naik}}\\ 
%	\small{Lecturer}\\
%	\small{School of Physics}\\
%	{Sambalpur University, Jyotivihar}\\
%	\vspace{0.03cm}
%	\small{and} \\
%	\vspace{0.03cm}
	\large{\textbf{Dr. Bivudutta Mishra}}\\
	\vspace{1.00cm} 
	\large{\em{Under the supervision of}}\\ 
	%\large{\em{Co-Supervisor}}\\ 
	\vspace{0.10cm} 
	\large{\textbf{Dr. Pradyumn Kumar Sahoo}}\\
%	\small{Assistant Professor}\\
%	\small{Deaprtment of Physics}\\  
%	{Indira Gandhi Institute of Technology, Sarang}\\ 
%\[
%\begin{array}{cc}
%\centering
%\large{\textbf{Dr. Sukanta Das}} & \large{\textbf{Dr. Pradipta Maji}} \\
%\small{Asst. Professor} &  \small{Asst. Professor}\\
%\small{\textbf{Dept. of Information Technology}} & \small{\textbf{Machine Intelligence unit}}\\
%\small{\textbf{Indian Institute of Engineering Science And Technology,}} & \small{\textbf{Indian Statistical institute, Kolkata}}\\
%\small{\textbf{Shivpur}} & \small{\textbf{ }}\\\\\\\\\\
%\end{array}
%\]
       \vspace{0.4in} 
	\small{\textbf{Department of Mathematics}}\\ 
	\small{\textbf{Birla Institute of Technology and Science-Pilani, Hyderabad Campus}}\\
	\small{\textbf{(Hyderabad, Telangana-500078)}}\\
	%\small{\textbf{West Bengal, India -- 711103}}\\ 
        \vspace{0.12in} 
	%\small{\textbf{\thedate}}\\ 
	\end{center} 

\newpage 


==> Thesis__Synopsis/1References.tex <==
\begin{thebibliography}{100}

%Chapter-1

\bibitem{Eddington/1920} F.W. Dyson, A.S. Eddington, C.R. Davidson, \textit{Phil. Trans. Roy. Soc. A} \textbf{220}, 291333 (1920).
\bibitem{Damour/1999} T. Damour, \textit{Einsteins Path}, Springer New York, 171-187 (1999).
\bibitem{Schwarzschild/1916a} K. Schwarzschild, \textit{Sitzungsber. Preuss. Akad. D. Wiss. Berlin (Math.Phys.)} \textbf{1916}, 189-196 (1916).
\bibitem{Schwarzschild/1916b} K. Schwarzschild, \textit{Sitzungsber. Preuss. Akad. D. Wiss. Berlin (Math.Phys.)} \textbf{1916}, 424-434 (1916).
\bibitem{Reissner/1916} H. Reissner, \textit{Annalen der Physik} \textbf{355} (9), 106120 (1916).
\bibitem{Nordstrom/1918} G. Nordstrom, \textit{Verhandl. Koninkl. Ned. Akad. Wetenschap.} \textbf{26}, 12381245 (1918).
\bibitem{Oppenheimer/1939} J. R. Oppenheimer, H. Snyder, \textit{Phys. Rev.} \textbf{56}, 455-459 (1939).


\bibitem{Weinberg/1989} S. Weinberg, \textit{Rev. Mod. Phys.} \textbf{61}, 1 (1989).

\bibitem{Velten/2014} H. E. S. Velten, R. F. Vom Marttens, W. Zimdahl, \textit{Eur. Phys. J. C} \textbf{74(11)}, 3160 (2014).

\bibitem{Weinberg/2013} D.H. Weinberg et al., \textit{Phys. Rep.}, \textbf{530(2)}, 87-255 (2013).
\bibitem{Valentino/2021} E. Di Valentino et al., \textit{Astropart. Phys.} \textbf{131}, 102605 (2021).
\bibitem{Riess/2019} A.G. Riess, \textit{Nature Rev. Phys.} \textbf{2(1)}, 10-12 (2019).

\bibitem{Ivanov/2020} M.M. Ivanov, M. Simonovic, M. Zaldarriaga,  J\textit{. Cosm. and Astropart. Phys.} \textbf{2020(05)}, 042 (2020).
\bibitem{Valentino/2021a} E. Di Valentino et al., \textit{Class. Quant. Grav.} \textbf{38(15)}, 153001 (2021).


\bibitem{Jimenez/2018} J. B. Jimenez, L. Heisenberg, T. Koivisto, \textit{Phys. Rev. D} \textbf{98(4)}, 044048 (2018).
% \bibitem{dm50c} C. L. Bennett et al., \textit{Astrophys. J. (supp.)}, \textbf{148}, 97 (2003).
% \bibitem{dm51c} E. Komatsu et al., \textit{Astrophys. J. (supp.)} \textbf{180}, 330 (2009).
% \bibitem{dm52c} M. Tegmark et al., \textit{Phys. Rev. D} \textbf{74}, 123507 (2006).
% \bibitem{dm53c} W. J. Percival et al., \textit{MNRAS} \textbf{381}, 1053 (2007).
% \bibitem{dm54c} E. Aubourg et al., \textit{Phys. Rev. D} \textbf{92}, 123516 (2015).
% \bibitem{dm55c} A. Cooray and R. Sheth, \textit{Phys. Reports} \textbf{372}, 1-129 (2002).
% \bibitem{dm56c} G. L. Bryan and M. L. Norman \textit{Astrophys. J.} \textbf{495}, 80-99 (1998).
% \bibitem{dm57c} A. F. Neto et al., \textit{MNRAS} \textbf{381}, 1450 (2007).
% \bibitem{dm58c} A. A. Dutton and A. V. Maccio, \textit{MNRAS} \textbf{441}, 3359 (2014).
% \bibitem{dm59c} A. D. Ludlow et al., \textit{MNRAS} \textbf{441}, 378 (2014).
% %NFW DM
% \bibitem{dm50} J. Dubinski and R. G. Carlberg, \textit{Astrophys. J.} \textbf{378}, 496 (1991).
% \bibitem{dm51}  L. Hernquis, \textit{Astrophys. J.} \textbf{356}, 359 (1990).
% \bibitem{dm52} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astrophys. J.} \textbf{462}, 563 (1996).
% \bibitem{dm53} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astrophys. J.} \textbf{490}, 493 (1997).
% \bibitem{dm54} D. Merritt et al., \textit{Astrophys. J.} \textbf{132}, 2685 (2006).
% \bibitem{dm55} J. Stadel et al., \textit{MNRAS} \textbf{398}, L21 (2009).
% \bibitem{dm56} J. F. Navarro et al., \textit{MNRAS} \textbf{402}, 21 (2010).
% \bibitem{dm57} J. Einasto, \textit{Trudy Astrofizicheskogo Instituta Alma-Ata} \textbf{5}, 87 (1965).
% \bibitem{dm58} D. Merritt et al., \textit{Astrophys. J.} \textbf{132}, 2685 (2006).
% \bibitem{dm59} A. A. Dutton and A. V. Maccio, \textit{MNRAS} \textbf{441}, 3359 (2014).
% %BEC DM
% \bibitem{dm60} S. J. Sin, \textit{Phys. Rev. D} \textbf{50}, 3650 (1994). 
% \bibitem{dm61} S. U. Ji and S. J. Sin, \textit{Phys. Rev. D} \textbf{50}, 3655 (1994).
% \bibitem{dm62} W. Hu, R. Barkana, and A. Gruzinov, \textit{Phys. Rev. Lett.} \textbf{85}, 1158 (2000).
% \bibitem{dm63} S. Khlebnikov, \textit{Phys. Rev. A} \textbf{66}, 063606 (2002).
% \bibitem{dm64} M. Nishiyama, M. Morita, and M. Morikawa, 	arXiv: astro-ph/0403571 (2004).
% \bibitem{dm65} F. Ferrer and J. A. Grifols, \textit{J. Cosmo. Astro. Phys.} \textbf{0412}, 012 (2004).
% \bibitem{dm66} J. A. Grifols, \textit{Astropart. Phys.} \textbf{25}, 98 (2006).
% \bibitem{dm67} C. G. Boehmer and T. Harko, \textit{JCAP} \textbf{0706}, 025 (2007).
% \bibitem{dm68} F. Dalfovo, S. Giorgini, L. P. Pitaevskii, and S. Stringari, \textit{Rev. Mod. Phys.} \textbf{71}, 463 (1999).
% \bibitem{dm69} T. Harko, P. Liang, S. D. Liang, and G. Mocanu, \textit{JCAP} \textbf{1511}, 027 (2015).
% \bibitem{Begeman} K. G. Begeman, A. H. Broeils, and R. H. Sanders, \textit{MNRAS} \textbf{249}, 523 (1991).
% \bibitem{Frenk4} W. J. G. de Blok, Stacy S. McGaugh, Albert Bosma, and Vera C. Rubin, \textit{Astrophys. J.} \textbf{552}, L23-L26 (2001).
% \bibitem{pi1} G. Gentile, P. Salucci, U. Klein, D. Vergani, and P. Kalberla, \textit{MNRAS} \textbf{351}, 903 (2004).
% \bibitem{pi2} S-H. Oh, W. J. G. de Blok, E. Brinks, F. Walter, and R. C. Kennicutt Jr, \textit{Astrono. J.} \textbf{141}, 193 (2011).
% \bibitem{pi3} Z. Xu, M. Tang, G. Cao, and S.-N. Zhang, \textit{Eur. Phys. J. C} \textbf{80}, 70 (2020).
% \bibitem{dm70} A. Burkert, \textit{Astrophys. J.} \textbf{447}, L25-L28, (1995).
% \bibitem{dm71} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{MNRAS} \textbf{275}, 720-740 (1995).
% \bibitem{dm72} M. Persic, P. Salucci, and F. Stel, \textit{MNRAS} \textbf{281}, 27 (1996).






% \bibitem{gr1}  T. P. Sotiriou, ``Modified Actions for Gravity: Theory and Phenomenology”, arXiv:gr-qc/0710.4438 (2007). 
% \bibitem{gr2} C. M. Will, ``Theory and Experiment in Gravitational Physics, revised edition", Cambridge University Press, Cambridge (1993).
% \bibitem{gr3} R. M. Wald, ``General Relativity", University of Chicago Press, United States of America (1984).
% \bibitem{gr4} A. Pais ``Subtle is the Lord: The Science and the Life of Albert Einstein”, Cambridge University Press (1982).
% \bibitem{gr5} W. Pauli, ``Theory of Relativity", Pergamon Press (1958).
% \bibitem{gr55} W. Rindler, ``Relativity: Special, General, and Cosmological", Second Edition, Oxford University Press (2006).
% \bibitem{gr6} K. S. Thorne and C. M. Will, \textit{Astrophys. J.} \textbf{163}, 595 (1971).
% \bibitem{gr7} V. A. Fock, ``The Theory of Space-Time and Gravitation", Pergamon Press, New York (1964).
% \bibitem{gr8} T. P. Sotiriou, V. Faraoni, and S. Liberati, \textit{Int. J. Mod. Phys. D} \textbf{17}, 399-423 (2008).
% \bibitem{otr1} R. D'Inverno, ``Introducing Einstein’s Relativity", Cambridge University Press, Cambridge (1998).
% % \bibitem{ot1} B. A. Dubrovin, A. T. Fomenko, and S. P. Novikov, ``Modern Geometry-Methods and Applications: Part I: The Geometry of Surfaces, Transformation Groups, and Fields", Second Edition, New York: Springer Verlag (1984).
% % \bibitem{ot2} L. D. Landau and E. M. Lifshitz, ``The Classical Theory of Fields", Amsterdam: Butterworth-Heinemann (1994).
% \bibitem{sp1} R. d'Inverno, ``Introducing Einstein’s Relativity", Clarendon Press (1992).
% \bibitem{sp2} C. W. Misner, K. S. Thorne, and J. A. Wheeler, ``Gravitation", W. H. Freeman and Co., San Francisco (1973).
% \bibitem{sp3} H. A. Buchdahl, \textit{MNRAS} \textbf{150}, 1-8 (1970).
% \bibitem{sp4} T. P. Sotiriou, V. Faraoni, and S. Liberati,
% \textit{Int. J. Mod. Phys. D} \textbf{17}, 399-423 (2008).
% \bibitem{sp5} J. M. Nester and H.-J. Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% \bibitem{sp6} J. B. Jimenez, L. Heisenberg, and T. S. Koivisto, \textit{Universe} \textbf{5}, 173 (2019).
% \bibitem{sp7} T. Padmanabhan, ``Theoretical Astrophysics: Volume 3, Galaxies and Cosmology", Theoretical Astrophysics Cambridge University Press (2000).
% \bibitem{sp8} V. Sahni and A. A. Starobinsky, \textit{Int. J. Mod. Phys. D} \textbf{9}, 373 (2000).
% \bibitem{Padmanabhan/2003}T. Padmanabhan, \textit{Phys. Rep.} \textbf{380}, 235 (2003).
% \bibitem{sp9} S. Weinberg, \textit{Rev. Mod. Phys.} \textbf{61}, 1-23 (1989).
% \bibitem{sp10} E. J. Copeland, M. Sami, and S. Tsujikawa, \textit{Int. J. Mod. Phys. D} \textbf{15}, 1753 (2006).
% \bibitem{sp11} L. Amendola and S. Tsujikawa, ``Dark Energy: Theory and Observations", Cambridge University Press (2015).
% \bibitem{sp12} L. Verde, T. Treu, and A. G. Riess, \textit{Nature Astron.} \textbf{3}, 891 (2019).
% \bibitem{sp13} A. G. Riess et al, \textit{Astrophys. J. Lett.} \textbf{934}, L7 (2022).
% \bibitem{sp14} E. Macaulay, I. K. Wehus, and H. K. Eriksen, \textit{Phys. Rev. Lett.} \textbf{111}, 161301 (2013).
% \bibitem{sp15} M. Asgari et al, (KiDS), \textit{Astron. Astrophys.} \textbf{645}, A104 (2021).
% \bibitem{sp16} E. Di Valentino \textit{et\,al.}, \textit{Class. Quant. Grav.} \textbf{38}, 153001 (2021),
% \bibitem{sp17}  S. Nojiri, S. D. Odintsov, and V. K. Oikonomou, \textit{Phys. Rept.} \textbf{692}, 1-104 (2017).

% \bibitem{mg1}  M. Ostrogradsky, \textit{Mem. Acad. St. Petersbourg} \textbf{6}, 385-517 (1850).
% \bibitem{mg2} Thomas P. Sotiriou and Valerio Faraoni, \textit{Rev. Mod. Phys.} \textbf{82}, 451-497 (2010).
% \bibitem{mg3} Th. Kaluza, \textit{Zum Unit atsproblem der Physik. Sitzungsber. Preuss. Akad. Wiss. Berlin} \textbf{1921}, 966-972 (1921).
% \bibitem{mg4} G. R. Dvali, Gregory Gabadadze, and Massimo Porrati, \textit{Phys. Lett. B} \textbf{485}, 208-214 (2000).
% \bibitem{mg5} Gabriel R. Bengochea and Rafael Ferraro, \textit{Phys. Rev. D} \textbf{79}, 124019 (2009).
% \bibitem{mg6} J. B. Jimenez, L. Heisenberg, and Tomi S. Koivisto, \textit{Universe} \textbf{5}, 173 (2019).
% \bibitem{mg7} T. Jacobson and D. Mattingly, \textit{Phys. Rev. D} \textbf{64}, 024028 (2001).
% \bibitem{mg8} S. Tsujikawa, \textit{Class. Quant. Grav.} \textbf{30}, 214003 (2013).
% \bibitem{mg9} M. Banados, \textit{Phys. Rev. D} \textbf{77}, 123534 (2008).








% \bibitem{sp18} R. P. Woodard, \textit{Lect. Notes Phys.} \textbf{720}, 403 (2007).
% \bibitem{sp19} A. A. Starobinsky, \textit{JETP Lett.} \textbf{86}, 157 (2007).
% \bibitem{sp20} A. A. Starobinsky, \textit{Phys. Lett. B} \textbf{91}, 99 (1980).
% \bibitem{sp21} Y. Akrami \textit{et\,al.} (Planck), \textit{Astron. Astrophys.} \textbf{641}, A10 (2020).
% \bibitem{sp22} W. Hu and I. Sawicki, \textit{Phys. Rev. D} \textbf{76}, 64004 (2007).
% \bibitem{sp23} S. Xavier, J. Mathew, and S. Shankaranarayanan, \textit{Class. Quant. Grav.} \textbf{37}, 225006 (2020).
% %STEGR
% \bibitem{fq0} Tomas Ortin, ``Gravity and strings", Cambridge Monographs on Mathematical Physics Cambridge Univ. Press (2004).
% \bibitem{fq00} James M. Nester and Hwei-Jang Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% \bibitem{fq000} Muzaffer Adak, M. Kalay, and Ozcan Sert, \textit{Int. J. Mod. Phys. D} \textbf{15}, 619-634 (2006).
% \bibitem{fq1} J. B. Jimenez, L. Heisenberg, and T. Kovisto, \textit{Phys. Rev. D} \textbf{98}, 044048 (2018).
% \bibitem{fq11} Igor Mol, \textit{Adv. Appl. Clifford Algebras} \textbf{27}, 2607-2638 (2017).
% \bibitem{fqt}Y. Xu et al.,	Eur. Phys. J. C \textbf{79}, 708 (2019).
% \bibitem{fq2} Avik De, Tee-How Loo, and Emmanuel N. Saridakis, \textit{JCAP} \textbf{03}, 050 (2024).
% %4D EGB
% \bibitem{egb1} D. Glavan and C. Lin, \textit{Phys. Rev. Lett.} \textbf{124}, 081301 (2020).
% \bibitem{egb2} D. Lovelock, \textit{J. Math. Phys.} \textbf{12}, 498 (1971).
% \bibitem{egb3} D. Lovelock, \textit{J. Math. Phys.} \textbf{13}, 874 (1972).
% \bibitem{egb4} T. Padmanabhan and D. Kothawala, \textit{Phys. Rep.} \textbf{531}, 115-171 (2013).
% \bibitem{egb6} C. Lanczos, \textit{Z. Phys.} \textbf{73}, 147-168 (1932).
% \bibitem{egb7} C. Lanczos, \textit{Ann. Math.} \textbf{39}, 842-850 (1938).
% \bibitem{egb5}  S. Chern, \textit{Ann. Math.} \textbf{46}, 674-84 (1945).
% %%%%%%%%%%%%%%%%%%%% END INTRODUCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-2 REFERENCES***********************************

% \bibitem{Laurentis} S. Capozziello and M. De Laurentis, \textit{Phys. Rept.} \textbf{509}, 167 (2011).
% \bibitem{Krssak} M. Krssak, R. J. van den Hoogen, J. G. Pereira, C. G. B\"ohmer, and A. A. Coley, \textit{Class. Quant. Grav.} \textbf{36}, 183001 (2019).
% \bibitem{Nester} James M. Nester and  Hwei-Jang Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% \bibitem{Kalay} M. Adak, M. Kalay, and O. Sert, \textit{Int. J. Mod. Phys.} \textbf{D15}, 619 (2006).
% \bibitem{Conroy} A. Conroy and T. Koivisto, \textit{Eur. Phys. J. C} \textbf{78}, 923 (2018).
% \bibitem{Jimenez} J. B. Jimenez, L. Heisenberg, and T. S. Koivisto, \textit{Phys. Rev. D} \textbf{98}, 044048 (2018).
% \bibitem{Soudi} I. Soudi, G. Farrugia, V. Gakis, J. L. Said, and E. N. Saridakis, \textit{Phys. Rev. D} \textbf{100}, 044008 (2019).
% \bibitem{Banos} R. Lazkoz, F. S. N. Lobo, M. O. Banos, and V. Salzano, \textit{Phys. Rev. D} \textbf{100}, 104027 (2019).
% \bibitem{Salzano} I. Ayuso, R. Lazkoz, and V. Salzano, \textit{Phys. Rev. D} \textbf{103}, 063505 (2021).
% \bibitem{Koivisto11} B. J. Barros, T. Barreiro, T. Koivisto, and N. J. Nunes, \textit{Phys. Dark Univ.} \textbf{30}, 100616 (2020).
% \bibitem{Anagnostopoulos} F. K. Anagnostopoulos, S. Basilakos, and E. N. Saridakis, \textit{Phys. Lett. B} \textbf{822}, 136634 (2021).
% \bibitem{Fell} F. D'Ambrosio, S. D. B. Fell, L. Heisenberg, and S. Kuhn \textit{Phys. Rev. D} \textbf{105}, 024042 (2022).
% \bibitem{Zhai} Rui-Hui Lin and Xiang-Hua Zhai, \textit{Phys. Rev. D} \textbf{103}, 124001 (2021).
% \bibitem{Wang2} W. Wang, H. Chen, and T. Katsuragawa, \textit{Phys. Rev. D} \textbf{105}, 024060 (2022).
% \bibitem{Calza} M. Calza and L. Sebastiani, \textit{Eur. Phys. J. C} \textbf{83}, 247 (2023).
% \bibitem{Moraes/2017} P. H. R. S. Moraes and P. K. Sahoo, \textit{Phys. Rev. D} \textbf{96}, 044038 (2017).
% \bibitem{Elizalde/2019} E. Elizalde and M. Khurshudyan, \textit{Int. J. Mod. Phys. D} \textbf{28}, 1950172 (2019).
% \bibitem{kimet/2018} Kimet Jusufi, \textit{Phys. Rev. D} \textbf{98}, 044016 (2018).
% \bibitem{Lobo/2005} F. S. N. Lobo, \textit{Phys. Rev. D} \textbf{71}, 084011 (2005).
% \bibitem{Francisco/2005} F. S. N. Lobo, \textit{Phys. Rev. D} \textbf{71}, 124022 (2005).
% \bibitem{Mauricio/2013} Mauricio Cataldo and Paola Meza, \textit{Phys. Rev. D} \textbf{87}, 064012 (2013).
% %\bibitem{Visser/2003} M. Visser, S. Kar, and N. Dadhich, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.90.201102}{\prl \,\ \textbf{90}, 201102 (2003)}.
% \bibitem{Newton/2020} Ksh. Newton Singh, Ayan Banerjee, Farook Rahaman, and M. K. Jasim, \textit{Phys. Rev. D} \textbf{101}, 084012 (2020).
% \bibitem{Visser/2003} M. Visser, S. Kar, and N. Dadhich, \textit{Phys. Rev. Lett.} \textbf{90}, 201102 (2003).
% \bibitem{Jusufi/2020} K. Jusufi, A. Banerjee, and S. G. Ghosh, \textit{Eur. Phys. J. C} \textbf{80}, 698 (2020).
% % \bibitem{Hassan1} Zinnat Hassan, Sanjay Mandal, P.K. Sahoo, \textit{Forts. Phys.} \textbf{69}, 2100023 (2021).
% % \bibitem{Mustafa} G. Mustafa, Z. Hassan, P.H.R.S. Moraes, P.K. Sahoo, \textit{Phys. Lett. B} \textbf{821}, 136612 (2021).
% % \bibitem{1} M. Calza and L. Sebastiani, \textit{arXiv}, arXiv:2208.13033 [gr-qc].
% % \bibitem{Sokoliuk} O. Sokoliuk, Z. Hassan, P.K. Sahoo, A. Baransky, \textit{Ann. Phys.} \textbf{443}, 168968 (2022).
% % \bibitem{Sahoo111} G. Mustafa, Z. Hassan, P. K. Sahoo, \textit{Ann. Phys.} \textbf{437}, 168751 (2022).
% % \bibitem{Hassan3} S. Mandal, G. Mustafa, Z. Hassan, P. K. Sahoo \textit{Phys. Dark Univ.} \textbf{35}, 100934 (2022)


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-3 REFERENCES*********(PLB paper)*****************************************

% % \bibitem{Jimenez/2018} J. B. Jim\'enez, L. Heisenberg, T. Koivisto, Phy. Rev. D, \textbf{98}, 044048 (2018).
% % \bibitem{maluf/2013} J. W. Maluf, \textit{Ann. Phys.} {\bf 525}, 339 (2013).
% % \bibitem{Ratanpal1} S.K. Maurya, B.S. Ratanpal, and M. Govender, \textit{Ann. Phys.} \textbf{382}, 36 (2017).
% % \bibitem{Ratanpal2} S. Gedela, R.K. Bisht, and N. Pant, Neeraj, \textit{Mod. Phys. Lett. A} \textbf{34}, 1950157 (2019).
% % \bibitem{Bhar1} P. Bhar, \textit{Eur. Phys. J. C} \textbf{79}, 138 (2019).
% % \bibitem{Bhar2} S. Gedela, R. K. Bisht, and N. Pant, \textit{Eur. Phys. J. A} \textbf{54}, 207 (2018).
% % %\bibitem{Bhar3} K. N. Singh, S. K. Maurya, and A. Errehymy, et al., \textit{Phys. Dark Univ.} \textbf{30}, 100620 (2020).
% % \bibitem{Hansraj} S. Hansraj and L. Moodly, \textit{Eur. Phys. J. C} \textbf{80}, 496 (2020).
% % \bibitem{Naidu1} N. F. Naidu, M. Govender, and S. D. Maharaj, \textit{Eur. Phys. J. C} \textbf{78}, 48 (2018).
% % \bibitem{Naidu2} J. Ospino and L. A. Nunez, \textit{Eur. Phys. J. C} \textbf{80}, 166 (2020).
% % \bibitem{Naidu3} S. C. Jaryal, \textit{Eur. Phys. J. C} \textbf{80}, 683 (2020).
% % \bibitem{Maurya4} S. K. Maurya, et al. \textit{Eur. Phys. J. C} \textbf{81}, 729 (2021).
% % \bibitem{Eiesland} J. Eiesland, \textit{Trans. Am. Math. Soc.} \textbf{27}, 213 (1925).
% % \bibitem{Eisenhart1} L. P. Eisenhart, \textit{Riemannian Geometry}, (Princeton University Press, Princeton, United States of America, 1966).
% % \bibitem{Karmarkar1} K. R. Karmarkar, \textit{Proc. Indian Acad. Sci. A} \textbf{27} 56 (1948).
% % \bibitem{Pandey1} S. N. Pandey and S. P. Sharma, \textit{Gen. Relativ. Gravit.} \textbf{14}, 113 (1981).
% % \bibitem{Gupta/1975} Y. K. Gupta, and M.P. Goel., \textit{Gen. Rel. Grav.} 6, 499 (1975).
% % \bibitem{Zia} M.F. Shamir and S. Zia, \textit{Astrophys. Space Sci.} \textbf{363}, 247 (2017).
% % \bibitem{Anchordoqui} L.A. Anchordoqui, D.F. Torres, M.L. Trobo, and S.E.P. Bergliaffa, \textit{Phys. Rev. D} \textbf{57}, 829 (1998).
% % \bibitem{Pavlovic/2015} P. Pavlovic, M. Sossich, \textit{Eur. Phys. J. C} \textbf{75}, 117 (2015).
% % \bibitem{Elizalde/2011} E. Elizalde, S. Nojiri, S.D. Odintsov, L. Sebastiani, S. Zerbini, \textit{Phys. Rev. D} \textbf{83}, 086006 (2011).
% % \bibitem{Tsujikawa/2008} S. Tsujikawa, \textit{Phys. Rev. D} \textbf{77}, 023507 (2008).

% % \bibitem{rahaman/2014} Farook Rahaman, P. K. F. Kuhfittig, Saibal Ray, and Nasarul Islam, {\it Eur. Phys. J. C} {\bf 74}, 2750 (2014).
% % \bibitem{ovgun/2016} A. {\" O}vg{\" u}n and M. Halilsoy, {\it Astrophys. Spa. Sci.} {\bf 361}, 214 (2016).
% % \bibitem{safonova/2002} Margarita Safonova, Diego F. Torres, and Gustavo E. Romero, {\it Phys. Rev. D} {\bf 65}, 023001 (2001).
% % \bibitem{bambi/2021} C. Bambi and D. Stojkovic, arXiv:2105.00881.

% % \bibitem{dai/2019} D.-C. Dai and D. Stojkovic, Phys. Rev. D {\bf 100}, 083513 (2019).
% % \bibitem{cramer/1995} J.G. Cramer et al., Phys. Rev. D {\bf 51}, 3117 (1995).
% % \bibitem{wang/2020} X. Wang et al., Phys. Lett. B {\bf 811}, 135930 (2020).
% % \bibitem{ohgami/2015} T. Ohgami and N. Sakai, Phys. Rev. D {\bf 91}, 124020 (2015).
% % \bibitem{torres/1998} D.F. Torres et al., Phys. Rev. D {\bf 58}, 123001 (1998).
% % \bibitem{shaikh/2018} R. Shaikh, Phys. Rev. D {\bf 98}, 024044 (2018).
% % \bibitem{nandi/2006} K.K. Nandi et al., Phys. Rev. D {\bf 74}, 024020 (2006).
% % \bibitem{jusufi/2018} K. Jusufi and A. \~A-vg\"{u}n, Phys. Rev. D {\bf 97}, 024042 (2018).
% % \bibitem{damour/2007} T. Damour and S.N. Solodukhin, Phys. Rev. D {\bf 76}, 024016 (2007).
% % \bibitem{Morris} M. S. Morris and K. S. Thorne, \textit{Am. J. Phys.} \textbf{56}, 395 (1988).
% % \bibitem{hawking/1973} S.W. Hawking and G.F.R. Ellis, The Large Scale Structure of Space-Time (Cambridge University Press, Cambridge, England, 1973).
% % \bibitem{visser/1995} M. Visser, Lorentzian Wormholes: from Einstein to Hawking (AIP Press, New York, United States of America, 1995).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-3 (GRG paper) REFERENCES***************************************************
% \bibitem{casimir}  H. B. G. Casimir,  D. Polder, \textit{Phys. Rev.} \textbf{73}, 360-372 (1948).
% \bibitem{lifshitz} I. E. Dzyaloshinskii, E. M. Lifshitz, and Lev P Pitaevskii,  \textit{Soviet Physics Uspekhi.} \textbf{4}, 153 (1961).
% \bibitem{experiment} S. K. Lamoreaux, \textit{ Phys. Rev. Lett.} \textbf{78}, 5-8 (1997).
% \bibitem{bressi} G. Bressi, G. Carugno, R. Onofrio, and G. Ruoso, \textit{Phys. Rev. Lett.} \textbf{88}, 041804 (2002).
% \bibitem{Garattini} R. Garattini, \textit{Eur. Phys. J. C} \textbf{79}, 951 (2019).
% \bibitem{rainbowsmolin}  J. Magueijo and L. Smolin, \textit{Class. Quant. Grav.} \textbf{21}, 1725 (2004).
% %\bibitem{sabinegup} S. Hossenfelder 
% %\textit{Living Rev. Relativity},\textbf{16}, 2, (2013).
% \bibitem{7} R. Garattini, \textit{Eur. Phys. J. C} \textbf{79}, 951 (2019).
% \bibitem{Channuie} D. Samart, T. Tangphati, and P. Channuie, \textit{Nucl. Phys. B} \textbf{980}, 115848 (2022).

% \bibitem{g1} M. Adak, O. Sert, M. Kalay, and M. Sari, \textit{Int. J. Mod. Phys. A} \textbf{28}, 1350167 (2013). 
% \bibitem{g2} M. Adak, M. Kalay, and O. Sert, \textit{Int. J. Mod. Phys. D} \textbf{15}, 619 (2006).
% \bibitem{g3} I. Mol, \textit{Adv. Appl. Clifford Algebras} \textbf{27}, 2607 (2017).
% \bibitem{g4} M. Krssak and E. N. Saridakis, \textit{Class. Quant. Grav.} \textbf{33}, 115009 (2016).
% \bibitem{rk} Rui-Hui Lin and Xiang-Hua Zhai, \textit{Phys. Rev. D} \textbf{103}, 124001 (2021).
% \bibitem{zee} A. Zee, ``Quantum Field Theory in a Nutshell", Second Edition, Princeton University Press (2010).
% \bibitem{paddy} T. Padmanabhan, ``Quantum Field Theory The Why, What and How", First Edition, Springer (2016).
% \bibitem{Bezerra} G. Alencar, V. B. Bezerra, and C. R. Muniz, \textit{Eur. Phys. J. C} \textbf{81}, 924 (2021).
% \bibitem{Fuenmayor} R. Avalos, E. Fuenmayor, and E. Contreras, \textit{Eur. Phys. J. C} \textbf{82}, 420 (2022).
% \bibitem{Khabibullin} A. R. Khabibullin et al., \textit{Class. Quant. Grav.} \textbf{23}, 627 (2006).
% %\bibitem{gupcasimir} A. M. Frassino, O. Panella, \textit{Phys. Rev. D}  \textbf{85} 045030 (2012).
% \bibitem{Solanki} R. Solanki, A. De, and P. K. Sahoo, \textit{Phys. Dark Univ.} \textbf{36}, 101053 (2022).
% \bibitem{Parbati} P. Sahoo, A. De, Tee-How Loo, and P. K. Sahoo, \textit{Comm. Theor. Phys.} \textbf{74}, 125402 (2022).
% \bibitem{Kazuharu} Z. Hassan, S. Ghosh, P. K. Sahoo, and K. Bamba, \textit{Eur. Phys. J. C} \textbf{82}, 1116 (2022).
% \bibitem{Visser} M. Visser, ``Lorentzian Wormholes: From Einstein to Hawking", First Edition, American Institute of Physics, New York
% (1996).
% \bibitem{Pradhan} A. Banerjee, A. Pradhan, T. Tangphati, and F. Rahaman, \textit{Eur. Phys. J. C} \textbf{81}, 1031 (2021).
% % \bibitem{adm0} R. M. Wald, \textit{General Relativity} (University of Chicago Press, Chicago, 1984).
% % \bibitem{adm1} R. Shaikh, \textit{Phys. Rev. D} \textbf{98}, 024044 (2018).
% % \bibitem{adm2} P. T. Chrusciel, Lectures on Energy in General Relativity, Krakow, 2010.
% %\bibitem{Visser3} M. Visser, S. Kar and N. Dadhich, \textit{Phys. Rev. Lett.} \textbf{90}, 201102 (2003).
% \bibitem{Channuie1} K. Jusufi, P. Channuie, and M. Jamil, \textit{Eur. Phys. J. C} \textbf{80}, 127 (2020).
% \bibitem{Baransky} O. Sokoliuk, S. Mandal, P. K. Sahoo, and A. Baransky, \textit{Eur. Phys. J. C} \textbf{82}, 280 (2022).
% % \bibitem{rainbowsmolin}  J. Magueijo, L. Smolin \textit{Class. Quantum Grav.} \textbf{21} 1725 (2004).
% % \bibitem{sabinegup} S. Hossenfelder 
% % \textit{Living Rev. Relativity},\textbf{16}, 2, (2013).
% \bibitem{regula} A. Kempf and G. Mangano  \textit{Phys. Rev. D} \textbf{55}, 7909 (1997).
% \bibitem{Tripathy} S. K. Tripathy, \textit{Phys. Dark Univ.} \textbf{31}, 100757 (2021).
% %\bibitem{Koivisto} J. B. Jimenez, L. Heisenberg, T. Koivisto, and S. Pekar, \textit{Phys. Rev. D} \textbf{101}, 103507 (2020).
% \bibitem{qedgup1} O. Panella, \textit{Phys. Rev. D} \textbf{76}, 045012 (2007).
% \bibitem{qedgup2} K. Nouicer, \textit{J. Phys. A} \textbf{38}, 10027 (2005).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-4 (CQG paper)*************************************************

% \bibitem{Rubin1} V. C. Rubin, W. K. Jr. Ford, and  N. Thonnard, \textit{Astrophys. J.} \textbf{238}, 471-487 (1980).
% \bibitem{Rubin2} F. Zwicky, \textit{Gen. Rel. Grav.} \textbf{41}, 207-224 (2009).
% \bibitem{Rubin3} P. A. R. Ade et al., \textit{Astron. Astrophys.} \textbf{594}, A13 (2016).
% \bibitem{Rahaman1} F. Rahaman, P. K. F. Kuhfittig, S. Ray, and N. Islam, \textit{Eur. Phys. J. C} \textbf{74}, 2750 (2014).
% \bibitem{Rahaman2} F. Rahaman, P. Salucci,  K. F. Kuhfittig, S. Ray, and  M. Rahaman, \textit{Ann. Phys.} \textbf{350}, 561 (2014).
% \bibitem{Rahaman3} J. F. Navarro, C. S. Frenk, and S. D. M. White,  \textit{Astrophys. J.} \textbf{462}, 563 (1996).
% \bibitem{Rahaman4} F. Rahaman, G. C. Shit, B. Sen, and S. Ray, \textit{Astrophys. Space Sci.} \textbf{361}, 37 (2016).
% \bibitem{Rahaman6} S. Islam, F. Rahaman, A. Ovgun, and M. Halilsoy,  \textit{Can. J. Phys.} \textbf{97}, 241 (2019).
% \bibitem{Rahaman5} P. Salucci and Ch. Frigerio Martins, \textit{EAS Publ. Ser.} \textbf{36}, 133 (2009).
% \bibitem{Jusufi1} K. Jusufi, M. Jamil, and M. Rizwan, \textit{Gen. Rel. Grav.} \textbf{51}, 102 (2019).
% \bibitem{Jusufi2} J. Einasto and U. Haud, \textit{Galaxy Astron. Astrophys.} \textbf{223}, 89 (1989).
% \bibitem{Jusufi3} K. G. Begeman, A. H. Broeils, and R. H. Sanders, \textit{MNRAS} \textbf{249}, 523 (1991).
% \bibitem{Milgrom1} M. Milgrom, \textit{Phys. Rev. Lett.} \textbf{117}, 141101 (2016).
% \bibitem{Milgrom2} M. Milgrom, \textit{Astrophys. J.} \textbf{270}, 365 (1983).
% \bibitem{Milgrom3} M. Milgrom, \textit{Astrophys. J.} \textbf{270}, 371 (1983).
% \bibitem{Milgrom4} B. C. Paul, \textit{Class. Quant. Grav.} \textbf{38}, 145022 (2021).
% \bibitem{sd1} J. L. Synge, \textit{MNRAS} \textbf{131}, 463 (1966).
% \bibitem{sd2} J. P. Luminet, \textit{Astron. Astrophys.} \textbf{75}, 228 (1979).
% \bibitem{sd3} H. Falcke, F. Melia, and E. Agol, \textit{Astrophys.  J.} \textbf{528}, L13 (2000).
% %\bibitem{sd4} V. Perlick and O. Y. Tsupko, \textit{Phys. Rep.} \textbf{947}, 1 (2022).
% \bibitem{sd5} K.  Akiyama et al., \textit{Astrophys.  J.} \textbf{875}, L1 (2019).
% \bibitem{sd6} K. Akiyama et al., \textit{Astrophys. J. Lett} \textbf{930}, L12 (2022).
% \bibitem{sd7} C. Bambi and K. Freese, \textit{Phys. Rev. D.} \textbf{79}, 043002 (2009).
% \bibitem{sd8} A. Abdujabbarov et al., \textit{Phys. Rev. D} \textbf{93}, 104004 (2016).
% \bibitem{sd9} X. Hou,  Z. Xu,  and  J. Wang, \textit{J.  Cosmo.  Astro.  Phys.} \textbf{2018}, 040 (2018).
% \bibitem{sd10} P. V. P. Cunha, N. A. Eiro, C. A. R. Herdeiro, and J. P. S. Lemos, \textit{J.  Cosmo.  Astro.  Phys.} \textbf{2020}, 035 (2020).
% \bibitem{sd11} M.  Afrin,  R.  Kumar,  and  S.  G.  Ghosh, \textit{MNRAS} \textbf{504}, 5927 (2020).
% % \bibitem{sd12} F.  Atamurotov,  U.  Papnoi,  and  K.  Jusufi, \textit{Class. Quant. Grav.} \textbf{39}, 025014 (2022).
% % \bibitem{sd13} X. Wang, P.-C. Li, C.-Y. Zhang, and M. Guo, \textit{Phys. Lett. B} \textbf{811}, 135930 (2020).
% % \bibitem{sd14} V. Perlick  and  O. Y. Tsupko, \textit{Phys. Rep.} \textbf{947}, 1 (2022).
% % \bibitem{sd15} M. Alloqulov et al., \textit{Chinese Phys. C} \textbf{48}, 025104 (2024).
% \bibitem{Einstein10} A. Einstein, \textit{Science} \textbf{84}, 506 (1936).
% \bibitem{Dyson} F. W. Dyson, A. S. Eddington, and C. Davidson, \textit{Philos. Trans. R. Soc. A} \textbf{220}, 291 (1920).
% \bibitem{Eddington} A. S. Eddington, ``Space, Time and Gravitation", Cambridge University Press, Cambridge, England (1920).
% \bibitem{Sahu} K. C. Sahu et al., \textit{Science} \textbf{356}, 1046 (2017).
% \bibitem{Bozza1} V. Bozza, S. Capozziello, G. Iovane, and G. Scarpetta , \textit{Gen. Rel. Grav.} \textbf{33}, 1535-1548 (2001).
% \bibitem{Virbhadra} K. S. Virbhadra and G. F. R. Ellis, \textit{Phys. Rev. D} \textbf{62}, 084003 (2000).
% \bibitem{Bozza22} V. Bozza, \textit{Phys. Rev. D} \textbf{66}, 103001 (2002).
% \bibitem{A1}  N. Tsukamoto,  \textit{Phys. Rev. D} \textbf{94}, 124001 (2016).
% \bibitem{A2} Y. Kumaran and A. Ovgun, \textit{Turk. J. Phys.} \textbf{45}, 247-267 (2021).
% \bibitem{A3} A. Ovgun, \textit{Turk. J. Phys.} \textbf{44}, 465-471 (2020).
% \bibitem{A4} W. Javed, R. Babar, and A. Ovgun, \textit{Phys. Rev. D} \textbf{99}, 084012 (2019).
% % \bibitem{A5} R. Shaikh and S. Kar, \textit{Phys. Rev. D} \textbf{96}, 044037 (2017).
% % \bibitem{A6} A. Ovgun, \textit{Phys. Rev. D} \textbf{98}, 044033 (2018).
% % \bibitem{A7} K. Jusufi and A. Ovgun, \textit{Phys. Rev. D} \textbf{97}, 024042 (2018).
% % \bibitem{A8} W. Javed et al, \textit{Eur. Phys. J. C} \textbf{82}, 1057 (2022).
% % \bibitem{A9}  S. N. Sajadi and N. Riazi, \textit{Can. J. Phys.} \textbf{98}, 1046-1054 (2020).
% % \bibitem{A10} W. Javed et al., \textit{Universe} \textbf{8}, 599 (2022).
% \bibitem{dz1} R. Ferraro and F. Fiorini, \textit{Phys. Rev. D} \textbf{84}, 083518 (2011).
% \bibitem{dz2} W. Wang, H. Chen, and T. Katsuragawa,  \textit{Phys. Rev. D} \textbf{105}, 024060 (2022).
% \bibitem{dz3} D. Zhao, \textit{Eur. Phys. J. C} \textbf{82}, 303 (2022).
% \bibitem{Hawking} S. W. Hawking and G. F. R. Ellis, ``The Large Scale Structure of Space-Time", Cambridge University Press, England (1973).
% \bibitem{Raychaudhuri} A. Raychaudhuri, \textit{Phys. Rev.} \textbf{98}, 1123 (1955).
% \bibitem{ws1} J. M. Bardeen, W. H. Press, and S. A. Teukolsky, \textit{Astrophys. J.} \textbf{178}, 347 (1972).
% \bibitem{ws2} K. Hioki and K.-ichi Maeda, \textit{Phys. Rev. D} \textbf{80}, 024042 (2009).
% \bibitem{ws3} S. E. Vazquez and E. P. Esteban, \textit{Nuovo Cimento B Serie} \textbf{119}, 489 (2004).
% \bibitem{ws4} P. G. Nedkova, V. Tinchev, and S. S. Yazadjiev,
% \textit{Phys. Rev. D} \textbf{88}, 124019 (2013).
% \bibitem{Virbhadra1} K. S. Virbhadra, D. Narasimha, and S. M. Chitre, \textit{Astron. Astrophys.} \textbf{337}, 1 (1998).
% %\bibitem{Virbhadra2} K. S. Virbhadra and G. F. R. Ellis, \textit{Phys. Rev. D} \textbf{62}, 084003 (2000).
% \bibitem{Virbhadra3} C. M. Claudel, K. S. Virbhadra, and G. F. R. Ellis, \textit{J. Math. Phys.} \textbf{42}, 818 (2001).
% %\bibitem{Bozza2} V. Bozza, \textit{Phys. Rev. D} \textbf{66}, 103001 (2002).
% \bibitem{Quinet} J. P. S. Lemos, F. S. N. Lobo, and S. Quinet de Oliveira, \textit{Phys. Rev. D} \textbf{68}, 064004 (2003).
% \bibitem{Tejeiro} J. M. Tejeiro and E. A. Larranaga, \textit{Rom. J. Phys.} \textbf{57}, 736 (2012).
% %\bibitem{g11} R. Shaikh, P. Banerjee, S. Paul, and T. Sarkar, \textit{JCAP} \textbf{07}, 028 (2019).
% \bibitem{r4} N. Godani and G. C. Samanta, \textit{Ann. Phys.} \textbf{429}, 168460 (2021).
% \bibitem{r1} R. Shaikh, P. Banerjee, S. Paul, and T. Sarkar, \textit{Phys. Lett. B} \textbf{789}, 270-275 (2019).
% \bibitem{r2} D. Samart, N. Autthisin, and P. Channuie, \textit{Anna. Physik} \textbf{535}, 2300039 (2023).
% \bibitem{r3} P. K. F. Kuhfittig, \textit{Eur. Phys. J. C} \textbf{74}, 2818 (2014).
% \bibitem{c1} F. Rahaman, G. C. Shit, B. Sen, and S. Ray, \textit{Astrophys. Space Sci.} \textbf{361}, 37 (2016).
% \bibitem{c2} F. Rahaman et al. \textit{Ann. Phys.} \textbf{350}, 561 (2014).
% %\bibitem{c3} K. Jusufi, M. Jamil, and M. Rizwan, \textit{Gen. Rel. Grav.} \textbf{51}, 102 (2019).
% \bibitem{c4} G. Mustafa, F. Atamurotov, and S. G. Ghosh, \textit{Phys. Dark Univ.} \textbf{40}, 101214 (2023).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-5 (ADP paper) REFERENCES***************************************************

% \bibitem{Zwiebach1} B. Zwiebach, \textit{Phys. Lett. B} \textbf{156}, 315 (1985).
% %\bibitem{Zwiebach2} M. J. Duff, B. E. W. Nilsson, and C. N. Pope, \textit{Phys. Lett. B} \textbf{173}, 69 (1986).
% \bibitem{Zwiebach3} D. J. Gross and J. H. Sloan, \textit{Nucl. Phys. B} \textbf{291}, 41 (1987).
% \bibitem{Zwiebach4} M.C. Bento and O. Bertolami, \textit{Phys. Lett. B} \textbf{368}, 198 (1996).
% %\bibitem{Lanczos} C. Lanczos, \textit{Ann. Math.} \textbf{39}, 842 (1938).
% \bibitem{Lovelock1} D. Lovelock, \textit{J. Math. Phys.} \textbf{12}, 498 (1971).
% \bibitem{Lovelock2} D. G. Boulware and S. Deser, \textit{Phys. Rev. Lett.} \textbf{55}, 2656 (1985).
% % \bibitem{Lovelock3} J. T. Wheeler, \textit{Nucl. Phys. B} \textbf{268}, 737 (1986).
% % \bibitem{Lovelock4} F. R. Tangherlini, \textit{Nuovo Cim.} \textbf{27}, 636 (1963).

% \bibitem{Lin1} D. Glavan and C. Lin, \textit{Phys. Rev. Lett.} \textbf{124}, 081301 (2020).
% \bibitem{Aoki1} K. Aoki, M.A. Gorji, and S. Mukohyama, \textit{Phys. Lett. B} \textbf{810}, 135843 (2020).
% \bibitem{Aoki2} K. Aoki, M.A. Gorji, and S. Mukohyama, \textit{J. Cosmo. Astro. Phys.} \textbf{2009}, 014 (2020).


% \bibitem{Lin2} R. A. Konoplya and A. Zhidenko, \textit{Phys. Dark Univ.} \textbf{30}, 100697 (2020).
% %\bibitem{Lin3} K. Hegde et al., \textit{arXiv} arXiv:2003.08778
% \bibitem{Lin4} C.-Y. Zhang, P.-C. Li, and M. Guo, \textit{Eur. Phys. J. C} \textbf{80}, 874 (2020).
% \bibitem{Lin5} H. Lu and Y. Pang, \textit{Phys. Lett. B} \textbf{809}, 135717 (2020).
% \bibitem{Lin6} M. S. Churilova, \textit{Phys. Dark Univ.} \textbf{31}, 100748 (2021).
% %\bibitem{Lin7} P. G. S. Fernandes, \textit{Phys. Lett. B} \textbf{805}, 135468 (2020).
% \bibitem{Lin8} D. V. Singh, S. G. Ghosh and S. D. Maharaj, \textit{Phys. Dark Univ.} \textbf{30}, 100730 (2020).
% \bibitem{Lin9} S. G. Ghosh and R. Kumar, \textit{Class. Quant. Grav.} \textbf{37}, 245008 (2020).
% \bibitem{Doneva1} D. D. Doneva and S. S. Yazadjiev, \textit{J. Cosmo. Astro. Phys.} \textbf{2021}, 024 (2021).
% \bibitem{Doneva2} R. A. Konoplya and A. Zhidenko, \textit{Phys. Rev. D} \textbf{102}, 064004 (2020).
% \bibitem{Doneva3} S.-W. Wei and Y.-X. Liu, \textit{Eur. Phys. J. Plus} \textbf{136}, 436 (2021).
% % \bibitem{Doneva4} R. Kumar and S. G. Ghosh, \textit{J. Cosmo. Astro. Phys.} \textbf{2020}, 053 (2020).
% % \bibitem{Doneva5} S. A. Hosseini Mansoori, \textit{Phys. Dark Univ.} \textbf{31}, 100776 (2021).
% \bibitem{Guo} M. Guo and P.-C. Li, \textit{Eur. Phys. J. C} \textbf{80}, 588 (2020).
% \bibitem{Mulryne} P. G. S. Fernandes, P. Carrilho, T. Clifton, and D. J. Mulryne, \textit{Class. Quantum Grav.} \textbf{39}, 063001 (2022).

% % \bibitem{Sisman} M. Gurses, T. C. Sisman, and B. Tekin, \textit{Eur. Phys. J. C} \textbf{80}, 647 (2020).
% % \bibitem{Carrilho1} Pedro G. S. Fernandes, P. Carrilho, T. Clifton, and D. J. Mulryne, \textit{Phys. Rev. D} \textbf{102}, 024025 (2020).
% % \bibitem{Carrilho2} R. A. Hennigar, D. Kubiznak, R. B. Mann, and C. Pollack, \textit{J. High Energ. Phys.} \textbf{2020}, 27 (2020).
% % \bibitem{Ai1} Wen Yuan Ai, \textit{Commun. Theor. Phys.} \textbf{72}, 095402 (2020).
% % \bibitem{Ai2} Fu-Wen Shu, \textit{Phys. Lett. B} \textbf{811}, 135907 (2020).
% % \bibitem{Ai3} S. Mahapatra, \textit{Eur. Phys. J. C} \textbf{80}, 992 (2020).
% % \bibitem{Ai4} J. Arrechea et al. \textit{Chinese Phys. C} \textbf{45} 013107 (2021).
% % \bibitem{Kobayashi1} T. Kobayashi, \textit{J. Cosmo. Astro. Phys.} \textbf{2020}, 013 (2020).
% % \bibitem{Kobayashi2} H. Lu and Yi Pang, \textit{Phys. Lett. B} \textbf{809}, 135717 (2020).
% % \bibitem{Kobayashi3} A. Casalino, A. Colleaux, M. Rinaldi, and S. Vicentini, \textit{Phys. Dark. Univ.} \textbf{31}, 100770 (2021).
% % \bibitem{Kobayashi4} L. Ma and H. Lu, \textit{Eur. Phys. J. C} \textbf{80}, 1209 (2020).

% \bibitem{Jusufi11} K. Jusufi, A. Banerjee, and S. G. Ghosh, \textit{Eur. Phys. J. C} \textbf{80}, 698 (2020).
% \bibitem{Jusufi22} N. Godani, D. V. Singh, G. C. Samanta, \textit{Phys. Dark Univ.} \textbf{35}, 100952 (2022).
% \bibitem{Jusufi33} Shweta, U. K. Sharma, and A. K. Mishra, \textit{Int. J. Geo. Mod. Phys.} \textbf{20} 2350140 (2023).
% \bibitem{Zwicky1} F. Zwicky, \textit{Helv. Phys. Acta} \textbf{6}, 110 (1933)
% \bibitem{Zwicky2} F. Zwicky, \textit{Astrophys. J.} \textbf{86}, 217 (1937).
% \bibitem{Oort1} J. Oort, \textit{Bull. Astron. Ins. Nether. V} \textbf{192} (1930).
% \bibitem{Oort2} J. Oort, \textit{Bull. Astron. Ins. Nether. V} \textbf{239} (1930).
% \bibitem{Diemand} J. Diemand et al., \textit{Nature} \textbf{454}, 735 (2008).
% \bibitem{Springel} V. Springel et al., \textit{MNRAS} \textbf{391}, 1685 (2008).
% %\bibitem{Pato} F. Iocco, M. Pato, G. Bertone, P. Jetzer, \textit{J. Cosmol. Astropart. Phys.} \textbf{2011}, 029 (2011).
% %\bibitem{Faber} T. Faber and M. Visser, \textit{MNRAS} \textbf{372}, 136 (2006).
% %\bibitem{Kalam} F. Rahaman, M. Kalam, A. DeBenedictis, A. Usmani, S. Ray, \textit{MNRAS} \textbf{389}, 27 (2008).
% %\bibitem{Filippov} K. K. Nandi, A. I. Filippov, F. Rahaman et al., \textit{MNRAS} 399, 2079 (2009).
% \bibitem{Rahaman66} F. Rahaman, G. C. Shit, B. Sen, S. Ray, \textit{Astrophys. Space Sci. }\textbf{361}, 37 (2016).
% \bibitem{Sarkar2} N. Sarkar, et al. \textit{Mod. Phys. Lett. A} \textbf{34}, 1950188 (2019).
% \bibitem{Rahaman8} P. K. F. Kuhfittig, \textit{Eur. Phys. J. C} \textbf{74}, 2818 (2014).

% \bibitem{Hennigar1} R. A. Hennigar, et al. \textit{J. High Energ. Phys.} \textbf{2020}, 27 (2020).
% \bibitem{Hennigar2} L. Ma and H. Lu, \textit{Eur. Phys. J. C} \textbf{80}, 1209 (2020).
% \bibitem{Hennigar3} A. casalino, et al. \textit{Phys. Dark Univ.} \textbf{31}, 100770 (2021).
% \bibitem{Eiesland} J. Eiesland, \textit{Trans. Am. Math. Soc.} \textbf{27}, 213 (1925).
% \bibitem{Eisenhart1} L. P. Eisenhart, \textit{Riemannian Geometry}, (Princeton University Press, Princeton, United States of America, 1966).
% \bibitem{Karmarkar1} K. R. Karmarkar, \textit{Proc. Indian Acad. Sci. A} \textbf{27} 56 (1948).
% \bibitem{Pandey1} S. N. Pandey and S. P. Sharma, \textit{Gen. Rel. Grav.} \textbf{14}, 113 (1981).
% \bibitem{Islam1} P. K. F. Kuhfittig, \textit{Eur. Phys. J. C} \textbf{ 74}, 2818 (2014).
% \bibitem{Islam3} F. Rahaman, P. Salucci, P. K. F. Kuhfittig, S. Ray, and M. Rahaman, \textit{Ann. Phys. }\textbf{350}, 561 (2014).
% \bibitem{Oort4} J. H.  Oort, \textit{Bull. Astro. Inst. Nether.} \textbf{3}, 275 (1927).
% \bibitem{Frenk2} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astro. J.}, \textbf{462}, 563 (1996).
% \bibitem{Frenk3} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astro. J.}, \textbf{490}, 493 (1997).
% \bibitem{Frenk44} D. Merritt et al., \textit{Astrophys. J.} \textbf{624}, L85 (2005).
% \bibitem{Frenk5} D. Merritt et al., \textit{Astrono. J.} \textbf{132}, 2685 (2006).
% \bibitem{Rizwan1} K. Jusufi, M. Jamil, and M. Rizwan, \textit{Gen. Rel. Grav.} \textbf{51}, 102 (2019).
% \bibitem{Rizwan2} Z. Xu, M. Tang, G. Cao, and S.-N. Zhang, \textit{Eur. Phys. J. C} \textbf{80}, 70 (2020).
% \bibitem{Rizwan4} G. Mustafa, S. K. Maurya, and S. Ray, \textit{Astrophys. J.} \textbf{941}, 170 (2022).
% % \bibitem{Burkertt} A. Burkert, \textit{Astro. J} \textbf{447}, L25-L28, (1995).
% % \bibitem{Stel} M. Persic, P. Salucci, F. Stel, \textit{MNRAS} \textbf{281}, 27 (1996).
% % \bibitem{Carlberg} J. Dubinski and R. G. Carlberg, \textit{Astro. J.} \textbf{378}, 496 (1991).
% \bibitem{Matos1} L. A. Urena-Lopez, T. Matos and R. Becerril, \textit{Class. Quant. Grav.} \textbf{19}, 6259 (2002).
% \bibitem{Matos2} T. Harko, \textit{J. Cosmo. Astro. Phys.} \textbf{05}, 022 (2011).
% % \bibitem{Hou1} X. Hou et al., \textit{J. Cosmo. Astro. Phys.} \textbf{2018}, 015 (2018).
% % \bibitem{Hou2} Z. Xu et al., \textit{J. Cosmo. Astro. Phys.} \textbf{2018}, 038(2018).
% \bibitem{Liempi1} M. Cataldo, L. Liempi, and P. Rodriguez, \textit{Phys. Lett. B} \textbf{757}, 130-135 (2016).
% \bibitem{Liempi2} F. S. N. Lobo, \textit{Phys. Rev. D} \textbf{71}, 084011 (2005).
% \bibitem{Liempi3} A. S. Nezhada, M. R. Mehdizadehb, and H. Golchin, \textit{Eur. Phys. J. Plus} \textbf{139}, 110 (2024).






% \bibitem{Sahdev} Kar and Sahdev, \textit{Phys. Rev. D} \textbf{52}, 2030 (1995).
% \bibitem{Anchordoqui} L. A. Anchordoqui et al., \textit{Phys. Rev. D} \textbf{57}, 829 (1998).
% \bibitem{Fayyaz1} M. F. Shamir and I. Fayyaz, \textit{Eur. Phys. J. C} \textbf{80}, 1102 (2020).
% \bibitem{Fayyaz2} A. Malik et al. \textit{Eur. Phys. J. C} \textbf{83}, 522 (2023).
% %\bibitem{Mustafa} G. Mustafa et al. \textit{Phys. Lett. B} \textbf{821}, 136612 (2021).
% \bibitem{Sarkar} S. Sarkar, N. Sarkar, and F. Rahaman \textit{Eur. Phys. J. C} \textbf{80}, 882 (2020).
% % \bibitem{Channuie11} K. Jusufi, P. Channuie, and M. Jamil, \textit{Eur. Phys. J. C} \textbf{80}, 127 (2020).
% % \bibitem{Hassan2} Z. Hassan, S. Ghosh, P. K. Sahoo, and V. S. Hari Rao, \textit{Gen. Relativ. Gravit.} \textbf{55}, 90 (2023).
% \bibitem{L. Herrera} L. Herrera, \textit{Phys. Rev. D} \textbf{97}, 044010 (2018).
% \bibitem{Gomez1} Alfonso Garcia-Parrado Gomez-Lobo, \textit{Class. Quantum Grav.} \textbf{25}, 015006 (2008).
% \bibitem{Gomez2} L. Herrera et al.,  \textit{Phys. Rev. D} \textbf{79}, 064025 (2009).
% \bibitem{Casadio1} R. Casadio et al., \textit{Eur. Phys. J. C} \textbf{79}, 826 (2019).
% \bibitem{Casadio2} E. Contreras and E. Fuenmayor, \textit{Phys. Rev. D} \textbf{103}, 124065 (2021).
% \bibitem{Casadio3} C. Arias, E. Contreras, E. Fuenmayor, and A. Ramos,\textit{ Ann. Phys.} \textbf{436}, 168671 (2022).
% %\bibitem{} R. Avalos, E. Fuenmayor, and E. Contreras, \textit{Eur. Phys. J. C} \textbf{82}, 420  (2022).
% \bibitem{Butt1} M. Sharif and I. I. Butt, \textit{Eur. Phys. J. C} \textbf{78}, 688 (2018).
% \bibitem{Butt2} Z. Yousaf, M. Yu. Khlopov, M. Z. Bhatti, and T. Naseer, \textit{MNRAS}  \textbf{495}, 4334-4346 (2020).
% \bibitem{Butt3} M. Zubair and M. Farooq, \textit{Eur. Phys. J. C} \textbf{83}, 507 (2023).
% \bibitem{Katz1} D. Lynden-Bell, J. Katz, J. Bicak, \textit{Phys. Rev. D} \textbf{75}, 024040 (2007).
% \bibitem{Katz2} K. K. Nandi, Y. Z. Zhang, R. G. Cai, and A. Panchenko, \textit{Phys. Rev. D} \textbf{79}, 024011 (2009).
% \bibitem{A. Wheeler} C. W. Misner, K. S. Thorne, and J. A. Wheeler, \textit{Gravitation} (Freeman, San Francisco, 1973), pp. 467 and 603.
% \bibitem{Manna1} P. Bhar, F. Rahaman, T. Manna, and A. Banerjee, \textit{Eur. Phys. J. C} \textbf{76}, 708 (2016).
% \bibitem{Manna2} F. Rahaman, S. Karmakar, I. Karar, and S. Ray, \textit{Phys. Lett. B} \textbf{746}, 73-78 (2015).
% \bibitem{Manna3} O. Sokoliuk, S. Mandal, P. K. Sahoo, and A. Baransky, \textit{Eur. Phys. J. C} \textbf{82}, 280 (2022).
% \bibitem{Rahaman7} F. Rahaman, P. K. F. Kuhfitting, S. Ray, and N. Islam, \textit{Eur. Phys. J. C} \textbf{74}, 2750 (2014).
% \bibitem{Atamurotov} G. Mustafa, F. Atamurotov, and Sushant G. Ghosh, \textit{Phys. Dark Univ.} \textbf{40}, 101214 (2023).
% \bibitem{Rizwan3} B. C. Paul, \textit{Class. Quant. Grav.} \textbf{38} 145022 (2021).
% %\bibitem{Sahoo} M. Tayde, Z. Hassan, and P. K. Sahoo, \textit{Nucl. Phys. B} \textbf{1000}, 116478 (2024).















































% % \bibitem{einstein} A. Einstein, Sitzungsber. Preuss. Akad. Wiss. Berlin (Math.Phys.) \textbf{1917}, 142 (1917).

% % \bibitem{desitter}W. de Sitter, Philosophical Problems in Science \textbf{63}, 205 (2017).

% % \bibitem{desitter2}W. de Sitter, MNRAS, \textbf{78}, 3 (1917).

% % \bibitem{friedman}A. Friedman, Zeitschrift für Physik \textbf{10}, 377 (1922).

% % \bibitem{lemaitre} G. Lemaitre, MNRAS \textbf{91}, 483 (1931).

% % \bibitem{penzias} A. A. Penzias, R. W. Wilson, Astrophys. J. \textbf{142}, 419 (1965).

% % \bibitem{riess/1998}A. G. Riess et al., Astron. J. \textbf{116}, 1009 (1998).
 
% % \bibitem{perlmutter/1999} S. Perlmutter et al., ApJ. \textbf{517}, 565 (1999).

% % \bibitem{planck/2015}P. A. R. Ade et al., Astron. Astrophys. \textbf{594}, A13 (2015).

% % \bibitem{dub} B. A. Dubrovin, A. T. Fomenko, S. P. Novikov, \textit{Modern Geometry-Methods and Applications: Part I: The Geometry of Surfaces, Transformation Groups, and Fields}, 2nd edition, (New York: Springer Verlag).

% % \bibitem{lan} L. D. Landau, E. M. Lifshitz, The Classical Theory of Fields, (Amsterdam: Butterworth-Heinemann, 1994).

% % \bibitem{hehl/1976} W. Hehl, et al., Rev. Mod. Phys. \textbf{48}, 393 (1976).

% % \bibitem{maluf}J. W. Maluf, 
% % %“The teleparallel equivalent of general relativity”, 
% % Annalen Phys. \textbf{525}, 339 (2013).

% % \bibitem{Haghani} Z. Haghani et al.,
% % %“Weyl-Cartan-Weitzenboeck gravity as a generalization of teleparallel gravity,” 
% % JCAP \textbf{1210}, 061 (2012).

% % \bibitem{nester}J. M. Nester, H. J. Yo,
% % % “Symmetric teleparallel general relativity,”
% %   Chin. J. Phys. \textbf{37}, 113 (1999).
  
% % \bibitem{olmo} G. J. Olmo, Int. J. Mod. Phys. D \textbf{20}, 413 (2011).

% % \bibitem{heisenberg} L. Heisenberg, Phys. Rep. \textbf{796}, 1 (2019).

% % \bibitem{heisenberg1} J. Beltr\'an Jim\'enez, L. Heisenberg, T. S. Koivisto, Universe \textbf{5}, 173 (2019).

% % \bibitem{r/1923} R. Weitzenb$\ddot{o}$ck, \textit{Invariantentheorie}, Noordhoff, Gronningen (1923).
% % \bibitem{Hayashi/1979} K. Hayashi, T. Shirafuji, Phys. Rev. D \textbf{19}, 3524 (1979).
% % \bibitem{Arcos/2004} H. I. Arcos, J. G. Pereira, Int. J. Mod. Phys. D \textbf{13}, 2193 (2004).
% % \bibitem{Maluf/1994} J. W. Maluf, J. Math. Phys. \textbf{35}, 335 (1994).


% % \bibitem{robert}H. P. Robertson, Astrophys. J. \textbf{82}, 284 (1935).

% % \bibitem{walker} A. G. Walker, Proc. Lon. Math. Soc. \textbf{42}, 90127 (1937).

% % \bibitem{1}W. Hillebrandt, J. C. Niemeyer, Ann. Rev. Astron. Astrophys. \textbf{38}, 191 (2000).

% % \bibitem{2} B. Leibundgut et al., ApJ. \textbf{466}, L21  (1996). 

% % \bibitem{3} S. Perlmutter et al., ApJ. \textbf{483}, 565 (1997).

% % \bibitem{4} B. Leibundgut, Ann. Rev. Astron. Astrophys. \textbf{39}, 67 (2001). 

% % \bibitem{7}J. Frieman, M. Turner, D. Huterer, Ann. Rev. Astron. Astrophys. \textbf{46}, 385 (2008).

% % \bibitem{9} J. L. Tonry et al., ApJ. \textbf{594}, 1 (2003).

% % \bibitem{10} B. Barris et al., ApJ. \textbf{602}, 571 (2004).

% % \bibitem{19}J. A. Holtzman et al., AJ. \textbf{136}, 2306 (2008); R. Kessler et al., ApJS. \textbf{185},  32 (2009).

% % \bibitem{18}J. Leaman et al., arXiv:1006.4611; W. D. Li et al., arXiv:1006.4612; W. D. Li et al., arXiv:1006.4613.

% % \bibitem{17} G. Folatelli et al., AJ. \textbf{139}, 120 (2010); G. Folatelli et al., AJ. \textbf{139} , 519 (2010).

% % \bibitem{16} Y. Copin et al., New Astronomy Rev. \textbf{50}, 436 (2006); R. A. Scalzo et al., ApJ. \textbf{713}, 1073 (2009).

% % \bibitem{15}G. Miknaitis et al., ApJ. \textbf{666}, 674 (2007); W. M. Wood-Vasey et al., ApJ. \textbf{666}, 694 (2007).

% % \bibitem{1314}P. Astier et al., Astron. Astrophys. \textbf{447}, 31 (2006);S. Baumont et al., Astron. Astrophys. \textbf{491}, 567 (2008); N. Regnault et al., arXiv:0908.3808; J. Guy et al., arXiv:1010.4743.

% % \bibitem{1112} A. G. Riess et al., ApJ. \textbf{607} 665 (2004); A. G. Riess et al., ApJ. \textbf{659}, 98 (2007). 

% % \bibitem{37} A. A. Penzias, R. W. Wilson, ApJ. \textbf{142} 419 (1965).

% % \bibitem{38} R. A. Alpher, H. Bethe, G. Gamow, Phys. Rev. D \textbf{73}, 803 (1948). 

% % \bibitem{39}G. F. Smoot et al., ApJ. \textbf{396}, Ll  (1992); C. L. Bennett et al., ApJ. \textbf{396},  L7 (1992). 

% % \bibitem{40} A. D. Miller et al., ApJL. \textbf{524}, L1 (1999); P. de Bernardlis et al., Nature

% % (London) \textbf{404}, 955 (2000); S. Hanany et al., ApJL. \textbf{545} L5 (2000).

% % \bibitem{41} P. J. E. Peebles, J. T. Yu, ApJ. \textbf{162}, 815 (1970).

% % \bibitem{42} J. R. Bond, G. Efstathiou, ApJ. \textbf{285} L45 (1984).

% % \bibitem{WAMP} D. N. Spergel et al., ApJS \textbf{148}, 175 (2003); H. V. Peiris et al., ApJS \textbf{148}, 213 (2003); D. N. Spergel et al., ApJS \textbf{170}, 377 (2007); E. Komatsu et al., ApJS \textbf{180}, 330 (2009).

% % \bibitem{Planck/2011} Planck Collaboration: arXiv: 1101.2022, arXiv: 1101.2023, arXiv: 1101.2024.

% % \bibitem{62} J. Silk, ApJ \textbf{151}, 459 (1968).

% % \bibitem{69} A. Albrecht et al., arXiv:astro-ph/0609591; J. Guzik, G. Bernstein, R. E. Smith, MNRAS \textbf{375}, 1329 (2007); H. J. Seo, D. J. Eisenstein, ApJ. \textbf{665} 14 (2007); R. E. Smith, R. Scoccimarro, R. K. Sheth, Phys. Rev. D \textbf{77}, 043525 (2008). 

% % \bibitem{72} M. Colless et al., arXiv:astro-ph/0306581.

% % \bibitem{73} D. G. York et al., AJ. \textbf{120}, 1579 (2000);  M. Tegmark et al., Phys. Rev. D \textbf{74}, 123507 (2006).

% % \bibitem{75} http://www.sdss3.org/dr8/.

% % \bibitem{136} E. Hubble, M. L. Humason, ApJ. \textbf{74}, 43  (1931).

% % \bibitem{138}W. L. Freedman et al., ApJ. \textbf{533}, 47 (2001).

% % \bibitem{139} A. Sandage et al., ApJ. \textbf{653}, 843 (2006).

% % \bibitem{140} A. G. Riess et al., ApJ. \textbf{699}, 539 (2009).

% % \bibitem{141}A. G. Riess et al., ApJ. \textbf{730}, 119 (2011).

% % \bibitem{145} W. L. Freedman, B. F. Madore, Annu. Rev. Astro. Astrophys. \textbf{48}, 673 (2010).

% % \bibitem{perkin} Miao Li, Xiao-Dong Li, Shuang Wang, Yi Wang, \textit{Dark Energy}
% % (Peking University Press-World Scientific Advanced Physics Series, 2014).

% % \bibitem{carroll/1992}S. M. Carroll et al., Annu. Rev. Astron. Astrophys. \textbf{30}, 499 (1992).
% % \bibitem{Sahni/2000} V. Sahni, A. Starobinski, Int. J. Mod. Phys. D, \textbf{9}, 373 (2000).

% % \bibitem{joyce/2016} A. Joyce et al., Ann. Rev. Nucl. Part. Sci., \textbf{66}, 95 (2016).

% % \bibitem{baker/2019} T. Baker et al., Rev. Mod. Phys. \textbf{93}, 15003 (2021).

% % \bibitem{peracaula/2019}J. S. Peracaula et al., Astrophys. J., \textbf{886}, L6 (2019); Y. Yerramsetti, et al., Eur. Phys. J. C, \textbf{79}, 1020 (2020); D. Wang, Phys. Dark Universe, \textbf{28}, 100545 (2020); D. Wang et al., Eur. Phys. J. C, \textbf{79}, 211 (2019); S. Arora et al., Class. Quan. Grav., 37, 205022 (2020); S. Bhattacharjee, P. K. Sahoo, Phys. Dark Universe, \textbf{28}, 100537 (2010).



% % \bibitem{bud} H. A. Buchdahl, Mon. Not. Roy. Astro. Soc. \textbf{150}, 1 (1970).

% % \bibitem{fr} A. A. Starobinsky, Physics Letters B \textbf{91}, 99 ( 1980); S .G. Chaudhury et al., Mon. Not. Roy. Astro. Soc., \textbf{485}, 5693 ( 2019); S. D. Odintsov, V. K Oikonomou, Phys. Rev. D  \textbf{101}, 044009 (2020);  A. G. Suvorov, Phys. Rev. D \textbf{99}, 124026 (2019); M. Zhang,R. B. Mann, Physi. Rev. D \textbf{100}, 084061 (2019); A. V. Astashenok, S. D. Odintsov, Mon. Not. Roy. Astro. Soc.  \textbf{493}, 78 (2020); P. Feola et al. Physi. Rev.D \textbf{101}, 044037 (2020).

% % \bibitem{Harko/2011}T Harko  et al., Phys. Rev. D \textbf{84}, 024020 (2011).

% % \bibitem{fg} D. Lovelock, J. Math. Phys., \textbf{12}, 498 (1971).

% % \bibitem{frlm} T. Harko, F. S. N. Lobo, Eur. Phys. J. C \textbf{70}, 373 (2010). 

% % \bibitem{ft} R. Ferraro,  F. Fiorini, Phys. Rev. D \textbf{75}, 084031 (2007).

% % \bibitem{ftb}S. Bahamonde, C. G. Böhmer, , M. Wright, Phys. Rev. D \textbf{92}, 104042 (2015).

% % \bibitem{ftg}G. Kofinas , E. N. Saridakis, Phys. Rev. D \textbf{90}, 084044 (2014).

% % %Chapter 2

% % %\bibitem{observations} A. G. Riess et al., Astron. J. \textbf{116}, 1009
% % %(1998); S. Perlmutter et al., Astrophys. J. \textbf{517}, 565 (1999); P.
% % %deBernardis et al., Nature \textbf{404}, 955 (2000); S. Perlmutter et al.,
% % %Astrophys. J. \textbf{598}, 102 (2003); M. Colless et al., Mon. Not. R.
% % %Astron. Soc. \textbf{328}, 1039 (2001); M. Tegmark et al., Phys. Rev. D 
% % %\textbf{69}, 103501 (2004); S. Cole et al., MNRAS 
% % %\textbf{362}, 505 (2005); V.Springel et al., Nature (London) \textbf{440},
% % %1137 (2006); P. A. R. Ade et al., Astron. Astrophys. \textbf{571}, A16
% % %(2014); P. Astier et al., Astron. Astrophys. \textbf{447}, 31 (2006); A. G.
% % %Riess et al., Astrophys. J. \textbf{659}, 98 (2007); D. N. Spergel et al.,
% % %Astrophys. J. Suppl. Ser. \textbf{148}, 175 (2003); H. V. Peiris et al.,
% % %Astrophys. J. Suppl. Ser. \textbf{148}, 213 (2003); D. N. Spergel et al.,
% % %Astrophys. J. Suppl. Ser. \textbf{170}, 377 (2007); E. Komatsu et al.,
% % %arXiv:0803.0547.
% % %
% % %\bibitem{alternate} B. Ratra, P. J. E Peebles, Phys. Rev. D \textbf{37},
% % %3406 (1988); R. R. Caldwell et al., Phys. Rev. Lett. \textbf{80}, 1582 1988;
% % %C. Armendariz-Picon et al., Phys. Rev. D \textbf{63}, 103510 (2001); T.
% % %Buchert, Gen. Relativ. Gravit. \textbf{32}, 105 (2000); P. Hunt, S. Sarkar,
% % %MNRAS \textbf{401}, 547 (2010); K. Tomita, Mon. Not. R.
% % %Astron. Soc. \textbf{326}, 287 (2001); B. Pandey, MNRAS 
% % %\textbf{485}, L73 (2019); B. Pandey, MNRAS \textbf{471},
% % %L77 (2017); K. A. Milton, Gravit. Cosmol.\textbf{\ 9}, 66 (2003); D. Easson
% % %et al., Phys. Lett. B \textbf{696}, 273 (2011); D. Pav\'on , N. Radicella,
% % %Gen. Relativ. Gravit. \textbf{45}, 63 (2013); N. Radicella, D. Pav\'on, Gen.
% % %Relativ. Gravit. \textbf{44}, 685 (2012).
% % %

% % %
% % %\bibitem{review} S. Nojiri et al., Phys. Rept. \textbf{692}, 1 (2017).
% % %\bibitem{snehasish}  P.K. Sahoo and S. Bhattacharjee, New Astronomy, \textbf{77}, 101351 (2020); R. Zaregonbadi, et al., Phys. Rev. D \textbf{94}, 084052 (2016); G. Sun and Y.-C. Huang, Int. J. Mod. Phys. D, \textbf{25}, 1650038 (2016); F. Rocha et al. arXiv:1911.08894 (2019); S.I. dos Santos, G.A. Carvalho, P.H.R.S. Moraes, C.H. Lenzi and M. Malheiro, Eur. Phys. J. Plus, \textbf{134}, 398 (2019); P.H.R.S. Moraes, J.D.V. Arban˜il and M. Malheiro, J. Cosm. Astrop. Phys. \textbf{06}, 005 (2016); P.H.R.S. Moraes and P.K. Sahoo, Eur. Phys. J. C \textbf{79}, 677 (2019); E. Elizalde and M. Khurshudyan, Phys. Rev. D, \textbf{99}, 024051 (2019); P.H.R.S. Moraes, W. de Paula and R.A.C. Correa, Int. J. Mod. Phys. D, \textbf{28}, 1950098 (2019); E. Elizalde and M. Khurshudyan, Phys. Rev. D, \textbf{98}, 123525 (2018); P.H.R.S. Moraes and P.K. Sahoo, Phys. Rev. D, \textbf{97}, 024007 (2018); P.K. Sahoo, P.H.R.S. Moraes and P. Sahoo, Eur. Phys. J. C, \textbf{78}, 46 (2018); P.K. Sahoo, P.H.R.S. Moraes, P. Sahoo and G. Ribeiro, Int. J. Mod. Phys. D, \textbf{27}, 1950004 (2018); P.H.R.S. Moraes and P.K. Sahoo, Phys. Rev. D, \textbf{96}, 044038 (2017); P.H.R.S. Moraes, R.A.C. Correa and R.V. Lobato, J. Cosm. Astrop. Phys., \textbf{07}, 029 (2017); T. Azizi, Int. J. Theor. Phys. \textbf{52}, 3486 (2013); M. Sharif and A. Siddiqa, Gen. Rel. Grav., \textbf{51}, 74 (2019);  M.E.S. Alves, P.H.R.S. Moraes, J.C.N. de Araujo and M. Malheiro, Phys. Rev. D, \textbf{94}, 024032 (2016); P.K. Sahoo and S. Bhattacharjee, Int. J. Theor. Phys, DOI: 10.1007/s10773-020-04414-3 [arXiv: 1907.13460]; S. Bhattacharjee and P. K. Sahoo, Eur. Phys. J. C. \textbf{80}, 289 (2020) [arXiv: 2002.11483]; 
% % % P. Sahoo et al, Mod. Phys. Lett. A, DOI: 10.1142/S0217732320500959 [arXiv: 1907.08682] ;S. Bhattacharjee and P. K. Sahoo, Phys. Dark. universe. \textbf{28}, 100537 (2020) [arXiv: 2003.14211]; S. Bhattacharjee and P. K. Sahoo, Eur. Phys. J. Plus, \textbf{135}, 86 (2020) [arXiv:2001.06569]; S. Bhattacharjee and P. K. Sahoo, Eur. Phys. J. Plus, DOI: 10.1140/epjp/s13360-020-00361-4.
% % \bibitem{cosmo7to9} G. R. Bengochea, R. Ferraro, Phys. Rev. D \textbf{79},
% % 124019 (2009); R. Ferraro, F. Fiorini, Phys. Rev. D \textbf{75}, 084031
% % (2007); E. V. Linder, Phys. Rev. D \textbf{81}, 127301 (2010).

% % \bibitem{reviewft} Y. F. Cai et al., Rept. Prog. Phys. \textbf{79},
% % 106901 (2016).

% % \bibitem{cosmoft} A. Paliathanasis et al., Phys. Rev. D \textbf{94}, 023525 (2016).

% % \bibitem{cosmo10to12} K. Hayashi, T. Shirafuji, Phys. Rev. D \textbf{19},
% % 3524 (1979); M. Tsamparlis, Phys. Lett. A \textbf{75}, 27 (1979); H. I.
% % Arcos, J.G. Pereira, Int. J. Mod. Phys. D \textbf{13}, 2193 (2004).

% % \bibitem{cosmo14} A. Einstein 1928, Sitz. Preuss. Akad. Wiss. p. 217; ibid
% % p. 224 [Translated by A. Unzicker, T. Case, (preprint: arXiv:
% % physics/0503046)]

% % \bibitem{cosmo19to20} K. Atazadeh, F. Darabi, Eur. Phys. J. C \textbf{72},
% % 2016 (2012); S. Basilakos et al., Phys. Rev. D \textbf{88}, 103526 (2013).

% % \bibitem{cosmo21} M. E. Rodrigues et al., Astroph. Space Sci. \textbf{357},
% % 129 (2015)

% % \bibitem{cosmo22to23} A. Paliathanasis et al., Phys. Rev. D \textbf{89},
% % 104042 (2014); S. Capozziello et al., JHEP \textbf{89}, 039 (2013).


% % \bibitem{inflation} K. Bamba et al., Phys. Rev. D \textbf{94}, 083513 (2016).

% % \bibitem{late} G. R. Bengochea, R. Ferraro, Phys. Rev. D \textbf{79}, 124019
% % (2009); K. Bamba et al., JCAP \textbf{01}, 021 (2011); R. Myrzakulov, Eur.
% % Phys. J. C \textbf{71}, 1752 (2011).

% % \bibitem{bounce} Y.F. Cai et al., Class. Quant. Grav. \textbf{28}, 215011
% % (2011); J. de Haro, J. Amor\'os, J. Phys. Conf. Ser. \textbf{600}, 012024
% % (2015); W. El Hanafy, G.
% % G. L. Nashed, Int. J. Mod. Phys. D \textbf{26}, 1750154 (2017).

% % \bibitem{bhatti/2017} M. Zaeem-ul-Haq Bhatti, Z.Yousaf, Sonia Hanif, Phys.
% % Dark Univ.,\textbf{16}, 34 (2017).

% % \bibitem{bhatti/2017a} M. Zaeem-ul-Haq Bhatti, Z.Yousaf, Sonia Hanif, Mod.
% % Phys. Lett. A, \textbf{32}, 1750042 (2017).

% % \bibitem{pacif} S. K. J. Pacif et al., Int. J. Geom. Meth. Mod. Phys. 
% % \textbf{14}, 1750111 (2017).

% % \bibitem{para} M. Chevallier, D. Polarski, Int. J. Mod. Phys. D \textbf{10},
% % 213 (2001); Mod. Phys. Lett. A. \textbf{35}, 2050011 (2020); S. del Campo et
% % al., Phys. Rev. D \textbf{86}, 083509 (2012); A. A. Mamon, K.Bamba, Eur.
% % Phys. J. C \textbf{78}, 862 (2018).

% % \bibitem{banerjee} N. Banerjee, S. Das, Gen. Relativ. Gravit. \textbf{37},
% % 1695 (2005).

% % \bibitem{olive21} S. Pan, A.Mukherjee, N.Banerjee, MNRAS 
% % \textbf{477}, 1189 (2018).

% % \bibitem{sahni} V. Sahni, T. D. Saini, A. A. Starobinsky, U. Alam: JETP
% % Lett. \textbf{77}, 201 (2003); U. Alam et al., MNRAS 
% % \textbf{344}, 1057 (2003).

% % \bibitem{sahni17to18} J. Albert et al. [SNAP Collaboration]: arXiv:0507458;
% % J. Albert et al. [SNAP Collaboration]: arXiv:0507459.

% % \bibitem{Omsahni} V. Sahni et al., Phys. Rev. D. \textbf{78}, 103502 (2008);
% % M. Shahalam1, Sasha Sami, Abhineet Agarwal, MNRAS 
% % \textbf{448} 2948 (2015); Abhineet Agarwal et al., Int. J. Mod. Phys. D %
% % \textbf{28} 1950083 (2019).

% % \bibitem{sahoo} P. H. R. S. Moraes, P. K. Sahoo, Eur. Phys. J. C. \textbf{77}%
% % , 480 (2017).

% % \bibitem{non39} R. M. Wald, General relativity (University of Chicago Press,
% % Chicago, 1984)

% % \bibitem{Poisson/2004} A. Raychaudhuri, Phys. Rev., \textbf{98} (1955) 1123; J.~Ehlers, Int. J. Mod. Phys. D,  \textbf{15}, 1573 (2006); S. Nojiri, S. D. Odintsov, Int. J. Geom. Methods Mod. Phys., \textbf{4}, 115 (2007).

% % \bibitem{energy} D. Liu, M. J. Reboucas, Phys.Rev. D. \textbf{86}, 083515
% % (2012); T. Azizi, M. Gorjizadeh, EPL \textbf{117}, 6 (2017);M. Zubair, Saira
% % Waheed, Astrophys Space Sci. \textbf{355}, 361 (2015).

% % \bibitem{sharov} G. S. Sharov, V. O. Vasiliev, Mathematical Modelling and
% % Geometry \textbf{6}, 1 (2018).

% % \bibitem{Hz1} C. H. Chuang, Y. Wang, MNRAS \textbf{435}%
% % , 255 (2013); C-H Chuang C-H. et al., MNRAS \textbf{433%
% % }, 3559 (2013); A. Font-Ribera et al., J. Cosmol. Astropart. Phys. \textbf{05%
% % }, 027 (2014); T. Delubac et al., Astron. Astrophys. \textbf{574}, id. A59,
% % 17 (2015); L.,erson et al., MNRAS \textbf{441}, 24
% % (2014); Y. Wang et al., MNRAS \textbf{469}, 3762
% % (2017); E. Gaztanaga et al. MNRAS \textbf{399}, 1663
% % (2009); C. Blake et al., MNRAS \textbf{425}, 405
% % (2012); N. G. Busca et al., Astro. Astrophys. \textbf{552}, A96 (2013); A.
% % Oka et al., MNRAS \textbf{439}, 2515 (2014); S. Alam
% % et al., MNRAS \textbf{470}, 2617 (2017); J. E.
% % Bautista et al., Astron. Astrophys. \textbf{603}, A12 (2017).

% % \bibitem{Hz2} J. Simon, L. Verde, R. Jimenez, Phys. Rev. D \textbf{71},
% % 123001 (2005); D. Stern et al., J. Cosmol. Astropart. Phys. \textbf{02}, 008
% % (2010); C. Zhang et al., Research in Astron. and Astrop. \textbf{14}, 1221
% % (2014); M. Moresco et al., J. Cosmol. Astropart. Phys. \textbf{8}, 006
% % (2012); M. Moresco, MNRAS: Letters., \textbf{450}, L16
% % (2015); M. Moresco M. et al., J. Cosmol. Astropart. Phys. \textbf{05}, 014
% % (2016); A. L. Ratsimbazafy et al., MNRAS \textbf{467},
% % 3239 (2017)

% % \bibitem{SNeIa} N. Suzuki et al., ApJ., \textbf{746}, 85 (2012).

% % \bibitem{padn} N. Padmanabhan, X. Xu, D. J. Eisenstein, R. Scalzo, A. J.
% % Cuesta, K. T. Mehta et al., MNRAS \textbf{427},
% % 2132 (2012).

% % \bibitem{6df} F. Beutler et al., MNRAS \textbf{416}, 3017 (2011).

% % \bibitem{boss} BOSS collaboration, L. Anderson et al., Mon. Not. Roy.
% % Astron. Soc. \textbf{441}, 24 (2014).

% % \bibitem{wig} C. Blake et al., MNRAS \textbf{425}, 405 (2012).

% % %\bibitem{adep} Ade P A R et al., Planck 2015 results. XIII. Cosmological
% % %parameters, Preprint arXiv:1502.01589 (2015)

% % \bibitem{waga} M. Vargas dos Santos, Ribamar R. R. Reis, J. Cosm. Astropart.
% % Phys., \textbf{1602}, 066 (2016).

% % \bibitem{gio} R. Giostri, M. V. d. Santos, I. Waga, R. R. R. Reis, M. O.
% % Calvao, B. L. Lago, JCAP \textbf{1203}, 027 (2012).

% % \bibitem{hing} G. Hinshaw et al., Astrophys. J. Suppl., \textbf{208},
% % 19 (2013).

% % \bibitem{non41to42} M. Visser, C. Barcelo. arXiv:gr-qc/0001099; C. Barcelo,
% % M. Visser, Int. J. Mod. Phys. D \textbf{11}, 1553 (2002).

% % \bibitem{Planck/2018} Planck Collaboration: arXiv:1807.06209.

% % \bibitem{Jaime/2019} B. S. Haridasu, V. V. Lukovic, M. Moresco, N. Vittorio,
% % J. Cosmol. Astropart. Phys. \textbf{10}, 015 (2018); J. R. Garza et al.,
% % Eur. Phys. J. C \textbf{79}, 890 (2019); Hai-Nan Lin, Xin Li, Li Tang, Chin.
% % Phys. C \textbf{43}, 075101 (2019); J. F. Jesus, R. Valentim, A. A. Escobal,
% % S. H. Pereira, arXiv: 1909.00090. 


% % %Chapter-3

% % %\bibitem{Capozziello_book} S. Capozziello, and V. Faraoni, \textit{Beyond Einstein Gravity: A Survey of Gravitational Theories for Cosmology and Astrophysics}, Springer Dordrecht, 2011. doi: 10.1007/978-94-007-0165-6.
% % %\bibitem{lv_papers} B. P. Abbott et al. (LIGO Scientific Collaboration and Virgo Collaboration), {\it Phys. Rev. Lett.}, {\bf 116} (2016) 061102; B. P. Abbott et al. (LIGO Scientific Collaboration and Virgo Collaboration),{\it Phys. Rev. Lett.},  {\bf 119} (2017) 161101; B. P. Abbott et al. (LIGO Scientific Collaboration and Virgo Collaboration), {\it Phys. Rev. Lett.},  {\bf 123} (2019) 011102.
% % %\bibitem{eht_papers} The Event Horizon Telescope Collaboration et al., {\it ApJL},  {\bf 875} (2019) L1; The Event Horizon Telescope Collaboration et al., {\it ApJL},  {\bf 875} (2019) L5. 

% % \bibitem{Lazkoz/2019} R. Lazkoz et al.,  Phys. Rev. D, {\bf 100}, 104027  (2019). 
% % \bibitem{Capozziello/2018} S. Capozziello et al., Phys. Lett. B, {\bf 781}, 99  (2018).

% % %\bibitem{Plank/2018} Planck Collaboration, arXiv:1807.06209.
% % \bibitem{Capozziello/2019} S. Capozziello et al., Int. J. Mod. Phys. D, \textbf{28}, 1930016 (2019). 
% % \bibitem{Riess/1998} A. G. Riess, et al., Astro. J., \textbf{116}, 1009 (1998); S. Perlmutter, et al., Astrophys. J., \textbf{517} 565 (1999); S. Perlmutter, et al., Astrophys. J., \textbf{598}  102 (2003); S. Cole, et al., Mon. N. Roy. Astro. Soc., \textbf{362}, 505 (2005); P. A. R. Ade, et al., Astron. Astrophys., \textbf{571}, A16 (2014). 
% % \bibitem{Santos/2007} J. Santos, et al., Phys. Rev. D, \textbf{76}, 083513  (2007).
% % \bibitem{Bertolami/2009} O. Bertolami, M. C. Sequeira, Phys. Rev. D, \textbf{79}, 104010 (2009).
% % \bibitem{Gracia/2011} N. M. Gracia et al., Phys. Rev. D, \textbf{83}, 104032  (2011).
% % \bibitem{Bamba/2017} K Bamba et al., Gen. Rel. Grav.,  \textbf{49}, 112 (2017).
% % \bibitem{Liu/2012} D. Liu, M. J. Rebouc,  Phys. Rev. D, \textbf{86}, 083515 (2012).
% % \bibitem{Sharif/2016} M. Sharif, A. Ikram, Eur. Phys. J. C, \textbf{76}, 640 (2016).
% % \bibitem{Sharif/2013} M. Sharif, M. Zubair, J. High Energy Physics, \textbf{2013}, 79 (2013).
% % \bibitem{Atazadeh/2014} K. Atazadeh, F. Darabi, Gen. Rel. Grav.,  \textbf{46}, 1664 (2014).
% % \bibitem{Yousaf/2018} Z. Yousaf et al. Int. J. Geom. Methods Mod. Phys.,  \textbf{15}, 1850146 (2018).
% % \bibitem{Moraes/2019} P.H.R.S. Moraes et al. Adv. Astron.,  \textbf{2019}, 8574798 (2019).
% % \bibitem{Harko/2018}T. Harko, et al., Phys. Rev. D, \textbf{98}, 084043 (2018). 
% % \bibitem{Visser/2000} M. Visser, C. Barcelo, COSMO-99, 98 (2000).
% % %\bibitem{Moraes/2017} P.H.R.S. Moraes, P.K. Sahoo, Eur. Phys. J. C, \textbf{77} 480 (2017).
% % \bibitem{Whinnett/2004} A. W. Whinnett, D. F. Torres, Astrophys. J., {\bf 603}, L133  (2004).
% % \bibitem{Calcagni_book} G. Calcagni, \textit{Classical and Quantum Cosmology}, Springer Switzerland, 2017.

% % %Chapter-4

% % %\bibitem{riess/1998} A. G. Riess, et al., \textit{Astron. J.} \textbf{116}, 1009 (1998);  S. Perlmutter, et al., \textit{Astrophys. J.} \textbf{517}, 565 (1999); S. Perlmutter, et al., \textit{Astrophys. J.} \textbf{598}, 102 (2003);  D. N. Spergel,  et al.,  \textit{Astrophys. J. Suppl. Ser.} \textbf{148}, 175 (2003); A. G. Riess, et al., \textit{Astrophys. J.} \textbf{659}, 98 (2007);  D. N. Spergel,  et al.,  \textit{Astrophys. J. Suppl. Ser.} \textbf{170}, 377 (2007).
% % %
% % %\bibitem{carroll/1992}S. M. Carroll et al., \textit{Annu. Rev. Astron. Astrophys.} \textbf{30}, 499 (1992); V. Sahni, A. Starobinski, \ijmpd, \textbf{9}, 373 (2000).
% % %
% % %\bibitem{yang/2010}R. J. Yang, S. N. Zhang, \mnras,  \textbf{407}, 1835 (2010).
% % %
% % %\bibitem{veltan/2014} H. E. S. Velten ey al., Eur. Phys. J. C, \textbf{74}, 3160 (2014).
% % %
% % %\bibitem{joyce/2016} A. Joyce et al., \textit{Ann. Rev. Nucl. Part. Sci.}, \textbf{66}, 95 (2016).
% % %
% % %\bibitem{baker/2019} T. Baker et al., (2019), arXiv:1908.03430.
% % %
% % %\bibitem{peracaula/2019}J. S. Peracaula et al., \textit{Astrophys. J.}, \textbf{886}, L6 (2019); S. Mandal et al., \textit{Phys. Dark Universe}, \textbf{28}, 100551 (2020); Y. Yerramsetti, et al., Eur. Phys. J. C, \textbf{79}, 1020 (2020); D. Wang, \textit{Phys. Dark Universe}, \textbf{28}, 100545 (2020); D. Wang et al., Eur. Phys. J. C, \textbf{79}, 211 (2019); S. Arora et al., \cqg, 37, 205022 (2020); S. Bhattacharjee and P. K. Sahoo, \textit{Phys. Dark Universe}, \textbf{28}, 100537 (2010).
% % %
% % %\bibitem{hehl/1995}F. W. Hehl et al., \textit{Phys. Rep.} \textbf{258}, 1 (1995); T. Ortin, \textit{Gravity and Strings} (Cambridge University Press, Cambridge, England, 2015).
% % %
% % %\bibitem{aldrovandi/2014}R. Aldrovandi and J. Pereira, \textit{Teleparallel Gravity. An Introduction}, Fundamental Theories of Physics Vol. 173 (Springer, Dordrecht, 2014).
% % %
% % %\bibitem{maluf/2013}J. W. Maluf, \textit{Ann. Phys.}, \textbf{525}, 339 (2013).
% % %
% % %\bibitem{haghani/2012} Z. Haghani et al., \jcap, \textbf{10}, 061 (2012).
% % %
% % %\bibitem{haghani/2013}Z. Haghani et al., Phys. Rev. D, \textbf{88}, 044024 (2013).
% % %
% % %\bibitem{nester/1999}J. M. Nester and H.-J. Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% % %
% % %\bibitem{ferraro/2008}R. Ferraro and F. Fiorini, Phys. Rev. D, \textbf{78}, 124019 (2008); E. V. Linder, Phys. Rev. D, \textbf{81}, 127301 (2010); Y.-F. Cai et al., \textit{Rep. Prog. Phys.} \textbf{79}, 106901 (2016); C.-Q. Geng et al., \textit{Phys. Lett. B}, \textbf{704}, 384 (2011); L. Jarv and A. Toporensky, Phys. Rev. D, \textbf{93}, 024051 (2016); J. B. Jim´enez et al., Phys. Rev. D, \textbf{98}, 044048 (2018); A. Conroy and T. Koivisto, Eur. Phys. J. C, \textbf{78}, 923 (2018).
% % %
% % %\bibitem{jarv/2018} L. J\"arv et al., Phys. Rev. D, \textbf{97}, 124025 (2018).
% % %
% % %\bibitem{hehl/1976} F. W. Hehl, et al., \textit{Rev. Mod. Phys.}, \textbf{48}, 393 (1976).

% % %\bibitem{Lazkoz/2019}R. Lazkoz et al.,Phys. Rev. D, \textbf{100}, 104027 (2019).

% % \bibitem{Mandal/2020} S. Mandal, P.K. Sahoo, J.R.L. Santos, Phys. Rev. D, \textbf{102}, 024057  (2020).

% % \bibitem{jianbo/2019} J. Lu et al., Eur. Phys. J. C, \textbf{79}, 530 (2019).

% % \bibitem{mikhel/2018} M. R\"unkla, O. Vilson, Phys. Rev. D, 98, 084034 (2018).

% % \bibitem{viktor/2020}V. Gakis, et al., Phys. Rev. D, \textbf{101}, 064024 (2020).

% % %\bibitem{Harko/2018} T. Harko, et al., Phys. Rev. D, \textbf{98}, 084043 (2018).

% % \bibitem{olmo/2015} G. J. Olmo, D. Rubiera-Garcia, Phys. Lett. B, \textbf{740}, 73 (2015).

% % \bibitem{einstein/1916}A. Einstein, Hamiltonsches Prinzip und allgemeine Relativit\"atstheorie, K\"oniglich Preu$\mathcal{B}$ische, Akademie der Wissenschaften (Berlin), Sitzungsberichte (1916), pp. 1111-1116.



% % %\bibitem{Jimenez/2018} J. B. Jim\'enez, L. Heisenberg, T. Koivisto, Phys. Rev. D, 
% % %\textbf{98}, 044048 (2018).

% % \bibitem{tomi/2018} T. Koivisto, Int. J. Geom. Methods Mod. Phys., \textbf{15}, 1840006 (2018).

% % \bibitem{Cattoen/2008}C. Cattoen, M. Visser, Phys. Rev. D, \textbf{78}, 063501 (2008); A. Aviles, et al., Phys. Rev. D, \textbf{87}, 044012 (2013); A. Aviles, et al., Phys. Rev. D, \textbf{86}, 123516 (2012); S. Capozziello, et al., Phys. Rev. D, \textbf{78}, 063504 (2008). 

% % \bibitem{will/2006}C. M. Will, Living Rev. Relativity, \textbf{9}, 3 (2006).


% % \bibitem{Scolnic/2018} D.~M.~Scolnic {\it et al.}, Astrophys.\ J.\  {\bf 859}, 101 (2018).

% % \bibitem{hobson/2009} M. P. Hobson, A. H. Jaffe, A. R. Liddle, P. Mukherjee, D.Parkison, \textit{Bayesian Methods in Cosmology}, (Cambridge University Press, Cambridge, 2009).

% % %Chapter-5







% % %\bibitem{Harko_2011} T. Harko et al., \textit{Phys. Rev. D}, {\bf 84}  (2011) 024020.

% % \bibitem{Ray_1955} A. Raychaudhuri, Phys. Rev., {\bf 98}, 1123 (1955).


% % \bibitem{Carroll_2004} S. Carroll, Spacetime and Geometry, An Introduction to GR (Addison Wesley, Boston 2004).

% % \bibitem{Hawking_1973} S.W. Hawking, G. F. R Ellis, The Large Scale Structure of Spacetime (Cambridge Univ Press, Cambridge 1973).

% % \bibitem{Bamba_2017} K. Bamba et al., Gen. Relativ. Gravit., {\bf 49}, 112 (2017).

% % \bibitem{Capo_2018} S. Capozziello et al., Phys. Lett. B, {\bf 781}, 99 (2018).

% % \bibitem{Atazadeh_2014} K. Atazadeh, F. Darabi, Gen. Relativ. Gravit., {\bf 46}, 1664 (2014).

% % \bibitem{Zubair_2015} M. Zubair, S. Waheed, Astrophys. Space. Sci., {\bf 355}, 361 (2015).

% % %\bibitem{Planck} Planck Collaboration, arXiv:1807.06209.

% % %\bibitem{Poisson/2004}  J.~Ehlers, Int. J. Modern Phys. D,  \textbf{15} (2006) 1573; S. Nojiri, S. D. Odintsov, \textit{Int. J. Geom. Methods Mod. Phys.}, \textbf{4} (2007) 115.

% % %\bibitem{Capozziello/2019} S. Capozziello et al., Int. J. Modern Phys. D, \textbf{28} (2019) 1930016.





% % %Chapter-6
% % %\bibitem{Capo/2011} S. Capozziello, M. De Laurentis, \href{https://www.sciencedirect.com/science/article/pii/S0370157311002432}{Phys. Rep. \textbf{509}, 167 (2011)}.
% % %
% % %\bibitem{Sari} E. N. Saridakis, et al., CANTATA, \href{https://arxiv.org/abs/2105.12582}{arXiv:2015.12582}.

% % %\bibitem{Jimenez/2018} J. B. Jimenez, L. Heisenberg, and T. Koivisto, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.98.044048}{Phys. Rev. D \,\ \textbf{98}, 044048 (2018)}.

% % %\bibitem{Lazkoz/2019} R. Lazkoz et al,, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.100.104027}{Phys. Rev. D \,\ \textbf{100}, 104027 (2019)}.

% % %\bibitem{Mandal/2020} S. Mandal, P.K. Sahoo, J.R.L. Santos, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.102.024057}{Phys. Rev. D \,\ \textbf{102}, 024057 (2020)}.

% % \bibitem{Mandal/2020a}S. Mandal, D. Wang, P.K. Sahoo, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.102.124029}{Phys. Rev. D \,\ \textbf{102}, 124029 (2020)}.

% % %\bibitem{Harko/2018}T. Harko et al,, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.98.084043}{Phys. Rev. D \,\ \textbf{98}, 084043 (2018)}.

% % \bibitem{Barros/2020} B. J. Barros et al., \href{https://www.sciencedirect.com/science/article/pii/S2212686420302387?via\%3Dihub}{Phys. Dark Universe \textbf{30}, 100616 (2020)}.
 
% % \bibitem{Jimenez/2020} J. B. Jimenez et al,, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.101.103507}{Phys. Rev. D \,\ \textbf{101}, 103507 (2020)}.

% % \bibitem{Hasan/2021}Z. Hasan, S. Mandal, P.K. Sahoo, \href{https://onlinelibrary.wiley.com/doi/10.1002/prop.202100023}{Fortschritte der Physik \textbf{69}, 2100023 (2021)}.

% % \bibitem{Solanki/2021}R. Solanki et al., \href{https://www.sciencedirect.com/science/article/pii/S2212686421000510?via\%3Dihub}{Phys. Dark Universe \textbf{32}, 100820 (2021)}.

% % \bibitem{Frus/2021} N. Frusciante, \href{https://www.scopus.com/record/display.uri?eid=2-s2.0-85101007939&origin=inward}{Phys. Rev. D \,\ \textbf{103}, 044021 (2021)}.

% % \bibitem{Flat/2021} K. Flathmann, M. Hohmann, \href{https://www.scopus.com/record/display.uri?eid=2-s2.0-85100981932&origin=inward}{Phys. Rev. D \,\ \textbf{103}, 044030 (2021)}.

% % \bibitem{Khyllep/2021} W. Khyllep, A. Paliathanasis, J. Dutta, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.103.103521}{Phys. Rev. D \,\ \textbf{103}, 103521 (2021)}.

% % \bibitem{Anag/2021} F. K. Anagnostopoulos, S. Basilakos, E. N. Saridakis, \href{https://www.sciencedirect.com/science/article/pii/S0370269321005748?via\%3Dihub}{Phys. Lett. B \,\ \textbf{822}, 136634 (2021)}.

% % \bibitem{Ata/2021} L. Atayde, N. Frusciante, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.104.064052}{Phys. Rev. D \,\ \textbf{104}, 064052 (2021)}.

% % \bibitem{Dial/2019}K. F. Dialektopoulos, T. S. Koivisto, S. Capozziello, \href{https://link.springer.com/article/10.1140/epjc/s10052-019-7106-8}{Eur. Phys. J. C \,\ \textbf{79}, 606 (2019)}. 

% % \bibitem{Ayu/2021}I. Ayuso, R. Lazkoz, V. Salzano, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.103.063505}{Phys. Rev. D \,\ \textbf{103}, 063505 (2021)}.

% % \bibitem{Amb/2020}F. D'Ambrosio, M. Garg, L. Heisenberg, \href{https://www.sciencedirect.com/science/article/pii/S0370269320307735}{Phys. Lett. B \,\ \textbf{811}, 135970 (2020)}.

% %\bibitem{baye}\href{http://www.cambridge.org/us/catalogue/catalogue.asp?isbn=9780521887946}{Bayesian Methods in Cosmology, edited by M. P. Hobson, A. H. Jaffe, A. R. Liddle, P. Mukherjee, and D. Parkison (Cambridge University Press, Cambridge, England, 2009)}.

% %\bibitem{Sharov/2018} G. S. Sharov, V. O. Vasiliev, \href{https://mmg.tversu.ru/images/publications/2018-611-abstract-references.pdf}{Mathematical Modelling and Geometry, \textbf{6}, 1 (2018)}.
% %
% %\bibitem{BAO1} C. H. Chuang, Y. Wang,\href{https://doi.org/10.1093/mnras/stt1290}{MNRAS \,\ \textbf{435}, 255 (2013)}.
% %
% %\bibitem{BAO2} C-H Chuang C-H. et al., \href{https://doi.org/10.1093/mnras/stt988}{MNRAS \,\ \textbf{ 433}, 3559  (2013)};  
% % 
% % \bibitem{BAO3} T.  Delubac  et  al.,  \href{https://www.aanda.org/articles/aa/full_html/2015/02/aa23969-14/aa23969-14.html}{Astron. Astrophys. \,\ \textbf{574}, 17 (2015)}; 
% %  
% % \bibitem{BAO4}L. Anderson et al., \href{https://doi.org/10.1093/mnras/stu523}{MNRAS \,\ \textbf{441}, 24 (2014)}; 
% % 
% %  
% % \bibitem{BAO5}S. Alam et al., \href{https://doi.org/10.1093/mnras/stx721}{MNRAS \,\ \textbf{470}, 2617 (2017)}. 
% % 
% % \bibitem{h1} J. Simon, L. Verde, R. Jimenez, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.71.123001}{ Phys. Rev. D \,\ \textbf{71}, 123001 (2005)}.
% % 
% % \bibitem{h2}D. Stern et al., \href{https://iopscience.iop.org/article/10.1088/1475-7516/2010/02/008/meta}{JCAP \,\ \textbf{02}, 008 (2010)}.
% %  
% %\bibitem{h3}M. Moresco, \href{https://doi.org/10.1093/mnrasl/slv037}{MNRAS \,\ \textbf{450},  L16 (2015)}.
% %
% %\bibitem{h4} A. L. Ratsimbazafy et al., \href{https://doi.org/10.1093/mnras/stx301}{MNRAS \,\ \textbf{467}, 3239 (2017)}.

% %\bibitem{Scolnic/2018}D. M. Scolnic et al., \href{https://iopscience.iop.org/article/10.3847/1538-4357/aab9bb}{Astrophys. J. \,\ \textbf{859}, 101 (2018)}.

% %\bibitem{capo/2014} S. Capozziello et al., \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.90.044016}{Phys. Rev. D \,\ \textbf{90}, 044016 (2014)}.

% %\bibitem{capo/2019} S. Capozziello, R. D'Agostino, Orlando Luongo, \href{https://www.worldscientific.com/doi/abs/10.1142/S0218271819300167}{Int. J. Modern Phys. D \,\ \textbf{28}, 1930016 (2019).}

% %\bibitem{capo/2011} S. Capozziello et al., \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.84.043527}{Phys. Rev. D \,\ \textbf{84}, 043527 (2011)}.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\end{thebibliography}

==> Thesis__Synopsis/variables.tex <==
%-------------------------------------------------------------------------------
%	DOCUMENT VARIABLES
%
%	Fill in the lines below to set the various variables for the document
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
% Your thesis title - this is used in the title and abstract
% Command: \ttitle
\thesistitle{Accelerated Expansion of the Universe in Nonmetricity-based Modified Gravity}
%-------------------------------------------------------------------------------
% The document type: Thesis / report, etc.
% Command: \doctype
\documenttype{\textbf{SYNOPSIS}}
%-------------------------------------------------------------------------------
% Your supervisor's name - this is used in the title page
% Command: \supname
\supervisor{\textbf{Prof. Pradyumn Kumar Sahoo}}
%-------------------------------------------------------------------------------
% The supervisor's position - Used on Certificate
% Command: \suppos
\supervisorposition{\textbf{Professor}}
%-------------------------------------------------------------------------------
% Supervisor's institute
% Command: \supinst
\supervisorinstitute{\textbf{BITS-Pilani, Hyderabad Campus}}
%-------------------------------------------------------------------------------
% Your Co-Supervisor's name
% Command: \cosupname
%\cosupervisor{Dr. Pradyumn Kumar Sahoo}
%-------------------------------------------------------------------------------
% Co-Supervisor's Position - Used on Certificate
% Command: \cosuppos
%\cosupervisorposition{Associate Professor}
%-------------------------------------------------------------------------------
% Co-Supervisor's Institute
% Command: \cosupinst
%\cosupervisorinstitute{BITS-Pilani, Hyderabad Campus}
%-------------------------------------------------------------------------------
% Your Examiner's name. Not currently used anywhere.
% Command: \examname
\examiner{}
%-------------------------------------------------------------------------------
% Name of your degree
% Command: \degreename
\degree{Ph.D. Research Scholar}
%-------------------------------------------------------------------------------
% The BITS Course Code for which this report is written
% COmmand: \ccode
\coursecode{\textbf{DOCTOR OF PHILOSOPHY}}
%\coursecode{BITS C799T}
%-------------------------------------------------------------------------------
% The name of the Course
% Command: \cname
\coursename{Thesis}
%-------------------------------------------------------------------------------
% Your name. Extend manually in case of multiple authors
% Command: \authornames
\authors{\textbf{GAURAV NARAYANRAO GADBAIL}}
%-------------------------------------------------------------------------------
% Your ID Number - used on the Title page and abstract
% Command: \idnum
\IDNumber{\textbf{2020PHXF0401H}}
%-------------------------------------------------------------------------------
% Your address
% Command: \addressnames
\addresses{}
%-------------------------------------------------------------------------------
% Your subject area
% Command: \subjectname
\subject{}
%-------------------------------------------------------------------------------
% Keywords for this report.
% Command: \keywordnames
\keywords{}
%-------------------------------------------------------------------------------
% University details
% Command: \univname
\university{\texorpdfstring{\href{http://www.bits-pilani.ac.in/} % URL
                {\textbf{Birla Institute of Technology and Science, Pilani}}} % University name
                {\textbf{Birla Institute of Technology and Science, Pilani}}}
%-------------------------------------------------------------------------------
% University details, in Capitals
% Command: \UNIVNAME
\UNIVERSITY{\texorpdfstring{\href{http://www.bits-pilani.ac.in/} % URL
                {\textbf{BIRLA INSTITUTE OF TECHNOLOGY AND SCIENCE, PILANI}}} % name in capitals
                {\textbf{BIRLA INSTITUTE OF TECHNOLOGY AND SCIENCE, PILANI}}}

%-------------------------------------------------------------------------------
% Campus Name
% Command: \campusname
%\campus{Hyderabad Campus}

%-------------------------------------------------------------------------------
% Campus Name, in capitals
% Command: \CAMPUSNAME
%\CAMPUS{HYDERABAD CAMPUS}


%-------------------------------------------------------------------------------
% Department Details
% Command: \deptname
\department{\texorpdfstring{\href{http://www.bits-pilani.ac.in/pilani/Mathematics/Mathematics} % Your department's URL
                {Mathematics}} % Your department's name
                {Mathematics}}
%-------------------------------------------------------------------------------
% Department details, in Capitals
% Command: \DEPTNAME
\DEPARTMENT{\texorpdfstring{\href{http://www.bits-pilani.ac.in/pilani/Mathematics/Mathematics} % Your department's URL
                {Mathematics}} % Your department's name in capitals
                {Mathematics}}
%-------------------------------------------------------------------------------
% Research Group Details
% Command: \groupname
\group{\texorpdfstring{\href{Research Group Web Site URL Here (include http://)}
                {Research Group Name}} % Your research group's name
                {Research Group Name}}
%-------------------------------------------------------------------------------
% Research Group Details, in Capitals
% Command: \GROUPNAME
\GROUP{\texorpdfstring{\href{Research Group Web Site URL Here (include http://)}
                {RESEARCH GROUP NAME (IN BLOCK CAPITALS)}}
                {RESEARCH GROUP NAME (IN BLOCK CAPITALS)}}
%-------------------------------------------------------------------------------
% Faculty details
% Command: \facname
\faculty{\texorpdfstring{\href{Faculty Web Site URL Here (include http://)}
                {Faculty Name}}
                {Faculty Name}}
%-------------------------------------------------------------------------------
% Faculty details, in Capitals
% Command: \FACNAME
\FACULTY{\texorpdfstring{\href{Faculty Web Site URL Here (include http://)}
                {FACULTY NAME (IN BLOCK CAPITALS)}}
                {FACULTY NAME (IN BLOCK CAPITALS)}}
%-------------------------------------------------------------------------------



==> declaration.tex <==
\noindent
\textbf{{\Huge \bfseries declaration}}

\vspace{1cm}

\noindent
I, \textbf{Nakidi Shravani}, declare that this thesis titled, ``\emph{A Posteriori} Error Analysis of Parabolic Partial Differential Equation with Small Random Input Data" and the work presented in it are my own. I confirm that:
	\begin{itemize}
		\item This work was done wholly or mainly while in candidature for a research degree at this
		University.
		\item No portion of this work referred to in this thesis has been submitted in support of an
		application for another degree or qualification of this or any other university or other
		institution of learning.
		\item  Where I have consulted the published work of others, this is always clearly attributed.
		\item  Where I have quoted from the work of others, the source is always given. With the
		exception of such quotations, this thesis is entirely my own work.
	\end{itemize}
	\vspace{1cm}
	\noindent Signature: \begin{minipage}{0.4\textwidth}
		\rule{6cm}{0.5pt}
	\end{minipage}
	\vspace{1cm}
	\\Date: \begin{minipage}{0.4\textwidth}
		\rule{6cm}{0.5pt}
	\end{minipage}
% \thispagestyle{empty}

% ~~ \vspace{3in}

% \begin{center}


% \em{\textbf{\Large{To \\[4pt] my mother Sai and brother Tiru}}}



% \end{center}


==> glossaries/CHANGES <==
glossaries change log:

v4.45 (2020-02-13):

 * glossaries-accsupp.sty:

   - new associated accessibility keys for the user fields

   - new commands: \glsaccessibility, \glsfieldaccsupp, \xglsfieldaccsupp,
     \glsshortaccsupp, \glsshortplaccsupp (determine Alt/ActualText/E
     according to the field)

   - added accessibility support to \glstext, \glsplural, \glsfirst,
     \glsfirstplural, \glssymbol, \glsname, \glsdesc,
     \glsdescplural, \glsuseri, \glsuserii, \glsuseriii, \glsuseriv,
     \glsuserv, \glsuservi and their case variants

   - bug fixes: 

     - added field existence checks for \gls...accessdisplay commands

     - removed symbol use backward compatibility as it causes
       interference

 * glossaries-prefix.sty:

   - new command \glsprefixsep

 * glossaries.sty:

   - new package options:

      disablemakegloss
      restoremakegloss
      writeglslabels

   - package option debug now also accepts value 'showaccsupp'

   - detokenize label before passing to \glsshowtarget

   - new commands: \glsentryparent, \glsshowtargetouter and \glsshowtargetfont

   - made robust: \ifglshaschildren, \ifglshassymbol, \ifglshaslong,
     \ifglshasshort, \ifglshasfield

   - Bug fix:

     - added existence check to \glsentrytitlecase

v4.44 (2019-12-06):

 * glossaries-prefix.sty:

   - add hook for glossaries-extra's record option.

v4.43 (2019-09-28):

 * glossaries.sty:

   - added check for LaTeX kernel 2019/10/01 (new kernel affects
     accent stripping of UTF-8 characters with \makenoidxglossaries)

v4.42 (2019-01-06):

 * glossaries.sty:

  - changed \edef to \protected@csedef in \glsfieldedef

  - changed \xdef to \protected@csxdef in \glsfieldxdef

  - added package option 'noglossaryindex' to counteract 'index'
    (if 'index' happens to be supplied as a global option)

  - automake option now takes 'immediate' as a value.

 * glossary-longbooktabs.sty:

  - removed superfluous \glspatchLToutput

v4.41 (2018-07-23):

 * glossaries.sty:

  - added package option kernelglossredefs (Warnings are now
    generated if the kernel commands \makeglossary and \glossary are
    used. These commands are deprecated with the glossaries package.
    If the originals are required, by a package or class that must
    be used with glossaries.sty for some reason, then use 
    kernelglossredefs=false, but beware of other possible conflicts.)

  - renamed some internal commands to avoid conflict
     \gls@debug@val, \gls@debug@nr
     \gls@seenoindex@val, \gls@seenoindex@nr
     \gls@numberedsection@val, \gls@numberedsection@nr
     \gls@translate@val, \gls@translate@nr
     \gls@nonumberlist@val, \gls@nonumberlist@nr

v4.40 (2018-06-01):

 * bug fix: corrected page number reference when
   using \makenoidxglossaries 

v4.39 (2018-05-23):

 * makeglossaries-lite.lua:

  - corrected version information

 * glossariesbegin.tex:

  - updated further information section

 * glossaries-user.tex:

  - updated some external links

v4.38 (2018-05-10):

 * glossaries.sty:

  - added \GlsEntryCounterLabelPrefix

  - bug fixes:

    - moved conditional inside \glsstepentry,
      \glsstepsubentry, \glsrefentry,
      \glsentrycounterlabel, \glssubentrycounterlabel, \glsentryitem,
      \glssubentryitem, \glsresetentrycounter, \glsresetsubentrycounter

    - removed spurious space in subentrycounter (printgloss) key

    - fixed use of entrycounter and subentrycounter in \setupglossaries

 * glossaries-accsupp.sty:

  - bug fixes:

   - added braces around argument of ActualText in \glsaccsupp

   - corrected field used in \showglonameaccess

v4.37 (2018-04-07):

 * glossaries.sty:

  - added \gls@begindocdefs

v4.36 (2018-03-07):

 * glossaries.sty:

  - bug fix (if \makeindex is used without \makeglossaries, 
    corrupted glossary information is written to the .idx file)

 * makeglossaries-lite.lua:

  - corrected check for double-quotes in \@istfilename
    (from \jobname when the .tex file name contains spaces)

  - added check for nil codepage

v4.35 (2017-11-14):

 * glossaries.sty:

  - bug fix (\glsadd breaks with sort=use)

v4.34 (2017-11-03):

 * glossaries.sty:

  - modified \glsshowtarget to check for math mode and inner

 * glossary-mcols.sty:

  - removed spurious space in mcolalttreespannav style

 * makeglossaries and makeglossaries-lite.lua:

  - added check for \glsxtr@resource

v4.33 (2017-09-20):

 * Removed makeglossaries.bat (TeX distributions on Windows
   convert the Perl script to makeglossaries.exe, so the
   .bat file isn't needed.)

 * makeglossaries and makeglossaries-lite.lua now have their
   version numbers synchronised with glossaries.sty

 * Added makeglossaries-lite.pod (to provide the
   makeglossaries-lite.1 man file)

 * Updated POD at the end of makeglossaries

 * Added example-glossaries-symbolnames.tex for use in any MWE 
   requiring symbols in the name fields.

 * Tidied up the user manual and guide for beginners.

 * glossaries.sty:

  - added package option nolangwarn

  - added package option esclocations

  - added \GlsSetXdyNumberGroupOrder

  - added starred form of \GlsSetXdyFirstLetterAfterDigits

v4.32 (2017-08-24):

 * glossaries.sty:

  - added debug=showtargets and associated commands
    \@glsshowtarget and \glsshowtarget

 * glossary-hypernav.sty:

  - added \@glsnavhypertarget

v4.31 (2017-08-10):

 * glossaries.sty:

  - Bug fix: 'nolist' option sets default style to \relax
    if currently set to 'list' to prevent trying to set an
    undefined style.

v4.30 (2017-06-11):

  * glossaries.sty:

   - Added sort=none option

   - Added \glosortentrieswarning

   - Added \@glo@autosee

   - Fixed bug occurring with \setupglossaries{sort=def}

   - Fixed bug in \@xdyuserlocationnames

   - Fixed bug in \@xdylocationclassorder

   - Added \@xdycrossrefhook

   - Added \@glo@check@sortallowed

   - Fixed bug in \printnoidxglossary with group skips in
     tabular styles

  * makeglossaries v2.21:

    - Fixed spelling mistake in warning message
      (\GlsAddLocation -> \GlsAddXdyLocation)

    - Adjusted range encap clash correction

v4.29:

  * glossaries-accsupp.sty: corrected check for glossaries-extra
    'accsupp' option.

  * glossaries.sty: moved definition of \@gls@currentlettergroup
    before \begin{theglossary} and made redefinitions of it within
    theglossary global to guard against scoping issues cause by
    tabular-like glossary styles.

  * glossary-hypernav.sty: added \glsnavhyperlinkname

v4.28:

  * glossaries.sty: added \glspatchtabularx

v4.27:

  * Version number updated in *.sty files, but no actual code
    change.

  * makeglossaries v2.20 and makeglossaries-lite.lua v1.3:

    - Added check for \glsxtr@makeglossaries

v4.26:

  * glossaries.sty:

    - added check for classicthesis.sty (if it's been loaded
      the default style is changed to "index" since the "list"
      style doesn't work with classicthesis.)

  * glossary-tree.sty:

    - new commands \glstreeitem, \glstreesubitem and
      \glstreesubsubitem provided for the "index" style
      to make the style easier to adjust.

    - replaced hard-coded \space with \glstreepredesc 
      or \glstreechildpredesc for all glossary-tree styles
      except for the alttree* styles.

  * glossary-mcol.sty:

    - The "mcolindex" and "mcolindexspannav" styles
      use the new \glstreeitem, \glstreesubitem and
      \glstreesubsubitem provided by glossary-tree.sty.

v4.25:

  * glossaries.sty:

    - bug fix
      http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=111

v4.24:

  * glossaries.sty:

    - added debug and seenoindex option

    - added \GlsSetWriteIstHook and \GlsSetQuote

    - added \@gls@extramakeindexopts for makeglossaries
      and makeglossaries-lite.lua (allow makeindex -g
      for German documents)

  * makeglossaries (2.19):

    - Improved check in &parse_for_xindy_nosort

    - Added check for \@gls@extramakeindexopts

  * makeglossaries-lite.lua (1.2):

    - Added check for nil codepage

v4.23

  * glossaries.sty:

    - added \glscurrentfieldvalue

  * tabular-like styles (glossary-long.sty etc):

    - bug fix (nogroupskip in tabular styles with "noidx" commands)
      http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=108

v4.22:

  * glossaries.sty:

    - added \gls@arabicpage

    - added \ifglswrallowprimitivemods

    - added \glsentrytitlecase

  * glossary-tree.sty:

    - new formatting commands \glstreegroupheaderfmt
      and \glstreenavigationfmt to
      make it easier to customize styles

    - new command \glsfindwidesttoplevelname

  * glossary-mcols.sty:

    - hard-coded \textbf replaced with
      \glstreegroupheaderfmt or \glstreenavigationfmt,
      as appropriate

    - added new styles mcolindexspannav, mcoltreespannav,
      mcoltreenonamespannav, mcolalttreespannav

  * glossary-list.sty:

    - new formatting commands \glslistgroupheaderfmt
      and \glslistnavigationitem to make it easier to 
      customize styles

    - fixed missing space before description in list
      style sub-entries.

  * glossary-super.sty:

    - fixed bug in super4col style

  * glossary-long.sty:

    - fixed bug in long style (typo in \glossentrydesc
      for sub-entries)

v4.21:

  * glossaries.sty:

    - Added warning if there's no default style.

  * glossary-longbooktabs.sty - new package

  * makeglossaries (2.18):

    - Added extra diagnostic if xindy's empty index key
      warning/error occurs.

    - Added check for makeindex's multiple encap warning
      and attempt to fix.

  * glossaries-user.tex:

    - Fixed typo: \DefineAcronymShortcuts should be
      \DefineAcronymSynonyms

v4.20:

  * makeglossaries (2.17) bug fix
   http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=101

  (No changes to any of the *.sty files, except the version number.)

v4.19:

  * glossaries.sty:

    - Added commands: \glsdoifexistsordo, 
      \doifglossarynoexistsordo 

    - Added some new internals that will be used by pending new
      package glossaries-extra.sty

  * glossary-tree.sty:

    - Added \glstreenamebox

v4.18:

  * mfirstuc removed from glossaries bundle and now
    needs to be installed separately

v4.17:

  * makeglossaries-lite.lua:

    - changed #! line "lua" to "texlua"

  * mwe-acr.tex and mwe-acr-desc.tex:

    - fixed misplaced \setacronymstyle

v4.16:

  * Added makeglossaries-lite.lua (Lua trimmed-down alternative 
    to Perl makeglossaries script. Doesn't have the full
    functionality of makeglossaries but doesn't require Perl.)

  * makeglossaries (Perl script):

    - fixed ngerman din5007 issue.

  * glossaries.sty:

    - new field-related commands:
      \glsaddstoragekey, \glsfielddef, \glsfieldedef,
      \glsfieldgdef, \glsfieldxdef, \glsfieldfetch,
      \ifglsfieldeq, \ifglsfielddefeq, \ifglsfieldcseq

    - new user command \glswriteentry to hook into mechanism
      that writes entry information to the external files

    - new user command \glspostlinkhook to hook into end of
      commands like \gls and \glstext.

    - Added new acronym styles "long-sp-short" and
      "long-sp-short-desc"

    - bug fix: \glsadd should use \@@do@wrglossary not
      \@do@wrglossary

v4.15:

  * glossaries.sty:

   - bug fix
     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=79

v4.14:

  * glossaries.sty:

    - Added \glsenableentrycount and associated commands
      and accompanying sample file sample-entrycount.tex 
      that illustrates them.

v4.13:

  * glossaries.sty:

    - provide a definition of \indexspace if not already defined
      for those styles that need it.

  * mfirstuc.sty (v1.10):

    - added \ecapitalisewords, \emakefirstuc

v4.12:

  * glossaries.sty:

    - Separated language-dependent code into separate
      modules to be independently installed, as required.

    - Fixed bugs:
      www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=67
      www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=69
      www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&category=glossaries&key=72

v4.11:

  * glossaries.sty:

    - Added \glsaddprotectedpagefmt

    - Put back the redefinition of \glossary (so that it takes an
      optional argument) removed in the previous version to 
      allow for packages that have hacked the internal glossary
      writing mechanism. (This may be removed or moved to a 
      compatibility mode in the future.)

    - Fixed backward compatibility support of deprecated
      sanitize=none option

    - Fixed bug introduced in v4.10 that caused a conflict with
      doc.sty

v4.10:

  * Added test file example-glossaries-url.tex 

  * glossaries.sty:

    - Added \glspercentchar and \glstildechar

    - Fixed problem with \Glsentryname (and \Glsname)
      when used with \setacronymstyle

    - No longer redefine \glossary but instead define
      a replacement internal command \gls@glossary, and 
      renamed \@glossary to \@gls@glossary

  * glossary-tree.sty:

    - Corrected location of space in alttree style with symbols

v4.09:

  * Fixed bug in \glsaddkey introduced in v4.08
    www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=64

v4.08:

  * New files: example-glossaries-*.tex

    These contain lorem ipsum dummy entries for testing
    new styles or constructing MWEs that require a lot of sample entries
    (to be placed on TeX's path)

  * glossaries.sty

   - new package option: automake

   - \newglossary now has a starred version where you don't need
     to specify the extensions

   - new commands: \forallacronyms, \newignoredglossary

   - new keys for \printglossary/\printnoidxglossary:
     entrycounter, subentrycounter, nopostdot

   - \gls etc now have a +-version (opposite of the *-version)
     that explicitly switches on the hyperlink with hyper=true
     (unlike the unstarred version that uses the default setting).

   - new commands for use within \glsentryfmt or \defglsentryfmt:
     \glsifhyperon and \glslinkvar (\glsifhyper now deprecated).

   - fixed bug that didn't correctly honour the hyper setting
     in commands like \glslink, \gls, glstext, etc under 
     certain situations.

   - fixed bug
     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=54

   - added \@gls@hyp@opt and removed now-redundant internal commands

   - removed some of the redundancy in commands like \gls

  * glossary-longragged.sty:

   - Fixed bug in altlongragged4col style that displayed the
     description instead of the symbol in the third column.

  * glossary-tree.sty:

   - Added \glstreenamefmt

  * mfirstuc.sty v1.09:

   - Added \MFUnocap

  * New package: mfirstuc-english.sty

  * makeglossaries

   - Fixed bug report
     http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=55

v4.07:

  * glossaries.sty:

   - Added \glsletentryfield

   - Bug fixes:
     - added optional argument to unstarred sectioning
       commands (used with package options numberedsection=nolabel
       and numberedsection=autolabel)

     - added \global prefix to definition of \@gls@loclist
       in \@gls@noidx@do in case a tabular-like style is used.

     - Fixed no case change bug in \Acrfullplfmt

v4.06:

  * glossaries.sty:

   - Added \glsifhyper

   - Fixed bookmark issue occurring with
     "numbers" and "symbols" package options
     in combination with hyperref.sty and translator.sty

v4.05:

  - Added missing glossaries-prefix.sty to tds

v4.04:

  * glossaries.sty:

   - new commands: \makenoidxglossaries, \printnoidxglossary
     and \printnoidxglossaries that use TeX to sort entries 
     instead of makeindex/xindy

   - new command: \glsnumberlistloop (for use with
     \makenoidxglossaries)

   - new package option: noredefwarn

   - moved definition of \glswrite to \makeglossaries so that write
     register is only allocated if required.

   - fixed bug in \defglsdisplayfirst

  * glossary-tree.sty:

   - fixed bug in alttree style


  * glossaries-accsupp.sty:

   - \compatibleglossentry and \compatiblesubglossentry:
     changed \newcommand to \def as they may or may not be
     defined depending on whether user has loaded glossaries
     separately from glossaries-accsupp

  * makeglossaries:

   - added -Q and -k switches

   - added extra diagnostics

v4.03:

  glossaries.sty:

   * Added \glsifhasfield

   * Changed default definition of \glswritefiles to \@empty
     instead of \relax

   * Fixed bug in \ifglsdescsuppressed

   * Added \glsdetoklabel

   * Added \glsdoifexistsorwarn

   * Changed \glossentryname etc to use \glsdoifexistsorwarn
     instead of \glsdoifexists

   * Added \renewacronymstyle

   * Fixed bug in dua acronym style

  glossaries-accsupp.sty:

   * Redefined acronym styles to use accessibility support

  makeglossaries v2.12:

   * Added check for backslashes in -x, -m and -d arguments


v4.02:

  glossaries.sty:

   * Added nameref value to 'numberedsection' package option

   * New package option: "index"

   * New package option: xindynoglsnumbers (equivalent to 
     xindy={glsnumbers=false})

   * Added \newacronymstyle, \setacronymstyle and associated
     commands. (Package options "smallcaps", "smaller",
     "description", "dua" and "footnote" now deprecated.)

   * New commands \acrfullfmt etc to govern the format of 
     \acrfull etc.

   * Made \makeglossaries preamble only

   * Bug Fixes:

     - \acrlong, \Acrlong, \ACRlong, \acrlongpl,
       \Acrlongpl and \ACRlongpl: removed \acronymfont and
       spurious parenthetical text.

     - \glsentryfull, \Glsentryfull, \glsentryfullpl,
       and \Glsentryfullpl: added missing \acronymfont

     - Fixed bug in "sanitize" package option (deprecated option,
       but still kept for backward compatibility).

v4.01:

  * Fixed bug in \CustomAcronymFields caused by missing comma.

  * Fixed valueless package options so that they can be passed via
    the document class.

v4.0:

  First stable release since v3.07.

v3.14a:

  * glossaries.sty

    - New package options: acronyms, xindygloss, notranslate

    - Modified savewrites option so that it can be set via
      \setupglossaries

    - Enabled compatible-3.07 option in \setupglossaries

    - Added \provideglossaryentry and \longprovideglossaryentry

    - Bug fix: fixed the default firstplural value to the value of
      the plural key.

  * glossaries-prefix.sty

    - New

  * makeglossaries v2.09:

    - added check for -q switch when issuing warnings

v3.13a:

  * glossaries.sty

    - Added \glsprestandardsort

    - Renamed \glossarymark to \glsglossarymark to prevent clash
      with memoir.

    - Made "translate" package option a choice key rather than boolean

    - Bug fix for \glsaddallunused: 
        set default value of optional argument to \@glo@types

    - Bug fix for \SetFootnoteAcronymDisplayStyle:
        added missing final argument of \ifglshaslong

    - Bug fix for \glossarystyle:
        replaced \ifdef with \ifcsdef

  * mfirstuc.sty (v1.08):

    - Made \makefirstuc and \capitalisewords robust

v3.12a:

  * glossaries.sty

    - Added \glsaddkey (allows the user to add their own custom 
      keys to glossary entries).

v3.11a:

  * glossaries.sty

    - Added \setupglossaries
      (http://www.dickimaw-books.com/cgi-bin/featuretracker.cgi?action=view&key=7)

    - Added \glsentryfmt and \defglsentryfmt
      and deprecated \glsdisplayfirst, \glsdisplay,
      \defglsdisplayfirst and \defglsdisplay
      (http://www.dickimaw-books.com/cgi-bin/featuretracker.cgi?action=view&key=13)

    - Added \longnewglossaryentry

    - Added \ifglshasshort and \ifglshaslong

    - Added check in \glsgetgrouptitle for non-Latin characters

    - Added compatible-3.07 package option

    - Added "symbols" and "numbers" package options
      (http://www.dickimaw-books.com/cgi-bin/featuretracker.cgi?action=view&key=16)

    - Added \printacronyms[opts] as a synonym for
      \printglossary[type=\acronymtype,opts]
      if "acronym" package option is used and
      "compatible-3.07" package has not been used
      and \printacronym doesn't already exist at the start
      of the document.

    - Added \showgloshort and \showglolong

    - Fixed bug in \@gls@noexpand@fields

    - Fixed bug in \gls@defglossaryentry that didn't set the default
      counter correctly

    - Now uses \mfirstucMakeUppercase instead of \MakeUppercase
      to be consistent with mfirstuc.

    - Now requires textcase (better handling of case changes)

  * mfirstuc (v1.07)

    - Added \mfirstucMakeUppercase to allow the user to switch from
      \MakeUppercase to another case changing command.

  * makeglossaries (v2.08)

    - Added -x and -m switches

v3.10a:

  * glossaries.sty

    - Added \providecommand to aux file in case user removes 
      the glossaries package from their document. (This ensures
      the next run doesn't throw a load of undefined control
      sequence errors when the aux file is parsed.)

    - Fixed new code (from v3.08a) so that document can still
      compile if entries are defined within the document after
      \printglossary or \printglossaries

v3.09a:

  * glossaries.sty

    - Added fix for \RecordChanges if doc.sty has been loaded

    - Fixed noexpand for symbolplural field
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=41)

    - Made \Glsentryname, \Glsentrytext etc robust

    - Fixed bug in footnote option
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=37)

    - Fixed bug where acronym starts with repeated letter
      (www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=34)

    - Added \glstextup which checks for \textulc
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=40)

v3.08a:

  * glossaries.sty

    - Changed the way information is written to external glossary
      files. Information is now written as just \glossentry{label}
      or \subglossentry{level}{label} instead of
      \glossaryentryfield{label}{name}{description}{symbol} or 
      \glossarysubentryfield{level}{label}{name}{description}{symbol} 
      This means that descriptions can span multiple paragraphs
      without exceeding makeindex's buffer.

    - Added \setglossarystyle (replaces \glossarystyle which is now
      just for backward compatibility)

    - New user commands: 

        \glossentryname, \Glossentryname,
        \glossentrydesc, \Glossentrydesc,
        \glossentrysymbol, \Glossentrysymbol,
        \glsexpandfields, \glsnoexpandfields,
        \glsaddallunused,
        \ifglshassymbol, ifglshasdesc

    - Added nogroupskip option to \printglossary

    - Added \gls@ifnotmeasuring

    - Made \glsseeformat, \glsseelist, \glsseeitem and \glssee robust

  * glossary-tree.sty

    - Added \par to end of theglossary environment for index style.
      (http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=38)

v3.07:

  * glossaries.sty

    - Fixed bug relating to nohypertypes list option

    - Added \setglossarypreamble (code provided by Michael Pock)

    - Modified \glspostdescription to adjust spacefactor before full
      stop. (Patch provided by Michael Pock.)

    - Added check for openright in \gls@doclearpage

    - Added \glsdoparenifnotempty

    - Made \findrootlanguage obsolete

makeglossaries:

    - Added languagemap to determine root language

v3.06:

  * glossaries.sty

    - Fixed incompatibility between glossaries and new version of babel.

  * makeglossaries

    - added babel dialect -> xindy language map

v3.05:

  * glossaries.sty

    - fixed bugs related to location numbering (Roman and Alph).

    - made \nopostdesc robust

    - clarified in the documentation that \makeglossaries must be
      used before cross-referenced entries

    - added missing 'nohypertypes' code

  * makeglossaries:

    - added "din5007" as the default to makeglossaries if the
      language is german

  * glossary-mcols.sty:

    - Fixed bug -> \begin{multicols}{2} replaced with \begin{multicols}{\glsmcols}

v3.04:

  * added 'nohypertypes' package option

  * added new commands: \GlsDeclareNoHyperList and \glsIfNoHyperType

  * added 'local' key to \glsdisp, \gls, \Gls and \GLS

  * added check for doc package

  * fixed bug in altlist that can cause an unintentional page break
    between entry and description.

  * fixed bug that causes extra space after glossary when using
    xindy

  * fixed bug that was introduced by the bug fix in 3.02 regarding wrong
    page number

  makeglossaries v2.05:
  * added -d option

v3.03:

  * fixed bug in \printglossary options: title now also sets
    toctitle if toctitle missing (as per documentation).

  * added sanitize={sort=false} option

  * added nopostdot package option

  * added nogroupskip package option

   glossary-inline.sty added:

   - \glsinlinenameformat
   - \glsinlinedescformat
   - \glsinlineemptydescformat
   - \glsinlinesubnameformat
   - \glsinlinesubdescformat
   - \glsinlinepostchild

v3.02:

  * new package options:

    - 'ucmark'
    - 'indexonlyfirst'
    - 'savenumberlist'

  * new glossary styles:

    - glossary-mcol.sty
    - glossary-inline.sty

  * new commands:

    - \glolinkprefix
    - \glsmoveentry
    - \renewglossarystyle
    - \ifglshaschildren
    - \ifglshasparent
    - \glsresetentrycounter
    - \glsentrynumberlist
    - \glsdisplaynumberlist

  * added check to \glswritefiles to see if glossary tokens have
    been defined in case savewrites option used and \makeglossaries
    omitted.

  * fixed bug in \showglossaryentries

  * fixed bug in \SmallNewAcronymDef

  * fixed unwanted space in
    \SetDescriptionFootnoteAcronymDisplayStyle

  * fixed [xindy] wrong page number bug for entries occurring in
    paragraph spanning page break

  * fixed bug in \Glsentryfull and \glsentryfullpl

  * swapped order of checks for babel and polyglossia

  mfirstuc v1.06:

  * added \capitalisewords, \xcapitalisewords

  makeglossaries v2.04:

  * fixed bug in &scan_aux

v3.01:

   * made commands like \glslink, \gls and \acrshort robust

   * Fixed bugs in commands like \acrfullpl which was missing the
     plural in some cases.

   * Removed \acronymfont from \acrfullformat as it's already used
     in the second argument passed to that command. (Causes a 
     problem with the "smaller" option.)

v3.0 (Major changes):

   * Documentation has been restructured:

     - glossaries-user: main user manual
     - glossariesbegin: cut-down introduction for beginners
     - mfirstuc-manual: user manual for mfirstuc package
     - glossaries.pdf: documented code for advanced users
     - glossary2glossaries: upgrading from glossary.sty to glossaries.sty

   * Added new package options:

     - entrycounter : number main (level 0) entries in the glossary.

     - counterwithin : set parent counter for the entry counter.

     - subentrycounter : number level 1 entries in the glossary.

     - sort : set the sort order to 
              - standard alphabetical (sort=standard),
              - order of definition (sort=def) 
              - order of use (sort=use)

     - seeautonumberlist : automatically activates the number list
                           for entries that use the "see" key.

     - savewrites : minimise number of \newwrite

     - compatible-2.07 :

         bug fixes in v3.0 have cause compatibility problems. This 
         package option will restore the old behaviour but bugs will 
         remain.  (Should mostly only effect documents that used
         \noist with a custom Xindy style file.)

   * \printglossary sets \currentglossary to the current glossary's
     label. (Allows custom glossary styles access to the glossary
     type.)

   * Modified internal workings of acronyms and:

     - Added starred versions of \acrshort etc.

     - Added "long", "short", "longplural" and "shortplural" keys
       (Reserved for use with \newacronym.)

     - Added analogous "longaccess", "shortaccess", "longpluralaccess"
       and "shortpluralaccess" keys for \newacronym in 
       glossaries-accsupp.sty

   * Added \glsseeitemformat to customise the text given in the link
     created by \glsseeitem.

   * \newglossaryentry key "nonumberlist" now boolean.

   * added debugging commands \showgloname etc.

   * now loads etoolbox:

     - replaced \DeclareRobustCommand with \newrobustcmd

     - replaced \@ifundefined with \ifcsundef

     - replaced \let...\undefined with \undef...

   * Bug Fixes:

     - now works with equation counter in amsmath's align
       environment.

     - Mixed counters now work with xindy option.

     - Fixed hyperlinks in location numbers where \theH<counter>
       has a prefix not present in \the<counter>.

     - If title specified in \printglossary but toctitle hasn't
       been specified, make toctitle same as supplied title.

     - \newglossaryentry "see" key and \glssee now sanitize and escape 
       special characters before writing to output file. (Allows
       user to redefine \seename any point before \printglossary or
       \printglossaries.)

     - \glshyperlink: Changed the default value of the optional argument
                      to \glsentrytext instead of \glsentryname.

   * mfirstuc.sty (v1.05):

     - added \glsmakefirstuc (replaces \@gls@makefirstuc) to make
       it easier to customise.

   makeglossaries (v2.02):

   * now displays version number on startup unless -q

   * added more diagnostics to give more helpful messages than
     those supplied by xindy or makeindex.

v2.07:

   * Fixed bug that ignored format key in \glsadd

   makeglossaries:

   * Fixed bug causing failure to process aux files containing \@input

v2.06:
   * Added \altnewglossary

   * added facility to customise acronyms if the predefined styles
     don't fit the user's requirements.

   * Serbian dictionary added (provided by Zoran Filipovic)

   makeglossaries:

   * Scans aux file for \@input in case \printglossary is in an
     imported file.

v2.05:
   * Fixed error in .ist file and in \glsdisp caused by a 
     misplace brace. (Patch provided by Sergiu Dotenco).

v2.04:
   * Improved support for multiple lists of acronyms.

   * Fixed bug that caused \glsadd to ignore counter option

   * Fixed bug that causes babel to override translator's definition
     of \glossaryname.

   * Added user1, ... , user6 keys.

   * Added polyglossia support

   * makeglossaries now creates stub output file if input file is
     empty

  glossaries-accsupp v0.2:
   * Added access keys.

   * Added support for acronyms.

  mfirstuc v1.04: 
   * fixed bug occurring when initial control sequence
     in the argument of \makefirstuc has more than one 
     argument.

v2.03:
   * Added check to see if \glossarymark has been defined

   * makeglossaries - failed file test messages printed to
     stdout instead of stderr (so that it doesn't interrupt
     latexmk).

   * Fixed bug when entries used at the start of a paragraph.

   * Added package option hyperfirst (boolean option to suppress
     hyperlink on first use).

   * Added pod to makeglossaries.

v2.02:
   * Renamed glossaries-dictionary-Brazil.dict to 
     glossaries-dictionary-Brazilian.dict

   * Replaced \@mkboth with \glossarymark in \glossarysection
     to make it easier for the user to override it

   * Fixed bug that generated no \printglossary warning when
     the glossary is placed in a group

   * translate=false option will now prevent automatic loading
     of translator package.

v2.01:
   * Documentation changes:
      - removed quick guide section from glossaries.pdf and replaced 
        it with a separate beginners guide (glossariesbegin.pdf)
      - added a section for front-end or script developers who
        want to access information from the aux file

   * Added new ragged right versions of long/super styles

   * Added 'nomain' package option to suppress the creation of the
     main glossary

   * Added 'nowarn' package option to suppress warnings

   * Removed unwanted full stops in transcript messages

   * Changed \linewidth to \hsize when setting lengths

   * Removed item_02 key from makeindex style file (no such key)

   * Moved \@do@wrglossary before term is displayed to prevent
     unwanted whatsit

v2.0 (1.20):
   * Fixed ngerman caption bug in glossaries-babel.sty

v1.19:

   * changed \acronymfont to use \textsmaller instead of \smaller
     (for "smaller" package option)

   * Added \glsdisp (similar to \glslink except that it uses
     \glsdisplay/glsdisplayfirst and unsets the first use flag)

   * Added experimental package glossaries-accsupp which 
     requires accsupp package.

v1.18:
   * fixed missing closing } in glossaries-babel.sty

   * added \glstarget so that glossary styles can be modified
     in the document without using internal commands.

   * glossary-super.sty isn't loaded if supertabular.sty isn't
     installed.

   * added nolong, nosuper, nolist, notree and nostyles package 
     options to prevent loading unnecessary packages.

   * added \oldacronym (emulates the old glossary package's 
     \newacronym command).

   * added sublistdotted style.

   * fixed bug caused by misspelt \glspagewidthlist (should be
     \glspagelistwidth).

   * fixed border in super4colheaderborder and 
     altsuper4colheaderborder styles.

   * fixed sort sanitization when package option sanitize={name=false}
     is used.

v1.17:
   * changed definition of \@glossary to prevent conflict with
     memoir

   * added check to determine if \printglossary is defined. (If
     it is, issue warning and redefine.)

   * provided means to suppress number list for specific entries

   * provided means to suppress description terminator for
     specific entries

   * added cross-referencing support

   * added hierarchical support

   * added xindy support

   * modified \glshypernumber to support \nohyperpage
     (code provided by Heiko Oberdiek)

   * added 2 and 3-page suffix support

   * added "order" package option to set word/letter ordering
     (only has an effect in combination with makeglossaries script)

   * added Brazilian dictionary (supplied by Thiago de Melo)

v1.16 :
   * fixed bug that causes footnote option to remove hyperlink
     for first use entries in glossaries other than the list
     of acronyms. (footnote option should only affect entries
     in \acronymtype glossary.)

   * Raised hypertarget so that links to glossary entries don't
     scroll off the top of the page.

   * Fixed expansion-related bug (thanks to fix provided by
     Ulrich Diez)

v1.15 :
   * added \glslabel

   * added altlong4col* and altsuper4col* styles

   * fixed PDF encoding problem caused when both translator
     and hyperref packages are being used

   * fixed bug when using smallcaps and smaller options that causes
     the long form in the list of acronyms to be the same for each 
     entry

   * Added warnings when rerun required when using glossary
     group hyper navigation

glossaries.perl v1.04:
   * add do_cmd_glslabel

   * changed links to the start of the relevant glossary entry
     rather than the entry's backlink

   * added implementation of starred forms of \gls etc

   * added frame related code if frames.pl has been loaded

v1.14 :
   * Fixed bug in \glsnavhyperlink that causes an error when used
     with hyperref and translator packages.

   * Added \glsautoprefix (specifies a prefix to the automatically
     generated label)

   * Added nonumberlist and numberedsection keys to \printglossary

   * Changed \glsnavigation so that it only lists the groups that
     are present. (This prevents unknown target warnings.)

   * Amended documentation.

mfirstuc v1.02 (18 June 2008):

   * Fixed bug that transfered grouping, (e.g 
     \makefirstuc{\emph{abc}xyz} moved the xyz into the \emph)

   * If group following initial command is empty, \MakeUppercase
     is applied to the command, e.g. \makefirstuc{\ae{}bc} now
     produces \MakeUppercase\ae{}bc.

v1.13 :
   * Fixed bug in long4colheaderborder that puts an extra row
     at the end of the glossary.

   * Fixed bug in \glstext etc that ignored 3rd argument (thanks
     to Franz Fischer for pointing this out).

   * Removed only preamble restriction on \newglossaryentry and
     \newacronym.

   * Added \glspluralsuffix.

   * Changed firstplural default so that it takes its value from
     the plural key if the first key is omitted.

   * Added \acrshortpl, \Acrshortpl, \ACRshortpl, \acrlongpl,
     \Acrlongpl, \ACRlongpl, \acrfullpl, \Acrfullpl, \ACRfullpl.

   * Fixed bugs in \Acrshort etc.

   * Add package options "smaller" and "shortcuts".

   * Acronym default plural forms now implemented for the additional
     acronym styles.

   * Fixed makeglossaries to allow filenames with spaces.

   * Fixed error in documentation describing \glsaddall
     - optional argument should be a key=value list.

   * Added Polish support (thanks to Piotr Formella for supplying
     the translations).

   * If babel is loaded and translator package is found on TeX's
     path, then the translator package will now be automatically 
     loaded.

mfirstuc v1.01 (13 May 2008):

   * Added \xmakefirstuc (expands argument before applying \makefirstuc)

v1.12 (8 March 2008):
   * Fixed bug that causes \glspl to print the plural short form
     on first use instead of the plural long form.

   * Added descriptionplural and symbolplural keys.

   * Added \glsshortkey, \glsshortpluralkey, \glslongkey and
     \glslongpluralkey.

   * Fixed bugs in \glsname, \glstext, \glsdesc etc.

   * Added a check for \hypertarget in addition to checking
     for \hyperlink (in the event that \hyperlink is defined
     but not \hypertarget).

   * Changed #! line in makeglossaries to use /usr/bin/env

   * Added package mfirstuc.sty which provides the command 
     \makefirstuc{<stuff>} which makes the first object of
     <stuff> uppercase unless <stuff> starts with a control
     sequence followed by a group, in which case the first
     object in the group is converted to uppercase. Examples:

     \makefirstuc{abc}        -> Abc
     \makefirstuc{\emph{abc}} -> \emph{Abc}
     \makefirstuc{{\'a}bc}    -> {\'A}bc
     \makefirstuc{\ae bc}     -> \AE bc
     \makefirstuc{{\ae}bc}    -> {\AE}bc

     (but don't do \makefirstuc{\ae{}bc} which produces \ae Bc.)

v1.11 (2 March 2008):
   * Fixed error in manual (glossary style is set using \glossarystyle
     not \setglossarystyle).

   * Changed the way the package is archived to make it compatible
     with TeX Live.

   * Improved error handling of makeglossaries and added --version
     and --help options.

v1.1 (22 Feb 2008):

   * New package options:

     - numberline: 
       inserts \numberline{} in \addcontentsline when used with
       the toc option.

     - numberedsection: 
       puts glossaries in numbered chapters/sections

     - translate:
       translate=false option prevents glossaries package from
       using pre-supplied translations.

     - description:
       changes definition of \newacronym to allow a description

     - footnote:
       changes definition of \newacronym to use a footnote on
       first use

     - smallcaps:
       changes definition of \newacronym to set acronyms in 
       small capitals

     - dua:
       changes definition of \newacronym to always expand
       acronyms

   * Added \setglossarysection
     - changes the section type used by the glossaries

   * Added listdotted glossary style.

   * No longer uses xspace package; uses amsgen instead.

   * Added \glsname, \glsdesc, \glssymbol, \glsfirst, \glstext, 
     \glsplural and \glsfirstplural.

   * Added support for translator package.

v1.08 (13 Oct 2007):
   * Added multilingual support
   * Fixed bug in listgroup and altlistgroup styles so that 
     \glsgroupheading uses \glsgetgrouptitle to get the group title 
     instead of displaying the label
   * Fixed typo in error message text when the description key
     is missing to \newglossaryentry.

v1.07 (13 Sep 2007):
   * Fixed bug causing incorrect page number for entries in the
     first paragraph of a page.

v1.06 (21 Aug 2007):
   * Changed the license text

v1.05 (10 Aug 2007):
   * Changed the default value of the sort key to just use the
     name key
   * Added \@mkboth to \glossarysection

v1.04 (3 Aug 2007):
   * Added \glstextformat

v1.03 (4 July 2007):
   * Added \glspostdescription

v1.02 (25 May 2007):
   * Added overview section in the documentation

v1.01 (17 May 2007):
   * Added number range facility (equivalent to makeindex's |( and |)
     formatting commands.)
   * Added a space after \delimN and \delimR in the ist file.

v1.0 (16 May 2007): Initial release


==> glossaries/INSTALL <==
INSTALLATION

The best (and recommended) method of installing is through your TeX package
manager (for example, `tlmgr install glossaries`), but if you need to use 
the manual method for some reason, follow the instructions below.

If you have downloaded the glossaries package using the TeX
Directory Structure (TDS), that is you have downloaded the archive
glossaries.tds.zip containing doc, tex, scripts and source
directories, you need to follow the "Installing from TDS"
instructions below.

If you have downloaded the following files:

glossaries.dtx
glossaries.ins
makeglossaries
makeglossaries.bat

You need to follow the "Installing from DTX and INS" instructions
below.

For further information on installing LaTeX packages see:

http://www.tex.ac.uk/cgi-bin/texfaq2html?label=installthings

INSTALLING FROM TDS
===================

Files in tex and doc directories should go in the corresponding
TEXMF directories (for example, ~/texmf or /usr/share/texmf-local/ or
C:\localtexmf\). The scripts/glossaries/ directory contains the Perl
script makeglossaries and the batch file makeglossaries.bat which
should go somewhere on your operating system's PATH. (Both files are
required for Windows, but only the Perl script is required for other
operating systems.) Similarly for makeglossaries-lite.lua, which is
a Lua alternative.

Example (on UNIX like systems):

unzip glossaries.tds.zip -d ~/texmf/

A minimal example file called minimalgls.tex is provided for testing
and debugging purposes and can be found in the package documentation
samples directory (doc/latex/glossaries/samples/). To test your
installation do:

latex minimalgls
makeglossaries minimalgls
latex minimalgls

The LaTeX2HTML style file, glossaries.perl, is located in 
source/latex/glossaries and should go in the LaTeX2HTML styles 
directory, if required.

INSTALLING FROM DTX AND INS
===========================

Run LaTeX on glossaries.ins to generate the package style files,
sample files and LaTeX2HTML style file:

latex glossaries.ins

To create the package documentation (glossaries-code.pdf):

pdflatex -jobname glossaries-code glossaries.dtx
makeindex -s gind.ist glossaries.idx
makeindex -s gglo.ist -o glossaries.gls glossaries.glo
makeglossaries glossaries
pdflatex -jobname glossaries-code glossaries.dtx
pdflatex -jobname glossaries-code glossaries.dtx

If TEXMF denotes the base directory of your local TeX installation (e.g.
/usr/share/texmf-local/ or C:\localtexmf\) then create the following
directories (if they don't already exist):

TEXMF/doc/latex/glossaries
TEXMF/doc/latex/glossaries/samples
TEXMF/tex/latex/glossaries
TEXMF/tex/latex/glossaries/base
TEXMF/tex/latex/glossaries/expl
TEXMF/tex/latex/glossaries/styles
TEXMF/tex/latex/glossaries/test-entries

Move the example-glossaries-*.tex files to
TEXMF/tex/latex/glossaries/test-entries/

Move the sample files (*.tex) to TEXMF/doc/latex/glossaries/sample/

Move the documentation (*.pdf) to TEXMF/doc/latex/glossaries/

Move glossaries.sty, glossaries-babel.sty,
glossaries-polyglossia.sty, glossaries-compatible-207.sty, 
glossaries-compatible-307.sty,
mfirstuc.sty and mfirstuc-english.sty to
TEXMF/tex/latex/glossaries/base/

Move glossaries-accsupp.sty to
TEXMF/tex/latex/glossaries/expl/

Move the other style files (glossary-*.sty) to
TEXMF/tex/latex/glossaries/styles/

Move makeglossaries to somewhere on your path, e.g. /usr/bin/.

If you are a Windows user, you will also need to move
makeglossaries.bat to the same location as makeglossaries, but you
will need to have Perl installed to be able to use makeglossaries.
(It is possible to use makeindex or xindy directly if you don't have
Perl installed. See the manual, glossaries.pdf, for details.)

A minimal example file called minimalgls.tex is provided for testing
and debugging purposes. This file is created along with all the other
sample files when you run glossaries.ins through LaTeX. To test your
installation do:

latex minimalgls
makeglossaries minimalgls
latex minimalgls

If you want to use the glossaries package with LaTeX2HTML:
move glossaries.perl to the LaTeX2HTML styles directory.


==> glossaries/makeglossaries <==
#!/usr/bin/env perl

# File    : makeglossaries
# Author  : Nicola Talbot
# Version : 4.45
# Description: simple Perl script that calls makeindex or xindy.
# Intended for use with "glossaries.sty" (saves having to remember
# all the various switches)

# This file is distributed as part of the glossaries LaTeX package.
# Copyright 2019 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

# This work consists of the files glossaries.dtx and glossaries.ins 
# and the derived files glossaries.sty, glossaries-prefix.sty,
# glossary-hypernav.sty, glossary-inline.sty, glossary-list.sty, 
# glossary-long.sty, glossary-longbooktabs.sty, glossary-longragged.sty,
# glossary-mcols.sty, glossary-super.sty, glossary-superragged.sty, 
# glossary-tree.sty, glossaries-compatible-207.sty, 
# glossaries-compatible-307.sty, glossaries-accsupp.sty, 
# glossaries-babel.sty, glossaries-polyglossia.sty, glossaries.perl.
# Also makeglossaries and makeglossaries-lite.lua.

my $version="4.45 (2020-01-18)";

# History:
# v4.43:
#   * No change.
# v4.41:
#   * No change.
# v4.40:
#   * No change.
# v4.39:
#   * No change.
# v4.38:
#   * No change.
# v4.37:
#   * No change.
# v4.36:
#   * No change.
# v4.35:
#   * No change.
# v4.34:
#   * Added check for \glsxtr@resource
# v4.33:
#   * Version number synchronized with glossaries.sty
# v2.21:
#   * Fixed spelling of \GlsAddXdyLocation
#   * Adjusted range encap clash
# v2.20 (2016/12/16)
#   * Added check for \glsxtr@makeglossaries
# v2.19 (2016/05/27)
#   * Improved check in &parse_for_xindy_nosort
# v2.18 (2016/01/24)
#   * Added &parse_for_xindy_nosort to help diagnose xindy's empty
#     index key warning/error.
#   * Added check for makeindex's multiple encap warning.
# v2.17 (2015/11/30)
#   * Escaped { in regular expressions.
#     http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=101
# v2.16 (2015/06/28)
#   * Added check for "german" and codepage that doesn't contain
#   "din5007", "duden" or "braille". If missing, "din5007-" is
#   prefixed to the codepage.
# v2.15 (2014/07/30)
#   * Removed hard-coded three character extension assumption
#     www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=55
#   * Added message to indicate the number of ignored glossaries
#     when the extension is specified.
# v2.14 (2014/03/06)
#   * Added -Q and -k options
# v2.13 (2014/01/21)
#   * Added check for leading and trailing quotes in filename
# v2.12 (2014/01/20)
#   * Added check for '*' in istfilename
#   * Fixed bug report
#   http://www.dickimaw-books.com/cgi-bin/bugtracker.cgi?action=view&key=33
#   * Added error text hashes
# v2.11 (2014/01/17):
#   * Added check for backslashes in -x, -m and -d paths
#   * Added double-quotes around $appname in &run_app
# v2.10 (2013/12/01):
#   * initialise $language to suppress warnings
# v2.09 (2013-11-12):
#   * added check for -q switch when issuing warnings.
# v2.08 (2013-10-14):
#   * added -x and -m options
# v2.07 (2013-06-17):
#   * added check for success on chdir if -d used
#   * added dialect map
# v2.06 (2013-04-21):
#   * added "din5007" as default if language is set to "german"
# v2.05 (2012-11-12):
#   * added -d option
# v2.04 (2012-04-19):
#   * fixed bug in &scan_aux
# v2.03 (2011-04-12):
#   * added warning about possibly needing 'nomain' package option
# v2.02 (2011-04-2):
#   * Prints version number at start of run unless -q
#   * Added more diagnostics.
# v2.01 (2010-09-29):
#   * Added 'use warnings'
# v2.0 (2010-06-30) :
#   * Made file handle local in &scan_aux
# v1.9 (2010-06-14) :
#   * Check for \@input
# v1.8 (2009-11-03) :
#   * Create an empty output file if the input file is empty
#     without calling xindy/makeindex
# v1.7 (2009-09-23) :
#   * Issue warning rather than error when empty/non existant file 
#     checks fail
# v1.6 (2009-05-24) :
#   * main glossary no longer automatically added
#     (only added if information in aux file)
#   * if file extension is specified, check added to ensure it
#     corresponds to a known glossary extension.
#   * added file existance test and file empty test
# v1.5 (2008-12-26) :
#   * added support for xindy
#   * picks up ordering information from aux file
# v1.4 (2008-05-10) :
#   * added support for filenames with spaces.
# v1.3 (2008-03-08) :
#   * changed first line from /usr/bin/perl -w to /usr/bin/env perl
#     (Thanks to Karl Berry for suggesting this.)
# v1.2 (2008-03-02) :
#   * added support for --help and --version
#   * improved error handling
# v1.1 (2008-02-13) :
#   * added -w and strict
#   * added check to ensure .tex file not passed to makeglossaries
#
# v1.0 (2007-05-10) : Initial release.

use Getopt::Std;
use strict;
# v2.01 added the following line
use warnings;
# v2.05 added $opt_d
# v2.08 added $opt_x and $opt_m
use vars qw($opt_q $opt_t $opt_o $opt_s $opt_p $opt_g $opt_c $opt_r
   $opt_l $opt_i $opt_L $opt_n $opt_C $opt_d $opt_x $opt_m $opt_Q
   $opt_k);


$Getopt::Std::STANDARD_HELP_VERSION = 1;

# v1.5 added -L <lang> for xindy (but language can be specified in 
# .tex file)
# v1.5 added -n (print the command that would be issued but
# don't actually run the command)
getopts('s:o:t:p:L:C:ilqQkrcgnd:x:m:');

unless ($#ARGV == 0)
{
   die "makeglossaries: Need exactly one file argument.\n",
       "Use `makeglossaries --help' for help.\n";
}

# v2.02: added:
print "makeglossaries version $version\n" unless ($opt_q);

# v2.07: added babel dialect -> xindy language map:
my %languagemap =
(
  'american'  => 'english',
  'austrian'  => 'german',
  'british'   => 'english',
  'francais'  => 'french',
  'frenchb'   => 'french',
  'germanb'   => 'german',
  'lsorbian'  => 'lower-sorbian',
  'magyar'    => 'hungarian',
  'naustrian' => 'german',
  'ngermanb'  => 'german',
  'ngerman'   => 'german', # v2.16
  'norsk'     => 'norwegian',
  'portuges'  => 'portuguese',
  'russianb'  => 'russian',
  'slovene'   => 'slovenian',
  'UKenglish' => 'english',
  'USenglish' => 'english',
  'ukraineb'  => 'ukrainian',
  'usorbian'  => 'upper-sorbian'
);

# v2.07 added check for success and for -q
# v2.05 added:

if ($opt_d)
{
  # v2.11 check for backslash character if on Windows
  $opt_d=~s/\\/\//g if $^O=~/Win/;

  if (chdir $opt_d)
  {
     print "Changed to '$opt_d'\n" unless ($opt_q);
  }
  else
  {
     die "Unable to chdir to '$opt_d' $!\n";
  }
}

# v2.02: added:
# v2.19: changed value
my $xdynotist = 2;
# v2.13: removed
#my $needcompatibilitymode=2;

# v2.13: added $istnotfound
my $istnotfound = 3;

# v2.13: added error text:
my %makeindex_error_text =
 (
   $xdynotist => "Style name indicates makeindex, but may be in xindy format.\n"
          . "Remember to use \\setStyleFile to specify the name\n"
          . "of the style file rather than redefining \\istfilename\n"
          . "explicitly.",
   $istnotfound => "Style file not found. (Have you used \\noist by mistake?)"
 );

my %xindy_error_text =
 (
   'nosort'    => "Sort key required for entries only containing command names.",
   'istnotxdy' =>
      "Style name has xdy extension, but may be in makeindex format.\n"
     . "Remember to use \\setStyleFile to specify the name\n"
     . "of the style file rather than redefining \\istfilename\n"
     . "explicitly.",
   'missingendquote' =>
       "You may have missed a \" character in a command such as \\GlsAddXdyLocation.",
    'nolanguage' =>
       "No language detected.\nHave you remembered to use \\printglossary\n".
       "or \\printglossaries in your document?",
    'nomain' =>
        "\nRemember to use package option 'nomain' if you don't\n".
        "want to use the main glossary.",
#v2.21: fixed spelling of \GlsAddXdyLocation
    'badlocation' =>
        "You may have forgotten to add a location \n"
        . "class with \\GlsAddXdyLocation or you may have \n"
        . "the format incorrect.\n",
    'comp207' => "You may need to add 'compatible-2.07' package option.",
    'noxdyfile' => "Style file not found. (Have you used \\noist by mistake?)"
 );

# define known extensions

# v1.6: removed adding main glossary here as there's no guarantee
# that it's been used. If it has been used, the information will
# be picked up later in the aux file
my %exttype = (
#   main => {in=>'glo', out=>'gls', 'log'=>'glg'},
 );

# v1.5 define require languages for xindy

my %language = ();
my %codepage = ();

my $ext = '';
my $name = $ARGV[0];

# v2.13 added:
#$name=~s/^"(.*)"$/$1/;
# v2.15: fix provided by Herb Schulz to allow for extensions that
# aren't exactly three characters:
# (HS) changes fix for 3 character extension limit
my ($basename,$extension) = ($name =~ m/^(.*?)(?:\.([^\.]*))?$/);
# (HS) end of changes fix for 3 character extension limit

# make sure $extension is defined. (If there was no match in the
# above, it cause an uninitialised error later.)
$extension = '' unless ($extension);

# Make sure users don't try passing the tex file:

#if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
#{
#  $name = substr($ARGV[0],0,length($ARGV[0])-4);
#
#  $ext = substr($ARGV[0],-3,3);
#
#  if (lc($ext) eq 'tex')
# (HS) changes fix for 3 character extension limit
#if (length($ARGV[0]) > 3 and substr($ARGV[0],-4,1) eq ".")
#{
#  $name = substr($ARGV[0],0,length($ARGV[0])-4);
#
#  $ext = substr($ARGV[0],-3,3);
#
#  if (lc($ext) eq 'tex')
  if (lc($extension) eq 'tex')
  {
     die("Don't pass the tex file to makeglossaries:\n"
        ."either omit the extension to make all the glossaries, "
        ."or specify one of the glossary files, e.g. $name.glo, to "
        ."make just that glossary.\n")
  }
#}
# (HS) end of fix for 3 character extension limit

# (HS) changes fix for 3 character extension limit
$ext = $extension;
$name = $basename;
# (HS) end of changes fix for 3 character extension limit

# v2.01 add check to see if aux file exists

unless (-e "$name.aux")
{
   die "Auxiliary file '$name.aux' doesn't exist. Have you run LaTeX?\n";
}

my $istfile = "";

my $glslist = "";

# should letter ordering be used? (v1.5 added)

my $letterordering = defined($opt_l);

# v2.19 added:
my $extramkidxopts = '';

# v4.34 added:
my $foundbib2glsresource = '';

# Check aux file for other glossary types,
# style file name and various other bits of information.

&scan_aux($name);

# has the style file been specified?
unless ($istfile)
{
   if ($foundbib2glsresource)
   {
      die "Found \\glsxtr\@resource in '$name.aux',\n",
          "but not found \\\@istfilename.\n",
          "You need to run bib2gls not makeglossaries.\n";
   }
   else
   {
      die "No \\\@istfilename found in '$name.aux'.\n",
          "Did your LaTeX run fail?\n",
          "Did your LaTeX run produce any output?\n",
          "Did you remember to use \\makeglossaries?\n";
   }
}

# v2.08 added $xindyapp and $makeindexapp
# By default assume they are on the operating system's path
my $xindyapp = ($opt_x ? $opt_x :'xindy');
my $makeindexapp = ($opt_m ? $opt_m :'makeindex');

# v2.11 check for backslash character if on Windows
if ($^O=~/Win/)
{
  $xindyapp=~s/\\/\//g;
  $makeindexapp=~s/\\/\//g;
}

# v1.5 save the general xindy switches

my $xdyopts = '';

# v2.01 replaced 'unless ($opt_L eq "")' with 'if ($opt_L)'
if ($opt_L)
{
  $xdyopts .= " -L $opt_L";
}

# save all the general makeindex switches

my $mkidxopts = '';

if ($opt_i)
{
   $mkidxopts .= " -i";
}

if ($letterordering)
{
   $mkidxopts .= " -l";
   $xdyopts .= " -M ord/letorder";
}

if ($opt_q)
{
# v2.01 removed following lines. (This script now deals with
# printing messages to STDOUT.)
   #$mkidxopts .= " -q";
   #$xdyopts .= " -q";
}

if ($opt_r)
{
   $mkidxopts .= " -r";
}

if ($opt_c)
{
   $mkidxopts .= " -c";
}

if ($opt_g)
{
   $mkidxopts .= " -g";
}

# v2.01 replaced 'unless ($opt_p eq "")' with 'if ($opt_p)'
if ($opt_p)
{
   $mkidxopts .= " -p $opt_p";
}

if ($extramkidxopts)
{
  $mkidxopts .= " $extramkidxopts";
}

# v2.01 replaced 'unless ($opt_s eq "")' with 'if ($opt_s)'
if ($opt_s)
{
   # v2.01 check if user has specified -s <file>.ist but aux file
   # indicates .xdy ought to be used and vice-versa. Also check if
   # requested style file exists

   unless (-e $opt_s)
   {
      die "\n",
         "Requested style file '$opt_s' doesn't exist.\n\n";
   }

   if ($istfile=~/\.xdy$/ and $opt_s!~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using xindy,\n",
        "but you have specified makeindex style file '$opt_s'\n",
        "Make sure you don't specify 'xindy' as a package option if\n",
        "you want to use makeindex.\n\n",
        "\\usepackage[makeindex]{glossaries}\n\n";
   }
   elsif ($istfile!~/\.xdy$/ and $opt_s=~/\.xdy$/)
   {
      die "\n",
        "The auxiliary file indicates that you should be using\n",
        "makeindex, but you have specified xindy style file '$opt_s'.\n",
        "Make sure you specify 'xindy' as a package option if you\n",
        "want to use xindy.\n\n",
        "\\usepackage[xindy]{glossaries}\n\n";
   }

   $istfile = $opt_s;
}

# Use xindy if style file ends with .xdy otherwise use makeindex

my $usexindy = ($istfile=~m/\.xdy\Z/);

if ($ext)
{
   # an extension has been specified, so only process
   # the specified file

   # v1.6 %thistype is no longer given a default value
   my %thistype;

   my $thislang = "";
   my $thiscodepage = "";

   my @types = ($glslist ? split /,/, $glslist : keys %exttype);

   foreach my $type (@types)
   {
      if ($exttype{$type}{'in'} eq $ext)
      {
         %thistype = %{$exttype{$type}};

         $thislang = $language{$type};

         $thiscodepage = $codepage{$type};

         last;
      }
   }

   # v1.6 If %thistype hasn't been defined, then the given
   # extension doesn't correspond to any known glossary type

   # v2.01 replaced deprecated 'defined(%thistype)' with %thistype
   unless (%thistype)
   {
      die "The file extension '$ext' doesn't correspond to any\n",
          "known glossary extension. Try running makeglossaries\n",
          "without an extension, e.g. makeglossaries \"$name\".\n";
   }

   my $outfile;

# v2.01 replaced 'if ($opt_o eq "")' with 'unless ($opt_o)'
   unless ($opt_o)
   {
      $outfile = "$name.$thistype{out}";
   }
   else
   {
      $outfile = $opt_o;
   }

   my $transcript;

# v2.01 replaced 'if ($opt_t eq "")' with 'unless ($opt_t)'
   unless ($opt_t)
   {
      $transcript = "$name.$thistype{'log'}";
   }
   else
   {
      $transcript = $opt_t;
   }

# v2.01 remove old transcript file

   unless ($opt_n)
   {
      unlink($transcript);
   }

   if ($usexindy)
   {
      &xindy("$name.$ext", $outfile, $transcript,$istfile,
        $thislang, $thiscodepage, $xdyopts, $opt_q, $opt_n, $xindyapp);
   }
   else
   {
      &makeindex("$name.$ext",$outfile,$transcript,$istfile,
                 $mkidxopts,$opt_q, $opt_n, $makeindexapp, 1);
   }


   # v2.15 added:

   my $num_omitted = $#types;

   if ($num_omitted == 1)
   {
      print "1 glossary ignored.\n" unless $opt_q;
   }
   elsif ($num_omitted > 1)
   {
      print "$num_omitted glossaries ignored.\n" unless $opt_q;
   }
}
else
{
   # no file extension specified so process all glossary types

   my @types = ($glslist ? split /,/, $glslist : keys %exttype);

   foreach my $type (@types)
   {
      my %thistype = %{$exttype{$type}};

      my $inputfile = "$name.$thistype{in}";

      my $outfile;

# v2.01 changed 'if ($opt_o eq "")' with 'unless ($opt_o)'
      unless ($opt_o)
      {
         $outfile = "$name.$thistype{out}";
      }
      else
      {
         $outfile = $opt_o;
      }

      # v1.7 print warnings to STDOUT instead of STDERR

      # v1.6 added file existence test
      unless (-e $inputfile)
      {
         # v2.09 suppress warning if -q switch in use
         print "Warning: File '$inputfile' doesn't exist.\n",
             "*** Skipping glossary '$type'. ***\n" unless ($opt_q);
         next;
      }

      unless (-r $inputfile)
      {
         print "Warning: No read access for '$inputfile' $!\n",
             "*** Skipping glossary '$type'. ***\n" unless ($opt_q);
         next;
      }

      my $transcript;

# v2.01 changed 'if ($opt_t eq "")' with 'unless ($opt)'
      unless ($opt_t)
      {
         $transcript = "$name.$thistype{'log'}";
      }
      else
      {
        $transcript = $opt_t;
      }

      # v1.6 added file empty test
      if (-z $inputfile)
      {
         my $message =
             "Warning: File '$inputfile' is empty.\n".
             "Have you used any entries defined in glossary '$type'?\n";

         if ($type eq 'main')
         {
            $message .=
               "Remember to use package option 'nomain' if you\n".
               "don't want to use the main glossary.\n";
         }

         # v2.09 suppress warning if -q switch in use
         warn $message unless $opt_q;

         # Write warning to transcript file.

         if (open TRANSFD, ">$transcript")
         {
            print TRANSFD $message;
            close TRANSFD;
         }

         # create an empty output file and move on to the next glossary

         if (open OFD, ">$outfile")
         {
            print OFD "\\null\n";
            close OFD;
         }
         else
         {
            warn "Unable to create '$outfile' $!\n";
         }

         next;
      }

# v2.01 remove old transcript file

      unless ($opt_n)
      {
         unlink($transcript);
      }

      if ($usexindy)
      {
         &xindy($inputfile,$outfile,$transcript,$istfile,
                $language{$type},$codepage{$type},
                $xdyopts,$opt_q,$opt_n, $xindyapp);
      }
      else
      {
         &makeindex($inputfile,$outfile,$transcript,
                    $istfile,$mkidxopts,$opt_q,$opt_n, $makeindexapp, 1);
      }
   }
}

sub scan_aux{
  my $name = shift;

  # v2.0 added
  local(*AUXFILE);

  if (open AUXFILE, "$name.aux")
  {
     while (<AUXFILE>)
     {
        #v2.14 added
        if (m/\\\@gls\@reference/ and not $glslist)
        {
           die "Your document has used \\makenoidxglossaries\n",
               "You don't need makeindex or xindy.\n";
        }

        if (m/\\glsxtr\@makeglossaries\{(.*)\}/)
        {
           #v2.20 added

           $glslist = $1;

           unless ($opt_q)
           {
              print "only processing subset '$glslist'\n";
           }
        }
        elsif (m/\\\@input\{(.+)\.aux\}/)
        {
           # v1.9 added
           # v2.17 escaped { in regex
           &scan_aux($1);

           # v2.04 added
           # (Fix provided by Daniel Grund) 
           next;
        }
        elsif (m/\\\@newglossary\s*\{(.*)\}\{(.*)\}\{(.*)\}\{(.*)\}/)
        {
           # v2.17 escaped { in regex

           $exttype{$1}{'log'} = $2;
           $exttype{$1}{'out'} = $3;
           $exttype{$1}{'in'}  = $4;

           unless ($opt_q)
           {
              print "added glossary type '$1' ($2,$3,$4)\n";
           }
        }
        elsif (m/\\\@istfilename\s*\{([^}]*)\}/)
        {
           # v2.17 escaped { in regex

           $istfile = $1;

           # check if double quotes were added to \jobname
           # v2.12 added check for xdy (bug ID 33)
           $istfile=~s/^"(.*)"\.(ist|xdy)$/$1.$2/;

           # v2.12 if on Windows, substitute any '*' with ' '
           # to compensate for MiKTeX bug
           # http://sourceforge.net/p/miktex/bugs/2301/

           if ($^O=~/Win/)
           {
              $istfile=~tr/\*/ /;
           }
        }
        elsif (m/\\\@xdylanguage\s*\{([^}]+)\}\{([^}]*)\}/)
        {
           # v1.5 added
           # v2.17 escaped { in regex

           $language{$1} = $2;
        }
        elsif (m/\\\@gls\@codepage\s*\{([^}]+)\}\{([^}]*)\}/)
        {
           # v1.5 added
           # v2.17 escaped { in regex

           $codepage{$1} = $2;
        }
        elsif (m/\\\@gls\@extramakeindexopts\{(.*)\}/)
        {
           # v2.19 added

           $extramkidxopts .= $1;
        }
        elsif (m/\\glsxtr\@resource/)
        {
           # v4.34 added

           # No error at this point as a hybrid method is allowed.
           # Error only occurs if no \@istfilename found.

           $foundbib2glsresource = 1;
        }

        # v1.5 added
        # Allow -l switch to override specification in aux file
        unless (defined($opt_l))
        {
           # v2.17 escaped { in regex
           if (m/\\\@glsorder\s*\{([^}]+)\}/)
           {
              my $ordering = $1;

              if ($ordering eq "word")
              {
                 $letterordering = 0;
              }
              elsif ($ordering eq "letter")
              {
                 $letterordering = 1;
              }
              else
              {
                 warn
                   "Unknown ordering '$ordering'\n",
                   "Assuming word ordering\n" unless ($opt_q);
                 $letterordering = 0;
              }
           }
        }
     }

     close AUXFILE;
  }
  else
  {
     warn "Unable to open $name.aux: $!\n";
  }
}

# v2.01 new subroutine run_app added
sub run_app{
   my($appname, $appargs, $trans, $quiet, $dontexec) = @_;

   local(*STATUS);

   my $status   = '';
   my $warnings = '';
   my $errno = 0;
   my $log = '';

   print "$appname $appargs\n" if ($dontexec or not $quiet);

   return if ($dontexec);

   # v2.11 added double-quotes around $appname
   # v2.14 added -k switch
   if (not $opt_k and open (STATUS, "\"$appname\" $appargs 2>&1 |"))
   {
      while (<STATUS>)
      {
         print unless ($quiet);

         $warnings .= $_ if (/WARNING:/);

         $status .= $_ unless (/^[\w]+ing/ or /^Finished/ or /^Usage:/);

         $log .= $_;
      }

      close STATUS;
   }
   else
   {
      unless ($opt_k)
      {
         $warnings = "Unable to fork \"$appname\" with redirection $!\n";

         # v2.14 added check for quiet switches
         warn $warnings,  
           "Retrying without redirection.\n" unless ($quiet or $opt_Q);
      }

      $status = `\"$appname\" $appargs`;

      $log = $status;

      print $status unless ($quiet);
   }

   if ($?)
   {
      # v2.14 Fixed error number assignment
      $errno = ($? >> 8);

      # v2.14 Added check for existence of transcript
      unless (-e $trans)
      {
         $log .= "\n$appname didn't create a transcript.\n";

         if (not $appname=~/\//)
         {
            # No path specified
            $log .= "Check that $appname has been installed and\nis on your system's PATH.\n";

            if (defined $ENV{PATH})
            {
               $log .= "Your PATH environment variable is set to: \n"
                    . $ENV{PATH} . "\n";
            }
            else
            {
               $log .= "I'm sorry, I can't detect your PATH environment variable\n";
            }

            $log .= "Try manually running:\n\"$appname\" $appargs\n";
         }
         elsif (not -e $appname)
         {
            if ($^O=~/Win/)
            {
               if (-e "$appname.exe" or -e "$appname.bat")
               {
                  $log .= "Try manually running:\n\"$appname\" $appargs\n";
               }
               else
               {
                  $log .= "File '$appname' doesn't exist.\n";
               }
            }
            else
            {
               $log .= "File '$appname' doesn't exist.\n";
            }
         }
         else
         {
            $log .= "Try manually running:\n\"$appname\" $appargs\n";
         }
      }

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n\n*** Unable to execute: '\"$appname\" $appargs' ***\n\n";
         print LOGFILE "Failed with error code $errno.\n\n";

         if ($log)
         {
            print LOGFILE "Status report:\n\n";
            print LOGFILE "$log", "\n";
         }

         print LOGFILE "Warnings:\n\n",$warnings, "\n" if $warnings;
         close LOGFILE;
      }
      else
      {
         warn "Unable to open '$trans' $!\n";
      }
   }

   if ($log=~/\(0 entries accepted,/
    or ( ($log=~/(\d+) warnings?/ and $1 gt 0))
    or $log=~/not found/)
   {
      # Attempt to diagnose what's gone wrong

      if (open TRANS, $trans)
      {
         while (<TRANS>)
         {
            if (/Index style file .* not found/)
            {
               $errno = $istnotfound;
               last;
            }
            elsif (/Unknown specifier ;/)
            {
               $errno = $xdynotist;
               last;
            }
            elsif (/## Warning \(.*\):\s*$/)
            {
               $warnings .= $_ . <TRANS>;
            }
         }

         close TRANS;
      }

   }

   return ($status, $warnings, $errno);
}

# v2.08 added $app parameter
sub makeindex{
   my($in,$out,$trans,$ist,$rest,$quiet,$dontexec,$app,$repairencaps) = @_;

   my $args = "$rest -s \"$ist\" -t \"$trans\" -o \"$out\" \"$in\"";

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app($app, $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($errno)
   {
      my $diagnostic = '';

      if ($makeindex_error_text{$errno})
      {
         $diagnostic = $makeindex_error_text{$errno};
      }
      else
      {
         $diagnostic = "Can't find diagnostic message for error code $errno";
      }

      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\nmakeglossaries diagnostic messages:\n$diagnostic\n";
         close LOGFILE;
      }

      die "\n***Call to makeindex failed***\n", 
        ($diagnostic ?
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"
        ),
        "Check '$trans' for details\n";
   }

   # 2.18: added check and repair for multiple encaps
   if ($warnings)
   {
      warn $warnings unless $quiet;

      if ($repairencaps and $warnings=~/multiple encaps/)
      {
         unless ($quiet)
         {
            print "Multiple encaps detected. Attempting to remedy.\n";
            print "Reading $in...\n";
         }

         # if $in can't be opened at this point something wrong
         # has occurred (otherwise how did makeindex manage to open
         # it?)

         open INFD, $in or die "Can't open '$in' $!\n";

         my @entries = ();

         while (<INFD>)
         {
            if (/\\glossaryentry\{(.*)\|([^\|]*)\}\{(.*?)\}/)
            {
               my %entry = 
                (
                   'entry' => $1,
                   'encap' => $2,
                   'location' => $3
                );

               my $add = 1;

               for (my $idx = 0; $idx <= $#entries; $idx++)
               {
                  my $existing = $entries[$idx];

                  if ($entry{'entry'} eq $existing->{'entry'}
                  and $entry{'location'} eq $existing->{'location'}
                  and $entry{'encap'} ne $existing->{'encap'})
                  {
                     $add = 0 if ($add == 1);

                     # Range encaps should take precedence.

                     if ($entry{'encap'}=~/^[\(\)]/)
                     {
                        $add = 2;

                        if ($existing->{'encap'}=~/^[\(\)]/)
                        {
                           # too complicated, keep both

                           last;
                        }
                        else
                        {
                           # remove existing

                           splice @entries, $idx, 1;

                           $idx--;
                        }
                     }
                     elsif ($existing->{'encap'}=~/^[\(\)]/)
                     {
                        if ($entry{'encap'}=~/^[\(\)]/)
                        {
                           # too complicated, keep both

                           $add = 1;
                           last;
                        }
                        # (otherwise drop new entry)
                     }
                     elsif (&encap_overrides($entry{'encap'},
                                   $existing->{'encap'}))
                     {
                        $entries[$idx] = \%entry;
                     }
                  } 
               }

               push @entries, \%entry if $add > 0;
            }
            else
            {
               warn "Abandoning attempt. Can't parse: $_" unless $quiet;

               close INFD;
               return;
            }
         }

         close INFD;

         if (open OUTFD, ">$in")
         {
            print "Writing $in...\n" unless $quiet;

            foreach my $entry (@entries)
            {
               print OUTFD '\\glossaryentry{',
                 $entry->{'entry'}, '|',
                 $entry->{'encap'}, '}{',
                 $entry->{'location'}, '}', "\n";
            }

            close OUTFD;

            print "Retrying\n" unless $quiet;

            &makeindex($in,$out,$trans,$ist,$rest,$quiet,$dontexec,$app,0);
         }
         else
         {
            warn "Can't open '$in' $!\n" unless $quiet;
         }
      }
   }
}

# 2.18 new
# This is a subroutine in case of possible extension.
# For example, what happens in the event of 'textbf' and 'emph'?
# Should one override the other or be combined? Combining is harder
# as it would need a corresponding LaTeX command. (bib2gls deals
# with this better through its --map-formats switcn.)
# 2.21 check for range encap moved earlier

sub encap_overrides{
  my ($newencap, $existing) = @_;

  ($existing=~/\\glsnumberformat\s*$/ or $newencap!~/\\glsnumberformat\s*$/ )
}

# v2.08 added $app parameter
sub xindy{
   my($in,$out,$trans,$ist,$language,$codepage,$rest,$quiet,
     $dontexec, $app) = @_;
   my($args, $langparam, $main, $retry);
   my($module);

   $module = $ist;
   $module=~s/\.xdy\Z//;

   if ($language)
   {
     # map babel names to xindy names

     $language = $languagemap{$language} if ($languagemap{$language});

     $langparam = "-L $language";
   }
   else
   {
     $langparam = "";
     # v2.10 initialise $language to suppress warnings
     $language = "";
   }

   # most languages work with xindy's default codepage, but
   # some don't, so if the codepage isn't specific, check
   # the known cases that will generate an error
   # and supply a default. (For all other cases, it's up to the 
   # user to supply a codepage.)

# v2.01 changed 'if ($codepage eq "")' to 'unless ($codepage)'
   unless ($codepage)
   {
      if ($language eq 'dutch')
      {
         $codepage = "ij-as-ij";
      }
      elsif ($language eq 'german')
      {
         $codepage = "din5007";
      }
      elsif ($language eq 'gypsy')
      {
         $codepage = "northrussian";
      }
      elsif ($language eq 'hausa')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'klingon')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'latin')
      {
         $codepage = "utf";
      }
      elsif ($language eq 'mongolian')
      {
         $codepage = "cyrillic";
      }
      elsif ($language eq 'slovak')
      {
         $codepage = "small";
      }
      elsif ($language eq 'spanish')
      {
         $codepage = "modern";
      }
      elsif ($language eq 'vietnamese')
      {
         $codepage = "utf";
      }
   }
   elsif ($language eq 'german' and $codepage!~/(din5007|duden|braille)/)
   {
#v2.16 added check for german din/duden

      $codepage = "din5007-$codepage";
   }


   my $codepageparam = "";

   if ($codepage)
   {
      $codepageparam = "-C $codepage";
   }

   $main = join(' ',
      "-I xindy",
      "-M \"$module\"",
      "-t \"$trans\"",
      "-o \"$out\"",
      "\"$in\"");

   $args = join(' ', $rest, $langparam, $codepageparam, $main);

# v2.01 replaced code with call to &run_app

   my ($status, $warnings, $errno) 
     = &run_app($app, $args, $trans, $quiet, $dontexec);

   return if ($dontexec);

   if ($status=~/Cannot locate xindy module for language ([^\s]+) in codepage ([^\s]+)/)
   {
      $args = join(' ', $rest, $langparam, $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying using default codepage.\n";

         warn $message;

         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($status=~/Cannot locate xindy module for language ([^\s]+)/
    and $1 ne 'general')
   {
      $args = join(' ', $rest, "-L general", $main);

      unless ($quiet)
      {
         my $message = "$&\nRetrying with -L general\n";

         warn $message;
         $retry .= $message;
      }

      ($status, $warnings, $errno) 
         = &run_app('xindy', $args, $trans, $quiet, $dontexec);

   }

   if ($errno)
   {
      # attempt further diagnostic

      my $diagnostic = '';

      if ($status=~/index 0 should be less than the length of the string/m)
      {
         $diagnostic = $xindy_error_text{nosort};

         $diagnostic .= &parse_for_xindy_nosort($in);
      }
      elsif ($status=~/variable .+ has no value/m)
      {
         # v2.19 fixed misspelt key
         $diagnostic = $xindy_error_text{istnotxdy};
      }
      elsif ($status=~/Could not find file /m)
      {
         # v2.19 added
         $diagnostic = $xindy_error_text{noxdyfile};
      }
      elsif ($status=~/Possible read-error due to ill-formed string " :sep/m)
      {
         $diagnostic = $xindy_error_text{missingendquote};
      }
      elsif (not $language)
      {
         # If the language hasn't been set, then it may be
         # because the document doesn't contain
         # \printglossaries/\printglossary or it may be
         # because the user has a customized style file that
         # contains the language settings.

          $diagnostic = $xindy_error_text{nolanguage};

          if ($in eq 'glo')
          {
             # or it may be that the user doesn't want to use the main
             # glossary and has forgotten to suppress it with the
             # "nomain" package option

             $diagnostic .= $xindy_error_text{nomain};
          }
      }

      # v2.19 added:
      if ($diagnostic and open LOGFILE, ">>$trans")
      {
         print LOGFILE "\nmakeglossaries diagnostic messages:\n\n$diagnostic\n";
         close LOGFILE;
      }

      die "\n***Call to xindy failed***\n", 
          ($diagnostic ? 
          "\nPossible cause of problem:\n\n".  $diagnostic . "\n\n":
          "\n"),
          "Check '$trans' for details\n";
   }

   # Check xindy warnings

   if ($status=~/^WARNING:/m)
   {
      my $diagwarn = '';

      if ($status=~/did not match any location-class/m)
      {
         $diagwarn = $xindy_error_text{badlocation};
      }

      if ($status=~/unknown attribute `pageglsnumberformat'/m)
      {
         $diagwarn .= $xindy_error_text{comp207};
      }

      if ($status=~/Would replace complete index key by empty string, ignoring/m)
      {
         $diagwarn .= $xindy_error_text{nosort};
         $diagwarn .= &parse_for_xindy_nosort($in);
      }

      if ($diagwarn)
      {
         warn "\n**Warning:**\n\n", $diagwarn, "\n";

         $warnings .= "\nmakeglossaries diagnostic messages:\n\n"
                   . $diagwarn;
      }
   }

   if ($retry or $warnings)
   {
      if (open LOGFILE, ">>$trans")
      {
         print LOGFILE "\n$warnings";

         if ($retry)
         {
            print LOGFILE "\nmakeglossaries messages:\n\n", $retry;
         }

         close LOGFILE;
      }
      else
      {
         warn "Unable to open '$trans' $!\n";
      }
   }
}

# v2.18 added:
sub parse_for_xindy_nosort{
  my ($in) = @_;

  my $msg = join("\n", "", 
                 "Attempting to determine which entries have problem sort keys.",
                 "Parsing '$in'");

  my %entries = ();

  if (open FD, $in)
  {
     while (<FD>)
     {
# v2.19 extra conditions added
        if (/:tkey \(\("((?:\\\\[a-zA-Z@]+ *)+)" "\\\\glossentry\{(.*)\}"\) \)/)
        {
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $label;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/([\\\s]+)//g;

           }
        }
        elsif (/:tkey \(\("(\\\\[a-zA-Z@]+ *{(?:\\\\[a-zA-Z@]+ *)+})+" "\\\\glossentry\{(.*)\}"\) \)/)
        {
# name in the form \cs{\cs}
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $1;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/^[a-zA-Z]+[:\-\.]//;
              $entries{$label}->{suggestion}=~s/([^\w]+)//g;
           }
        }
        elsif (/:tkey \(\("(\$\s*(?:\{?\\\\[a-zA-Z@]+ *\}?)+\$)" "\\\\glossentry\{(.*)\}"\) \)/)
        {
# name in the form $\cs$
           my $label = $2;

           unless ($entries{$label})
           {
              $entries{$label}->{sort} = $1;
              $entries{$label}->{suggestion} = $label;
              $entries{$label}->{suggestion}=~s/^[a-zA-Z]+[:\-\.]//;
              $entries{$label}->{suggestion}=~s/([^\w]+)//g;
           }
        }
     }

     close FD;

     my @labels = keys %entries;

     my $n = $#labels+1;

     if ($n == 0)
     {
        $msg .= "\nCouldn't find anything! Sorry, I'm stumped.";
     }
     else
     {
        $msg .= ($n == 1 ? "\n1 problematic entry found:\n"
                         : "\n$n problematic entries found:\n");

        foreach my $label (@labels)
        {
           my $thisentry = $entries{$label};

           $msg .= "\nLabel: '$label'. Sort value : '$thisentry->{sort}'";
           $msg .= "\n(Try adding sort={$thisentry->{suggestion}} to the definition.)";
        }
     }
  }
  else
  {
     $msg .= "\nFailed to open '$in' $!\n";
  }

  $msg;
}

sub HELP_MESSAGE{
   print "\nSyntax : makeglossaries [options] <filename>\n\n";
   print "For use with the glossaries package to pass relevant\n";
   print "files to makeindex or xindy.\n\n";
   print "<filename>\tBase name of glossary file(s). This should\n";
   print "\t\tbe the name of your main LaTeX document without any\n";
   print "\t\textension.\n";
   print "\nGeneral Options:\n\n";
   print "-o <gls>\tUse <gls> as the output file.\n";
   print "\t\t(Don't use -o if you have more than one glossary.)\n";
   print "-q\t\tQuiet mode.\n";
   print "-Q\t\tSilence unable to fork warning.\n";
   print "-k\t\tDon't try to use piped redirection.\n";
   print "-l\t\tLetter ordering.\n";   
   print "-s <sty>\tEmploy <sty> as the style file.\n";
   print "-t <log>\tEmploy <log> as the transcript file.\n";
   print "\t\t(Don't use -t if you have more than one glossary\n";
   print "\t\tor the transcripts will be overwritten.)\n";
   print "-d <directory>\tDirectory in which the .aux, .glo etc files are located.\n",
     "\t\t(Default is the directory in which <filename> resides.)\n";
   print "-n\t\tPrint the command that would normally be executed,\n",
         "\t\tbut don't execute it.\n";

   print "\nXindy Options:\n\n";
   print "-L <language>\tUse <language>.\n";
   print "-x <file>\tFull path to xindy executable.\n",
    "\t\t(Default assumes xindy is on the operating system's path.)\n";

   print "\nMakeindex Options:\n";
   print "(See makeindex documentation for further details on these ";
   print "options.)\n\n";
   print "-c\t\tCompress intermediate blanks.\n";
   print "-g\t\tEmploy German word ordering.\n";
   print "-p <num>\tSet the starting page number to be <num>.\n";
   print "-r\t\tDisable implicit page range formation.\n";
   print "-m <file>\tFull path to makeindex executable.\n",
    "\t\t(Default assumes makeindex is on the operating system's path.)\n";
}

sub VERSION_MESSAGE{

   my $verYear = '';

   if ($version=~/(\d{4})-\d{2}-\d{2}/)
   {
      $verYear = "-$1";
   }

   print "Makeglossaries Version $version\n";
   print "Copyright (C) 2007$verYear Nicola L C Talbot\n";
   print "This material is subject to the LaTeX Project Public License.\n";
}

1;

=head1 NAME

makeglossaries  - Calls makeindex/xindy for LaTeX documents using glossaries package

=head1 SYNOPSIS

B<makeglossaries> [B<-o> I<file>] [B<-q>] [B<-Q>] [B<-k>] [B<-n>]
[B<-s> I<file>] [B<-t> I<file>] [B<-L> I<language>] [B<-c>] [B<-g>] [B<-l>]
[B<-p> I<num>] [B<-r>] [B<-d> I<aux dir>] [B<-m> I<file>] [B<-x> I<file>]
[B<--version>] [B<--help>] I<basename>

=head1 DESCRIPTION

B<makeglossaries> is designed for use with LaTeX documents that
use the glossaries package. The mandatory argument I<basename> should
be the name of the LaTeX document without the .tex extension. 
B<makeglossaries> will read the auxiliary file to determine whether
B<makeindex> or B<xindy> should be called. All the information
required to be passed to the relevant indexing application should
also be contained in the auxiliary file, but may be overridden by
the option arguments to B<makeglossaries>.

=head1 OPTIONS

=over 4

=item B<-q>

Quiet mode. Reduces chatter to standard output.

=item B<-Q>

Silences warning about being unable to fork.

=item B<-k>

Don't try forking with piped redirection. (Lessens the
effect of -q)

=item B<-n>

Print the commands that would normally be executed but don't run them.

=item B<-o> I<file>

Use I<file> as the output file. (Only suitable for documents 
containing a single glossary, otherwise each glossary will be
overridden.)

=item B<-s> I<file>

Use I<file> as the style file. Note that if you use this option,
you need to know whether B<makeindex> or B<xindy> will be called, as
they have different style files.

=item B<-t> I<file>

Use I<file> as the transcript file.

=item B<-l>

Letter ordering.

=item B<-L> I<language>

This option only has an effect if B<xindy> is called. Sets the
language. See B<xindy> documentation for further details.

=item B<-c>

Compress intermediate blanks (B<makeindex> only).

=item B<-g>

Employ German word ordering (B<makeindex> only).

=item B<-p> I<num>

Sets the starting page number to be I<num> (B<makeindex> only).

=item B<-r>

Disable implicit page range formation (B<makeindex> only).

=item B<-d> I<aux dir>

Specify the directory the .aux, .glo etc files are located.
Defaults to the parent directory of the base file I<filename>.

=item B<-m> I<file>

Specify the full path name for B<makeindex> to I<file> in the 
event that B<makeindex> isn't on the operating system's path.

=item B<-x> I<file>

Specify the full path name for B<xindy> to I<file> in the 
event that B<xindy> isn't on the operating system's path.

=item B<--version>

Prints version number and exits.

=item B<--help>

Prints help message and exits.

=back

=head1 REQUIRES

Perl, Getopt::Std, and makeindex or xindy (depending on glossaries
package options).

=head1 LICENSE

This is free software distributed under the LaTeX Project Public 
License. There is NO WARRANTY.
See L<http://www.latex-project.org/lppl.txt> for details.

=head1 AUTHOR

Nicola L. C. Talbot,
L<http://www.dickimaw-books.com/>

=head1 RECOMMENDED READING

The glossaries manual:

	texdoc glossaries

=cut


==> glossaries/makeglossaries-lite.1 <==
.\" Automatically generated by Pod::Man 4.12 (Pod::Simple 3.39)
.\"
.\" Standard preamble:
.\" ========================================================================
.de Sp \" Vertical space (when we can't use .PP)
.if t .sp .5v
.if n .sp
..
.de Vb \" Begin verbatim text
.ft CW
.nf
.ne \\$1
..
.de Ve \" End verbatim text
.ft R
.fi
..
.\" Set up some character translations and predefined strings.  \*(-- will
.\" give an unbreakable dash, \*(PI will give pi, \*(L" will give a left
.\" double quote, and \*(R" will give a right double quote.  \*(C+ will
.\" give a nicer C++.  Capital omega is used to do unbreakable dashes and
.\" therefore won't be available.  \*(C` and \*(C' expand to `' in nroff,
.\" nothing in troff, for use with C<>.
.tr \(*W-
.ds C+ C\v'-.1v'\h'-1p'\s-2+\h'-1p'+\s0\v'.1v'\h'-1p'
.ie n \{\
.    ds -- \(*W-
.    ds PI pi
.    if (\n(.H=4u)&(1m=24u) .ds -- \(*W\h'-12u'\(*W\h'-12u'-\" diablo 10 pitch
.    if (\n(.H=4u)&(1m=20u) .ds -- \(*W\h'-12u'\(*W\h'-8u'-\"  diablo 12 pitch
.    ds L" ""
.    ds R" ""
.    ds C` ""
.    ds C' ""
'br\}
.el\{\
.    ds -- \|\(em\|
.    ds PI \(*p
.    ds L" ``
.    ds R" ''
.    ds C`
.    ds C'
'br\}
.\"
.\" Escape single quotes in literal strings from groff's Unicode transform.
.ie \n(.g .ds Aq \(aq
.el       .ds Aq '
.\"
.\" If the F register is >0, we'll generate index entries on stderr for
.\" titles (.TH), headers (.SH), subsections (.SS), items (.Ip), and index
.\" entries marked with X<> in POD.  Of course, you'll have to process the
.\" output yourself in some meaningful fashion.
.\"
.\" Avoid warning from groff about undefined register 'F'.
.de IX
..
.nr rF 0
.if \n(.g .if rF .nr rF 1
.if (\n(rF:(\n(.g==0)) \{\
.    if \nF \{\
.        de IX
.        tm Index:\\$1\t\\n%\t"\\$2"
..
.        if !\nF==2 \{\
.            nr % 0
.            nr F 2
.        \}
.    \}
.\}
.rr rF
.\"
.\" Accent mark definitions (@(#)ms.acc 1.5 88/02/08 SMI; from UCB 4.2).
.\" Fear.  Run.  Save yourself.  No user-serviceable parts.
.    \" fudge factors for nroff and troff
.if n \{\
.    ds #H 0
.    ds #V .8m
.    ds #F .3m
.    ds #[ \f1
.    ds #] \fP
.\}
.if t \{\
.    ds #H ((1u-(\\\\n(.fu%2u))*.13m)
.    ds #V .6m
.    ds #F 0
.    ds #[ \&
.    ds #] \&
.\}
.    \" simple accents for nroff and troff
.if n \{\
.    ds ' \&
.    ds ` \&
.    ds ^ \&
.    ds , \&
.    ds ~ ~
.    ds /
.\}
.if t \{\
.    ds ' \\k:\h'-(\\n(.wu*8/10-\*(#H)'\'\h"|\\n:u"
.    ds ` \\k:\h'-(\\n(.wu*8/10-\*(#H)'\`\h'|\\n:u'
.    ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'^\h'|\\n:u'
.    ds , \\k:\h'-(\\n(.wu*8/10)',\h'|\\n:u'
.    ds ~ \\k:\h'-(\\n(.wu-\*(#H-.1m)'~\h'|\\n:u'
.    ds / \\k:\h'-(\\n(.wu*8/10-\*(#H)'\z\(sl\h'|\\n:u'
.\}
.    \" troff and (daisy-wheel) nroff accents
.ds : \\k:\h'-(\\n(.wu*8/10-\*(#H+.1m+\*(#F)'\v'-\*(#V'\z.\h'.2m+\*(#F'.\h'|\\n:u'\v'\*(#V'
.ds 8 \h'\*(#H'\(*b\h'-\*(#H'
.ds o \\k:\h'-(\\n(.wu+\w'\(de'u-\*(#H)/2u'\v'-.3n'\*(#[\z\(de\v'.3n'\h'|\\n:u'\*(#]
.ds d- \h'\*(#H'\(pd\h'-\w'~'u'\v'-.25m'\f2\(hy\fP\v'.25m'\h'-\*(#H'
.ds D- D\\k:\h'-\w'D'u'\v'-.11m'\z\(hy\v'.11m'\h'|\\n:u'
.ds th \*(#[\v'.3m'\s+1I\s-1\v'-.3m'\h'-(\w'I'u*2/3)'\s-1o\s+1\*(#]
.ds Th \*(#[\s+2I\s-2\h'-\w'I'u*3/5'\v'-.3m'o\v'.3m'\*(#]
.ds ae a\h'-(\w'a'u*4/10)'e
.ds Ae A\h'-(\w'A'u*4/10)'E
.    \" corrections for vroff
.if v .ds ~ \\k:\h'-(\\n(.wu*9/10-\*(#H)'\s-2\u~\d\s+2\h'|\\n:u'
.if v .ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'\v'-.4m'^\v'.4m'\h'|\\n:u'
.    \" for low resolution devices (crt and lpr)
.if \n(.H>23 .if \n(.V>19 \
\{\
.    ds : e
.    ds 8 ss
.    ds o a
.    ds d- d\h'-1'\(ga
.    ds D- D\h'-1'\(hy
.    ds th \o'bp'
.    ds Th \o'LP'
.    ds ae ae
.    ds Ae AE
.\}
.rm #[ #] #H #V #F C
.\" ========================================================================
.\"
.IX Title "MAKEGLOSSARIES-LITE 1"
.TH MAKEGLOSSARIES-LITE 1 "2020-02-14" "perl v5.30.1" "makeglossaries-lite Lua Script"
.\" For nroff, turn off justification.  Always turn off hyphenation; it makes
.\" way too many mistakes in technical documents.
.if n .ad l
.nh
.SH "NAME"
makeglossaries\-lite  \- Calls makeindex/xindy for LaTeX documents using glossaries package
.SH "SYNOPSIS"
.IX Header "SYNOPSIS"
\&\fBmakeglossaries\fR [\fB\-o\fR \fIfile\fR] [\fB\-q\fR] [\fB\-n\fR]
[\fB\-s\fR \fIfile\fR] [\fB\-t\fR \fIfile\fR] [\fB\-L\fR \fIlanguage\fR] [\fB\-c\fR] [\fB\-g\fR]
[\fB\-l\fR] [\fB\-p\fR \fInum\fR] [\fB\-r\fR] [\fB\-m\fR \fIfile\fR] [\fB\-x\fR \fIfile\fR]
[\fB\-\-version\fR] [\fB\-\-help\fR] \fIbasename\fR
.SH "DESCRIPTION"
.IX Header "DESCRIPTION"
\&\fBmakeglossaries-lite\fR is cut-down Lua alternative to the
\&\fBmakeglossaries\fR Perl script. It's designed for use with LaTeX documents that
use the glossaries package. Some options that are available to
\&\fBmakeglossaries\fR aren't available with \fBmakeglossaries-lite\fR.
The mandatory argument \fIbasename\fR should
be the name of the LaTeX document without the .tex extension. 
\&\fBmakeglossaries-lite\fR will read the auxiliary file to determine whether
\&\fBmakeindex\fR or \fBxindy\fR should be called. All the information
required to be passed to the relevant indexing application should
also be contained in the auxiliary file, but may be overridden by
the option arguments to \fBmakeglossaries-lite\fR.
.SH "OPTIONS"
.IX Header "OPTIONS"
.IP "\fB\-q\fR" 4
.IX Item "-q"
Quiet mode. Reduces chatter to standard output.
.IP "\fB\-n\fR" 4
.IX Item "-n"
Print the commands that would normally be executed but don't run
them.
.IP "\fB\-o\fR \fIfile\fR" 4
.IX Item "-o file"
Use \fIfile\fR as the output file. (Only suitable for documents 
containing a single glossary, otherwise each glossary will be
overridden.)
.IP "\fB\-s\fR \fIfile\fR" 4
.IX Item "-s file"
Use \fIfile\fR as the style file. Note that if you use this option,
you need to know whether \fBmakeindex\fR or \fBxindy\fR will be called, as
they have different style files.
.IP "\fB\-t\fR \fIfile\fR" 4
.IX Item "-t file"
Use \fIfile\fR as the transcript file.
.IP "\fB\-l\fR" 4
.IX Item "-l"
Letter ordering.
.IP "\fB\-L\fR \fIlanguage\fR" 4
.IX Item "-L language"
This option only has an effect if \fBxindy\fR is called. Sets the
language. See \fBxindy\fR documentation for further details.
.IP "\fB\-c\fR" 4
.IX Item "-c"
Compress intermediate blanks (\fBmakeindex\fR only).
.IP "\fB\-g\fR" 4
.IX Item "-g"
Employ German word ordering (\fBmakeindex\fR only).
.IP "\fB\-p\fR \fInum\fR" 4
.IX Item "-p num"
Sets the starting page number to be \fInum\fR (\fBmakeindex\fR only).
.IP "\fB\-r\fR" 4
.IX Item "-r"
Disable implicit page range formation (\fBmakeindex\fR only).
.IP "\fB\-m\fR \fIfile\fR" 4
.IX Item "-m file"
Specify the full path name for \fBmakeindex\fR to \fIfile\fR in the 
event that \fBmakeindex\fR isn't on the operating system's path.
.IP "\fB\-x\fR \fIfile\fR" 4
.IX Item "-x file"
Specify the full path name for \fBxindy\fR to \fIfile\fR in the 
event that \fBxindy\fR isn't on the operating system's path.
.IP "\fB\-\-version\fR" 4
.IX Item "--version"
Prints version number and exits.
.IP "\fB\-\-help\fR" 4
.IX Item "--help"
Prints help message and exits.
.SH "REQUIRES"
.IX Header "REQUIRES"
texlua and makeindex or xindy (depending on glossaries package options).
.SH "LICENSE"
.IX Header "LICENSE"
This is free software distributed under the LaTeX Project Public 
License. There is \s-1NO WARRANTY.\s0
See <http://www.latex\-project.org/lppl.txt> for details.
.SH "AUTHOR"
.IX Header "AUTHOR"
Nicola L. C. Talbot,
<http://www.dickimaw\-books.com/>
.SH "RECOMMENDED READING"
.IX Header "RECOMMENDED READING"
The glossaries manual:
.PP
.Vb 1
\&        texdoc glossaries
.Ve


==> glossaries/makeglossaries.1 <==
.\" Automatically generated by Pod::Man 4.12 (Pod::Simple 3.39)
.\"
.\" Standard preamble:
.\" ========================================================================
.de Sp \" Vertical space (when we can't use .PP)
.if t .sp .5v
.if n .sp
..
.de Vb \" Begin verbatim text
.ft CW
.nf
.ne \\$1
..
.de Ve \" End verbatim text
.ft R
.fi
..
.\" Set up some character translations and predefined strings.  \*(-- will
.\" give an unbreakable dash, \*(PI will give pi, \*(L" will give a left
.\" double quote, and \*(R" will give a right double quote.  \*(C+ will
.\" give a nicer C++.  Capital omega is used to do unbreakable dashes and
.\" therefore won't be available.  \*(C` and \*(C' expand to `' in nroff,
.\" nothing in troff, for use with C<>.
.tr \(*W-
.ds C+ C\v'-.1v'\h'-1p'\s-2+\h'-1p'+\s0\v'.1v'\h'-1p'
.ie n \{\
.    ds -- \(*W-
.    ds PI pi
.    if (\n(.H=4u)&(1m=24u) .ds -- \(*W\h'-12u'\(*W\h'-12u'-\" diablo 10 pitch
.    if (\n(.H=4u)&(1m=20u) .ds -- \(*W\h'-12u'\(*W\h'-8u'-\"  diablo 12 pitch
.    ds L" ""
.    ds R" ""
.    ds C` ""
.    ds C' ""
'br\}
.el\{\
.    ds -- \|\(em\|
.    ds PI \(*p
.    ds L" ``
.    ds R" ''
.    ds C`
.    ds C'
'br\}
.\"
.\" Escape single quotes in literal strings from groff's Unicode transform.
.ie \n(.g .ds Aq \(aq
.el       .ds Aq '
.\"
.\" If the F register is >0, we'll generate index entries on stderr for
.\" titles (.TH), headers (.SH), subsections (.SS), items (.Ip), and index
.\" entries marked with X<> in POD.  Of course, you'll have to process the
.\" output yourself in some meaningful fashion.
.\"
.\" Avoid warning from groff about undefined register 'F'.
.de IX
..
.nr rF 0
.if \n(.g .if rF .nr rF 1
.if (\n(rF:(\n(.g==0)) \{\
.    if \nF \{\
.        de IX
.        tm Index:\\$1\t\\n%\t"\\$2"
..
.        if !\nF==2 \{\
.            nr % 0
.            nr F 2
.        \}
.    \}
.\}
.rr rF
.\"
.\" Accent mark definitions (@(#)ms.acc 1.5 88/02/08 SMI; from UCB 4.2).
.\" Fear.  Run.  Save yourself.  No user-serviceable parts.
.    \" fudge factors for nroff and troff
.if n \{\
.    ds #H 0
.    ds #V .8m
.    ds #F .3m
.    ds #[ \f1
.    ds #] \fP
.\}
.if t \{\
.    ds #H ((1u-(\\\\n(.fu%2u))*.13m)
.    ds #V .6m
.    ds #F 0
.    ds #[ \&
.    ds #] \&
.\}
.    \" simple accents for nroff and troff
.if n \{\
.    ds ' \&
.    ds ` \&
.    ds ^ \&
.    ds , \&
.    ds ~ ~
.    ds /
.\}
.if t \{\
.    ds ' \\k:\h'-(\\n(.wu*8/10-\*(#H)'\'\h"|\\n:u"
.    ds ` \\k:\h'-(\\n(.wu*8/10-\*(#H)'\`\h'|\\n:u'
.    ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'^\h'|\\n:u'
.    ds , \\k:\h'-(\\n(.wu*8/10)',\h'|\\n:u'
.    ds ~ \\k:\h'-(\\n(.wu-\*(#H-.1m)'~\h'|\\n:u'
.    ds / \\k:\h'-(\\n(.wu*8/10-\*(#H)'\z\(sl\h'|\\n:u'
.\}
.    \" troff and (daisy-wheel) nroff accents
.ds : \\k:\h'-(\\n(.wu*8/10-\*(#H+.1m+\*(#F)'\v'-\*(#V'\z.\h'.2m+\*(#F'.\h'|\\n:u'\v'\*(#V'
.ds 8 \h'\*(#H'\(*b\h'-\*(#H'
.ds o \\k:\h'-(\\n(.wu+\w'\(de'u-\*(#H)/2u'\v'-.3n'\*(#[\z\(de\v'.3n'\h'|\\n:u'\*(#]
.ds d- \h'\*(#H'\(pd\h'-\w'~'u'\v'-.25m'\f2\(hy\fP\v'.25m'\h'-\*(#H'
.ds D- D\\k:\h'-\w'D'u'\v'-.11m'\z\(hy\v'.11m'\h'|\\n:u'
.ds th \*(#[\v'.3m'\s+1I\s-1\v'-.3m'\h'-(\w'I'u*2/3)'\s-1o\s+1\*(#]
.ds Th \*(#[\s+2I\s-2\h'-\w'I'u*3/5'\v'-.3m'o\v'.3m'\*(#]
.ds ae a\h'-(\w'a'u*4/10)'e
.ds Ae A\h'-(\w'A'u*4/10)'E
.    \" corrections for vroff
.if v .ds ~ \\k:\h'-(\\n(.wu*9/10-\*(#H)'\s-2\u~\d\s+2\h'|\\n:u'
.if v .ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'\v'-.4m'^\v'.4m'\h'|\\n:u'
.    \" for low resolution devices (crt and lpr)
.if \n(.H>23 .if \n(.V>19 \
\{\
.    ds : e
.    ds 8 ss
.    ds o a
.    ds d- d\h'-1'\(ga
.    ds D- D\h'-1'\(hy
.    ds th \o'bp'
.    ds Th \o'LP'
.    ds ae ae
.    ds Ae AE
.\}
.rm #[ #] #H #V #F C
.\" ========================================================================
.\"
.IX Title "MAKEGLOSSARIES 1"
.TH MAKEGLOSSARIES 1 "2020-02-14" "perl v5.30.1" "makeglossaries Perl Script"
.\" For nroff, turn off justification.  Always turn off hyphenation; it makes
.\" way too many mistakes in technical documents.
.if n .ad l
.nh
.SH "NAME"
makeglossaries  \- Calls makeindex/xindy for LaTeX documents using glossaries package
.SH "SYNOPSIS"
.IX Header "SYNOPSIS"
\&\fBmakeglossaries\fR [\fB\-o\fR \fIfile\fR] [\fB\-q\fR] [\fB\-Q\fR] [\fB\-k\fR] [\fB\-n\fR]
[\fB\-s\fR \fIfile\fR] [\fB\-t\fR \fIfile\fR] [\fB\-L\fR \fIlanguage\fR] [\fB\-c\fR] [\fB\-g\fR] [\fB\-l\fR]
[\fB\-p\fR \fInum\fR] [\fB\-r\fR] [\fB\-d\fR \fIaux dir\fR] [\fB\-m\fR \fIfile\fR] [\fB\-x\fR \fIfile\fR]
[\fB\-\-version\fR] [\fB\-\-help\fR] \fIbasename\fR
.SH "DESCRIPTION"
.IX Header "DESCRIPTION"
\&\fBmakeglossaries\fR is designed for use with LaTeX documents that
use the glossaries package. The mandatory argument \fIbasename\fR should
be the name of the LaTeX document without the .tex extension. 
\&\fBmakeglossaries\fR will read the auxiliary file to determine whether
\&\fBmakeindex\fR or \fBxindy\fR should be called. All the information
required to be passed to the relevant indexing application should
also be contained in the auxiliary file, but may be overridden by
the option arguments to \fBmakeglossaries\fR.
.SH "OPTIONS"
.IX Header "OPTIONS"
.IP "\fB\-q\fR" 4
.IX Item "-q"
Quiet mode. Reduces chatter to standard output.
.IP "\fB\-Q\fR" 4
.IX Item "-Q"
Silences warning about being unable to fork.
.IP "\fB\-k\fR" 4
.IX Item "-k"
Don't try forking with piped redirection. (Lessens the
effect of \-q)
.IP "\fB\-n\fR" 4
.IX Item "-n"
Print the commands that would normally be executed but don't run them.
.IP "\fB\-o\fR \fIfile\fR" 4
.IX Item "-o file"
Use \fIfile\fR as the output file. (Only suitable for documents 
containing a single glossary, otherwise each glossary will be
overridden.)
.IP "\fB\-s\fR \fIfile\fR" 4
.IX Item "-s file"
Use \fIfile\fR as the style file. Note that if you use this option,
you need to know whether \fBmakeindex\fR or \fBxindy\fR will be called, as
they have different style files.
.IP "\fB\-t\fR \fIfile\fR" 4
.IX Item "-t file"
Use \fIfile\fR as the transcript file.
.IP "\fB\-l\fR" 4
.IX Item "-l"
Letter ordering.
.IP "\fB\-L\fR \fIlanguage\fR" 4
.IX Item "-L language"
This option only has an effect if \fBxindy\fR is called. Sets the
language. See \fBxindy\fR documentation for further details.
.IP "\fB\-c\fR" 4
.IX Item "-c"
Compress intermediate blanks (\fBmakeindex\fR only).
.IP "\fB\-g\fR" 4
.IX Item "-g"
Employ German word ordering (\fBmakeindex\fR only).
.IP "\fB\-p\fR \fInum\fR" 4
.IX Item "-p num"
Sets the starting page number to be \fInum\fR (\fBmakeindex\fR only).
.IP "\fB\-r\fR" 4
.IX Item "-r"
Disable implicit page range formation (\fBmakeindex\fR only).
.IP "\fB\-d\fR \fIaux dir\fR" 4
.IX Item "-d aux dir"
Specify the directory the .aux, .glo etc files are located.
Defaults to the parent directory of the base file \fIfilename\fR.
.IP "\fB\-m\fR \fIfile\fR" 4
.IX Item "-m file"
Specify the full path name for \fBmakeindex\fR to \fIfile\fR in the 
event that \fBmakeindex\fR isn't on the operating system's path.
.IP "\fB\-x\fR \fIfile\fR" 4
.IX Item "-x file"
Specify the full path name for \fBxindy\fR to \fIfile\fR in the 
event that \fBxindy\fR isn't on the operating system's path.
.IP "\fB\-\-version\fR" 4
.IX Item "--version"
Prints version number and exits.
.IP "\fB\-\-help\fR" 4
.IX Item "--help"
Prints help message and exits.
.SH "REQUIRES"
.IX Header "REQUIRES"
Perl, Getopt::Std, and makeindex or xindy (depending on glossaries
package options).
.SH "LICENSE"
.IX Header "LICENSE"
This is free software distributed under the LaTeX Project Public 
License. There is \s-1NO WARRANTY.\s0
See <http://www.latex\-project.org/lppl.txt> for details.
.SH "AUTHOR"
.IX Header "AUTHOR"
Nicola L. C. Talbot,
<http://www.dickimaw\-books.com/>
.SH "RECOMMENDED READING"
.IX Header "RECOMMENDED READING"
The glossaries manual:
.PP
.Vb 1
\&        texdoc glossaries
.Ve


==> glossaries/samples/database1.tex <==
% This is a sample database of glossary entries
% Only those entries used in the document with \glslink, \gls,
% \glspl, and uppercase variants will have entries in the
% glossary. Note that the type key is not used, as the
% glossary type can be specified in \loadglsentries

\newglossaryentry{array}{name=array,
description={A list of values identified by a numeric value}}

\newglossaryentry{binary}{name=binary,
description={Pertaining to numbers represented in base 2}}

\newglossaryentry{comment}{name=comment,
description={A remark that doesn't affect the meaning of the 
code}}

\newglossaryentry{global}{name=global,
description={Something that maintains its state when it leaves
the current group}}

\newglossaryentry{local}{name=local,
description={Something that only maintains its state until
it leaves the group in which it was defined/changed}}



==> glossaries/samples/database2.tex <==
% This is a sample database of glossary entries
% Only those entries used in the document with \glslink, \gls,
% \glspl, and uppercase variants will have entries in the
% glossary. Note that the type key is not used, as the
% glossary type can be specified in \loadglsentries

% Don't need to worry about makeindex special characters
\newglossaryentry{quote}{name={"},
description={the double quote symbol}}

\newglossaryentry{at}{name={@},
description={the ``at'' symbol}}

\newglossaryentry{excl}{name={!},
description={the exclamation mark symbol}}

\newglossaryentry{bar}{name={\ensuremath{|}},
description={the vertical bar symbol}}

\newglossaryentry{hash}{name={\#},
description={the hash symbol}}


